Assurance via workflow+ modelling and conformance

We propose considering assurance as a model management enterprise: saying that a system is safe amounts to specifying three workflows modelling how the safety engineering process is defined and executed, and checking their conformance. These workflows are based on precise data modelling as in functional block diagrams, but their distinctive feature is the presence of relationships between the output data of a process and its input data; hence, the name ``WorkflowPlus'', WF+ . A typical WP^+ model comprises three layers: (i) process and control flow, (ii) dataflow (with input-output relationships), and (iii) argument flow or constraint derivation. Precise dataflow modelling signifies a crucial distinction of (WP+)-based and GSN-based assurance, in which the data layer is mainly implicit. We provide a detailed comparative analysis of the two formalisms and conclude that GSN does not fulfil its promises.

==> MCSTRregular.tex <==
%% This is file `MCSTR.sty'. 

% Version History
% 1.0 Initial version

\NeedsTeXFormat{LaTeX2e}
\ProvidesPackage{MCSTR}[2011/05/11 v1.1]
\message{MCS-TR style 2011/05/11 v1.1 by Nick A(Adapted from GSD-TR.sty by Yingfei (adapted from GRACE-TR.sty created by Zhenjiang Hu and Kiminori Matsuzaki))}
\ProcessOptions\relax

\usepackage{graphicx}

%% Cover
\def\MCSTRtitle#1{\gdef\@MCSTR@title{#1}}
\def\MCSTRauthor#1{\gdef\@MCSTR@author{#1}}
\def\MCSTRdate#1{\gdef\@MCSTR@date{#1}}
\def\MCSTRid#1{\gdef\@MCSTR@id{#1}}
\def\MCSTRcommunicatedBy#1{\gdef\@MCS@communicated{#1}}
\def\@MCS@date{\today}
\def\@MCS@title{Please Set MCSTRtitle}
\def\@MCS@author{Please Set MCSTRauthor}
\def\@MCS@id{Please Set MCSTRid}

\def\MCSTRmakecover{%
	\bgroup%
	% save original dimension
	\newdimen\dimen@orgtextheight
	\dimen@orgtextheight=\textheight
	% set layout for title pages
	\setlength{\parindent}     { 0pt}
	\setlength{\voffset}       {-1in}        % ... this is not recommended
	\setlength{\topmargin}     { 0pt}
	\setlength{\headheight}    { 0pt}
	\setlength{\headsep}       { 0pt}
	\setlength{\footskip}      { 0pt}
	\setlength{\textheight}    {\paperheight}
	\setlength{\hoffset}       {-1in}             % ... this is not recommended
	\setlength{\evensidemargin}{ 0pt}
	\setlength{\oddsidemargin} { 0pt}
	\setlength{\textwidth}     {\paperwidth}
	\setlength{\marginparsep}  { 0pt}
	\setlength{\marginparwidth}{ 0pt}
	% set font size for title pages
	\def\sizeHEADER      {\@setfontsize{\HEADER}      {\@xipt} {12}}
	\def\sizeTITLE       {\@setfontsize{\TITLE}       {\@xviipt}{20}}
	\def\sizeAUTHOR      {\@setfontsize{\AUTHOR}      {\@xivpt} {16}}
	\def\sizeCOMMUNICATED{\@setfontsize{\COMMUNICATED}{\@xiipt} {14}}
	\def\sizeDATE        {\@setfontsize{\DATE}        {\@xiipt} {14}}
	\def\sizeORGANIZATION{\@setfontsize{\ORGANIZATION}{\@xipt}  {13}}
	\def\sizeURL         {\@setfontsize{\URL}         {\@xipt}  {12}}
	\def\sizeCOPYRIGHT   {\@setfontsize{\COPYRIGHT}   {\@xipt}  {14}}
	% definition of boxes
	% header
	\newbox\HEADERbox\setbox\HEADERbox=%
	\vtop{\hsize=14cm\sffamily\sizeHEADER\begin{center}%
			McSCert TECHNICAL REPORT%
	\end{center}}
	% title
	\newbox\TITLEbox\setbox\TITLEbox=%
	\vtop{\hsize=14cm\bfseries\sizeTITLE%
		\begin{center}\@MCSTR@title\end{center}}
	% author
	\newbox\AUTHORbox\setbox\AUTHORbox=%
	\vtop{\hsize=12cm\begin{center}%
			\sizeAUTHOR\@MCSTR@author%
			\@ifundefined{@MCSTR@communicated}%
			{}%
			{\\\vspace{10pt}\sizeCOMMUNICATED%
				(Communicated by \@MCSTR@communicated)}%
	\end{center}}
	% number and date
	\newbox\DATEbox\setbox\DATEbox=%
	\vtop{\hsize=100mm
		\parfillskip=0pt\noindent\sizeDATE\@MCSTR@id\hfill\@MCSTR@date\par}
	% organization and url
	\newbox\ORGANIZATIONbox\setbox\ORGANIZATIONbox=%
	\vtop{\hsize=200mm\begin{center}%
			{\sffamily \sizeORGANIZATION
				McMaster Centre for Software Certification\\
				McMaster University\\
				1280 Main Street West, Hamilton, Ontario, Canada L8S 4L8
				\vspace{5mm}}
			{\sffamily\bfseries \sizeURL
				WWW page: https://www.mcscert.ca
			}
	\end{center}}
	% copyright
	\newbox\COPYRIGHTbox\setbox\COPYRIGHTbox=%
	\vtop{\hsize=140mm\sffamily\sizeCOPYRIGHT
		
		\smallskip
		
		The McSCert technical reports are published as a means to ensure timely
		dissemination of scholarly and technical work on a non-commercial
		basis. Copyright and all rights therein are maintained by the authors
		or by other copyright holders, notwithstanding that they have offered
		their works here electronically. It is understood that all persons
		copying this information will adhere to the terms and constraints
		invoked by each author's copyright. These works may not be reposted
		without the explicit permission of the copyright holder.}
	% some important lengths
	% length between leftside and center
	\newdimen\dimen@covercenter
	\dimen@covercenter=105mm
	% length between top and header (fixed point)
	\newdimen\dimen@coverheader 
	\dimen@coverheader=30mm
	% length between header and title (fixed point)
	\newdimen\dimen@covertitle  
	\dimen@covertitle=60mm
	\advance\dimen@covertitle  -\dimen@coverheader
	\advance\dimen@covertitle  -\ht\HEADERbox
	\advance\dimen@covertitle  -\dp\HEADERbox
	% length between title and author, between author and date (fixed length)
	\newdimen\dimen@coverauthor
	\dimen@coverauthor=15mm
	\newdimen\dimen@coverdate
	\dimen@coverdate=13mm
	% length between date and logo
	\newdimen\dimen@logo
	\dimen@logo=35mm
	% length between date and organization (fixed point)
	\newdimen\dimen@organization 
	\dimen@organization=160mm
	\advance\dimen@organization  -\dimen@coverheader
	\advance\dimen@organization  -\ht\HEADERbox
	\advance\dimen@organization  -\dp\HEADERbox
	\advance\dimen@organization  -\dimen@covertitle
	\advance\dimen@organization  -\ht\TITLEbox
	\advance\dimen@organization  -\dp\TITLEbox
	\advance\dimen@organization  -\dimen@coverauthor
	\advance\dimen@organization  -\ht\AUTHORbox
	\advance\dimen@organization  -\dp\AUTHORbox
	\advance\dimen@organization  -\dimen@coverdate
	\advance\dimen@organization  -\ht\DATEbox
	\advance\dimen@organization  -\dp\DATEbox
	% length between top and copyright (fixed point)
	\newdimen\dimen@copyright
	\dimen@copyright=220mm
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	% title page
	\thispagestyle{empty}
	\vbox{\hsize=\textwidth
		\vspace*{\dimen@coverheader}
		\hspace*\dimen@covercenter\hspace*{-.5\wd\HEADERbox}\box\HEADERbox\par
		\vspace*{\dimen@covertitle}
		\hspace*\dimen@covercenter\hspace*{-.5\wd\TITLEbox}\box\TITLEbox\par
		\vspace*{\dimen@coverauthor}
		\hspace*\dimen@covercenter\hspace*{-.5\wd\AUTHORbox}\box\AUTHORbox\par
		\vspace*{\dimen@coverdate}
		\hspace*\dimen@covercenter\hspace*{-.5\wd\DATEbox}\box\DATEbox\par
		\vspace*{\dimen@logo}
		\centerline{\includegraphics[height=3cm]{mcslogo}\hspace{1cm}\raisebox{0.5cm}{\includegraphics[height=2.5cm]{maclogo}}}
		\vspace*{\dimen@organization}
		\hspace*\dimen@covercenter\hspace*{-.5\wd\ORGANIZATIONbox}\box\ORGANIZATIONbox\par
	}\vspace*{-\textheight}\vfill % this is needed for the 1st page
	\clearpage
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	% Copyright Page
	\thispagestyle{empty}
	\vbox{\hsize=\textwidth
		\vspace*{\dimen@copyright}
		\hspace*\dimen@covercenter\hspace*{-.5\wd\COPYRIGHTbox}\box\COPYRIGHTbox
	}
	% set \textheight before clearpage for main paper
	\setlength{\textheight}{\dimen@orgtextheight} 
	\clearpage%
	\setcounter{page}{1}%
	\egroup%
}
%% End of file
 


==> abstract-big.tex <==
%Paper deadline is April 29.
%
%“Foundations” and “Practice and Innovation” papers must not exceed 10 pages (including figures and appendices, excluding references). All papers may include 1 additional page for references.
\begin{abstract}
Assurance is a demonstration that a complex system (such as a car) possesses an important property, such as safety, with a high level of confidence. 
Currently dominant approaches to building assurance safety cases (SC) are focused on goal structuring and/or logical inference. In contrast, we propose considering assurance as a model management enterprise: saying that a system is safe amounts to a) specifying three workflows modelling the safety engineering process (SEP) of the manufacturer (Wf1), its execution for particular product (Wf0), and a set of standards and other normative documents collectively defining some {\em normative} workflow (Wf20, and b) checking whether Wf0 conforms to Wf1 and Wf1 conforms to Wf2. These workflows are based on precise data modelling as in functional block diagrams,  but their special distinctive feature is the presence of multiple relationships between the output data of a process and its input data; hence, the name ``\workflow'' (\WF). 

A typical \WF-model comprises three layers: (i) process and control flow, (ii) dataflow (with input-output relationships), and (iii) argument flow or constraint derivation. It is the dataflow layer that bounds all ingredients into a single \WF-model and makes our assurance methodology both process-based and  product-oriented. Precise dataflow modelling also signifies a crucial distinction of \WF-based and GSN-based assurance, in which the data layer is mainly implicit. 

In the paper, the methodology above is supported with the following technical contributions. 
a) We show how \WF-modelling and conformance can effectively be done with class diagrams (which can further be developed into a specialized profile). 
%
b) We provide \WF\ with precise metamodels, a formal semantics, and an initial mathematical analysis of its foundations based on category theory.  A notable result we obtained in this way is compositionality of \WF, namely that a complex workflow can be encapsulated as a black-box process, which makes it possible to consider workflows of workflows (and so on)
%
%c) We manage the validation aspect of conformance checking by considering it as an aspect in the technical sense, \ie, as a cross-cutting concern spreading over the entire workflow, and present a simple metamodel weaving mechanism and show how it works with an example. 
%
c) For comparison of GSN- and \WF-based assurance, we take a sample SC  presented in the GSN Community Standard, rebuild it on WF+-foundations, and analyze the two SCs. The results of this analysis are then checked against the results of a known empirical survey of building and assessing SCs, and demonstrate that \WF-based assurance can fix many of inherited problems in  GSN-based SCs. 
\end{abstract}


	\endinput
Assurance is a demonstration that a complex system (such as a car or a communication network)  possesses an important%, complex 
property, such as safety or security, with a high level of confidence. 
In contrast to currently dominant approaches to building assurance cases, which are focused on goal structuring and/or logical inference, we propose considering assurance as a model transformation (MT) enterprise: saying that a system possesses an assured property amounts to saying that a particular {\em assurance view} of the system comprising the {\em  assurance data}, satisfies acceptance criteria posed as {\em assurance constraints}. While the MT realizing this view is very complex, we show that it can be decomposed into elementary MTs via a hierarchy of refinement steps. The transformations at the bottom level are ordinary MTs that can be executed for data specifying the system, thus providing the assurance data to be checked against the assurance constraints. In this way, assurance amounts to traversing the hierarchy from the top to the bottom and assuring the correctness of each MT in the path.  
Our approach has a precise mathematical foundation (rooted in process algebra and category theory) --- a necessity if we are to model precisely and then analyze our assurance cases. We discuss the practical applicability of the approach, and argue that it has several advantages over \deleted{the} existing approaches.  


%A now widely used approach for assurance justification and assessment is to delegate the assurance argument to the manufacturer of the system, who builds a corresponding document (called an assurance case) and submits it to a licensing body. 


==> figures/GSNAnnotated-1.tex <==
\begin{figure}
%\begin{wrapfigure}{R}{0.35\textwidth}
%\vspace{-1cm}
\centering
    \includegraphics[%scale=0.6%0.4
                    width=0.5\textwidth%
                    %height=0.12\textheight%
                    %angle=180
                 ]%
                 {figures/GSNannotated-1.pdf}
\caption{GSN Example annotated with data (orange blocks) and process executions (green)}%, logical statement (red) and inference (blue). }
	\label{fig:GSNAnnotated-1}
\vspace{-.6cm}
%\end{wrapfigure}
\end{figure}


==> figures/GSNAnnotated.tex <==
\begin{figure}
%\begin{wrapfigure}{R}{0.35\textwidth}
%\vspace{-1cm}
\centering
    \includegraphics[%scale=0.6%0.4
                    width=0.5\textwidth%
                    %height=0.12\textheight%
                    %angle=180
                 ]%
                %\vspace{-0.5cm}
                 {figures/GSNannotated.pdf}
\caption{GSN Example annotated with data (orange \& blocks), process executions (green \& purple), logical propositions(red) and inference (pale-blue). %\textcolor{red}{WHITE FONT in dark blocks would be better. Probably all green-orange arrows are better to make equally transparent (?)}
}\label{fig:GSNannotated}
\vspace{-.6cm}
%\end{wrapfigure}
\end{figure}


==> figures/TR/GSNAnnotatedPD.tex <==
\begin{figure*}
%\begin{wrapfigure}{R}{0.35\textwidth}
%\vspace{-1cm}
\centering
    \includegraphics[%scale=0.6%0.4
    				angle=90,
                    width=1\textwidth%
                    %height=0.12\textheight%
                    %angle=180
                 ]%
                 {figures/TR/GSNannotatedPDpic.pdf}
\caption{GSN Example annotated with data (orange/grey) and processes (green) blocks.% \& purple), logical propositions(red) and inference (pale-blue). %\textcolor{red}{WHITE FONT in dark blocks would be better. Probably all green-orange arrows are better to make equally transparent (?)}
}\label{fig:GSNannotated-PD}
\vspace{-.6cm}
%\end{wrapfigure}
\end{figure*}
%\end{document}
%(./sections/recoverSem.tex
%
%! LaTeX Error: File `figures/TR/GSNannotated-PD.tex' not found.


==> figures/TR/GSNAnnotatedTR.tex <==
\begin{figure*}
%\begin{wrapfigure}{R}{0.35\textwidth}
%\vspace{-1cm}
\centering
    \includegraphics[%scale=0.6%0.4
    				angle=90,
                    width=1\textwidth%
                    %height=0.12\textheight%
                    %angle=180
                 ]%
                 {figures/GSNannotated.pdf}
\caption{GSN Example annotated with data (orange \& blocks), process executions (green \& purple), logical propositions(red) and inference (pale-blue). %\textcolor{red}{WHITE FONT in dark blocks would be better. Probably all green-orange arrows are better to make equally transparent (?)}
}\label{fig:GSNannotated}
\vspace{-.6cm}
%\end{wrapfigure}
\end{figure*}


==> figures/TR/PD.tex <==
\begin{figure*}
%\begin{wrapfigure}{R}{0.35\textwidth}
%\vspace{-1cm}
\centering
    \includegraphics[%scale=0.6%0.4
    				angle=90,
                    width=1\textwidth%
                    %height=0.12\textheight%
                    %angle=180
                 ]%
                 {figures/TR/PDpic.pdf}
\caption{GSN Example annotated with data (orange/grey) and processes (green) blocks.% \& purple), logical propositions(red) and inference (pale-blue). %\textcolor{red}{WHITE FONT in dark blocks would be better. Probably all green-orange arrows are better to make equally transparent (?)}
}\label{fig:GSNannotated-PD}
\vspace{-.6cm}
%\end{wrapfigure}
\end{figure*}
%\end{document}
%(./sections/recoverSem.tex
%
%! LaTeX Error: File `figures/TR/GSNannotated-PD.tex' not found.


==> figures/TR/PDDRI.tex <==
\begin{figure*}
%\begin{wrapfigure}{R}{0.35\textwidth}
%\vspace{-1cm}
\centering
    \includegraphics[%scale=0.6%0.4
    				angle=90,
                    width=1\textwidth%
                    %height=0.12\textheight%
                    %angle=180
                 ]%
                 {figures/TR/PDDRIpic.pdf}
\caption{GSN Example annotated with data (orange), processes (green), dataflow, reviews (purple) and inferences (blue).% \& purple), logical propositions(red) and inference (pale-blue). %\textcolor{red}{WHITE FONT in dark blocks would be better. Probably all green-orange arrows are better to make equally transparent (?)}
}\label{fig:GSNannotated-PDDRI}
\vspace{-.6cm}
%\end{wrapfigure}
\end{figure*}


==> figures/TR/aspWeavingTR.tex <==
\begin{figure}
%\newcommand\enp{\ensuremath{\mathsf{ep}}}
%\begin{wrapfigure}{R}{0.45\columnwidth}
 \vspace{-0.5cm}
	\centering
\begin{diagram}%[small]  %
[w=20ex,h=20ex]
   \dbox{M_\main}&\lTo^{w_\enp} & \dbox{M_\entry} %& \lDashto^{\over{f}} &  {D_Z} 
\\ %row 2
	\dDashto<{e^*} & \mathsf{[PO]} %\swTilearrow{[po]} 
	 &\dTo>{e}
\\  % row 3\
	M_\main{+}M_\adv& \lDashto^{w^*} &\dbox{M_\adv}%& \lTo^f&\dbox{O}
\end{diagram}
%\caption{Aspect weaving}\label{fig:aspWeaving}
\vspace{-1ex}
%\end{wrapfigure}
\end{figure}

==> figures/TR/lostFile.tex <==
\begin{figure*}
%\begin{wrapfigure}{R}{0.35\textwidth}
%\vspace{-1cm}
\centering
    \includegraphics[%scale=0.6%0.4
    				angle=90,
                    width=1\textwidth%
                    %height=0.12\textheight%
                    %angle=180
                 ]%
                {figures/TR/GSNannotatedPDpic.pdf}
                  %{figures/TR/lostFilePic.pdf}
\caption{GSN Example annotated with data (orange/grey) and processes (green) blocks.% \& purple), logical propositions(red) and inference (pale-blue). %\textcolor{red}{WHITE FONT in dark blocks would be better. Probably all green-orange arrows are better to make equally transparent (?)}
}\label{fig:GSNannotated-PD}
\vspace{-.6cm}
%\end{wrapfigure}
\end{figure*}
%\end{document}
%(./sections/recoverSem.tex
%
%! LaTeX Error: File `figures/TR/GSNannotated-PD.tex' not found.


==> figures/TR/wfpMetamodel.tex <==
\begin{figure*}
%\begin{wrapfigure}{R}{0.35\textwidth}
%\vspace{-1cm}
\centering
    \includegraphics[%scale=0.6%0.4
                    width=0.95\textwidth%
                    %width=0.95\textwidth
                    %height=0.12\textheight%
                    %angle=180
                 ]%
                 {figures/sources/wfp-metamodel.png}
                 %\vspace{-0.5cm}
\caption{Metamodel for \wfp  \label{fig:wfp-metamodel}}
%\vspace{-.6cm}
%\end{wrapfigure}
\end{figure*}


==> figures/gsn2wf2gsn-schema.tex <==
\begin{figure}
%\begin{wrapfigure}{R}{0.35\textwidth}
%\vspace{-1cm}
\centering
    \includegraphics[%scale=0.6%0.4
                    width=0.495\textwidth%
                    %height=0.12\textheight%
                    %angle=180
                 ]%
                 {figures/gsn2wf2gsn-schema}
\caption{From GSN to WF+ -- a full complex version of \figref{fig:gsn2wf2gsn-simple}  ...  \label{fig:gsn2wf2gsn}}
%\vspace{-1cm}
%\end{wrapfigure}
\end{figure}

==> figures/gsn2wf2gsn-schemaSimple.tex <==
\begin{figure}[h]
%\begin{wrapfigure}{R}{0.35\textwidth}
%\vspace{-1cm}
\centering
    \includegraphics[%scale=0.6%0.4
                    width=0.485\textwidth%
                    %height=0.12\textheight%
                    %angle=180
                 ]%
                 {figures/gsn2wf2gsn-schemaSimple}
\caption{From GSN to WF+ -- a simple version. Perhaps, some elements of \figref{fig:gsn2wf2gsn} should be shown here too\label{fig:gsn2wf2gsn-simple}}
%\vspace{-1cm}
%\end{wrapfigure}
\end{figure}

==> figures/gsnEx-modified2.tex <==
\begin{figure*}
%\begin{wrapfigure}{R}{0.35\textwidth}
%\vspace{-1cm}
\centering
    \includegraphics[%scale=0.6%0.4
                    width=0.95\textwidth%
                    %height=0.12\textheight%
                    %angle=180
                 ]%
                 {figures/gsnEx-modified2.png}
\caption{Example modified ...  \label{fig:gsnEx-modified2}}
%\vspace{-1cm}
%\end{wrapfigure}
\end{figure*}

==> figures/sem-fwk.tex <==
\newlength{\cw}
\newlength{\ch}
\cw=5ex
\ch=6ex

\begin{figure}
%\begin{wrapfigure}{R}{0.35\columnwidth}
 %\vspace{-0.5cm}
	\centering
%	\begin{tabular}{ll}
	\begin{tabular}{l}
\begin{diagram}%[small]  % reading
[w=\cw,h=\ch]
   \dbox{D_X}&\lDashto^{\over{e}} & D_{Y}& \lDashto^{\over{f}} &  {D_Z} 
\\ %row 2
	\dTo<{t_X} & \neTilearrow{[pb]} &\dDashto~{{t_Y}}
	& \neTilearrow{[pb]} &\dDashto>{{t_Z}}
\\
	\dbox{M}& \lTo^e &\dbox{N}& \lTo^f&\dbox{O}
\end{diagram}
\\[10pt]
(a) %\vspace{5pt}
Reading via PB
%\\[10pt]
%\begin{diagram}%[small] % writing
%	[w=\cw,h=\ch]
%	\dbox{D_X}&\rDashto^{\over{e}} & D_{Y}& \rDashto^{\over{f}} &  {D_Z} 
%	\\
%	\dTo<{t_X} & \neTilearrow{[gen]} &\dDashto~{{t_Y}}
%	& \neTilearrow{[gen]} &\dDashto>{{t_Z}}
%	\\
%	\dbox{M}& \rTo^e &\dbox{N}& \rTo^f&\dbox{O}
%\end{diagram}
%\\[5pt]
%(b) Writing via generation
%\end{tabular}
%&\hspace{-2ex}
 \\ [10pt ]%======
%\begin{tabular}{l}
\begin{diagram}%[small]  % van kampen diag
		[w=3ex,h=4ex]
% row 1
&&\dbox{D_{X_2}}&\rDashto^{\widehat{\ovr{r_1}}}&&&D_{\mrginst}&
\\ % row 2
&\ruTo^{\ovr{r_2} }&&\poop&&\ruDashto<{\widehat{\ovr{r_2}}}&&
\\ % row 3
\dbox{\Corr_X}&\rTo^{\ovr{r_1}}&&&\dbox{D_{X_1}}&&\dDashto~{t_\mrginst}
\\ % row 4
&\pbop&\dTo>{t_{X_2}} && \dTo>{t_{X_1}}&&&
\\ % row 5
\dTo~{t_{12}}&&\dbox{M_2}&\rDashto^{\hat r_1}
                      &&&\mrgmm&
\\ % row 6
&\ruTo^{r_2}&&\poop&&\ruDashto^{\hat r_2}&&&
\\ % row 7
\dbox{\Corr_M}&\rTo^{r_1}&&&\dbox{M_1}&&&&
\\
%&&&&&&&
\end{diagram}
\\ [20pt]
(b) Writing via merging
%\end{tabular}
\end{tabular}
\caption{Main dataflow mechanisms (nodes denoting derived data graphs are not framed and derived mappings are dashed) %Dataflow via pullbacks (pb)}
}\label{fig:sem-fwk}
\vspace{-3ex}
%\end{wrapfigure}
\end{figure}

==> figures/wfExample-dataFlow.tex <==
\begin{figure*}
%\begin{wrapfigure}{R}{0.45\columnwidth}
%\vspace{-1cm}
\centering
    \includegraphics[%scale=0.6%0.4
                    width=0.95\textwidth%
                    %height=0.12\textheight%
                    %angle=180
                 ]%
                 {figures/wfExample-dataFlow.png}
\caption{Metadata definition for the dataflow in \figri}
\label{fig:wfExample-dataFlow}
\vspace{-5mm}
%\end{wrapfigure}
\end{figure*}

==> figures/wfExample-depFlow+meta.tex <==
\begin{figure}
%\begin{wrapfigure}{R}{0.45\columnwidth}
%\vspace{-1cm}
\centering
% start the left subfig
%\subfloat[Example of WF+ dependency flow]{
\begin{minipage}[t]{0.475\columnwidth}
\centering
    \includegraphics[%scale=0.6%0.4
                    width=0.95\textwidth%
                    %height=0.12\textheight%
                    %angle=180
                 ]%
                 {figures/wfMetamod-depflow-OLD.png}
                 \caption{Example of WF+ dependency flow
  \label{fig:wfExample-depFlow}              
} 
\end{minipage}% end left subfig
\hspace{5pt}
% start thre right subfig
\begin{minipage}[t]{0.475\columnwidth}
	\centering
	\includegraphics[%scale=0.6%0.4
	width=0.95\textwidth%
	%height=0.12\textheight%
	%angle=180
	]%
	{figures/wfMetamod-depflow-OLD.png}
	\caption{Metamodel of dependency flow (@Nick: select the best notations for constr and polish)
		\label{fig:depFlow-meta}              
	} 
\end{minipage}% end left subfig
% subfloat option does not work :(:( ))
%% start the right subfig
%\subfloat[Metamodel of WF+ dependency flow]{
%	\includegraphics[%scale=0.6%0.4
%	width=0.45\columnwidth%
%	%height=0.12\textheight%
%	%angle=180
%	]%
%	{figures/depFlow-meta.png}
%	\label{fig:wfExample-metadepFlow}              
%} % end left subfig
%\caption{Example of WF+ dependency flow}
%\label{fig:wfExample-depFlow}
%\vspace{-5mm}
%\end{wrapfigure}
\end{figure}

==> figures/wfExample-depFlow-1.tex <==
\begin{figure}
%\begin{wrapfigure}{R}{0.45\columnwidth}
%\vspace{-1cm}
\centering
    \includegraphics[%scale=0.6%0.4
                    width=0.75\columnwidth%
                    %height=0.12\textheight%
                    %angle=180
                 ]%
                 {figures/wfExample-depFlow.png}
\caption{Dependency flow: an example}
\label{fig:wfExample-depFlow}
\vspace{-5mm}
%\end{wrapfigure}
\end{figure}

==> figures/wfExample-depFlow.tex <==
\begin{figure}
%\begin{wrapfigure}{R}{0.45\columnwidth}
%\vspace{-1cm}
\centering
    \includegraphics[%scale=0.6%0.4
                    width=0.75\columnwidth%
                    %height=0.12\textheight%
                    %angle=180
                 ]%
                 {figures/wfExample-depFlow.png}
\caption{Example of a WF+ schema}
\label{fig:wfExample-depFlow}
%\vspace{-5mm}
%\end{wrapfigure}
\end{figure}

==> figures/wfExample-full.tex <==
\begin{figure*}
%\begin{wrapfigure}{R}{0.45\columnwidth}
%\vspace{-1cm}
\centering
    \includegraphics[%scale=0.6%0.4
                    width=0.95\textwidth%
                    %height=0.12\textheight%
                    %angle=180
                 ]%
                 {figures/wfExample-full.png}
\caption{Our running example of WF+}
\label{fig:wfExample-full}
\vspace{-5mm}
%\end{wrapfigure}
\end{figure*}

==> figures/wfExample-metadepFlow.tex <==
\begin{figure}
%\begin{wrapfigure}{R}{0.45\columnwidth}
%\vspace{-1cm}
\centering
% start the left subfig
\subfloat[Example of WF+ dependency flow]{
    \includegraphics[%scale=0.6%0.4
                    width=0.5\columnwidth%
                    %height=0.12\textheight%
                    %angle=180
                 ]%
                 {figures/wfExample-depFlow.png}
  \label{fig:wfExample-depFlow}              
} % end left subfig
\hspace{1in}
% start the right subfig
\subfloat[Metamodel of WF+ dependency flow]{
	\includegraphics[%scale=0.6%0.4
	width=0.5\columnwidth%
	%height=0.12\textheight%
	%angle=180
	]%
	{figures/wfExample-metadepFlow.png}
	\label{fig:wfExample-metadepFlow}              
} % end left subfig


\caption{Example of WF+ dependency flow}
\label{fig:wfExample-depFlow}
\vspace{-5mm}
%\end{wrapfigure}
\end{figure}

==> figures/wfExample-schema.tex <==
\begin{figure}
%\begin{wrapfigure}{R}{0.45\columnwidth}
%\vspace{-1cm}
\centering
    \includegraphics[%scale=0.6%0.4
                    width=0.75\columnwidth%
                    %height=0.12\textheight%
                    %angle=180
                 ]%
                 {figures/wfExample-depFlow.png}
\caption{Example of a WF+ schema}
\label{fig:wfExample-schema}
%\vspace{-5mm}
%\end{wrapfigure}
\end{figure}

==> figures/wfMetamod-flow.tex <==
\begin{figure}
%\begin{wrapfigure}{R}{0.45\columnwidth}
%\vspace{-1cm}
\centering
    \includegraphics[%scale=0.6%0.4
                    width=0.99\columnwidth%
                    %height=0.12\textheight%
                    %angle=180
                 ]%
                 {figures/wfMetamod-flow.png}
\caption{Metamodel of WF+ (it includes the content of metamodel in \figri\ but it's not shown).Default multiplicities are as in \figri}
\label{fig:wfMetamod-flow}
%\vspace{-5mm}
%\end{wrapfigure}
\end{figure}

==> figures/wfMetamod-full-horiz.tex <==
\begin{figure*}
	\centering
	\begin{tabular}{c@{\quad}c}
		    \includegraphics[%scale=0.6%0.4
		width=0.375\textwidth%
		%height=0.12\textheight%
		%angle=180
		]%
		{figures/wfMetamod-lib.png}
		&
			\includegraphics[%scale=0.6%0.4
		width=0.6\textwidth%
		%height=0.12\textheight%
		%angle=180
		]%
		{figures/wfMetamod-flow.png}
		\\ [10pt]
		(a) Process library metamodel
		&
		(b) WF+ metamodel (includes the content of metamodel (a) but it's not shown). 
		\end{tabular}
	\caption{Main Metamodels. The default multiplicity of a (un)directed end is (*)1. \label{fig:wfMetamod-full}}
\end{figure*}

\endinput

\begin{figure*}
%\begin{wrapfigure}{R}{0.45\columnwidth}
%\vspace{-1cm}
\centering
\begin{minipage}[t]{0.4\linewidth}
\centering
    \includegraphics[%scale=0.6%0.4
                    width=0.4\textwidth%
                    %height=0.12\textheight%
                    %angle=180
                 ]%
                 {figures/wfMetamod-lib.png}
                 \caption{Process library metamodel}  \label{fig:wfMetamod-libb}              
\end{minipage}% end left subfig
\hspace{5pt}
% start thre right subfig
\begin{minipage}[t]{0.6\linewidth}
	\centering
	\includegraphics[%scale=0.6%0.4
	width=0.6\textwidth%
	%height=0.12\textheight%
	%angle=180
	]%
	{figures/wfMetamod-flow.png}
	\caption{WF+ metamodel (it includes thr content of ... but it is not shown)	\label{fig:depFlow-meta}              
	} 
\end{minipage}% end left subfig
% subfloat option does not work :(:( ))
\end{figure}

==> figures/wfMetamod-full-vert.tex <==
\begin{figure}
	%\centering
	\begin{tabular}{p{1.\columnwidth}} %{}} %{c@{\quad}c}
			\includegraphics[%scale=0.6%0.4
		width=1.\columnwidth%
		%height=0.12\textheight%
		%angle=180
		]%
		{figures/wfMetamod-flow.png}
		\\ %[10pt]
		(a) WF+ metamodel (includes the content of metamodel (b), which is not shown)
		\\ [10pt]
				    \includegraphics[%scale=0.6%0.4
		width=0.375\textwidth%
		%height=0.12\textheight%
		%angle=180
		]%
		{figures/wfMetamod-lib.png}
		\\ %[10pt]
		(b) Process library metamodel
			\end{tabular}
	\caption{Main Metamodels. For associations, the default multiplicity of a (un)directed end is (*)1. The black diamond end has multiplicity 1 by default. %For {\bf undirected ones, the default multiplicity is *. 
		\label{fig:wfMetamod-full}}
\end{figure}

\endinput

\begin{figure*}
%\begin{wrapfigure}{R}{0.45\columnwidth}
%\vspace{-1cm}
\centering
\begin{minipage}[t]{0.4\linewidth}
\centering
    \includegraphics[%scale=0.6%0.4
                    width=0.4\textwidth%
                    %height=0.12\textheight%
                    %angle=180
                 ]%
                 {figures/wfMetamod-lib.png}
                 \caption{Process library metamodel}  \label{fig:wfMetamod-libb}              
\end{minipage}% end left subfig
\hspace{5pt}
% start thre right subfig
\begin{minipage}[t]{0.6\linewidth}
	\centering
	\includegraphics[%scale=0.6%0.4
	width=0.6\textwidth%
	%height=0.12\textheight%
	%angle=180
	]%
	{figures/wfMetamod-flow.png}
	\caption{WF+ metamodel (it includes thr content of ... but it is not shown)	\label{fig:depFlow-meta}              
	} 
\end{minipage}% end left subfig
% subfloat option does not work :(:( ))
\end{figure}

==> figures/wfMetamod-lib+flow.tex <==
\begin{figure}
%\begin{wrapfigure}{R}{0.45\columnwidth}
%\vspace{-1cm}
\centering
% start the left subfig
%\subfloat[Example of WF+ dependency flow]{
\begin{minipage}[t]{0.475\columnwidth}
\centering
    \includegraphics[%scale=0.6%0.4
                    width=0.95\textwidth%
                    %height=0.12\textheight%
                    %angle=180
                 ]%
                 {figures/wfMetamod-depflow-OLD.png}
                 \caption{Example of WF+ dependency flow
  \label{fig:wfExample-depFlow}              
} 
\end{minipage}% end left subfig
\hspace{5pt}
% start thre right subfig
\begin{minipage}[t]{0.475\columnwidth}
	\centering
	\includegraphics[%scale=0.6%0.4
	width=0.95\textwidth%
	%height=0.12\textheight%
	%angle=180
	]%
	{figures/wfMetamod-depflow-OLD.png}
	\caption{Metamodel of dependency flow (@Nick: select the best notations for constr and polish)
		\label{fig:depFlow-meta}              
	} 
\end{minipage}% end left subfig
% subfloat option does not work :(:( ))
%% start the right subfig
%\subfloat[Metamodel of WF+ dependency flow]{
%	\includegraphics[%scale=0.6%0.4
%	width=0.45\columnwidth%
%	%height=0.12\textheight%
%	%angle=180
%	]%
%	{figures/depFlow-meta.png}
%	\label{fig:wfExample-metadepFlow}              
%} % end left subfig
%\caption{Example of WF+ dependency flow}
%\label{fig:wfExample-depFlow}
%\vspace{-5mm}
%\end{wrapfigure}
\end{figure}

==> figures/wfMetamod-lib.tex <==
\begin{figure}
%\begin{wrapfigure}{R}{0.45\columnwidth}
%\vspace{-1cm}
\centering
    \includegraphics[%scale=0.6%0.4
                    width=0.75\columnwidth%
                    %height=0.12\textheight%
                    %angle=180
                 ]%
                 {figures/wfMetamod-lib.png}
\caption{Process library metamodel. The default multiplicity of an (un)directed end is (*)1.
}
\label{fig:wfMetamod-lib}
\vspace{-5mm}
%\end{wrapfigure}
\end{figure}

==> getPackages-ll.tex <==
%\usepackage{GSDTR}
\usepackage{enumitem}
\usepackage[stable]{footmisc}
\usepackage[retainorgcmds]{IEEEtrantools}
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
%\usepackage{bickham}
%--------
\usepackage[english]{babel}
\usepackage{hyperref}
\usepackage{tikz}
\usepackage{lipsum}
%\usepackage{boondox-cal}
%\usepackage{boondox-calo}
\usepackage{dutchcal}     %<--- ?
\usepackage[leqno]{amsmath}
\usepackage{fancybox}
\usepackage{graphicx}
\usepackage{wrapfig}
\usepackage{lineno}
\usepackage[misc,geometry]{ifsym}
\usepackage{graphicx}
\usepackage{color}
\usepackage{xcolor}
\definecolor{applegreen}{rgb}{0.55, 0.71, 0.0}
\definecolor{caribbeangreen}{rgb}{0.0, 0.8, 0.6}
\usepackage[normalem]{ulem}
\usepackage{ucs}
\usepackage{url}
\usepackage{makeidx}
\usepackage{amssymb}

\usepackage[all]{xy}
\usepackage{xspace}
\usepackage{subfig}

\usepackage{algorithm}
\usepackage{verbatim}
\usepackage{multirow}
%=== previosly were in macros

\usepackage{rotating}
\usepackage{lscape}
\usepackage{epsfig}
\usepackage{color}
\usepackage{float}
\usepackage{amsbsy,wasysym}
\usepackage{amsfonts}
\usepackage{amstext}
\usepackage{amssymb}
\usepackage{mathrsfs}
\usepackage{array}
\usepackage{latexsym}
\usepackage{xspace}
%\usepackage[figurename=Fig.]{caption}




==> getPackages-old.tex <==
%-- from TR-32
\usepackage{makeidx}  % was but commneted in my packages
\usepackage{epstopdf}
\usepackage[bookmarks=true,colorlinks=true,linkcolor=black,%
citecolor=black,urlcolor=black,filecolor=black,bookmarksnumbered=true]%
{hyperref}  %  I do have hyperref but w/out any option!
\usepackage{enumerate}
%\usepackage{subfigure}  I have it
%\usepackage{amsmath,amssymb}
\usepackage[usenames,dvipsnames]{color} % no options in my packages. I also have {xcolor}
%%--
\usepackage[final]{changes}
\usepackage{booktabs} % For formal tables
\usepackage[T1]{fontenc}
\usepackage{enumitem}
%%\usepackage{GSDTR}
 \usepackage{dutchcal}
\usepackage{fancybox}
\usepackage{graphicx}
\usepackage{wrapfig}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage{lipsum}
\usepackage{lineno} 
%\usepackage{hyperref}
\usepackage[misc,geometry]{ifsym}
\usepackage{graphicx}
%\usepackage{color}
\usepackage[normalem]{ulem}
\usepackage{ucs}
\usepackage{url}
%\usepackage{makeidx}	  
\usepackage{amsbsy}
\usepackage[nointegrals]{wasysym}
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{amstext}
\usepackage{amssymb}

\usepackage{xspace}
\usepackage{wrapfig}
\usepackage{subfigure}
\usepackage{algorithm}
\usepackage{verbatim}
\usepackage{multirow}
%=== previosly were in macros

\usepackage{rotating}
\usepackage{lscape}
\usepackage{epsfig}
%\usepackage{color}
\usepackage{float}
\usepackage{mathrsfs}
\usepackage{array}
\usepackage{latexsym}
\usepackage{xspace}

\usepackage{cite}

\usepackage{amsmath,amssymb,amsfonts}
\usepackage{textcomp}
\usepackage{xcolor}



==> getPackages.tex <==
%\usepackage{GSDTR}
\usepackage{enumitem}
\usepackage[stable]{footmisc}
\usepackage[retainorgcmds]{IEEEtrantools}
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
%\usepackage{bickham}
%--------
\usepackage[english]{babel}
\usepackage{hyperref}
\usepackage{tikz}
\usepackage{lipsum}
%\usepackage{boondox-cal}
%\usepackage{boondox-calo}
\usepackage{dutchcal}     %<--- ?
\usepackage[leqno]{amsmath}
\usepackage{fancybox}
\usepackage{graphicx}
\usepackage{wrapfig}
\usepackage{lineno}
\usepackage[misc,geometry]{ifsym}
\usepackage{graphicx}
\usepackage{color}
\usepackage{xcolor}
\definecolor{applegreen}{rgb}{0.55, 0.71, 0.0}
\definecolor{caribbeangreen}{rgb}{0.0, 0.8, 0.6}
\usepackage[normalem]{ulem}
\usepackage{ucs}
\usepackage{url}
\usepackage{makeidx}
\usepackage{amssymb}

\usepackage[all]{xy}
\usepackage{xspace}
\usepackage{subfig}

\usepackage{algorithm}
\usepackage{verbatim}
\usepackage{multirow}
%=== previosly were in macros

\usepackage{rotating}
\usepackage{lscape}
\usepackage{epsfig}
\usepackage{color}
\usepackage{float}
\usepackage{amsbsy,wasysym}
\usepackage{amsfonts}
\usepackage{amstext}
\usepackage{amssymb}
\usepackage{mathrsfs}
\usepackage{array}
\usepackage{latexsym}
\usepackage{xspace}
%\usepackage[figurename=Fig.]{caption}




==> macros/4lenses/macros4drawingTiles.tex <==
%\newcommand\xx{\!\!}
%\newcommand\xxx{\!\!\!}
%\newcommand\xxxx{\xxx\xx}

\newcommand\qryincl[2]{\mathsf{i}_{#1}^{#2}}
\newcommand\qryinclq[1]{\qryincl{#1}{Q}}
\newcommand\liftqryincl[2]{\ovr{\mathsf{i}_{#1}^{#2}}}
\newcommand\liftqryinclq[1]{\liftqryincl{#1}{Q}}


\newcommand\arrONarr{\stackrel{\mbox{$\longrightarrow$}}{\smash{\longrightarrow}}}
\newcommand\eeTilearrow[1]{\stackrel{#1}{\smash{\arrONarr}}}
%\newcommand\seTilearrow[2]{\searrow\xxx\xx\searrow{\mathsf{#1}_{#2}^{\mathstrut}}}

% NE staff
%\newcommand\mrklab[1]{\diagopername{#1}}
\newcommand\neTilearrowAB[2]{\mrklab{#1}
           \lefteqn{\,\nearrow\xxx\xx\nearrow}{\mrklab{#2}}
}
\newcommand\neqExeLabel{\neTilearrow{qEx}{e}}
\newcommand\seqExeLabel{\seTilearrow{qEx}{e}}
\newcommand\sevExeLabel{\seTilearrow{vEx}{e}}
\newcommand\nevExeLabel{\neTilearrow{vEx}{e}}
\newcommand\nePBLabel{\neTilearrow{p}{b}}
\newcommand\sePBLabel{\seTilearrow{p}{b}}
\newcommand\neCommLabel{\neTilearrow{[;]}{\xx}}
% SE staff
%\newcommand\seTilearrow[2]{\mrklab{#1}
%           \lefteqn{\searrow\xxx\xx\searrow}{\mrklab{#2}}
%}



\newcommand\seTilearrowHru[1]{%\mrklab{#1}
%           \lefteqn{\searrow\xxx\xx\searrow}{\mrklab{#2}}
 \lefteqn%
 {~~#1}{\searrow\xxx\xx\searrow}
} %
%%%% Oct 13 %%%%%
%\renewcommand\seTilearrowHru[1]{%\mrklab{#1}
%%           \lefteqn{\searrow\xxx\xx\searrow}{\mrklab{#2}}
% \lefteqn%
% {#1}{\searrow\xxx\xx\searrow}
%} %
%%%%%%%%%%%%%%%



%\newcommand\swTilearrowHru[1]{%\mrklab{#1}
%%           \lefteqn{\searrow\xxx\xx\searrow}{\mrklab{#2}}
% \lefteqn%
%         {~~#1}{\swarrow\xxx\xx\swarrow}
%}

\newcommand\ssTilearrow[2]{\downarrow\xxx\xx\downarrow^{#1_{#2}^{\mathstrut}}}
\newcommand\ssTilearrowHru[1]{\lefteqn%
{~~#1} \downarrow\xx\xx\downarrow}

% short names
\newcommand\seTilelabel[1]{\seTilearrowHru{#1}}
\newcommand\swTilelabel[1]{\swTilearrowHru{#1}}
\newcommand\ssTilelabel[2]{\ssTilearrowHru{#1}}


\newcommand\sefPrpLabel{\seTilearrow{[fPp}{]}}

% SW stuff
%\newcommand\swTilearrow[2]{\mrklab{#1}
%           \lefteqn{\mrklab{#2}}{\swarrow\xxx\xx\swarrow}
%}

%\renewcommand\swTilearrow[2]{{#1}
%           %\lefteqn
%           {\swarrow\xxx\xx\swarrow}{{#2}}
%}

\newcommand\swbPrpLabel{\swTilearrow{[bPp}{]}}

%\newcommand\swTilearrow[2]{\swarrow\xxx\xx\swarrow^{#1_{#2}^{\mathstrut}}}
% NN stuff
\newcommand\nnTilearrow[2]{\downarrow\xxx\xxx\xx\downarrow^{#1_{#2}^{\mathstrut}}}
\renewcommand\nnTilearrow[2]{\mrklab{#1}\!
           \lefteqn{\uparrow\xxx\xx\uparrow}{\mrklab{#2}}
}
%\renewcommand\nnTilearrow[2]{\mrklab{#1}^{
%              {\uparrow}\!{\uparrow}
%            } %{\mrklab{#2}}
%}
\newcommand\nnsubstLabel{\nnTilearrow{subst~}{}}

\newcommand\seselabel{~~~\seTilearrow{}{}~~~}
\newcommand\swswlabel{~~~\swTilearrow{}{}~~~}



\newcommand\rBlockarrow{\rule{0.25pt}{4.pt}\xx\Rrightarrow}
\newcommand\lBlockarrow{\Lleftarrow\xx\rule{0.25pt}{4.pt}}
\newcommand\sBlockarrow{\downarrow\xx\downarrow\xx\downarrow}
\renewcommand\sBlockarrow{\Downarrow\xxx\Downarrow}
\newcommand\rBlockarrowII{\mbox{$\sqsubset\xx\sqsupset$}\xx\LARGE{\rhd}}


==> macros/4lenses/macros4spaceNames.tex <==
\newcommand\colfunct{\ensuremath{\mathsf{Col}}}

% now spaces
\newcommand\metamodname[1]{\ensuremath{\mathsf{#1}}}
\renewcommand\metamodname[1]{\ensuremath{{\pmb{#1}}}}
\newcommand\metamapsymb[1]{\ensuremath{\pmb{#1}}}
\newcommand\classname[1]{\ensuremath{\pmb{#1}}}  %\itshape{\textbf{#1}}}
\newcommand\spacenam[1]{\ensuremath{\mathbf{#1}}}
%\newcommand\spacenamind[1]{\mathbf{#1}}
%\newcommand\arralgnam[1]{\ensuremath{{\pmb #1}}}
%\newcommand\spaalt{\arralgnam{alt}}

\newcommand\cfwkclass{\classname{CFwk}}
\newcommand\scclass{\classname{SCase}}
\newcommand\T{\classname{T}}

\newcommand\spaA{\ensuremath{\spacenam{A}}}
\newcommand\spaB{\ensuremath{\spacenam{B}}}
\newcommand\spaC{\ensuremath{\spacenam{C}}}

\newcommand\mmm{\ensuremath{\metamodname{M}}}
\newcommand\mmmd{\ensuremath{\mmm_\Delta}}
\newcommand\mmmdpri{\ensuremath{\mmm_\Delta^\priv}}
\newcommand\mmmdpub{\ensuremath{\mmm_\Delta^\pub}}
\newcommand\mmmob{\ensuremath{\mmm_\bullet}}
\newcommand\mmn{\ensuremath{\metamodname{N}}}
\newcommand\mmmn{\ensuremath{\metamodname{N}}}
\newcommand\mmnd{\ensuremath{\mmn_\Delta}}
\newcommand\mmndpri{\ensuremath{\mmn_\Delta^\priv}}
\newcommand\mmndpub{\ensuremath{\mmn_\Delta^\pub}}
\newcommand\mmnob{\ensuremath{\mmn_\bullet}}
\newcommand\mmmnob{\mmnob}
\newcommand\mmi{\ensuremath{\metamodname{I}}}
\newcommand\mmid{\ensuremath{\mmi_\Delta}}
\newcommand\mmiob{\ensuremath{\mmi_\bullet}}
\newcommand\mmj{\ensuremath{\metamodname{J}}}
\newcommand\mmjd{\ensuremath{\mmj_\Delta}}
\newcommand\mmjob{\ensuremath{\mmj_\bullet}}
\newcommand\mmo{\ensuremath{\metamodname{O}}}
\newcommand\mmr{\ensuremath{\metamodname{R}}}
\newcommand\mmrop{\ensuremath{\metamodname{R}^{{\circ}}}}
\newcommand\mmkop{\ensuremath{\metamodname{K}^{{\circ}}}}
\newcommand\mmrr{\ensuremath{\mmr_\bullet}}
\newcommand\mmrl{\ensuremath{{_\bullet}\mmr}}
\newcommand\mmk{\ensuremath{\metamodname{K}}}
\newcommand\mmkr{\ensuremath{\mmk_\bullet}}
\newcommand\mmkl{\ensuremath{{_\bullet}\mmk}}

\newcommand\mml{\ensuremath{\metamodname{L}}}
\newcommand\mms{\ensuremath{\metamodname{S}}}
\newcommand\mmsd{\ensuremath{\mms_\Delta}}
\newcommand\mmsob{\ensuremath{\mms_\bullet}}
\newcommand\mmv{\ensuremath{\metamodname{V}}}
\newcommand\mmvd{\ensuremath{\mmv_\Delta}}
\newcommand\mmld{\ensuremath{\mml_\Delta}}
\newcommand\mmrd{\ensuremath{\mmr_\Delta}}
\newcommand\mmvob{\ensuremath{\mmv_\bullet}}
\newcommand\mmrob{\ensuremath{\mmr_\bullet}}
\newcommand\mmlob{\ensuremath{\mml_\bullet}}
%\newcommand\ma{\trajectname{A}}
%\newcommand\mb{\trajectname{B}}

\newcommand\mmq{\metamodname{Q}}
%\newcommand\mmr{\metamodname{R}}
\newcommand\mmmrn{\metamodname{MRN}}

\endinput

\newcommand\mma[1]{\ensuremath{\metamodname{A}_{#1}}}
\newcommand\mmb[1]{\ensuremath{\metamodname{B}_{#1}}}
\newcommand\mmc[1]{\ensuremath{\metamodname{C}_{#1}}}
\newcommand\mmm[1]{\ensuremath{\metamodname{M}_{#1}}}
\renewcommand\mmm[1]{\ensuremath{\metamodname{V}_{#1}}}
\newcommand\mmn[1]{\ensuremath{\metamodname{N}_{#1}}}
\renewcommand\mmn[1]{\ensuremath{\metamodname{S}_{#1}}}
\newcommand\mmo[1]{\ensuremath{\metamodname{O}_{#1}}}
\newcommand\mmr[1]{\ensuremath{\metamodname{R}_{#1}}}
\newcommand\mmk[1]{\ensuremath{\metamodname{K}_{#1}}}
\newcommand\mms[1]{\ensuremath{\metamodname{S}_{#1}}}
\newcommand\mmv[1]{\ensuremath{\metamodname{V}_{#1}}}



\newcommand\mmmsub[1]{\ensuremath{\metamodname{M}^-_{#1}}}
\newcommand\mmnsub[1]{\ensuremath{\metamodname{N}^-_{#1}}}

\newcommand\mmmton{\metamodname{M_N}}
\newcommand\mmmx{\metamodname{M_N}}



%\newcommand\mmo{\metamapsymb{O}}
%\newcommand\mmr{\metamapsymb{r}}
%\newcommand\mmu{\metamapsymb{u}}
%\newcommand\mmv{\metamapsymb{v}}

% dyn metamod
\newcommand\dmmm[1]{\ensuremath{\spacenam{M}_{#1}}}
\newcommand\dmmn[1]{\ensuremath{\spacenam{N}_{#1}}}
\newcommand\dmmo[1]{\ensuremath{\spacenam{O}_{#1}}}


==> macros/document.tex <==
\definechangesauthor[name={Zinovy}, color=blue]{zd}




\newcommand{\mynote}[2]{
    \fbox{\bfseries\sffamily\scriptsize#1}
    {\small$\blacktriangleright$
    \textcolor{blue}{\textsf{\emph{#2}}}
    $\blacktriangleleft$}}
\newcommand\kb[1]{\mynote{KB}{#1}}
\newcommand\zd[1]{\mynote{ZD}{#1}}
\newcommand\hq[1]{\mynote{H}{#1}}
\newcommand\zdzd[1]{\mynote{ZD}{#1}}
\newcommand\ma[1]{\mynote{MA}{#1}}
\newcommand\mannum{\xspace}

% Zinovy's macros
%  to disable them,   comment \endinput command far below

\newcommand\hg[2]{\hgmargin{#1}\textcolor{blue}{#2}}

%== margin notes
\newcommand\mymarginfoot[1]{ % #1 - the author #2 - the text
           \footnote{{{\textit{{\footnotesize #1}}}} }}
\newcommand\mymarginnew[1]{%
                     \marginpar{\vspace{-1em}\flushleft\textit{\footnotesize\textcolor{blue} {#1}}}} 
    \newcommand\mymarginNew[2]{%
    	\marginpar{\vspace{#2}\flushleft\textit{\footnotesize\textcolor{blue} {#1}}}}    
       
       
       
       
\newcommand\zdmargin[1]{\mymarginnew{ZD:~#1}}
\newcommand\zdmarginNew[2]{\mymarginnew{ZD:~#1}{#2}}
\newcommand\skmargin[1]{\mymarginnewpurple{SK:~#1}}


% highlighting
\newcommand\hlight[2]{%
\textcolor{blue} {#1} % #1 - the piece to highlught
 {\mymarginnew{#2}} %#2 - margin note
 }
\newcommand\hlightNew[3]{%
	\textcolor{blue} {#1} % #1 - the piece to highlught
	{\mymarginNew{#2}{#3} %#2 - margin note
}}

 \newcommand\hlightpurple[2]{%
\textcolor{blue} {#1} % #1 - the piece to highlught
 {\mymarginnew{#2}} %#2 - margin note
 }

\newcommand\zdhlight[2]{\hlight{#1}{ZD:~#2}}
\newcommand\zdhl[2]{\hlight{#1}{ZD:~#2}}
\newcommand\zdhll[3]{\hlightNew{#1}{ZD:~#2}{#3}}


\newcommand\awhlight[2]{\hlight{#1}{AW:~#2}}
\newcommand\skhlight[2]{\hlightpurple{#1}{SK:~#2}}
\newcommand\zdnew[2]{\hlight{#1}{ZD:~#2}}
\newcommand\zdnewok[2]{{#1}}
\newcommand\sknew[2]{\hlightpurple{#1}{SK:~#2}}

% text modification
\def\modiffy#1#2#3#4#5{%
{\small\underline{\sf{#1}}}% the author
{{#2}}% the piece to delete
{%\textcolor{red}
\mymarginnew{#3}}% reason why
{#4 }%separator
{{#5}}% the piece to insert
}%
% separators
\newcommand\interArrow{\textcolor{red}{\mbox{$\Rightarrow$}}}
\renewcommand\interArrow{{}}
% specializing modiffy
\newcommand{\modify}[3]{%  #1 the piece to delete, #2--insert, #3--margin note
\modiffy{}%#1
{\textcolor{red}{\sout{#1}}}%#2
{\textcolor{blue}{#3}\vspace{-5em}}%#3 do not forget to place here your initials, say, ZD:
{\interArrow}%#4
{\textcolor{blue}{#2}}%#5
}
%

%==========
% text modification
\def\modiffyNew#1#2#3#4#5#6{%
	{\small\underline{\sf{#1}}}% the author
	{{#2}}% the piece to delete
	{%\textcolor{red}
		\mymarginNew{#3}{#6}}% reason why
	{#4 }%separator
	{{#5}}% the piece to insert
	%{#6}
}%
% separators
%\newcommand\interArrow{\textcolor{red}{\mbox{$\Rightarrow$}}}
\renewcommand\interArrow{{}}

% specializing modiffyNew
\newcommand{\modifyNew}[4]{%  #1 the piece to delete, #2--insert, #3--margin note
	\modiffyNew%
	{}%#1
	{\textcolor{red}{\sout{#1}}}%#2
	{\textcolor{blue}{#3}}%#3 do not forget to place here your initials, say, ZD:
	%{{#3}}
	{}%#4
	{\textcolor{blue}{#2}}%#5
	{#4} % #6
}
%


\newcommand\zdmod[3]{\modify{#1}{#2}{ZD:~#3}}
\newcommand\zdmodd[4]{\modifyNew{#1}{#2}{ZD:~#3}{#4}}
\newcommand\skmod[3]{\modify{#1}{#2}{SK:#3}}

\newcommand\zdmodok[3]{\modifyok{#1}{#2}{ZD:#3}}
\newcommand\zdmoddok[3]{\modiffyok{#1}{#2}{ZD:#3}}

\newcommand\zdmodno[3]{\modifyno{#1}{#2}{ZD:#3}}
\newcommand\zdmoddno[3]{\modiffyno{#1}{#2}{ZD:#3}}

\newcommand{\modifyok}[3]{{#2}}
\newcommand{\modiffyok}[4]{{#2}}

\newcommand{\modifyno}[3]{{#1}}
\newcommand{\modiffyno}[4]{{#1}}


\newcommand\hgmod[3]{\modify{#1}{#2}{H:#3}}
\newcommand\hgmodok[3]{\modifyok{#1}{#2}{ZD:#3}}
\newcommand\hgmodno[3]{\modifyno{#1}{#2}{ZD:#3}}

% new  stuff
\newcommand{\new}[2]{%
\modiffy{}{} %#1,#2
{\textcolor{blue}{#2}}%#3 do not forget to place here your initials, say, ZD:
{}%#4
{\textcolor{blue}{#1}}%#5
}
%
\newcommand\newok[2]{#1}
\newcommand\newno[2]{}


\endinput

% == remove comments by
\renewcommand\zdmargin[1]{}
\renewcommand\zdmod[3]{#2}
\renewcommand\skmargin[1]{}
\renewcommand\hlight[2]{#1}
\renewcommand\modify[3]{{#2}}
\renewcommand\modiffy[5]{{#5}}
\renewcommand\new[2]{{#1}}{}
%\renewcommand\del[2]{}
%\renewcommand{\zdmodify}[3]{{#2}}


\endinput

\renewcommand{\yxmodify}[2]{{#2}}
\renewcommand{\yxmodiffy}[3]{{#3}}
\renewcommand{\zdmodify}[2]{{#2}}
\renewcommand{\kcmodify}[2]{{#2}}
%\renewcommand\zdmargin[1]{}
\renewcommand\yxmargin[1]{}


==> macros/macros-general-prev.tex <==
% == rotation command
%\rotatebox[origin=c]{45}{$xxx$} 
\newcommand\qqquad{\qquad\quad}
\newcommand\qqqquad{\qquad\qquad}
%\newcommand{\tmapleft[2]}{\ensuremath{#1}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% == my font discipline for defs for Springer ==

\newenvironment{defin}[1][]{\ifthenelse{\equal{#1}{}}{\definition}{\definition[#1]}\rm}{\enddefinition}
\newenvironment{propo}[1][]{\ifthenelse{\equal{#1}{}}{\proposition}{\proposition[#1]}\rm}{\endproposition}
\newenvironment{remar}[1][]{\ifthenelse{\equal{#1}{}}{\remark}{\remark[#1]}\rm}{\endremark}
% \newtheorem{defin}{Definition}
% \newtheorem{corol}{Corollary}
% \newtheorem{theorem}{Theorem}
% \newtheorem{propo}{Proposition}
% \newtheorem{rema}{\textit{Remark}}
% \newtheorem{example}{Example}

%% ATTENTION PLS !
%  for Elsevieer, the above macros don't work, but versions below do work
% \let\oldexample=\example
% \let\endoldexample=\endexample
% \renewenvironment{example}{\vspace{-0.6em}\begin{oldexample}}{\end{oldexample}\vspace{-0.35em}}

% \let\olddefin=\defin
% \let\endolddefin=\enddefin
% \renewenvironment{defin}{\vspace{-0.6em}\begin{olddefin}}{\end{olddefin}\vspace{-0.5em}}

% \let\oldpropo=\propo
% \let\endoldpropo=\endpropo
% \renewenvironment{propo}{\vspace{-0.6em}\begin{oldpropo}}{\end{oldpropo}\vspace{-0.5em}}

% \let\oldrema=\rema
% \let\endoldrema=\endrema
% \newenvironment{rema}{\vspace{-0.6em}\begin{oldrema}}{\end{oldrema}\vspace{-0.5em}}

% \let\oldcorol=\corol
% \let\endoldcorol=\endcorol
% \newenvironment{corol}{\vspace{-0.6em}\begin{oldcorol}}{\end{oldcorol}\vspace{-0.5em}}

% \let\oldtheorem=\theorem
% \let\endoldtheorem=\endtheorem
% \renewenvironment{theorem}{\vspace{-0.6em}\begin{oldtheorem}}{\end{oldtheorem}\vspace{-


% math operations

\newcommand\opname[1]{\ensuremath{\mathsf{#1}}}
\newcommand\colim{\opname{colim}}
\newcommand\limcat{\opname{lim}}

%===== Calligraph. Literals ======
\newcommand\niceletter[1]{\ensuremath{{\cal #1}}}
\newcommand\nicex[1]{\niceletter{#1}}
\newcommand\nia{\nicex{A}}
\newcommand\nib{\nicex{B}}
\newcommand\nid{\nicex{D}}
\newcommand\nie {\nicex{E}}
\newcommand\nik {\nicex{K}}
\newcommand\nil {\nicex{L}}
\newcommand\nim{\nicex{M}}

\newcommand\nio{\nicex{O}}
\newcommand\nip{\nicex{P}}
\newcommand\nir{\nicex{R}}
\newcommand\nit{\nicex{T}}
\newcommand\niu{\nicex{U}}
\newcommand\niw{\nicex{W}}
\newcommand\nix{\nicex{X}}


% Domain-codomain/source-target/ident
\newcommand\cod[1]{\ensuremath{{#1}^\bullet}}
\newcommand\dom[1]{\ensuremath{^\bullet{#1}}}
\newcommand\so{\ensuremath{\mathsf{src}}}
\newcommand\ta{\ensuremath{\mathsf{trg}}}
\renewcommand\so{\ensuremath{\mathsf{s}}} % was src
\renewcommand\ta{\ensuremath{\mathsf{t}}}  % was trg
\newcommand\ldom[1]{\ensuremath{$\Box #1 $}}
\newcommand\rdom[1]{\ensuremath{$#1 \Box $}}
\newcommand\id[1]{\opname{id}_{{#1}}}
\renewcommand\id{\opname{id}}

% fig and others references
\newcommand\figref[1]{Fig.~\ref{#1}}
\newcommand\exref[1]{Ex.~\ref{#1}}
\newcommand\defref[1]{Definition~\ref{#1}}
\newcommand\tabref[1]{Table~\ref{#1}}
\newcommand\diagref[1]{(\ref{#1})}
%\newcommand\eqref[1]{\ref{#1}}
\newcommand\sectref[1]{Sect.~\ref{#1}}
\newcommand\secref[1]{Sect.~\ref{#1}}
\newcommand\appref[1]{Appendix~\ref{#1}}
%\newcommand\eqref[1]{(\ref{#1})}
%===============================================


% my macros for Formulas 

% roman font in math formulas
\newcommand\rmand{\mbox{ and }}
\newcommand\rmor{\mbox{ or }}
\newcommand\rmxor{\mbox{ xor }}

\newcommand\eqdef{\ensuremath{\stackrel{\mathrm{def}}{=}}}

% semantic brackets 
\newcommand\respace{\!}%\!\!}
\newcommand\lsemm{\left[ \respace\left[ }
\newcommand\rsemm{\right]\respace\right]}
\newcommand\semm[1]{\mbox{$\lsemm\, \mathit{#1} \, \rsemm$}}

% less blank space
\newcommand\timm{{\times}}
\newcommand\inn{{\in}}
\newcommand\subsett{{\subset}}
\newcommand\supsett{{\superset}}

%Suggestive Names for MathSymbols
\newcommand\superset{\supset}
\newcommand\subeq{{\subseteq}}
\newcommand\supeq{{\supseteq}}
\newcommand\sqsubeq{{\sqsubseteq}}
\newcommand\sqsupeq{{\sqsupseteq}}
\newcommand\varno{{\varnothing}}
\newcommand\subsetarr{\ensuremath{\hookrightarrow}}
\newcommand\supsetarr{\ensuremath{\hookleftarrow}}

\newcommand\this{\ensuremath{\underline{\mathrm{this}}}}
\newcommand\self{\ensuremath{\underline{\mathrm{self}}}}


\newcommand\ovr[1]{\ensuremath{\overline{#1}}}
\newcommand\und[1]{\ensuremath{\underline{#1}}}


\newcommand\rarr{{\rightarrow}}
%\newcommand\lar{\leftarrow}
\newcommand\larr{{\leftarrow}}
\newcommand\ifff{\Leftrightarrow}
\newcommand\iffarrow{\Leftrightarrow}
\newcommand\bottom{\perp}
\newcommand\disj{\vee}
\newcommand\sdisj{\stackrel{!}{\vee} }
\newcommand\conj{\wedge}
%\newcommand\mathand{\,\&\,}
\renewcommand\neg{\sim}
\newcommand\ded{\vdash}
\newcommand\semded{\models}
\newcommand\synent{\ensuremath{\vdah}}
\newcommand\sement{\ensuremath{\models}}

\newcommand\njoin[2]{\mathbin{${#1}\triangleright\!\triangleleft\;{#2}$}}

%\newcommand\ifthenelse[3]{{\bf if}#1{\bf then}#2{\bf else}#3}


\newcommand\true{\nmf{true}}
\newcommand\false{\nmf{false}}

% Operations 

\newcommand\image[2]{\opname{Image}_{#1}{#2}}
\newcommand\img[2]{\image{#1}{#2}}
%\newcommand\range[2]{\Operation{Range}_{#1}({#2})}

%\newcommand\aut{\ensuremath{\operation{Aut}}}
\newcommand\isoind{\opname{iso}}
\newcommand\iso{\isoind}

\newcommand\coimage[2]{\opname{CoIm}_{#1}{#2}}
\newcommand\coim[2]{\coimage{#1}{#2}}

\renewcommand\restriction[2]{#1\left\lceil_{#2}\mathstrut\right.}
\renewcommand\restriction[2]{#1\upharpoonright_{#2}\mathstrut}
\newcommand\restr[2]{\restriction{#1}{#2}}

\newcommand\idmap[1]{\Operation{id}_{#1}}

\newcommand\Inverse[1]{\left (\mathstrut {#1} \right )^{-1}}
%\newcommand\inverse[1]

%  Comprehension

\newcommand\comprehension[2]{\ensuremath{\left\{{#1}\left|\;{#2}\right.\right\}}}
\renewcommand\comprehension[2]{\ensuremath{\left\{{#1}| \;{#2}\right\}}}  % big brackets
\renewcommand\comprehension[2]{\ensuremath{\{{#1}| \;{#2}\}}}
\newcommand\compr[2]{\comprehension{#1}{#2}}
\newcommand\tuplecompr[2]
{\left\langle{#1}\left|\;{#2}\right.\right\rangle}
\newcommand\tuple[1]{\left\langle\mathstrut {#1}\right\rangle}
\newcommand\cotuplecompr[2]
{\left\rangle\mathstrut {#1}\left|\;{#2}\right.\right\langle}
\newcommand\cotuple[1]{\left\rangle\mathstrut {#1}\right\langle\;}
\newcommand\family[2]{\left(\mathstrut #1 \right)_{#2}}
\newcommand\famm[2]{\family{#1}{#2}}
% big brackets
\newcommand\comprfam[2]{\left(\mathstrut{#1}\left|\;{#2}\right.\right)}
\newcommand\famcompr[2]{\left(\mathstrut{#1}\left|\;{#2}\right.\right)}
% normal brackets
\renewcommand\comprfam[2]{(\mathstrut{#1}\left|\;{#2}\right.)}
\renewcommand\famcompr[2]{(\mathstrut{#1}\left|\;{#2}\right.)}
\newcommand\newfamm[2]{\compfamily{#1}{#2}}
\newcommand\arrfamm[4]{\family{%
		\lar{#1}{#2}{#3}%
	}{#4}}


\newcommand\cotimes{+}
\newcommand\noteq{\ne}
\newcommand\mybigcup[2]{\bigcup\compr{#1}{#2}}
\newcommand\mybigcap[2]{\bigcap\compr{#1}{#2}}

\newcommand\myprod[1]{{#1 \prod}}



%-- categories names
\newcommand\catname[1]{\mbox{\bfseries\itshape #1}}
%\newcommand\cat[1]{\catname{#1}}
\newcommand\catnameind[1]{{\pmb #1}}
\newcommand\categoryop[1]{\mbox{\bfseries\itshape #1}$^{\mathrm{op}}$}



%\renewcommand\cat[1]{\catname{#1}}
\newcommand\CC{\catname{C}}

\newcommand\graphcat{\catname{Graphs}}
\newcommand\setcat{\catname{Set}}
\newcommand\twocat{\catname{2}}
\newcommand\relcat{\catname{Rel}}
\newcommand\catcat{\catname{Cat}}
\newcommand\natset{\catname{Nat}}
\newcommand\gracat{\catname{Graphs}}
\newcommand\rgracat{\catname{rGraphs}}
\newcommand\twogracat{\catname{2Graphs}}
\newcommand\dbgracat{\catname{dblGraphs}}
\newcommand\posetcat{\catname{Posets}}
\newcommand\reprcat{\catname{Repr}}
\newcommand\schemacat{\catname{Schema}}
%\newcommand\catname[1]{\mbox{\boldmath $#1$}}



%=== word shorcuts
% \newcommand\eg{e.g.}
% \newcommand\ie{i.e.}
% \newcommand\etal{\textit{et al}}
%\newcommand\fwk{framework}
%\newcommand\traj{trajector}
%\newcommand\traj{trajector}
%\newcommand\syncon{synchronization}
%\newcommand\Syncon{Synchronization}
\newcommand\symmen{symmetrization}
\newcommand\Symmen{Symmetrization}


\endinput




\setlength{\marginparwidth}{3cm}
%\setlegth{\marginparsep}{1.5mm}
%\setlength{\marginparpush}{5mm}
%

\makeatletter
  \def\fps@figure{tp}
\makeatother

\newcommand{\backgro}[2]{\par\noindent\framebox[\textwidth]{
\begin{minipage}{0.98\textwidth}
\setlength{\parindent}{0.5cm} \noindent \textbf{Background: #1} #2
\end{minipage}}\smallskip}

%%%% macros %%%
%\newtheorem{defin}{Definition}%[section]
%\renewcommand{\thedefin}{\Alph{defin}}

\newcounter{defCounter}
\newenvironment{defin}[1][]{
\refstepcounter{defCounter}
\begin{trivlist}
\item[\hskip \labelsep {\bfseries Definition \arabic{defCounter} (#1) }]}%
{\end{trivlist}}



%\newcommand\xxx[4]{{\it #1}\mbox{$_{#3}^{#4}{#2}$}}
%\newcommand{\s}{\star}
%\newcommand\mrk[1]{\mbox{$\langle${\tt #1}$\rangle$}}
%=================================================
% 1  Fonts and letters
%============================================

%=====================================================
% 2  Mathematical shtuchki
%=========================================================


% New Symbols allowed to use in MathMode (!)
%========= General =============
\newcommand\mylist[2]{\mbox%
                          {$#1_1,\ldots,#1_{#2}$}}

\newcommand\iidots[2]{\mbox{
                            $#1=1,\ldots,#2$
                      }}
\newcommand\ijdots[3]{\mbox{
                            $#1=#2,\ldots,#3$
                      }}
\newcommand{\vare}{\varepsilon}
\newcommand\nr{\normalsize\rm}
\newcommand\tril{\triangleleft}
\newcommand\eqdef{\stackrel{\rm def}{=}}
\newcommand\trir{\triangleright}
\newcommand\bc{\bigcirc}







%(4)%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  Abbreviations of words from pre_gen
%%%%%%%%%%%%%%%%%%%%%

%\newcommand\ql{query \lan} comment for ISMIS'96
\newcommand\sync{synchronous}
\newcommand\async{asynchronous}
\newcommand\syncn{synchronization}
\newcommand\syncd{synchronized}
\newcommand\Sync{Synchronous}
\newcommand\Async{Asynchronous}
\newcommand\Syncn{Synchronization}
\newcommand\Syncd{Synchronized}

\newcommand\sce{scenario}

\newcommand\eqe{equivalence}
\newcommand\eqt{equivalent}

\newcommand\intn{intuition}
\newcommand\intv{intuitive}
\newcommand\coa{coalgebra}
\newcommand\ispartof{\ittt{isPartOf}}
\newcommand\isPartOf{\ittt{isPartOf}}
\newcommand\IsPartOf{\ittt{isPartOf}}

\newcommand\of{\ittt{(isPart)Of}}
\newcommand\Of{\ittt{Of}}
\newcommand\arrdl{ArrDL}
\newcommand\elmsl{ElmSL}

\newcommand\isa{\ittt{isA}}
\newcommand\IsA{\ittt{isA}}
\newcommand\isA{\ittt{isA}}


\newcommand\subst{\ittt{subst}}


\newcommand\OOAD{OOA\&D}
\newcommand\oid{o-id}

\newcommand\pred{predicate}

\newcommand\interstan{interstate relation}
\newcommand\intrel{interstate relation}
\newcommand\demon{demonstration}
\newcommand\demoe{demonstrate}
\newcommand\asson{association}
\newcommand\config{configuration}
\newcommand\asscon{association configuration}
\newcommand\ass{associative}
\newcommand\assive{associative}
\newcommand\aggrn{aggregation}
\newcommand\attrn{attribution}
\newcommand\abbrn{abbreviation}
\newcommand\gen{generalization}
\newcommand{\iden}{identification}
\newcommand\idey{identity}
\newcommand\qualn{qualification}
\newcommand\reprn{representation}
\newcommand\situn{situation}
\newcommand\speln{specialization}
\newcommand\spen{specialization}
\newcommand\spel{specialization}
\newcommand\spec{specification}
\newcommand\implen{implmentation}
\newcommand\impleg{implmenting}
\newcommand\strul{structural} %\strul

\newcommand\spenisa{\spen\ \isa-arrow}
\newcommand\genisa {\gen\  \isa-arrow}

\newcommand\visun{visualization}


%\newcommand\gen{generalization}
\newcommand\repr{representation}

\newcommand\visn{visualization}


%\newcommand{\oid}{object identity}
\newcommand{\oids}{object identities}



\newcommand\datamod[1]{{\rm #1}}

\newcommand\ERC{\datamod{ERC\mbox{$^+$}}}
\newcommand\ercd{\ERC-diagram}
\newcommand\ER{\datamod{ER}}
\newcommand\EER{\datamod{EER}}
\newcommand\RM{\datamod{RM}}
\newcommand\RMT{\datamod{RM/T}}
\newcommand\RDM{\datamod{RDM}}
\newcommand\VO{\datamod{VO}}
\newcommand\OOO{\datamod{OO}}
\newcommand\SDM{\datamod{SDM}}
\newcommand\FDM{\datamod{FDM}}
\newcommand\IFO{\datamod{IFO}}
\newcommand\Oid{\datamod{Oid}}
\newcommand\RO{\datamod{RO}}
\newcommand\ROP{\datamod{RO\mbox{$^+$}}}
\newcommand\Flogic{\datamod{F-logic}}
\newcommand\SkeDM{\datamod{SkeDM}}
\newcommand\Diagr{\datamod{Diagrams}}

\newcommand\datatrend[1]{{\bf #1}}

\newcommand\eer{\datatrend{eer}}
\newcommand\ooo{\datatrend{oo}}
\newcommand\pl{\datatrend{pl}}
\newcommand\skeske{\datatrend{ske}}

\newcommand\msour{multisource}
\newcommand\sour{source}

\newcommand\abbr{abbreviat}
\newcommand\lega{legacyless}


\newcommand\Ass{Associative}



\newcommand{\ider}{identifier}
\newcommand{\deor}{descriptor}

\newcommand\dombs{domain-based sketch}
\newcommand\ms{multisource}
\newcommand\mt{multitarget}
\newcommand\refin{refinement}
\newcommand\db{database}
\newcommand{\grab}{graph-based }
\newcommand{\spef}{specification}
%\newcommand\spec{specification}
\newcommand{\grabs}{\grab\spef}
\newcommand{\lan}{language}
\newcommand{\sgd}{\spel$\!$/\gen distinction }
\newcommand\qr{query }
\newcommand\qrs{queries}

%%%%% Integration %%%%%%%%%%%%%

\newcommand{\integ}{integration}
\newcommand{\intd}{integrated}
\newcommand{\di}{data integration }
\newcommand{\dbi}{database integration }
\newcommand{\vi}{view integration }
\newcommand{\si}{schema integration}
\newcommand{\sdi}{schema and data integration }
%-------------------------------------
\newcommand{\cmod}{conceptual modeling}
\newcommand{\smod}{semantic modeling}
\newcommand{\dbs}{data base}
\newcommand{\dml}{data model}
%\newcommand{\dm}{data model}%{dm}%{DM} % an abbreviation
\newcommand\const{constraint}
\newcommand{\attr}{attribute}
%=====================================
\newcommand\cdb{component \db}
\newcommand\dincy{data inconsistency}
\newcommand\corr{correspondence}
\newcommand\lang{language}
%------
\newcommand\corinf{correspondence information}
\newcommand\corrinf{correspondence information}

\newcommand\coras{correspondence assertion}
\newcommand\corass{correspondence assertions}
\newcommand\corda{correspondence data}
\newcommand\coreq{\corr\ equation}
\newcommand\coreqs{\corr\ equations}

\newcommand\dacorr{data \corr}
\newcommand\cors{\corr\ \ske}
\newcommand\corss{\corr\ \skes}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\relship}{relationship}
%----------------------------------------
\newcommand{\Spc}{Spaccapietra {\em et al} }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\ske{sketch}
\newcommand\skes{sketches}
\newcommand\cske{component sketch}
\newcommand\cskes{component sketches}
\newcommand\eroo{\cite{ER95}}
%%%%%%%%%%%% Romanic abbreviations  %%%%%%%%%%%%
\newcommand\eg{e.g.}
\newcommand\ie{i.e.}
\newcommand\wrt{w.r.t.}
\newcommand\etc{{\em etc}}
\newcommand\etal{{\em et al}}
\newcommand\ala{{\em a la }}
\newcommand\apriori{{\em a priori}}
\newcommand\adhoc{{\em ad hoc}}
\newcommand\dejure{{\em de jure}}
\newcommand\defacto{{\em de facto}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\newcommand{\sign}{signature}
%\newcommand{\constr}{constructivizab}% *le or *ility
%\newcommand{\cat}{category}
%\newcommand{\cats}{categories}
%\newcommand{\ct}{category theory\ } %y or ies
%\newcommand\mor{morphism}
%\newcommand\amor{automorphism}
%\newcommand\alg{algebra}
%%\newcommand\inst{institution}
%=============================

%(5)\newcommand\entails{\Rightarrow}
%\newcommand\implies{\Rightarrow}
%-------------------------------------
%\newcommand\dom[1]{\mathit{Dom}(#1)}
%\newcommand\cod[1]{\mathit{Cod}(#1)}
\newcommand\rg[1]{\mathit{Rg}(#1)}
\newcommand\DOM[1]{\Box #1}
\newcommand\COD[1]{#1 \Box}

\newcommand\tabname[1]{\mbox{$\ittt{Tab}\_#1$}}
%\newcommand\multisource[
\newcommand\mytilde[1]{\widetilde{#1}}
\newcommand\sempr[1]{\mytilde{\semm{#1}}}

\newcommand\mycount[1]{{\bf count}{(#1)}}
\newcommand\gragen[1]{\left[\mathstrut #1 \right]}

\newcommand\respace{\!}%\!\!}
\newcommand\lsemm{\left[ \respace\left[ }
\newcommand\rsemm{\right]\respace\right]}
\newcommand\semm[1]{\mbox{$\lsemm\, \mathit{#1} \, \rsemm$}}
\newcommand\semmind[2]{\mbox{$\lsemm\, \mathit{#1} \, \rsemm^{#2}$}}



\newcommand\semmindex[1]{\lsemm\, \mathit{#1} \, \rsemm}
\newcommand\semmstar[1]{\semm{#1}^{*}}
\newcommand\lbesemm{\left< \respace\left<}
\newcommand\rbesemm{\right> \respace\right>}
\newcommand\besemm[1]{\mbox{$\lbesemm\, \mathit{#1} \, \rbesemm$}}



%(6)%\newcommand\informalPar[1]{\nicex{{#1}$}}
%\newcommand\infParind[1]{\cal #1}
%Contents:
%--- semiotics
%--- Skesig
%--- Varset
%--- Behset



%%==== Semiotics =====
%
%%\newcommand\formalPar[1]{\mbox{$\mathrm{#1}$}}
%\newcommand\frmParind[1]{\mathrm{#1}}
%
%\newcommand\informalParBold[1]{\mbox{${\cal #1}$}}
%\newcommand\formalPar[1]{\mbox{$\mathrm #1$}}
%
%\newcommand\object[2]{\mbox{${\mathsf{#1}}_{#2}$}}
%%\newcommand\object[2]{\mbox{$#1_{#2}$}}
%\newcommand\universe[1]{\mbox{$\mathbf{#1}$}}
%%\newcommand\objectind[1]{\mathsf{#1}}
%\newcommand\objectind[1]{\mathsf{#1}}
%\newcommand\universeind[1]{\mathbf{#1}}
%
%\newcommand\proc[1]{\mbox{\sffamily\bfseries #1}}
%\newcommand\procind[2]{\mbox{${\mathrm{#1}}_{\mathrm #2}$}}
%\newcommand\linf{\informalParBold{L}}
%\newcommand\minf{\mbox{$\informalPar{M}(\diag{})$}}
%\newcommand\mdinf{\mbox{$\informalPar{M}(\diag{})$}} % the same as above
%\newcommand\mdfrm{\mbox{$\formalPar{M}(\diag{})$}} % the same as above
%\newcommand\uinf{\informalPar{U}}
%
%\newcommand\meaninf{\informalPar{M}}
%\newcommand\meanfrm[1]{\mbox{$\formalPar{M}_{#1}$}}
%\newcommand\diag[1]{\object{D}{#1}} %\mbox{$D$}}
%\newcommand\diagob[1]{\object{D}{#1}} %\mbox{$D$}}
%\newcommand\diags{\mbox{$\mathit{Diags}$}}
%\newcommand\graph{\mbox{$\mathit{Graph}$}}
%\newcommand\skeob[1]{\object{S}{#1}}
%\newcommand\modelob[1]{\object{M}{#1}}
%\newcommand\sigob[1]{\object{\mbox{$\Sigma$}}{#1}}
%\newcommand\skediag{\skeob{}[\diag{}]}
%\newcommand\meaninfdiag{\meaninf[\diag{}]}
%\newcommand\meanfrmdiag{\meanfrm[\diag{}]}
%% synonyms
%\newcommand\meanifdiag{\meaninf[\diag{}]}
%\newcommand\meanfdiag{\meanfrm[\diag{}]}

%=======================
%==== Skesig
%\newcommand\so[1]{source(#1)}
%\newcommand\ta[1]{target(#1)}
\newcommand\U{{\cal U}}
\newcommand\M{{\cal M}}
\newcommand\Set{{\mathbf Set}}
\newcommand\Varset{{\mathbf Varset}}
\newcommand\univ{\mbox{$\mathbf U$}}
\newcommand\univind{{\mathbf U}}
\newcommand\skesig{\mbox{$\Sigma$}}

%%%% macro\Skesig.tex %%%%  June 29

\newcommand\mrkid{\mrk{ID}}
\newcommand\imID{\mbox{ID?}} %$^*$}}
\newcommand\mrkidd{\imID} % marker of IDDeficient
\newcommand\prodid{\mbox{$\times$-\ider}}
\newcommand\plusid{\mbox{$+$-\ider}}
\newcommand\prodkey{\mbox{$\times$-key}}
\newcommand\pluskey{\mbox{$+$-key}}

\newcommand\ID{\mrk{ID}}
\newcommand\IDplus{\mrk{ID$^+$}}
\newcommand\IDprod{\mrk{ID$^\times$}}

\newcommand\andiden{\emph{and}-\iden}
\newcommand\oriden{\emph{or}-\iden}


\newcommand\ssta{\mbox{${\mathsf S}_{\mathrm sta}$}}
\newcommand\sdyn{\mbox{${\mathsf S}_{\mathrm dyn}$}}

%\newcommand\mrk[1]{\mbox{[${\tt #1}$]}}
%\newcommand\mrk[1]{\mbox{[${\mathbf{#1}}$]}}
%\newcommand\mrkop[1]{\mbox{$\langle{\tt #1}\rangle$}}
\newcommand\mrkop[1]{\mbox{$\langle{\mathbf{#1}}\rangle$}}
\newcommand\mrkopr[1]{\mbox{$\mathbf{[{#1}\rangle}$}}
\newcommand\mrkopl[1]{\mbox{$\mathbf{\langle{#1}]}$}}
\newcommand\mrksemiop[1]{\mbox{$\langle{\tt #1}]$}}
\newcommand\mrkNode[1]{\mbox{${\tt #1}$}}
\newcommand\mrkn[1]{\mrkNode{#1}}
\newcommand\mrktt[1]{{\tt #1}}
\newcommand\mrkopright[1]{\mbox{$[${\tt #1}$\rangle$}}
\newcommand\mrkopleft[1]{\mbox{$\langle${\tt #1}$]$}}
%%%%%%%%%%%%%  Begin Key commands %%%%%%%%%%%%%%%%%%%%%%%

\newcommand\PredicateSignature{\Pi}
\newcommand\OperationSignature{\Sigma}
\newcommand\predFromOperSig{\Sigma_{pr}}
\newcommand\BaseSignature{\bf B}
\newcommand\DomainBase{\bf B}

\newcommand\ConstraintLanguage{CL}
\newcommand\dolan%DomainLanguage{\Delta}
{\mbox{$\Delta $}}

\newcommand\dolanm{\Delta}

\newcommand\adtm{ADT}
\newcommand\adt{{\sl \adtm}}
\newcommand\dolanadt{\dolan_{\adtm}}
\newcommand\sigadt{{\it Sig}_{\adtm}}
\newcommand\semmadt{\semm{}_{\adtm}}

\newcommand\dbauxm{DBD}
\newcommand\dbaux{{\sl \dbauxm}}
\newcommand\dolandbaux{\dolan_{\dbauxm}}
\newcommand\sigdbaux{{\it Sig}_{\dbauxm}}
\newcommand\semmdbaux{\semm{}_{\dbauxm}}

\newcommand\ba{D}
\newcommand\domba{\mbox{$\Domain(\ba)$}}
\newcommand\bam{\BasicDomainMarkerSymbol}          %  B  for using in math mode
%\newcommand\V{\mbox{$\TheValueUniverse_{\dolanm}$}}%

\newcommand\Pred{{\it Pred}}
\newcommand\Oper{{\it Op}}
\newcommand\Base{{\it Base}}
\newcommand\Dom{{\it Dom}}
\newcommand\Domain{{\it Dom}}
\newcommand\pool{V}

\newcommand\ArityMap{{\it Shp}}
\newcommand\ArityGraph{D}
\newcommand\AritySketch{{\cal D}}
\newcommand\ArityInclusion{\mbox{\Large $\iota$}}

\newcommand\rms{\rm\scriptsize}   % for writing, eg, \D^{\rms in}

\newcommand\PredicateMarkerSymbol{P}
\newcommand\OperationMarkerSymbol{F}
\newcommand\BasicDomainMarkerSymbol{B}

\newcommand\PredicateDiagramSet[1]{\PredicateMarkerSymbol^{#1}}%P^#1}
\newcommand\OperationDiagramSet[1]{\OperationMarkerSymbol^{#1}}%F^#1}
\newcommand\BasicDomainDiagramSet[1]{\BasicDomainMarkerSymbol^{#1}}%B^#1}

\newcommand\AGraph{G}
\newcommand\g{\mbox{$\AGraph$}}
\newcommand\gm{\AGraph}

\newcommand\ASketchSymbol{S}
\newcommand\ASketch{\mathsf \ASketchSymbol}
\newcommand\s{\mbox{$\ASketch$}}
\newcommand\sind{\ASketch}
\newcommand\sm{\ASketch}
\newcommand\sprim{\mbox{$\ASketch'$}}
\newcommand\sbipr{\mbox{$\ASketch''$}}


\newcommand\TheUniverseSymbol{U}
\newcommand\TheUniverseSketch{\cal \TheUniverseSymbol}
\newcommand\TheObjectUniverse{Obj }%{\cal O}
\newcommand\TheTimeUniverse{\cal T}%{T}
\newcommand\TheHistoryUniverse{\cal \TheTimeUniverse^*}%}
\newcommand\TheValueUniverse{Val}%{\cal V}

\newcommand\ASketchAlgebra{\cal A}
\newcommand\ABaseSubSketch{\cal B}    % base subsketch of

\newcommand\APermutation{\pi}

%===================================================

\newcommand\Mod[1]{\mbox{{\bf Mod}$(#1)$}}
\newcommand\Ext[1]{\mbox{{\bf Ext}$(#1)$}}
\newcommand\Inst[1]{\mbox{{\bf Inst}$(#1)$}}

%%%%%%%%%%%%%   End Key commands %%%%%%%%%%%%%%%%%


%%%%%%%%%%%%    Useful Abbreviations %%%%%%%%%%%%

%%% Sketchi


\newcommand\sdom{\mbox{$\s_{\DomainBase}$}}
\newcommand\sdomm{\s_{\DomainBase}}

\newcommand\newb{\mbox{$\DomainBase$}}
\newcommand\bm{\DomainBase}

\newcommand{\bs}{\mbox{$\ABaseSubSketch$}}
\newcommand\bsm{\ABaseSubSketch}

\newcommand\skespe{{\bf \ASketchSymbol}}

\newcommand\gras{{\it Gra}\skeob}
\newcommand\doms{{\it Dom}\skeob}
\newcommand\clas{{\it Cla}\skeob}
\newcommand\rels{{\it Rel}(\skeob)}

\newcommand\R{\nicex{ R$}}
\newcommand\OO{\mbox{$\TheObjectUniverse$}}
%\newcommand\T{\mbox{$\TheTimeUniverse$}}
%\newcommand\Hist{\mbox{$\TheHistoryUniverse}}
%\newcommand\V{\mbox{$\TheValueUniverse_{\bm}$}}%

\renewcommand\u{\mbox{$\TheUniverseSketch$}}
\newcommand\um{\TheUniverseSketch}
\newcommand\upred{\mbox{$\TheUniverseSketch_{\predsigm}$}}
\newcommand\uoper{\mbox{$\TheUniverseSketch_{\opersigm}$}}

\newcommand\predsig{\mbox{$\PredicateSignature$}}
\newcommand\predsigm{\PredicateSignature}
\newcommand\opersig{\mbox{$\OperationSignature$}}
\newcommand\opersigm{\OperationSignature}
\newcommand\predopsig{\mbox{$\predFromOperSig$}}
%\newcommand\pros{\predopsig}
\newcommand\prosm{\predFromOperSig}
\newcommand\basesig{\mbox{\BaseSignature}}
\newcommand\basesigm{{\BaseSignature}}
\newcommand\clan{\mbox{$\ConstraintLanguage$}}
\newcommand\clanm{\ConstraintLanguage}
\newcommand\colan{\mbox{\ConstraintLanguage}}
\newcommand\clanform{\mbox{$\ConstraintLanguage=(\Pred,\arimap,\semm{})$}}
\newcommand\colanm{\ConstraintLanguage}
%\newcommand\dolan{\mbox{\DomainLanguage}}
%\newcommand\dolanm{\DomainLanguage}

\newcommand\pis{$\PredicateSignature $-sketch}
\newcommand\sis{$\OperationSignature $-sketch}
\newcommand\siprs{$\predFromOperSig$-sketch}
\newcommand\sia{$\OperationSignature $-algebra}
\newcommand\clans{$\Constraint Language$-sketch}

\newcommand\arimap{\ArityMap}
\newcommand\arimapin{\mbox{\ArityMap$^{\rms in}$}}

\newcommand\os{\mbox{$\overline{\s}$}}
%\newcommand\go{\mbox{$G_{({\cal O})}$}}

\newcommand\pip{\mbox{$\APermutation^{+}$}}
\newcommand\depipComp{\mbox{$\delta \comp\APermutation^{+}$}}
\newcommand\depip{\mbox{$\APermutation^{+}\delta $}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%                                  %%%%%%%%%%%%%%%%%
%%%%%%%%%%            A R I T I E S         %%%%%%%%%%%%%%%%%%
%%%%%%%%%%                                  %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand\pr{\mbox{$\PredicateMarkerSymbol$}}  % $P$ for using in text mode
\newcommand\op{\mbox{$\OperationMarkerSymbol$}}  % $F$ for using in text mode
%\newcommand\ba{\mbox{$\BasicDomainMarkerSymbol$}}  % $P$ for using in text mode


\newcommand\myprm{\PredicateMarkerSymbol}        %  P  for using in math mode
\newcommand\opm{\OperationMarkerSymbol}          %  F  for using in math mode
%\newcommand\bam{\BasicDomainMarkerSymbol}       %  B  for using in math mode

%%%%   functions to put the arg
%%%%   as subindex near \pr,\op and \ba

\newcommand\prix[1]{\myprm_{#1}}
\newcommand\opix[1]{\opm_{#1}}
\newcommand\baix[1]{\bam_{#1}}

%%%----  end functions

\newcommand\pri{$\myprm_{i}$}    %  \pr_i for using in text mode
\newcommand\opi{$\opm_{j}$}      %  \op_j for using in text mode
\newcommand\bai{$\bam_{l}$}      %  \ba_l for using in text mode

\newcommand\prim{\myprm_{i}}     %  \pr_i for using in math mode
\newcommand\opim{\opm_{j}}       %  \op_j for using in math mode
\newcommand\baim{\bam_{l}}       %  \ba_l for using in text mode
%======================================
%  eto makrosy funcciy
\renewcommand\Pr[1]{\PredicateDiagramSet{#1}}  % P^#1
\newcommand\Op[1]{\OperationDiagramSet{#1}}    % F^#1
\newcommand\Ba[1]{\BasicDomainDiagramSet{#1}}  % B^#1
%  a eto ih znacheniya
\newcommand\PrS{\Pr{\s}}      % P^\s
\newcommand\OpS{\Op{\s}}      % F^\s
\newcommand\BaS{\Ba{\s}}      % B^\s
%\newcommand\domba{$\Domain(\ba)$}

\newcommand\PrU{\Pr{\u}}      % P^\u
\newcommand\OpU{\Op{\u}}      % F^\u
\newcommand\BaU{\Ba{\u}}      % B^\u

%------------------------------------------------
% eto makrosy funkciy s 2 argumwntami
\newcommand\Prix[2]{\Pr{#1}_{#2}}              % a set P^#1_#2
\newcommand\Opix[2]{\Op{#1}_{#2}}              % a set F^#1_#2
\newcommand\Baix[2]{\Ba{#1}_{#2}}              % a set B^#1_#2
% a eto b nih podstavleny indexy i ostalsya 1 argument
\newcommand\Pri[1]{$\Prix{#1}{i}$}             % a set og diag, P^#1_i
\newcommand\Opi[1]{$\Opix{#1}{j}$}             % a set of diag, F^#1_j
\newcommand\Bai[1]{$\Baix{#1}{l}$}             % a set of diag, B^#1_l
% a eto znacheniya
\newcommand\PriS{\Pri{\s}}      % Pi^\s
\newcommand\OpiS{\Opi{\s}}      % Fj^\s
\newcommand\BaiS{\Bai{\s}}      % Bl^\s

\newcommand\PriU{\Pri{\u}}      % Pi^\u
\newcommand\OpiU{\Opi{\u}}      % Fj^\u
\newcommand\BaiU{\Bai{\u}}      % Bl^\u

%  a eto dlya mat mode
\newcommand\Prim[1]{\Prix{#1}{i}}     %  a set of diagr,  P^#1_i for using in math mode
\newcommand\Opim[1]{\Opix{#1}{j}}     %  a set of diagr,  F^#1_j for using in math mode
\newcommand\Baim[1]{\Baix{#1}{l}}     %  a set of diagr,  B^#1_#2 for using in math mode
%====================================================

%\newcommand\pool{V}
\newcommand\vx[1]{\mbox                                  % D_arg
                      {$\pool_{#1}$}}
\newcommand\vinx[1]{\mbox                                % D^in_arg
                      {$\pool^{\mbox\rms in}_{#1}$}}
\newcommand\voutx[1]{\mbox                               % D^out_arg
                      {$\pool^{\mbox\rms out}_{#1}$}}
%============================================================

%\newcommand\ArityGraph{D}
%\newcommand\AritySketch{\D}                             % \D - nice D
\newcommand\sprx[1]{\mbox                                %  D_arg
                      {$\ArityGraph_{#1}$}}
\newcommand\sopx[1]{\mbox                                % \D_arg
                      {$\AritySketch_{#1}$}}
\newcommand\sinx[1]{\mbox                                % \D^in_arg
                      {$\AritySketch^{\rms in}_{#1}$}}
\newcommand\soutx[1]{\mbox                               % \D^out_arg
                      {$\AritySketch^{\rms out}_{#1}$}}

%-----   marker-subindex version
\newcommand\spr{\sprx{\myprm}}         %  D_{prop marker}
\newcommand\sop{\sopx{\opm}}         % \D_{oper marker}
\newcommand\sinop{\sinx{\opm}}       % \D^in_{oper mark}
%-----   i-subindex version
\newcommand\spri{\sprx{i}}          %  D_{i}
\newcommand\sopi{\sopx{j}}          % \D_{j}
\newcommand\sinopi{\sinx{j}}        % \D^in_{j}



\newcommand\opshaxy[2]{\inclar{#1_{#2}}  % arg1_arg2: D^in_arg2 -->D_arg2
                            {\sinx{#2}}
                              {\sopx{#2}}
                       }
%\newcommand\ArityInclusion{i}
\newcommand\opsha{\opshaxy{\ArityInclusion}{\opm}}   %i_f: D^in_f   --> D_f
\newcommand\opshai{\opshaxy{\ArityInclusion}{\opim}} %i_f: D^in_f_j --> D_f_j

%----------------------------------------

%\newcommand\ArityMap{{\it Shp}}
\newcommand\arix[1]{\mbox
                        {$\ArityMap({#1})$}}         % Shp(arg)
\newcommand\ariinx[1]{\mbox
                        {$\ArityInclusion_{#1}$}}    % \iota_{arg}

\newcommand\aripr{\arix{\myprm}}                  % Shp(p)
\newcommand\ariop{\arix{\opm}}                  % Shp(f)
\newcommand\arinc{\ariinx{\opm}}                % \iota_f

\newcommand\aripri{\arix{\prim}}                % Shp(p_i)
\newcommand\ariopi{\arix{\opim}}                % Shp(f_j)
\newcommand\arinci{\ariinx{\opim}}              % \iota_j

%-----------------------------------------
\newcommand\sepr{\semm{\pr}}
\newcommand\seop{\semm{\op}}
\newcommand\sepri{\semm{\pri}}
\newcommand\seopi{\semm{\op}}


\newcommand\opv{\mbox{\Oper$^+$}}

%\endinput

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%              %%%%%%%%%%%%%%%
%%%%%%%%%%%  Old Macros %%%%%%%%%%%%%%%%
%%%%%%%%%%              %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\newcommand\sig{\mbox{$\PredicateSignature$}}
%\newcommand\gra{{\bf G}}
%\newcommand\sigo{\mbox{$\Sigma_1$}}
%\newcommand\grao{\mbox{${\bf G}_1$}}
%% OOPS! \newcommand\inst{\mbox{$\lar{\vare }{S}{W}$}}
%%\newcommand\sch{\Category{Schema} }
%
%
%\newcommand\instVareps{\mbox{$\lar{\vare }{S}{W}$}}
%\newcommand\inste{\mbox{$\lar{e}{S}{W}$}}
%\newcommand\emor[1]{\lar{e}{#1}{\u}}
%\newcommand\sv{\mbox{$S_V$}}
%\newcommand\sr{\mbox{$S_R$}}
%\newcommand\vmor{\lar{v}{\sv}{\ovrs{}}}
%\newcommand\rmor{\lar{r}{S}{\ovrs{R}}}
%\newcommand\vpair{\mbox{$V=(\sv,v)$}}
%\newcommand\rpair{\mbox{$R=(\sr,r)$}}
%===
%==== Varset
%% macros for writing formulas with varsets and varfunctions

%%%%%%%%%    ..\dke96\macro\varset.tex    %%%%%%%
%\renewcommand\c{\mbox{$\AClass$}}                    %   C
%\newcommand\cm{\AClass}                              %   C
%\newcommand\ce{\mbox{$\semm{\AClass}$}}              % ||C||

%\newcommand\ceind[1]{\mbox{$\semm{\AClass}^{#1}$}}   % ||C||^#1

%\newcommand\cindeind[2]{\mbox{$\semm{\AClass_{#1}}^{#2}$}}
% apply:
%\newcommand\cet{\ceind{\ltt}}                         % ||C||^t
%\newcommand\ceu{\ceind{\ltu}}                         % ||C||^u
\newcommand\ObjStt{\ittt{ObjStt}}
\newcommand\C{\textit{C}}
\newcommand\D{\textit{D}}

\newcommand\ot[1]{\mbox{$o^{\ltt_{#1}}$}}
\newcommand\otm{o^\ltt}
\newcommand\ou[1]{\mbox{$o^{\ltu_{#1}}$}}
\newcommand\otu{o^\ltu}

\newcommand\cet{\mbox{$\semm{C}^{\ltt}$}}                         % ||C||^t
\newcommand\ceti{\mbox{$\semm{C}^{\ltt_i}$}}                         % ||C||^t
\newcommand\ceu{\mbox{$\semm{C}^{\ltu}$}}                         % ||C||^t
\newcommand\ceprt{\mbox{$\sempr{C}^{\ltt}$}}                         % ||C||^t
\newcommand\cepru{\mbox{$\sempr{C}^{\ltu}$}}                         % ||C||^t


\newcommand\cetu{\mbox{$\vphantom{\semm{AClass}}^{\ltt}\!\semm{\AClass}^{\ltu}$}}
\newcommand\ceut{\mbox{$\vphantom{\semm{AClass}}^{\ltu}\!\semm{\AClass}^{\ltt}$}}
\newcommand\detu{\mbox{$\vphantom{\semm{AClass}}^{\ltt}\!\semm{\TargetClass}^{\ltu}$}}
\newcommand\fetu{\mbox{$\vphantom{\semm{AClass}}^{\ltt}\!\semm{\TargetClass_f}^{\ltu}$}}
\newcommand\djetu{\mbox{$\vphantom{\semm{AClass}}^{\ltt}\!\semm{\TargetClass_j}^{\ltu}$}}
\newcommand\dietu{\mbox{$\vphantom{\semm{AClass}}^{\ltt}\!\semm{\TargetClass_i}^{\ltu}$}}
\newcommand\deut{\mbox{$\vphantom{\semm{AClass}}^{\ltu}\!\semm{\TargetClass}^{\ltt}$}}
\newcommand\ceprtu{\mbox{$\vphantom{\sempr{AClass}}^{\ltt}\sempr{\AClass}^{\ltu}$}}
\newcommand\deprtu{\mbox{$\vphantom{\sempr{AClass}}^{\ltt}\sempr{\TargetClass}^{\ltu}$}}



\newcommand\cesu{\mbox{$\vphantom{\semm{AClass}}^{\lts}\!\semm{\AClass}^{\ltu}$}}
\newcommand\cest{\mbox{$\vphantom{\semm{AClass}}^{\lts}\!\semm{\AClass}^{\ltt}$}}
\newcommand\cett{\mbox{$\vphantom{\semm{AClass}}^{\ltt}\!\semm{\AClass}^{\ltt}$}}

\newcommand\dest{\mbox{$\vphantom{\semm{AClass}}^{\lts}\!\semm{\TargetClass}^{\ltt}$}}
\newcommand\desu{\mbox{$\vphantom{\semm{AClass}}^{\lts}\!\semm{\TargetClass}^{\ltu}$}}

\newcommand\cestart{\mbox{${\semmstar{C}}^{\ltt}$}}                         % ||C||^t
\newcommand\cestaru{\mbox{${\semmstar{C}}^{\ltu}$}}                         % ||C||^t
\newcommand\cestartu{\mbox{${}^{\ltt}{\semmstar{C}}^{\ltu}$}}

\newcommand\ceto{\mbox{$\semm{\AClass}^{\ltt}_{o}$}}
\newcommand\ceuo{\mbox{$\semm{\AClass}^{ \ltu}_{o}$}}

\newcommand\cestarto{\mbox{${\semmstar{\AClass}}^{\ltt}_{o}$}}
\newcommand\cestaruo{\mbox{${\semmstar{\AClass}}^{ \ltu}_{o}$}}

%======================================================================

%  ----  Basic Command -----------

\newcommand\LogicalTime{\cal T}
\newcommand\SetOfHistories{\LogicalTime^*}
\newcommand\AHistory{H}%J}

%\newcommand\IndexingXupYdownZ[3]{\mbox{$#1^{#2}_{#3}$}}
%\newcommand\IntRelSymb{\varepsilon}%rho}
%\newcommand\IntRelSymb{\mbox{\Large$\iota$}}%rho}
%\newcommand\IntersttMap{\mbox{\ittt same}}%rho}

\newcommand\AClass{C}
\newcommand\SourceClass{C}
\newcommand\TargetClass{D}
\newcommand\e{E}
\newcommand\AReference{f}
\newcommand\AnotherReference{g}
%\newcommand\Identifier{\mbox{\Large$\iota$}}
\renewcommand\g{g}
%\newcommand\h{h}
%\newcommand\hind{h}


\newcommand\farr{\lar{\AReference}{\SourceClass}{\TargetClass}}
\newcommand\farris{\lar{\AReference_i}{\SourceClass}{\TargetClass_i}}
\newcommand\farrit{\lar{\AReference_i}{\SourceClass_i}{\TargetClass}}
\newcommand\ffams{\mbox{$\f=\famm{\farris}{i\in I}$}}
\newcommand\ffamt{\mbox{$\f=\famm{\farrit}{i\in I}$}}

\newcommand\garr{\lar{\AnotherReference}{\SourceClass}{\TargetClass}}
\newcommand\garrit{\lar{\AnotherReference_i}{\SourceClass}{\TargetClass_i}}
\newcommand\garris{\lar{\AnotherReference_i}{\SourceClass_i}{\TargetClass} }
\newcommand\gfams{\mbox{$\g=\famm{\garris}{i\in I}$}}
\newcommand\gfamt{\mbox{$\g=\famm{\garrit}{i\in I}$}}


\newcommand\iarr{\lar{\AReference}{\SourceClass}{\TargetClass}}
\newcommand\iarris{\lar{\Identifier_j}{\SourceClass}{\TargetClass_j}}
\newcommand\iarrit{\lar{\Identifier_j}{\SourceClass_j}{\TargetClass} }
\newcommand\ifams{\mbox{$\Identifier=\famm{\iarris}{j\in J}$}}
\newcommand\ifamt{\mbox{$\Identifier=\famm{\iarrit}{j\in J}$}}


\newcommand\AMoment{t}%j}
\newcommand\EarlierMoment{t}%j}
\newcommand\LaterMoment{u}%k}
\newcommand\EarlierEarlierMoment{s}%i}
\newcommand\LaterLaterMoment{v}%l}

\newcommand\ttt{t1,t2}

\newcommand\IndexingXupYdownZ[3]{\mbox{$#1^{#2}_{#3}$}}

%%%%%%%%%%%%%%%%%%%%%%
% -- Abbreviations ----
%%%%%%%%%%%%%%%%%%%%%%%%%%                    sket}}


\newcommand\T{\mbox{$\LogicalTime$}}
\newcommand\Tm{\LogicalTime}
\newcommand\Hist{\mbox{$\SetOfHistories$}}
\newcommand\Histm{\SetOfHistories}
\newcommand\IntersttMap{\mbox{\ittt{same}}}%rho}
\newcommand\same[2]{\mbox{$\IntersttMap^{#1}_{#2}$}}
\newcommand\inter[2]{\same{#1}{#2}}
\newcommand\interpr[2]{\mbox{$\mytilde\IntersttMap^#1_#2$}}
% \IndexingXupYdownZ{\IntRelSymb}{#1}{#2}}  %\vare^#1_#2
%\newcommand\interpr[2]%
%      {\IndexingXupYdownZ{\mytilde{\IntRelSymb}}{#1}{#2}}  %\vare^#1_#2

%%% The new version t is denoted by \ltt, u is denoted by  \ltu etc

\newcommand\ttu{\EarlierMoment\LaterMoment}   %tu
\newcommand\logtimet{\EarlierMoment}               %t
\newcommand\ltt{\EarlierMoment}               %t
%\newcommand\tu{\LaterMoment}                  %u
\newcommand\ltu{\LaterMoment}                  %u
\newcommand\ttlu{\mbox{$\ltt\le\ltu$}}         % t =< u
\newcommand\tleu{\mbox{$\ltt\le\ltu$}}         % t =< u
\newcommand\tlu{\mbox{$\ltt<\ltu$}}            % t < u
\newcommand\logtimes{\EarlierEarlierMoment}        %s
\newcommand\lts{\EarlierEarlierMoment}               %t
\newcommand\ltv{\LaterLaterMoment}             %l
\newcommand\tv{\LaterLaterMoment}             %l

\newcommand\J{\AHistory}                      %J

\newcommand\intertu[1]{\inter{\ltt\to\ltu}{#1}}       % \eps^tu_#1
\newcommand\interut[1]{\inter{\ltt\gets\ltu}{#1}}       % \eps^tu_#1
\newcommand\intertuut[1]{\inter{\ltt\leftrightarrow\ltu}{#1}}       % \eps^tu_#1

\newcommand\intertt[1]{\inter{\ltt\to\ltt}{#1}}                 % \eps^tu_#1

\newcommand\interst[1]{\inter{\lts\to\ltt}{#1}}       % \eps^tu_#1
\newcommand\interts[1]{\inter{\lts\gets\ltt}{#1}}       % \eps^tu_#1

\newcommand\intersu[1]{\inter{\lts\to\ltu}{#1}}       % \eps^tu_#1
\newcommand\interus[1]{\inter{\ltu\gets\lts}{#1}}       % \eps^tu_#1

%\newcommand\interst[1]{\inter{\lts\to\ltt}{#1}}                 % \eps^tu_#1
%\newcommand\intersu[1]{\inter{\lts\to\ltu}{#1}}                 % \eps^tu_#1

\newcommand\domintertu[1]{\ldom{\intertu{#1}}}  %\Box\eps^tu_#1
\newcommand\codintertu[1]{\rdom{\intertu{#1}}}  %\eps^tu_#1\Box

\newcommand\sametuut[1]{\mbox{$\same{\ltt\leftrightarrow\ltu}{#1}$}}       % \eps^tu_#1
\newcommand\sametu[1]{\mbox{$\same{\ltt\to\ltu}{#1}$}}       % \eps^tu_#1
\newcommand\sameut[1]{\mbox{$\same{\ltt\gets\ltu}{#1}$}}       % \eps^tu_#1
\newcommand\samectu{\mbox{$\same{\ltt\to\ltu}{\cm}$}}       % \eps^tu_#1
\newcommand\samecut{\mbox{$\same{\ltt\gets\ltu}{\cm}$}}       % \eps^tu_#1
\newcommand\samedtu{\mbox{$\same{\ltt\to\ltu}{\dm}$}}       % \eps^tu_#1
\newcommand\samedut{\mbox{$\same{\ltt\gets\ltu}{\dm}$}}       % \eps^tu_#1

\newcommand\samett[1]{\same{\ltt\to\ltt}{#1}}                 % \eps^tu_#1

\newcommand\samest[1]{\same{\lts\to\ltt}{#1}}       % \eps^tu_#1
\newcommand\samets[1]{\same{\lts\gets\ltt}{#1}}       % \eps^tu_#1
\newcommand\samecst{\same{\lts\to\ltt}{\cm}}       % \eps^tu_#1
\newcommand\samects{\same{\lts\gets\ltt}{\cm}}       % \eps^tu_#1
\newcommand\samedst{\same{\lts\to\ltt}{\dm}}       % \eps^tu_#1
\newcommand\samedts{\same{\lts\gets\ltt}{\dm}}       % \eps^tu_#1



\newcommand\samesu[1]{\same{\lts\to\ltu}{#1}}       % \eps^tu_#1
\newcommand\sameus[1]{\same{\ltu\gets\lts}{#1}}       % \eps^tu_#1

%\newcommand\samest[1]{\same{\lts\to\ltt}{#1}}                 % \eps^tu_#1
%\newcommand\samesu[1]{\same{\lts\to\ltu}{#1}}                 % \eps^tu_#1

\newcommand\domsametu[1]{\ldom{\sametu{#1}}}  %\Box\eps^tu_#1
\newcommand\codsametu[1]{\rdom{\sametu{#1}}}  %\eps^tu_#1\Box


%  Apply:
\newcommand\interctt{\inter{\ltt\to\ltt}{\cm}}                 % \eps^tu_#1
\newcommand\intercst{\inter{\lts\to\ltt}{\cm}}                 % \eps^tu_#1
\newcommand\interctu{\inter{\ltt\to\ltu}{\cm}}                 % \eps^tu_#1
\newcommand\intercsu{\inter{\lts\to\ltu}{\cm}}                 % \eps^tu_#1

\newcommand\intercut{\inter{\ltt\leftarrow\ltu}{\cm}}                 % \eps^tu_#1

\newcommand\interprctt{\interpr{\ltt\ltt}{\cm}}                 % \eps^tu_#1
\newcommand\interprcst{\interpr{\lts\ltt}{\cm}}                 % \eps^tu_#1
\newcommand\interprctu{\interpr{\ltt\ltu}{\cm}}                 % \eps^tu_#1
\newcommand\interprcsu{\interpr{\lts\ltu}{\cm}}                 % \eps^tu_#1

\newcommand\dominterctu{\domintertu{\cm}}  %\Box\eps^tu_#1
\newcommand\codinterctu{\codintertu{\cm}}  %\eps^tu_#1\Box

%----------------------------------------------
%% Classes and arrows
%-------------------------------------------------

%\renewcommand\c{\mbox{$\AClass$}}                    %   C
\newcommand\cm{\AClass}                              %   C
\newcommand\ce{\mbox{$\semm{\AClass}$}}              % ||C||

%--- function:
\newcommand\ceind[1]{\mbox{$\semm{\AClass}^{#1}$}}   % ||C||^#1

\newcommand\cindeind[2]{\mbox{$\semm{\AClass_{#1}}^{#2}$}}
% apply:
%\newcommand\cet{\mbox{$\semm{C}^{\ltt}$}}                         % ||C||^t
%\newcommand\ceu{\mbox{$\semm{C}^{\ltu}$}}                         % ||C||^t
%\newcommand\cetu{\mbox{${}^{\ltt}\semm{\AClass}^{\ltu}$}}
\newcommand\ces{\ceind{\lts}}                         % ||C||^u
\newcommand\cev{\ceind{\tv}}                         % ||C||^u


\newcommand\ceJ{\ceind{\J}}

\newcommand\objeq[2]{\simeq^{#1}_{#2}}
\newcommand\eqJ[1]{\objeq{\J}{#1}}

\newcommand\ciet{\cindeind{i}{\ltt}}                         % ||C_i||^t
\newcommand\ctet{\cindeind{t}{\ltt}}                         % ||C_t||^t
\newcommand\cjet{\cindeind{j}{\ltt}}                         % ||C_i||^t
\newcommand\cket{\cindeind{k}{\ltt}}                         % ||C_t||^t
\newcommand\clet{\cindeind{l}{\ltt}}                         % ||C_i||^t


\newcommand\cieJ{\ceind{\J}}
%\newcommand\cjeJ{\ceind{\J}}

% function:
\newcommand\cind[1]{\mbox{$\AClass^{#1}$}}           %      C^#1
\newcommand\cindl[2]{\mbox{$_{#1}\AClass^{#2}$}}     % _{#1}C^{#2}
\newcommand\cindr[2]{\mbox{$\AClass_{#1}^{#2}$}}     %      C_{#1}^{#2}

%\newcommand\ceind[1]{\mbox{$\semm{\AClass}^{#1}$}}           %      C^#1
\newcommand\ceindl[2]{\mbox{$_{#1}\semm{\AClass}^{#2}$}}     % _{#1}C^{#2}
\newcommand\ceindr[2]{\mbox{$\semm{\AClass}_{#1}^{#2}$}}     %      C_{#1}^{#2}

%  apply:
\newcommand\ctu{\mbox{$^{\ltt}\!\AClass^{\ltu}$}}
\newcommand\ctplusu{\cindr{+\ltu}{\ltt}}
\newcommand\ctnullu{\cindr{0\ltu}{\ltt}}
\newcommand\cuminust{\cindl{-\ltt}{\ltu}}
\newcommand\cunullt{\cindl{0\ltt}{\ltu}}

%\newcommand\cetu{\cind{\ltt\ltu}}
\newcommand\cetplusu{\ceindr{+\ltu}{\ltt}}
\newcommand\cetnullu{\ceindr{0\ltu}{\ltt}}
\newcommand\ceuminust{\ceindl{-\ltt}{\ltu}}
\newcommand\ceunullt{\ceindl{0\ltt}{\ltu}}

% the same for D

%\renewcommand\d{\mbox{$\TargetClass$}}                    %   D
\newcommand\dm{\TargetClass}                              %   D

\newcommand\de{\mbox{$\semm{\TargetClass}$}}              % ||D||
\newcommand\deind[1]{\mbox{$\semm{\TargetClass}^{#1}$}}   % ||D||^#1
\renewcommand\det{\deind{\ltt}}                         % ||C||^t
\newcommand\deu{\deind{\ltu}}                         % ||C||^u
\newcommand\des{\deind{\lts}}                         % ||C||^u
\newcommand\dev{\deind{\tv}}                         % ||C||^u

\newcommand\deJ{\deind{\J}}

\newcommand\dindeind[2]{\mbox{$\semm{\TargetClass_{#1}}^{#2}$}}
%  apply
\newcommand\dies{\dindeind{i}{\lts}}                         % ||C||^t
\newcommand\djet{\dindeind{j}{\ltt}}                         % ||C||^t
\newcommand\djeu{\dindeind{j}{\ltu}}                         % ||C||^t
%\newcommand\djetu{\dindeind{j}{\ltt}}                         % ||C||^t
\newcommand\dieJ{\deind{\J}}
\newcommand\djeJ{\deind{\J}}
\newcommand\diet{\dindeind{i}{\ltt}}                         % ||C||^t
\newcommand\dieu{\dindeind{i}{\ltu}}                         % ||C||^t
%\newcommand\djetu{\dindeind{j}{\ltt}}                         % ||C||^t


\newcommand\dind[1]{\mbox{$\TargetClass^{#1}$}}           %      C^#1
\newcommand\dindl[2]{\mbox{$_{#1}\TargetClass^{#2}$}}     % _{#1}D^{#2}
\newcommand\dindr[2]{\mbox{$\TargetClass_{#1}^{#2}$}}     %      D_{#1}^{#2}

%\newcommand\deind[1]{\mbox{$\semm{\TargetClass}^{#1}$}}           %      C^#1
\newcommand\deindl[2]{\mbox{$_{#1}\semm{\TargetClass}^{#2}$}}     % _{#1}D^{#2}
\newcommand\deindr[2]{\mbox{$\semm{\TargetClass}_{#1}^{#2}$}}     %      D_{#1}^{#2}


% apply
\newcommand\dtu{\mbox{$^{\ltt}\!\TargetClass^{\ltu}$}}
\newcommand\detplusu{\deindr{+\ltu}{\ltt}}
\newcommand\detnullu{\deindr{0\ltu}{\ltt}}
\newcommand\deuminust{\deindl{-\ltt}{\ltu}}
\newcommand\deunullt{\deindl{0\ltt}{\ltu}}


%\newcommand\f{\mbox{$\AReference$}}                    %   f
\newcommand\fm{\AReference}                              %   f
%\newcommand\find[1]{\mbox{$\AReference^{#1}$}}           %      f^#1
%\newcommand\findl[2]{\mbox{$_{#1}\AReference^{#2}$}}     % _{#1}C^{#2}
%\newcommand\findr[2]{\mbox{$\AReference_{#1}^{#2}$}}     %      C_{#1}^{#2}

\newcommand\feind[1]{\mbox{$\semm{\AReference}^{#1}$}}           %      f^#1
\newcommand\feindl[2]{\mbox{$_{#1}\semm{\AReference}^{#2}$}}     % _{#1}C^{#2}
\newcommand\feindr[2]{\mbox{$\semm{\AReference}_{#1}^{#2}$}}     %      C_{#1}^{#2}

\newcommand\ftu{\find{\ttu}}

\newcommand\fe{\mbox{$\semm{\AReference}$}}              % ||f||
\renewcommand\feind[1]{\mbox{$\semm{\AReference}^{#1}$}}   % ||f||^#1
\newcommand\fet{\feind{\ltt}}
\newcommand\fes{\feind{\lts}}
\newcommand\feu{\feind{\ltu}}
\newcommand\fev{\feind{\tv}}
\newcommand\feJ{\feind{\J}}

\newcommand\femt{\mbox{$\semm{\AReference^{-1}}^{\ltt}$}}


\newcommand\findeind[2]{\mbox{$\semm{\AReference_{#1}}^{#2}$}}
\newcommand\fieu[1]{\findeind{#1}{\ltu}}
\newcommand\fiet[1]{\findeind{#1}{\ltt}}
\newcommand\fies[1]{\findeind{#1}{\lts}}                         % ||C||^t
%\newcommand\fiet{\findeind{i}{\ltt}}                         % ||C||^t
\newcommand\fjet{\findeind{j}{\ltt}}                         % ||C||^t
\newcommand\fket{\findeind{k}{\ltt}}                         % ||C||^t
\newcommand\flet{\findeind{l}{\ltt}}                         % ||C||^t
\newcommand\fkeu{\findeind{k}{\ltu}}                         % ||C||^t

\newcommand\fetplusu{\feindr{+\ltu}{\ltt}}
\newcommand\fetnullu{\feindr{0\ltu}{\ltt}}
\newcommand\feuminust{\feindl{-\ltt}{\ltu}}
\newcommand\feunullt{\feindl{0\ltt}{\ltu}}



%\newcommand\diet{\dindeind{i}{\ltt}}                         % ||C||^t
%\newcommand\djes{\dindeind{j}{\lts}}                         % ||C||^t

\newcommand\fieJ{\feind{\J}}
\newcommand\fjeJ{\feind{\J}}

\newcommand\fgcomp{\mbox{$\f(\g_1,\ldots,\g_m)$}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% The old version where \tj denotes t, \tk denotes u  etc
%%% The new version see on line 185

\newcommand\tjk{\EarlierMoment\LaterMoment}   %jk
\newcommand\tj{\EarlierMoment}               %j
\newcommand\tk{\LaterMoment}                  %k
\newcommand\tjlk{\mbox{$\tj\le\kt$}}
\newcommand\ti{\EarlierEarlierMoment}        %i
\newcommand\tl{\LaterLaterMoment}             %l

%\newcommand\J{\AHistory}                      %J

\newcommand\interjk[1]{\inter{\tjk}{#1}}                 % \eps^jk_#1
\newcommand\dominterjk[1]{\ldom{\interjk{#1}}}  %\Box\eps^jk_#1
\newcommand\codinterjk[1]{\rdom{\interjk{#1}}}  %\eps^jk_#1\Box

\newcommand\interjj[1]{\inter{\tj\tj}{#1}}                 % \eps^jk_#1
\newcommand\interij[1]{\inter{\ti\tj}{#1}}                 % \eps^jk_#1
%\newcommand\interjk[1]{\inter{\tj\tk}{#1}}                 % \eps^jk_#1
\newcommand\interik[1]{\inter{\ti\tk}{#1}}                 % \eps^jk_#1


\newcommand\intercjj{\inter{\tj\tj}{\cm}}                 % \eps^jk_#1
\newcommand\intercij{\inter{\ti\tj}{\cm}}                 % \eps^jk_#1
\newcommand\intercjk{\inter{\tj\tk}{\cm}}                 % \eps^jk_#1
\newcommand\intercik{\inter{\ti\tk}{\cm}}                 % \eps^jk_#1

\newcommand\domintercjk{\dominterjk{\cm}}  %\Box\eps^jk_#1
\newcommand\codintercjk{\codinterjk{\cm}}  %\eps^jk_#1\Box

\newcommand\interdjj{\inter{\tj\tj}{\dm}}                 % \eps^jk_#1
\newcommand\interdij{\inter{\ti\tj}{\dm}}                 % \eps^jk_#1
\newcommand\interdjk{\inter{\tj\tk}{\dm}}                 % \eps^jk_#1
\newcommand\interdik{\inter{\ti\tk}{\dm}}                 % \eps^jk_#1

%----------------------------------------------
%% Classes and arrows
%-------------------------------------------------

%\renewcommand\c{\mbox{$\AClass$}}                    %   C
%\newcommand\cm{\AClass}                              %   C

%\newcommand\ce{\mbox{$\semm{\AClass}$}}              % ||C||
%\newcommand\ceind[1]{\mbox{$\semm{\AClass}^{#1}$}}   % ||C||^#1
\newcommand\cej{\ceind{\tj}}                         % ||C||^j
\newcommand\cek{\ceind{\tk}}                         % ||C||^k
%\newcommand\ceJ{\ceind{\J}}
%--- function:
%\newcommand\cindeind[2]{\mbox{$\semm{\AClass_{#1}}^{#2}$}}
% apply:
\newcommand\ciej{\cindeind{i}{\tj}}                         % ||C_i||^j
\newcommand\cjej{\cindeind{j}{\tj}}                         % ||C_j||^j
\renewcommand\cieJ{\ceind{\J}}
\newcommand\cjeJ{\ceind{\J}}

% function:
%\newcommand\cind[1]{\mbox{$\AClass^{#1}$}}           %      C^#1
%\newcommand\cindl[2]{\mbox{$_{#1}\AClass^{#2}$}}     % _{#1}C^{#2}
%\newcommand\cindr[2]{\mbox{$\AClass_{#1}^{#2}$}}     %      C_{#1}^{#2}
%  apply:
\newcommand\cjk{\cind{\tj\tk}}
\newcommand\cjplusk{\cindr{+\tk}{\tj}}
\newcommand\cjnullk{\cindr{0\tk}{\tj}}
\newcommand\ckminusj{\cindl{-\tj}{\tk}}
\newcommand\cknullj{\cindl{0\tj}{\tk}}


% the same for D

%\renewcommand\d{\mbox{$\TargetClass$}}                    %   D
%\renewcommand\dm{\TargetClass}                              %   D

%\newcommand\de{\mbox{$\semm{\TargetClass}$}}              % ||D||

%\newcommand\deind[1]{\mbox{$\semm{\TargetClass}^{#1}$}}   % ||D||^#1
%\newcommand\dindeind[2]{\mbox{$\semm{\AClass_{#1}}^{#2}$}}

%\newcommand\dind[1]{\mbox{$\TargetClass^{#1}$}}           %      C^#1
%\newcommand\dindl[2]{\mbox{$_{#1}\TargetClass^{#2}$}}     % _{#1}D^{#2}
%\newcommand\dindr[2]{\mbox{$\TargetClass_{#1}^{#2}$}}     %      D_{#1}^{#2}



%  Apply:
\newcommand\dej{\deind{\tj}}                         % ||C||^j
\newcommand\dek{\deind{\tk}}                         % ||C||^k
%\newcommand\deJ{\deind{\J}}

\newcommand\diei{\dindeind{i}{\ti}}                         % ||C||^j
\newcommand\djej{\dindeind{j}{\tj}}                         % ||C||^j
%\newcommand\dieJ{\deind{\J}}
%\newcommand\djeJ{\deind{\J}}

\newcommand\djk{\dind{\tj\tk}}
\newcommand\djplusk{\dindr{+\tk}{\tj}}
\newcommand\djnullk{\dindr{0\tk}{\tj}}
\newcommand\dkminusj{\dindl{-\tj}{\tk}}
\newcommand\dknullj{\dindl{0\tj}{\tk}}


%\renewcommand\f{\mbox{$\AReference$}}                    %   f
%\newcommand\fm{\AReference}                              %   f
%\newcommand\find[1]{\mbox{$\AReference^{#1}$}}           %      f^#1
\newcommand\fjk{\find{\tjk}}

%\newcommand\fe{\mbox{$\semm{\AReference}$}}              % ||f||
%\newcommand\feind[1]{\mbox{$\semm{\AReference}^{#1}$}}   % ||f||^#1
\newcommand\fej{\feind{\tj}}
\newcommand\fei{\feind{\ti}}
\newcommand\fek{\feind{\tk}}
\newcommand\fel{\feind{\tl}}

%\newcommand\feJ{\feind{\J}}

%\newcommand\findeind[2]{\mbox{$\semm{\AClass_{#1}}^{#2}$}}
%\newcommand\diei{\dindeind{i}{\ti}}                         % ||C||^j
%\newcommand\djej{\dindeind{j}{\tj}}                         % ||C||^j
 \newcommand\fiei{\findeind{i}{\ti}}                         % ||C||^j
 \newcommand\fjej{\findeind{j}{\tj}}                         % ||C||^j
%\newcommand\fieJ{\feind{\J}}
%\newcommand\fjeJ{\feind{\J}}

%\newcommand\fgcomp{\mbox{$\f(\g_1,\ldots,\g_m)$}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand\Distinctctu{\mbox{$^{\ltt}\!\semm{\ittt{Distinct}_{\cm}}^{\ltu}$}}
\newcommand\Distinctcst{\mbox{$^{\lts}\!\semm{\ittt{Distinct}_{\cm}}^{\ltt}$}}
\newcommand\Samectu{\mbox{$^{\ltt}\!\semm{\ittt{Same}_{\cm}}^{\ltu}$}}
\newcommand\Samecst{\mbox{$^{\lts}\!\semm{\ittt{Same}_{\cm}}^{\ltt}$}}
%=============
%%%%% Behset
\newcommand\xstatei[3]{\mbox{${\mathit {#1}state}^{#3}_{#2}$}}
\newcommand\statei[2]{\xstatei{}{#1}{#2}}
\newcommand\xstate[2]{\xstatei{#1}{}{#2}}
%\newcommand\tstatei[1]{\statei{#1}{\ltt}}

\newcommand\attrName[1]{{\mathit #1}}
\newcommand\methName[1]{{\mathit #1}}
\newcommand\statepoint[1]{#1}

%%%%%
% discussing string-based  vs graph-based logics
\newcommand\cmlang{{\bf L}}
\newcommand\myindex[1]{\mbox{\scriptsize{#1}}}
\newcommand\mathsymbol[1]{\mbox{$#1$}}
%\newcommand\repr{\mathsymbol{r}}
\newcommand\world%{\ittt{world}}
{\mathsymbol{\cal W}}
\newcommand\cmter%{\ittt{computer}}
{\mathsymbol{\cal C}}
\newcommand\topos{\mathsymbol{\cal S}}


%----------------------
\newcommand\viewob[1]{\object{V}{#1}}
\newcommand\thob[1]{\object{T}{#1}}
\newcommand\uniob[1]{\object{U}{#1}}
\newcommand\uniobmath[1]{\objectmath{U}{#1}}
\newcommand\uniobind[1]{\objectind{U}{#1}}

\newcommand\UNI{\universe{U}}
\newcommand\UNIind{\universeind{U}}
\newcommand\UNImath{\universeind{U}} % the same
\newcommand\Setsind{\universeind{Sets}}

\newcommand\particularUni[1]{\mbox{$\mathbf{#1}$}}
\newcommand\particularUniInd[1]{\mathbf{#1}}
\newcommand\Sets{\particularUni{Sets}}
\newcommand\Varsets{\particularUni{VarSets}}
\newcommand\Behsets{\particularUni{BehSets}}
\newcommand\Sketches{\particularUni{Sketches}}


\newcommand\skeproc{\proc{ske}}
\newcommand\arrdlproc{\procind{Formal}{ArrDL}}
\newcommand\elmslproc{\procind{Formal}{ElmSL}}

%\newcommand\formalPar[1]{\mbox{$\mathrm #1$}}
\newcommand\formalParBold[1]{\mbox{$#1$}}
\newcommand\lf{\formalParBold{L}}
\newcommand\mf{\formalPar{M(D)}}
\newcommand\uf{\formalPar{U}}
\newcommand\df{\formalPar{D}}
\newcommand\tdf{\mbox{$\thob(\diag)$}}
\newcommand\sdf{\mbox{$\skeob{}(\diag)$}}

\newcommand\str{\formalPar{\sigma}}
%(7)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Created on May 4,2001
%============================================
% Part 1: pure italic writing of names
%        formerly file italic.tex
%--------------------------------------------
% Part 2: commands for semantics extensions of classes
%         like [[Person]]^t or {^t}[[SamePerson]]^{u}
%        formerly file employ.tex
%===========================================

\newcommand\operarrow[2]{\mbox{{\sffamily%\itshape
                                         #1}$_{#2}$}}
\newcommand\projop[1]{\operarrow{p}{#1}}
%\newcommand\concatop{\operarrow{concat}{}}
%\newcommand\pairop{\operarrow{pair}{}}
%\newcommand\idop[1]{\operarrow{id}{#1}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\newcommand\ltt{\mbox{$t$}}
%\newcommand\ltu{\mbox{$u$}}
%\newcommand\lts{\mbox{$s$}}

%

\newcommand\Emplsem[1]{\mbox{$\semm{\Empl}^{#1}$}}
\newcommand\Emplt{\Emplsem{\ltt}}
\newcommand\Emplu{\Emplsem{\ltu}}
\newcommand\Empls{\Emplsem{\lts}}
\newcommand\Empltu{\mbox{$^{\ltt}\!\semm{\Empl}^{\ltu}$}}
\newcommand\Emplst{\mbox{$^{\lts}\!\semm{\Empl}^{\ltt}$}}
\newcommand\SameEmpltu{\mbox{$^{\ltt}\!\semm{\SameEmpl}^{\ltu}$}}
\newcommand\SameEmplst{\mbox{$^{\lts}\!\semm{\SameEmpl}^{\ltt}$}}

\newcommand\Compsem[1]{\mbox{$\semm{\Comp}^{#1}$}}
\newcommand\Compt{\Compsem{\ltt}}
\newcommand\Compu{\Compsem{\ltu}}
\newcommand\Comps{\Compsem{\lts}}
\newcommand\Comptu{\mbox{$^{\ltt}\!\semm{\Comp}^{\ltu}$}}
\newcommand\Compst{\mbox{$^{\lts}\!\semm{\Comp}^{\ltt}$}}
\newcommand\SameComptu{\mbox{$^{\ltt}\!\semm{\SameComp}^{\ltu}$}}
\newcommand\SameCompst{\mbox{$^{\lts}\!\semm{\SameComp}^{\ltt}$}}

\newcommand\Engrsem[1]{\mbox{$\semm{\Engr}^{#1}$}}
\newcommand\Engrt{\Engrsem{\ltt}}
\newcommand\Engru{\Engrsem{\ltu}}
\newcommand\Engrs{\Engrsem{\lts}}
\newcommand\Engrtu{\mbox{$^{\ltt}\!\semm{\Engr}^{\ltu}$}}
\newcommand\Engrst{\mbox{$^{\lts}\!\semm{\Engr}^{\ltt}$}}

\newcommand\Mngrsem[1]{\mbox{$\semm{\Mngr}^{#1}$}}
\newcommand\Mngrt{\Mngrsem{\ltt}}
\newcommand\Mngru{\Mngrsem{\ltu}}
\newcommand\Mngrs{\Mngrsem{\lts}}
\newcommand\Mngrtu{\mbox{$^{\ltt}\!\semm{\Mngr}^{\ltu}$}}
\newcommand\Mngrst{\mbox{$^{\lts}\!\semm{\Mngr}^{\ltt}$}}

\newcommand\John[1]{\mbox{$\ittt{John}^{#1}$}}

\newcommand\Marr{\ittt{Married}}
\newcommand\Marrsem[1]{\mbox{$\semm{\Marr}^{#1}$}}
\newcommand\Marrt{\Marrsem{\ltt}}
\newcommand\Marru{\Marrsem{\ltu}}
\newcommand\Marrs{\Marrsem{\lts}}
\newcommand\Marrtu{\mbox{$^{\ltt}\!\semm{\Marr}^{\ltu}$}}
\newcommand\Marrst{\mbox{$^{\lts}\!\semm{\Marr}^{\ltt}$}}

\newcommand\Famy{\ittt{Family}}
\newcommand\Famysem[1]{\mbox{$\semm{\Famy}^{#1}$}}
\newcommand\Famyt{\Famysem{\ltt}}
\newcommand\Famyu{\Famysem{\ltu}}
\newcommand\Famys{\Famysem{\lts}}
\newcommand\Famytu{\mbox{$^{\ltt}\!\semm{\Famy}^{\ltu}$}}
\newcommand\Famyst{\mbox{$^{\lts}\!\semm{\Famy}^{\ltt}$}}
\newcommand\Famytt{\mbox{$^{\ltt}\!\semm{\Famy}^{\ltt}$}}
\newcommand\Familytu{\mbox{$^{\ltt}\!\semm{\Famy}^{\ltu}$}}
\newcommand\Familyst{\mbox{$^{\lts}\!\semm{\Famy}^{\ltt}$}}

\newcommand\Friendship{\ittt{Friendship}}
\newcommand\Friship{\ittt{Friendship}}
\newcommand\Frishiptu{\mbox{$^{\ltt}\!\semm{\Friship}^{\ltu}$}}
\newcommand\Frishipst{\mbox{$^{\lts}\!\semm{\Friship}^{\ltt}$}}


\newcommand\Matr{\ittt{Matrimony}}
\newcommand\Matrsem[1]{\mbox{$\semm{\Matr}^{#1}$}}
\newcommand\Matrt{\Matrsem{\ltt}}
\newcommand\Matru{\Matrsem{\ltu}}
\newcommand\Matrs{\Matrsem{\lts}}
\newcommand\Matrtu{\mbox{$^{\ltt}\!\semm{\Matr}^{\ltu}$}}
\newcommand\Matrst{\mbox{$^{\lts}\!\semm{\Matr}^{\ltt}$}}

\newcommand\Distincttu{\mbox{$^{\ltt}\!\semm{\ittt{Distinct}}^{\ltu}$}}
\newcommand\Distinctst{\mbox{$^{\lts}\!\semm{\ittt{Distinct}}^{\ltt}$}}
\newcommand\Sametu{\mbox{$^{\ltt}\!\semm{\ittt{Same}}^{\ltu}$}}
\newcommand\Samest{\mbox{$^{\lts}\!\semm{\ittt{Same}}^{\ltt}$}}

\newcommand\Wom{\ittt{Woman}}
\newcommand\Womsem[1]{\mbox{$\semm{\Wom}^{#1}$}}
\newcommand\Womt{\Womsem{\ltt}}
\newcommand\Womu{\Womsem{\ltu}}
\newcommand\Woms{\Womsem{\lts}}
\newcommand\Womtu{\mbox{$^{\ltt}\!\semm{\Wom}^{\ltu}$}}
\newcommand\Womst{\mbox{$^{\lts}\!\semm{\Wom}^{\ltt}$}}

%\newcommand\Man{\ittt{Man}}
\newcommand\Mansem[1]{\mbox{$\semm{\Man}^{#1}$}}
\newcommand\Mant{\Mansem{\ltt}}
\newcommand\Manu{\Mansem{\ltu}}
\newcommand\Mans{\Mansem{\lts}}
\newcommand\Mantu{\mbox{$^{\ltt}\!\semm{\Man}^{\ltu}$}}
\newcommand\Manst{\mbox{$^{\lts}\!\semm{\Man}^{\ltt}$}}

\newcommand\Husbsem[1]{\mbox{$\semm{\Husb}^{#1}$}}
\newcommand\Husbt{\Husbsem{\ltt}}
\newcommand\Husbu{\Husbsem{\ltu}}
\newcommand\Husbs{\Husbsem{\lts}}
\newcommand\Husbtu{\mbox{$^{\ltt}\!\semm{\Husb}^{\ltu}$}}
\newcommand\Husbst{\mbox{$^{\lts}\!\semm{\Husb}^{\ltt}$}}


\newcommand\mysemm[2]{\mbox{$\semm{#1}^{#2}$}}

\newcommand\isarrt{\mysemm{\isa}{\ltt}}
\newcommand\isarru{\mysemm{\isa}{\ltu}}

\newcommand\wifet{\mysemm{\wife}{\ltt}}
\newcommand\wifeu{\mysemm{\wife}{\ltu}}

\newcommand\husbt{\mysemm{\husb}{\ltt}}
\newcommand\husbu{\mysemm{\husb}{\ltu}}

\newcommand\mdatet{\mysemm{\mDate}{\ltt}}
\newcommand\mdateu{\mysemm{\mDate}{\ltu}}

\newcommand\liveset{\mysemm{\livesAt}{\ltt}}
\newcommand\liveseu{\mysemm{\livesAt}{\ltu}}

\newcommand\income{\ittt{income}}
\newcommand\WMHsem[2]{\mbox{$
      (\semm{\Wom}^{#1}\times\semm{\Man}^{#1}\times\semm{\House}^{#1})
\times
      (\semm{\Wom}^{#2}\times\semm{\Man}^{#2}\times\semm{\House}^{#2})
                            $}
                     }
\newcommand\WMHtu{\WMHsem{\ltt}{\ltu}}


\newcommand\WMWMsem[2]{\mbox{$(\semm{\Wom}^{#1}\times\semm{\Man}^{#1})
                        \times(\semm{\Wom}^{#2}\times\semm{\Man}^{#2})
                             $}
                        }
\newcommand\WMWMtu{\WMWMsem{\ltt}{\ltu}}


\newcommand\myview[1]{\mbox{$V_{#1}$}}
\newcommand\IndI{1}
\newcommand\SWAggr{2}
\newcommand\AggrI{3}
\newcommand\TWAggrG{4}
\newcommand\IndII{5}
\newcommand\TWAggrS{6}
\newcommand\LAggr{7}
\newcommand\LLAggr{8}
\newcommand\SWLAggr{9}
\newcommand\STWAggr{10}
\newcommand\DelAggr{11}
\newcommand\TotAggr{12}
\newcommand\WQual{13}
 \newcommand\LQual{14}
\newcommand\AttrI{15}
\newcommand\SWLQual{16}
\newcommand\STWQual{17}
\newcommand\AttrII{18}



%(8)
%\newcommand\s{\mbox{$S$}}
%\newcommand\os{\mbox{$\overline{S}$}}
%\newcommand\ovr[1]{\mbox{$\overline{#1}$}}
\newcommand\into[1]{\stackrel{#1}{\hookrightarrow}}
\newcommand\repgra{\nicex{ R$}}
\newcommand\rgra{\repgra}
\newcommand\nds[1]{\mbox{$\mathit{Nds}#1$}}
\newcommand\arrs[1]{\mbox{$\mathit{Arrs}#1$}}
\newcommand\ndsr{\nds{\rgra}}
\newcommand\arrsr{\arrs{\rgra}}

\newcommand\dersetmath{\mathit{Der}}
\newcommand\derset{\mbox{$\dersetmath$}}
\newcommand\derop{\mbox{$\mathbf{der}$}}
\newcommand\algebra[1]{\mbox{$\alpha^{#1}$}}
\newcommand\algu{\algebra{\uskemath}}

%\newcommand\inss[1]{\lar{I}{\ske{#1}}{\uske}}
%\newcommand\ovri{\mbox{$\overline{I}$}}
%\newcommand\ovrinss[1]{\lar{\ovri_{#1}}{\ovrs{#1}}{\uske}}

\newcommand\ovrske[1]{\mbox{$\overline{\ske{#1}}$}}
\newcommand\ovrs[1]{\mbox{$\overline{\ske{#1}}$}}
%-----------------------------
\newcommand\sv{\mbox{$\ske{V}$}}
\newcommand\sr{\mbox{$\ske{R}$}}
\newcommand\vmor{\lar{v}{\sv}{\ovrske{}}}
\newcommand\rmor{\lar{r}{S}{\ovrske{R}}}
\newcommand\emor{\lar{e}{S}{\U}}
\newcommand\vpair{\mbox{$V=(\sv,v)$}}
\newcommand\rpair{\mbox{$R=(\sr,r)$}}



%\newcommand\dbinst{\lar{e}{S}{W} }

%---------------------------------------------------


\newcommand\ovrsig[1]{\mbox{$\overline{\sigma _{#1}}$}}
\newcommand\ovrg[1]{\mbox{$\overline{G_{#1}}$}}
%-----------------------------------------
\newcommand\ovrp{\mbox{$\overline{\pi }$}}%{#1}}$}}
\newcommand\ovreps{\mbox{$\overline{\vare}$}}     % overlined epsilon


%\renewcommand\endinput{}
%\newcommand\comp{\mathbin{\triangleright\!\!\triangleright}}
\newcommand\state[2]{\mbox{${\mathit{state}}^{#1}_{#2}$}}
\newcommand\starInherit{*-inherit}

\newcommand\sig{\mbox{$\Sigma $}}
\newcommand\sigm{\Sigma}
\newcommand\defitemotstup[1]{\par\smallskip\noindent (#1)}


\newcommand\arity[1]{\mbox{$\mathit{Arity}(#1)$}}
\newcommand\predsem[2]{\mbox{$\semm{#1}^{#2} $}}
\newcommand\psem[1]{\predsem{P}{#1}}
\newcommand\psemu{\psem{\ucatmath}}
\newcommand\lsig{\mbox{$\Lambda $}}

%%%
\newcommand\Attr{\mbox{$\mathit{Attr}$}}
\newcommand\Var{\mbox{$\mathit{Var}$}}
\newcommand\relcat{\mbox{$\categoryname{Rel}$}}
\newcommand\relske{\mbox{$\sketchname{Rel}$}}
\newcommand\itte[1]{\mbox{\textit{#1}}}
\newcommand\dbcat{\mbox{$\categoryname{DB}$}}

\newcommand\skecat[1]{\mbox{$\categoryname{Sketch}(\sig_{#1})$}}
\newcommand\sigcat{\mbox{$\categoryname{Sign}$}}

\newcommand\funor{\mbox{$\Phi$}}
\newcommand\funarr{\lar{f}{X}{Y}}
\newcommand\currfun{\mbox{\lar{\Map{A}{\_}}{\catset}{\catset}}}
\newcommand\curra{\Map{A}{\_}}

% \newcommand\ {\itte{ }}
\newcommand\target{\itte{target}}
\newcommand\source{\itte{source}}
\newcommand\conof{\itte{consistsOf}}
\newcommand\marker{\itte{marker}}
\newcommand\Node{\itte{Node}}
\newcommand\nodeit{\ittt{node}}
\newcommand\Arrow{\itte{Arrow}}
\newcommand\arrow{\ittt{arrow}}
\newcommand\diagramit{\itte{diagram}}
\newcommand\graphit{\itte{graph}}
\newcommand\shape{\itte{shape}}
\newcommand\predecl{\itte{predicate\_declarations}}
\newcommand\statements{\itte{statements}}
\newcommand\carrier{\itte{carrier}}
\newcommand\arityshape{\itte{arity\_shape}}


% semiotics
%% MACROS OF Dec 3
\newcommand\formalObj[1]{\mbox{\sffamily #1}}
\newcommand\formalOper[1]{\mbox{{\bfseries\sffamily #1}}}
\newcommand\informalObj[1]{\mbox{\textit #1}}
\newcommand\informalOper[1]{\mbox{{\bfseries\itshape #1}}}

\newcommand\lzzl{\formalObj{l}}  %logic
\newcommand\ml{\informalObj{ML}}  % modeling language

\newcommand\f{\formalObj{F}}
\renewcommand\c{\informalObj{C}}
\newcommand\derf{\formalOper{Der}}
\newcommand\deri{\informalOper{Un}}
\newcommand\derff{\derf.\f}
\newcommand\deric{\deri(\c)}
\newcommand\FormalInterpret[1]{\mbox{$\formalObj{i}_f$}}
\newcommand\SubstantInterpret[1]{\mbox{$\informalObj{i}_s$}}


%====================================

\newcommand\informalPar[1]{\nicex{{#1}$}}
\newcommand\infParind[1]{\cal #1}
\newcommand\formalPar[1]{\mbox{$\mathrm{#1}$}}
\newcommand\frmParind[1]{\mathrm{#1}}

\newcommand\informalParBold[1]{\mbox{${\cal #1}$}}
%\newcommand\formalPar[1]{\mbox{$\mathrm #1$}}

\newcommand\object[2]{\mbox{${\mathsf{#1}}_{#2}$}}
%\newcommand\object[2]{\mbox{$#1_{#2}$}}
\newcommand\universe[1]{\mbox{$\mathbf{#1}$}}
%\newcommand\objectind[1]{\mathsf{#1}}
\newcommand\objectind[1]{\mathsf{#1}}
\newcommand\objectmath[1]{\mathsf{#1}} % the same
\newcommand\universeind[1]{\mathbf{#1}}
\newcommand\umath[1]{\mathbf{U}_{#1}}

\newcommand\proc[1]{\mbox{\sffamily\bfseries #1}}
\newcommand\procind[2]{\mbox{${\mathrm{#1}}_{\mathrm #2}$}}
\newcommand\linf{\informalParBold{L}}
\newcommand\minf{\mbox{$\informalPar{M}(\diag{})$}}
\newcommand\mdinf{\mbox{$\informalPar{M}(\diag{})$}} % the same as above
\newcommand\mdfrm{\mbox{$\formalPar{M}(\diag{})$}} % the same as above
\newcommand\uinf{\informalPar{U}}

\newcommand\meaninf{\informalPar{M}}
\newcommand\meanfrm[1]{\mbox{$\formalPar{M}_{#1}$}}

\newcommand\diags{\mbox{$\mathit{Diags}$}}
\newcommand\graph{\mbox{$\mathit{Graph}$}}

\newcommand\diaob[1]{\object{D}{#1}} %\mbox{$D$}}
\newcommand\diagob[1]{\object{D}{#1}} %the same \mbox{$D$}}
\newcommand\diag[1]{\object{D}{#1}} %the same \mbox{$D$}}
\newcommand\diaind{\objectind{D}}

\newcommand\graob[1]{\object{G}{#1}}
\newcommand\graind{\objectind{G}}
\newcommand\gra[1]{\graob{#1}}

\newcommand\skeob[1]{\object{S}{#1}}
\newcommand\skeind{\objectind{S}}

\newcommand\modelob[1]{\object{M}{#1}}
\newcommand\modelind{\objectind{M}}

\newcommand\sigob[1]{\object{\mbox{$\Sigma$}}{#1}}
\newcommand\skediag{\skeob{}[\diag{}]}

\newcommand\meaninfdiag{\meaninf[\diag{}]}
\newcommand\meanfrmdiag{\meanfrm[\diag{}]}
% synonyms
\newcommand\meanifdiag{\meaninf[\diag{}]}
\newcommand\meanfdiag{\meanfrm[\diag{}]}

%%% diags, sketchs, specs, and their semantic interpretaions
\newcommand\objectWithInd[3]{\mbox{$\mathsf{#1}_{#2}^{#3}$}}
\newcommand\sketch[1]{\objectWithInd{S}{#1}{}}
\renewcommand\ske[1]{\sketch{#1}}
%\newcommand\graph[1]{\objectWithInd{S}{#1}{}}
\renewcommand\diag[1]{\objectWithInd{D}{#1}{}}
%\newcommand\inst[2]{\mbox{$\mathit{Inst}^{#2}{(#1)}$}}
%\newcommand\instob[2]{\mbox{$\mathit{Inst}^{#2}{(#1)}$}}


%\newcommand\diaob[1]{\mbox{$\diag{#1}$}}
%\newcommand\skeob{\mbox{$S$}}
\newcommand\graofske{\mbox{$G_\skeind$}}
\newcommand\graske{\graofske}
\newcommand\diaofske{\mbox{$D_\skeind$}}
\newcommand\diaske{\diaofske}


\renewcommand\eg{e.g.}
\renewcommand\C{\mbox{$C$}}

\newcommand\ext[1]{\mbox{$\mathit{Ext}(#1)$}}
\renewcommand\stt[1]{\mbox{$\mathit{Stt}(#1)$}}
\newcommand\GCS{{\bf (GCS)}}
\newcommand\AET{{\bf (AET)}}



%\newcommand\tuple[1]{\left [ \mathstrut {#1} \right ]}
\newcommand\pmrk[1]{\mbox{[{\sf #1}]}}
\newcommand\omrk[1]{\mbox{[{\sf #1} $\rangle $}}

% used in Intro
\newcommand\lanfrm{\formalPar{FL}}
\newcommand\flan{\formalPar{FL}} %the same
\newcommand\flanind{\frmParind{FL}}

\newcommand\x{\diag{}}   %\mbox{$D$}}
\renewcommand\s{\skeob{}}%\mbox{$S$}}
%\newcommand\mix{\mbox{$\meaninf$}} %(\x)
%\newcommand\mfx{\mbox{$\meanfrm{\flanind}$}} %(\x)
\newcommand\mix{\mbox{$\meaninf(\x)$}}
\newcommand\mfx{\mbox{$\meanfrm{}(\x)$}}

%\newcommand\flan{\mbox{$\meanfrm(\x)$}}

\newcommand\spex[1]{\mbox{$\skeob{#1}$}} %(\mix)$}}
\newcommand\spem[1]{\mbox{$\skeob{#1}$}} %(\mix)$}}
\newcommand\spexl  {\mbox{$\skeob{\flanind}$}} %(\x)$}}
\newcommand\speml  {\mbox{$\skeob{}$}} %(\mfx)$}}

\newcommand\dateit{\ittt{date}}

% used in dGetStartViaAss
\newcommand\nis{\nicex{ S$}}
\newcommand\niv{\nicex{ V$}}
\newcommand\nivind{{V}}
\newcommand\nisind{{S}}

\newcommand\mrkdual[3]{\mbox{${#2}\stackrel{{\cal\scriptsize #1}}{[><]}{#3}$}} %{[>^{\mathrm{#1}}<]}$}}
\newcommand\sgv{single-valued}
\newcommand\assgenpred{\mbox{$[\Uparrow]$}}
\newcommand\SepPred{\mrk{1-1}  }
\newcommand\CovPred{\mrk{cover}}
\newcommand\MemPred{\mrk{$\in$}}

\newcommand\binAss{1}
\newcommand\assCla{2}
\newcommand\reiAss{3}
\newcommand\terAss{4}
\newcommand\quaAss{5}
\newcommand\skeo{\skeob{\binAss}}
\newcommand\skei{\skeob{\assCla}}
\newcommand\skeii{\skeob{\reiAss}}
\newcommand\skeiii{\skeob{\terAss}}
\newcommand\skeiv{\skeob{\quaAss}}
%\newcommand\diaob[1]{\diag{#1}}
\newcommand\diao{\diaob{\binAss}}
\newcommand\diai{\diaob{\assCla}}
\newcommand\diaii{\diaob{\reiAss}}
\newcommand\diaiii{\diaob{\terAss}}
\newcommand\diaiv{\diaob{\quaAss}}


\newcommand\visfunctor{\mbox{{\sffamily\bfseries vis}}}
\newcommand\skefunctor{\mbox{{\sffamily\bfseries ske}}}

%used in eAssonBySke
\newcommand\sale{\ittt{sale}}
\newcommand\Show{\ittt{Show}}
\renewcommand\show{\ittt{show}}
\newcommand\seat{\ittt{seat}}
\newcommand\perf{\ittt{perf}}
\newcommand\Performance{\ittt{Performance}}
\newcommand\Ticket{\ittt{Ticket}}
\newcommand\ticket{\ittt{sale}}
\newcommand\Integer{\ittt{Integer}}

\newcommand\mastr[1]{\mbox{$\mathbf{#1}$}}
\newcommand\extofcla[1]{\mastr{\semm{\mathit #1}}}
\newcommand\behofcla[1]{\mastr{\besemm{\mathit{#1}}}}
\newcommand\sttofcla[1]{\lar{\statemap{}{\mathit{#1}}}{\extofcla{#1}}{\behofcla{#1}}}

%\newcommand\tlu{\mbox{$t<u$}}
%\newenvironment\mathitext%
%{
%\begin{displaymath}
%\mbox{ }
%\end{displaymath}
%} {}
\newcommand\cEngine{\ittt{carEngine}}
\newcommand\carEngine{\ittt{carEngine}}


\newcommand\mrkmon[2]{\mbox{\mrk{1-1}$^{#1}_{\mathit{#2}}$}}
\newcommand\mrkfro[2]{\mbox{\mrk{fro}$^{#1}_{\mathit{#2}}$}}
\renewcommand\mrkid[2]{\mbox{\mrk{id}$^{#1}_{\mathit{#2}}$}}
\newcommand\mrkstrongid[2]{\mbox{\mrk{id!}$^{#1}_{\mathit{#2}}$}}
\newcommand\mrkdel[2]{\mbox{\mrk{del}$^{#1}_{\mathit{#2}}$}}
\newcommand\mrkins[2]{\mbox{\mrk{ins}$^{#1}_{\mathit{#2}}$}}

\newcommand\mathand{\mbox{ and }}
\newcommand\mathor{\mbox{ or }}
\newcommand\mathif{\mbox{ if }}
\newcommand\maththen{\mbox{ then }}
\newcommand\mathiff{\mbox{ iff }}
%\newcommand\ofit{\ittt{of}}
\newcommand\wholeit{\ittt{whole}}
\newcommand\Wholeit{\ittt{Whole}}
\newcommand\partit{\ittt{part}}
\newcommand\stateit{\ittt{state}}
\newcommand\prokol{{\mathbf +}\!\!\!\!\circ}

\newcommand\mixsemm[1]{\mbox{$\lbesemm\, {\mathit #1} \, \rsemm$}}

\newcommand\logrule[2]{\frac{\mathstrut #1}{\mathstrut #2}}
\newcommand\logruleFig[2]{\frac{\mathstrut #1}{\mathstrut #2}}
\newcommand\logruleRow[2]{\mbox{if $#1$ then $#2$}}
\newcommand\logruleFigText[2]{\mbox{$
\frac{\mbox{\rule[-1ex]{0pt}{3ex} #1}}{\mbox{\rule{0pt}{3ex} #2}} $}
}
\newcommand\logruleRowText[2]{\mbox{if #1 then #2}}


\newcommand\ClassIndInd[3]{\mbox{$^{#1}\!\semm{\mathit{#2}}^{#3}$}}
\newcommand\ClassBeh[1]{\mbox{$\besemm{\mathit{#1}}$}}

\newcommand\refInd[2]{\mbox{$\semm{\mathit{#1}}^{\mathit{#2}}$}}
\newcommand\refBehInd[2]{\mbox{$\besemm{\mathit{#1}}^{\mathit{#2}}$}}
\newcommand\refIndBeh[2]{\mbox{$\besemm{\mathit{#1}}^{\mathit{#2}}$}}




\renewcommand\same[2]{\mbox{${\mathit{same}}^{#1}_{\mathit{#2}}$}}
\newcommand\samemap[2]{\mbox{${\mathit{same}}^{#1}_{\mathit{#2}}$}}
%\newcommand\sametu[1]{\samemap{tu}{#1}}
\newcommand\delset[3]{\mbox{$\semm{#3}^{#1}\mathsf{Del}^{#1\rightarrow #2}$}}
\newcommand\deltu[1]{\delset{t}{u}{#1}}
\newcommand\newset[3]{\mbox{$\semm{#3}^{#1}\mathsf{New}^{#2\rightarrow #1}$}}
\newcommand\newut[1]{\newset{u}{t}{#1}}
\newcommand\newts[1]{\newset{t}{s}{#1}}
%\newcommand\insut[1]{\newset{t}{u}{#1}}
%\newcommand\newut[1]{\newset{t\leftarrow u}{#1}} %  correct
%\newcommand\newtu[1]{\newset{t\leftarrow u}{#1}} % incorrect, to match old
%\newcommand\newts[1]{\newset{s\leftarrow t}{#1}} %correct,
%\newcommand\newst[1]{\newset{s\leftarrow t}{#1}} %incorrect, to match old
\newcommand\statemap[2]{\mbox{${\mathit{state}}^{#1}_{\mathit{#2}}$}}



\newcommand\ofit{\ittt{of}}
\newcommand\ofmap[1]{\refInd{of}{#1}}
%\newcommand\ofit{\ofmap{}}
\newcommand\oft{\ofmap{t}}
\newcommand\ofu{\ofmap{u}}

\newcommand\ofindit{\mbox{$\semm{{\mathit of}_i}^{t}$}}
%\newcommand\ofindiu{\mbox{$\semm{{\mathit of}_i}^{u}$}}
\newcommand\ofiu{\mbox{$\semm{{\mathit of}_i}^{u}$}}
%
\newcommand\isit{\ittt{is}}
\newcommand\ismap[1]{\refInd{is}{#1}}
%\newcommand\isit{\ismap{}}
\newcommand\ist{\ismap{t}}
\newcommand\isu{\ismap{u}}


\newcommand\isindt{\mbox{$\semm{{\mathit is}_i}^{t}$}}
\newcommand\isindu{\mbox{$\semm{{\mathit is}_i}^{u}$}}
%

\newcommand\hasit{\ittt{has}}
\newcommand\hasmapbeh{\besemm{has}}
\newcommand\hasbeh{\besemm{has}}
\newcommand\hasbehind[1]{\besemm{has}_{#1}}


\newcommand\supmap[1]{\refInd{sup}{#1}}
\newcommand\supit{\supmap{}}
\newcommand\supt{\supmap{t}}
\newcommand\supu{\supmap{u}}
%
\newcommand\supbeh{\besemm{sup}}
%
\newcommand\submap[1]{\refInd{sub}{#1}}
\newcommand\subit{\submap{}}
\newcommand\subt{\submap{t}}
\newcommand\subu{\submap{u}}

\newcommand\isamap[1]{\refInd{isA}{#1}}
\newcommand\isait{\isamap{}}
\newcommand\isat{\isamap{t}}
\newcommand\isau{\isamap{u}}
\newcommand\isabeh{\besemm{\isa}}

\newcommand\Persontu{\ClassIndInd{t}{Person}{u}}
\newcommand\Persont{\ClassIndInd{}{Person}{t}}
\newcommand\Personu{\ClassIndInd{}{Person}{u}}
\newcommand\PersonBeh{\ClassBeh{Person}}

\newcommand\Drivertu{\ClassIndInd{t}{Driver}{u}}
\newcommand\Drivert{\ClassIndInd{}{Driver}{t}}
\newcommand\Driveru{\ClassIndInd{}{Driver}{u}}



\newcommand\Cart{\ClassIndInd{}{Car}{t}}
\newcommand\Caru{\ClassIndInd{}{Car}{u}}
\newcommand\Cartu{\ClassIndInd{t}{Car}{u}}
\newcommand\SameCartu{\ClassIndInd{t}{SameCar}{u}}
\newcommand\CarBeh{\ClassBeh{Car}}
\newcommand\Carbeh{\ClassBeh{Car}}
\newcommand\Ownershiptu{\ClassIndInd{t}{Ownership}{u}}
\newcommand\Ownershipt{\ClassIndInd{}{Ownership}{t}}
\newcommand\Ownershipu{\ClassIndInd{}{Ownership}{u}}



\newcommand\Ownership{\ittt{Ownership}}
\newcommand\owner{\ittt{owner}}
%\newcommand\car{\ittt{car}}
%\newcommand\property{\ittt{property}}

%\newcommand\Engine{\ittt{Engine}}
%\newcommand\Eng{\ittt{Eng}}
\newcommand\Enginetu{\ClassIndInd{t}{Engine}{u}}
\newcommand\Enginet{\ClassIndInd{}{Engine}{t}}
\newcommand\Engineu{\ClassIndInd{}{Engine}{u}}
\newcommand\EngineBeh{\ClassBeh{Engine}}
\newcommand\Enginebeh{\ClassBeh{Engine}}
\newcommand\Engbeh{\ClassBeh{Engine}}
\newcommand\BodyBeh{\ClassBeh{Body}}
\newcommand\ChassisBeh{\ClassBeh{Chassis}}


%\newcommand\Engine{\ittt{Engine}}
%\newcommand\Eng{\ittt{Eng}}
%\newcommand\Body{\ittt{Body}}
%\newcommand\BodyBeh{\ClassBeh{Body}}
%\newcommand\Chassis{\ittt{Chassis}}
%\newcommand\ChassisBeh{\ClassBeh{Chassis}}
%%\newcommand\PartName{Part}

%\newcommand\drives{\ittt{drives}}
\newcommand\drivest{\refInd{drives}{t}}
\newcommand\drivesu{\refInd{drives}{u}}
\newcommand\drivesbeht{\refBehInd{drives}{t}}
\newcommand\drivesbehu{\refBehInd{drives}{u}}
\newcommand\drivesbehv{\refBehInd{drives}{v}}
\newcommand\drivesbeh{\refBehInd{drives}{}}

\newcommand\fuelat{\refInd{fuelAmount}{t}}
%\newcommand\fuelAm{\ittt{fuelAmount}}
%\newcommand\tankVo{\ittt{tankVolume}}
%\newcommand\fillTa{\ittt{fillTank}}
%\newcommand\car{\ittt{car}}

\newcommand\tankvt{\refInd{tankVolume}{t}}
\newcommand\tankvu{\refInd{tankVolume}{u}}

\newcommand\cart{\refInd{car}{t}}
\newcommand\caru{\refInd{car}{u}}

\newcommand\prst{\refInd{prs}{t}}
\newcommand\prsu{\refInd{prs}{u}}

\newcommand\enginet{\refInd{engine}{t}}
\newcommand\engineu{\refInd{engine}{u}}

\newcommand\persont{\refInd{person}{t}}
\newcommand\personu{\refInd{person}{u}}



\newcommand\PersonP{\Person$^+$}
\newcommand\PersonM{\Person$^-$}
\newcommand\CarP{\Car$^+$}
\newcommand\CarM{\Car$^-$}


\newcommand\floatRange[1]{\mrk{Float(#1)}}

%\newcommand\Car{\ittt{Car}}


\newcommand\becar{\besemm{\Car}}
\newcommand\beCar{\besemm{\Car}}
\newcommand\lt{$t$}
\newcommand\tstate{\statei{}{\ltt}}
\newcommand\stts{\statepoint{s}}



% === composition: begin
\newcommand\ipart[1]{\mbox{$\mathit{Part}_{#1}$}}
\newcommand\ipartmath[1]{\mathit{Part}_{#1}}
\newcommand\ipartbeh[1]{\mbox{$\besemm{\ipart{#1}}$}}

\newcommand\imeth[1]{\mbox{$\mathit{Meth}_{#1}$}}
\newcommand\imethbeh[1]{\mbox{$\besemm{\imeth{#1}}$}}
\renewcommand\imeth[1]{\mbox{$\mathit{Meth}_{#1}$}}
\newcommand\imethstar[1]{\mbox{$\mathit{Meth}^*_{#1}$}}
\newcommand\istameth[1]{\imethstar{#1}} %the same

\newcommand\iiface[1]{\mbox{$\mathbf{IFace}_{#1}$}}
\newcommand\iifacestar[1]{\mbox{$\mathbf{IFace}^*_{#1}$}}
\newcommand\iistaface[1]{\iifacestar{#1}} %the same


\newcommand\prodspace{\mbox{$\prod_{i}\ipartbeh{i}$}}
\newcommand\prodspa{\mbox{$\prod_{i}\ipartbeh{i}$}}
\newcommand\wholespace{\mbox{$\prod_{i}^*\ipartbeh{i}$}}

\newcommand\prodmeths{\mbox{$%\prod_{i}\imeth{i}
                             \methsset{prod}$}}
\newcommand\wholemeths{\mbox{$%\prod^*_{i}\imeth{i}
                             \someofmethsset{Prod}$}}
\newcommand\prodmethsbeh{\mbox{$\besemm{\prodmeths}$}}
\newcommand\wholemethsbeh[2]{\mbox{$\besemm{\someofmeths{#1}{#2}}$}}
\newcommand\prodiface{\mbox{$%\prod_{i}\iiface{i}
                              \iface{Prod}$}}
\newcommand\wholeiface{\mbox{$%\prod^*_{i}\iiface{i}
                               \ifacepartial{Prod}$}}



%\newcommand\reductmap[1]{\mbox{$\mathit{red}^*_{\mathit{#1}}$}}
\newcommand\reductmap[2]{\mbox{$\mathit{red}^{\mathit{#1}}_{\mathit{#2}}$}}
%\newcommand\reductmapstar[1]{\mbox{$\mathit{red}^*_{\mathit{#1}}$}}
\newcommand\red[2]{\reductmap{#1}{#2}}
\newcommand\redsta[1]{\reductmapstar{#1}}
\newcommand\projectmap[1]{\mbox{$\mathit{proj}_{\mathit{#1}}$}}
%\renewcommand\proj[1]{\projectmap{#1}}
\newcommand\fproj[1]{\mbox{$\pi_{#1}$}}


%==== composition: end =========

\renewcommand\Eng[1]{\mbox{$\mathit{Eng}^#1$}}
\renewcommand\eng[1]{\mbox{$\mathit{eng}^#1$}}
\newcommand\ETOC{\Eng{*}} %Engine methods transferred TO Cars
\newcommand\etoc{\eng{*}}
\newcommand\Etocbeh{\besemm{\Engine^*}}
\newcommand\etocind{EngIntoCar}
\newcommand\ctoeind{CarToEng}

\newcommand\me{\mbox{$m$}}
\newcommand\Me{\mbox{$\mathit{Meth}$}}

%\newcommand\meths1]{\mbox{$\mathit{meth}^{\mathit{#1}}$}}
\newcommand\methsset[1]{\mbox{$\mathit{#1}\mathsf{Meth}$}}
%the same
\newcommand\meths[1]{\mbox{$\mathit{#1}\mathsf{Meth}$}}
%  in short
\newcommand\mset[1]{\methsset{#1}}

\newcommand\imset[1]{\mbox{\methsset{}$_{#1}$}}
\newcommand\someofmethsset[1]{\mbox{$\mathit{#1}^{*}\mathsf{Meth}$}}
% in short
\newcommand\somset[1]{\someofmethsset{#1}}

\newcommand\iface[1]       {\mbox{$\mathit{#1}  \mathbf{IFace}$}}
\newcommand\ifacepartial[1]{\mbox{$\mathit{#1}^*\mathbf{IFace}$}}

\newcommand\methsbody[2]{\mbox{$\besemm{\mathit{#1}}^{\mathit{#2}}$}}
%  in short
\newcommand\mbody[2]{\methsbody{#1}{#2}}
\newcommand\msbody[2]{\mbox{$\besemm{\methsset{#1}}^{\mathit{#2}}$}} % the same
\newcommand\mmbody[1]{\msbody{#1}{}}



\newcommand\someofmethsiface[1]{\mbox{$\ifacepartial{#1}$}}
\newcommand\somface[1]{\someofmethsiface{#1}}

\newcommand\someofmethsbody[2]{\mbox{$\besemm{\someofmethsset{#1}}^{#2}$}}
\newcommand\sombody[2]{\someofmethsbody{#1}{#2}}

\newcommand\miface{\iface{\me}}

\newcommand\categoryname[1]{\mathbf{#1}}
\newcommand\sketchname[1]{\mathsf{#1}}

\newcommand\setcatmath{\categoryname{Sets}}
\newcommand\setskemath{\sketchname{Set}}
\newcommand\vsetcatmath{\categoryname{VarSet}}
\newcommand\bsetcatmath{\categoryname{BehSet}}
\newcommand\coalgcatmath{\categoryname{coAlg}}
\newcommand\coalgske{\sketchname{coAlg}}
\newcommand\erske{\sketchname{ER}}
\newcommand\ercat{\categoryname{ER}}
\newcommand\vsetske{\sketchname{VarSet}}
\newcommand\bsetske{\sketchname{BehSet}}

\newcommand\setcat{\mbox{$\setcatmath$}}
\renewcommand\setcat{\mbox{$\categoryname{Sets}$}}
\newcommand\gracat{\mbox{$\categoryname{Graphs}$}}
\newcommand\posetcat{\mbox{$\categoryname{Posets}$}}
\newcommand\catcat{\mbox{$\categoryname{Cats}$}}


\newcommand\vsetcat{\mbox{$\vsetcatmath$}}
\newcommand\bsetcat{\mbox{$\bsetcatmath$}}
\newcommand\coalgcat{\mbox{$\coalgcatmath$}}
\newcommand\setske{\mbox{$\setskemath$}}


\newcommand\univcat{\mbox{$\categoryname{U}$}}
\newcommand\ucatmath{\categoryname{U}}
\newcommand\univske{\mbox{$\sketchname{U}$}}
\newcommand\uskemath{\sketchname{U}}
\newcommand\ucat{\univcat}
\newcommand\uske{\univske}

\newcommand\instus[2]{\inst{\ske{#1}}{\ucatmath_{#2}}}
\newcommand\uni[1]{\mbox{$\univcat_{#1} $}}

\newcommand\reuniv{\univcat}
\newcommand\mapcatmath{\categoryname{Map}}
\newcommand\mapcat{\categoryname{Map}}
\newcommand\Map[2]{\mbox{$\mapcatmath(#1,#2)$}}
\newcommand\cariface{\iface{\car}}

\newcommand\rePlug{\ittt{rePlug}}
%=====================
%\input{../../Tools/Macros/m01-macroLogic.tex}

%=====================
%\input{../../Tools/Macros/m05-myStyle(razdels).tex}
\newtheorem{mydef}{\noindent Definition}
%\newtheorem{remark}{Remark}
\newtheorem{termin}{\noindent Terminology}

%% ===========================================================
%%the version where razdels are inside subsections not sections
%\newcounter{Razdel}[subsection]
%\newcommand\beginRazd[1]%
%{
%\renewcommand\theRazdel{\thesubsection.\arabic{Razdel}}
%\par%\smallskip
%\noindent\refstepcounter{Razdel}%
%{\bf \thesubsection.\arabic{Razdel} #1} %\mylabel{#2}
%}
%%==========================================================

%% =========================================================
%%the version where razdels are inside sections not subsections
%\newcounter{RazDel}[section]
%\newcommand\beginRazD[1]%  2nd argument is dummy and inherited from old verion
%{
%\renewcommand\theRazDel{\thesection.\arabic{RazDel}}
%\par%\smallskip
%\noindent\refstepcounter{RazDel}%
%{\bf \thesection.\arabic{RazDel} #1} %\mylabel{#2}
%}
%%==============================================================
%
%%\newcommand\EndRazD{\qquad\qquad\mbox{$\diamondsuit$}\par\medskip}
%%\newcommand\EndRazd{\qquad\qquad\mbox{$\diamondsuit$}\par\medskip}
%
%\newcommand\EndRazD{\par\smallskip}
%\newcommand\EndRazd{\par\smallskip}
%%\renewcommand\EndRazD{\mbox{\textbf{endRemark} $\blacktriangleright$}\par\smallskip}
%%\renewcommand\EndRazd{\mbox{\textbf{endRemark} $\blacktriangleright$}\par\smallskip}
%\newcommand\remends{\par\smallskip}
%                   %{\mbox{\textbf{endRemark} $\blacktriangleright$}}
%
%
%\newenvironment{razdel}[2]{\beginRazd{#1}{Razd#2}}{\endRazd}
%\newenvironment{razd}[2]{\beginRazd{{%\itshape
%                                      \bfseries #1}}}{\EndRazd}
%%\newenvironment{razD}[2]{\beginRazD{#1}{RazD#2}}{\EndRazD}
%\newenvironment{razD}[2]{\beginRazD{{%\itshape
%                                      \bfseries #1}}}{\EndRazD}
%\newenvironment{razzD}[1]{\beginRazD{{%\itshape
%                                      \bfseries #1}}}{\EndRazD}
%
%% 1st argument is the title of the razdel,
%% 2nd - dummy, formerly it was for the label
%
%
%\newenvironment{defi}[1]{\beginRazdel{Definition.}  {Defi#1}}{\endRazdel}
%\newenvironment{cons}[1]{\beginRazdel{Construction.}{Cons#1}}{\endRazdel}
%\newenvironment{prop}[1]{\beginRazdel{Proposition.} {Prop#1}}{\endRazdel}
%\newenvironment{theo}[1]{\beginRazdel{Theorem.}     {Theo#1}}{\endRazdel}
%\newenvironment{coro}[1]{\beginRazdel{Corollary.}   {Coro#1}}{\endRazdel}
%\newenvironment{exam}[1]{\beginRazdel{Example.}     {Exam#1}}{\endRazdel}
%%\newenvironment{rema}[1]{\beginRazdel{Remark.}      {Rema#1}}{\endRazdel}
%\newenvironment{warn}[1]{\beginRazdel{Warning.}     {Warn#1}}{\endRazdel}
%\newenvironment{desc}[1]{\beginRazdel{Description.} {Desc#1}}{\endRazdel}
%\newenvironment{disc}[1]{\beginRazdel{Discussion.}  {Disc#1}}{\endRazdel}
%\newenvironment{conv}[1]{\beginRazdel{Convention.}  {Conv#1}}{\endRazdel}
%\newenvironment{nota}[1]{\beginRazdel{Notation.}    {Nota#1}}{\endRazdel}
%
%\newcommand\equnref[1]{Equation~(\ref{Equn#1})}
%\newcommand\equlref[1]{equality~(\ref{Equl#1})}
%%\newcommand\diagref[1]{(\ref{#1})}
%\newcommand\consref[1]{Construction~\ref{Cons#1}}
%\newcommand\defref[1]{Definition~\ref{#1}}
%\newcommand\propref[1]{Proposition~\ref{Prop#1}}
%\newcommand\discref[1]{Discussion~\ref{Disc#1}}
%\newcommand\convref[1]{Convention~\ref{Conv#1}}
%\newcommand\notaref[1]{Notation~\ref{Nota#1}}
%\newcommand\descref[1]{Description~\ref{Desc#1}}
%\newcommand\remaref[1]{Remark~\ref{Rema#1}}
%\newcommand\examref[1]{Example~\ref{Exam#1}}
%\newcommand\cororef[1]{Corollary~\ref{Coro#1}}
%\newcommand\razdref[1]{Section~\ref{Razd#1}}
%%\newcommand\appref[1]{appendix~\ref{App#1}}    see pre_gen.tex
%%\newcommand\sectref[1]{section~\ref{Sect#1}}   ....
%%\newcommand\sectsectref[1]{sections~\ref{Razd#1}}
%%\newcounter{Razdel}[subsection]
%\newcommand\NachRazd[2]%
%{
%%\renewcommand\theRazdel{\thesubsection.\arabic{Razdel}}
%\par\medskip\noindent%\refstepcounter{Razdel}%
%{\it #1} \mylabel{#2} }
%%\newcommand\end{\qquad\qquad\mbox{$\diamondsuit$}\par\medskip}
%
%\newenvironment{Example}{\NachRazd{Example}}{\end}
%\newenvironment{Remark} {\NachRazd{Remark}}{\end}
%\newenvironment{Warning}{\NachRazd{Warning}}{\end}
%=====================
%\input{../../Tools/Macros/m10-MMt-CASCON-Macros.tex}
\newcommand\instarr[1]{\mbox{$\lar{\statemap}{\igra{}{}}{#1}$}}
\newcommand\instarrt[1]{\mbox{$ \lar{\statemap}{\igraph{t}{}}{#1}$}}

\newcommand\idop{\mrksemiop{\times id}}
\newcommand\idos{\mrksemiop{+id}}

\newcommand\idoP{\mrkop{prod}}
\newcommand\idoS{\mrkop{sum}}

\newcommand\recop{\mrkop{rec}}
\newcommand\varop{\mrkop{var}}
%\newcommand\sumop{\mrkop{var}}

\renewcommand\owner{\textit{owner}}
\newcommand\types{\nicex{ T$}}

%% for Kleisly arrows section

\newcommand\ssma{\mbox{$S$}}
\newcommand\tsma{\mbox{$T$}}
\newcommand\usma{\mbox{$U$$$}}
\newcommand\mapelement{\mbox{$\rightsquigarrow$}}
\newcommand\mapel{\mapelement}

\newcommand\klear[3]{\mbox{$#1\!: #2 \rightsquigarrow #3$}}
\newcommand\kleare[2]{\mbox{$#1 \rightsquigarrow #2$}}
\newcommand\lare[2]{\mbox{$#1 \rightarrow #2$}}
%==============================================

\newcommand\corrce{correspondence}






%%% 1. Collections
%
%==1.1 Categories
% macros for names moved to macros4names.tex
%\newcommand\catname[1]{\mbox{\bfseries\itshape #1}}
%%\newcommand\catname[1]{\mbox{\boldmath $#1$}}
%\newcommand\cat[1]{\catname{#1}}
%\newcommand\categoryop[1]{\mbox{\bfseries\itshape #1}$^{\mathrm{op}}$}
%\newcommand\catnamei[1]{{\pmb #1}}



%\newcommand\idmap[1]{\operator{id}_{#1}}
%\renewcommand\f{\mbox{$\phi$}}
%\renewcommand\c{\catname{C}}
%\renewcommand\b{\catname{B}}
%\renewcommand\r{\catname{R}}





\newcommand\clonet{\mbox{${\nia}_\mathrm{Top}$}}
\newcommand\clonem{\mbox{${\nia}_\mathrm{MMt}$}}
%
% -- overlined letters for clones ---
%\newcommand\clonet{\mbox{$\overline{\nia}_\mathrm{Top}$}}
%\newcommand\clonem{\mbox{$\overline{\nia}_\mathrm{MMt}$}}



%==1.2 Classes of nodes/arrows
\newcommand\indclassofitems[1]{{\cal #1}}
\newcommand\classofitems[1]{\mbox{$\indclassofitems{#1}$}}
\newcommand\coi[1]{\classofitems{#1}}
\newcommand\incls{\coi{I}}
\newcommand\covers{\coi{C}}
\newcommand\univs{\coi{U}}
%\renewcommand\diags{\classofitems{D}}
\renewcommand\diags{\mathit{Diags}}
\newcommand\inddiags{\indclassofitems{D}}

%\newcommand\attrset[1]{\mbox{\textit{attrs}$(#1)$}}
%\newcommand\refset[1]{\mbox{\textit{refs}$(#1)$}}
%\newcommand\varset[1]{\mbox{\textit{vars}$(#1)$}}
%\newcommand\classtab[1]{\mbox{\textsf{tab}$_#1$}}
%\newcommand\attrtab[1]{\mbox{\textsf{aTab}$_#1$}}
%\newcommand\reftab[1]{\mbox{\textsf{rTab}$_#1$}}



%===1.3 Languages
\newcommand\querylanguage[1]{\nicex{ QL_{#1}$}}
\newcommand\ql{\querylanguage}
\newcommand\qlmath[1]{{\cal QL}_{#1}}

%%% 2. MMt Objects
\renewcommand\modelob[1]{\mbox{$M_{#1}$}}
\newcommand\schemaobsymbol{S}
\newcommand\typeSyssymbol{Types}
\newcommand\instanceGraphSymbol{I}
\newcommand\relschemaobsymbol{R}
\newcommand\skeobsymbol{S}
\newcommand\universesymbol{U}
\newcommand\valueUniverseGraphSymbol{U}
\newcommand\UniverseGraphSymbol{U}
\newcommand\schemaob[1]{\mbox{${\mathit \schemaobsymbol}_{#1}$}}
%\newcommand\typesys[1]{\mbox{${\mathit \schemaobsymbol}_{#1}$}}
\newcommand\instgra[2]{\mbox{${\mathit \instanceGraphSymbol}_{#1}^{#2}$}}
\newcommand\igra[2]{\instgra{#1}{#2}}
\newcommand\itogra[1]{\instgra{}{#1}}
\newcommand\irefgra[1]{\instgra{ref}{#1}}
\newcommand\iattgra[1]{\instgra{attr}{#1}}
\newcommand\iobjgra[1]{\instgra{obj}{#1}}

\newcommand\uvalgra[1]{\mbox{$\mathit{\universesymbol Val}_{#1}$}}
\newcommand\utupgra[1]{\mbox{$\mathit{\universesymbol Tuple}_{#1}$}}
\newcommand\uval{\uvalgra{}}
\newcommand\utup{\utupgra{}}
\renewcommand\uniob[1]{\mbox{$\mathsf{\universesymbol}_{#1}$}}

\newcommand\relsob[1]{\mbox{${\mathit \relschemaobsymbol}_{#1}$}}
\newcommand\newrelske[1] {\mbox{${\mathsf R}_{#1}$}}
\newcommand\newrelinst[2]{\mbox{${\mathsf Q}_{#1}^{#2}$}}

\newcommand\schemaOB[2]{\mbox{${\mathit \schemaobsymbol}_{#1}^{#2}$}}

\newcommand\claske[1]{\mbox{${\mathsf\skeobsymbol}_{\mathit{cla}#1}$}}
\newcommand\refske[1]{\mbox{${\mathsf\skeobsymbol}_{\mathit{ref}#1}$}}
\newcommand\attrske[1]{\mbox{${\mathsf\skeobsymbol}_{\mathit{attr}#1}$}}
\newcommand\objrefske[1]{\mbox{${\mathsf\skeobsymbol}_{\mathit{objRef}#1}$}}


\renewcommand\skeob[1]{\mbox{${\mathsf\skeobsymbol}_{#1}$}}
\newcommand\skeobind[1]{{\mathsf \skeobsymbol}_{#1}}
\newcommand\indskeob[1]{\skeobind{#1}}

\newcommand\typeske[1]{\mbox{$\mathsf{Type}_{#1}$}}
\newcommand\typemap[1]{\mbox{$\mathsf{type}_{#1}$}}
\newcommand\typeskeind{\mathsf{Type}}
\newcommand\typemapind[1]{\mathsf{type}_{#1}}

\renewcommand\statemap{\mbox{$\sigma$}}
\newcommand\statemapind{\sigma}




%\newcommand\gs{\mbox{$G_{\indskeob{}}$}}
%\newcommand\ds{\mbox{$\diags_{\indskeob{}}$}}
%\newcommand\gsi[1]{\mbox{$G_{\indskeob{#1}}$}}
%\newcommand\dsi[1]{\mbox{$\G_{\indskeob{#1}}$}}

%%% 2.1  Vectors of objects (bold objects)
%\newcommand\fullvector[3]{}
%\newcommand\vectorobject[1]{\mbox{$\boldsymbol{#1}$}} % see macros4names
\newcommand\multisch{\vectorobject{\schemaobsymbol}}
\newcommand\multiSch{\vectorobject{\schemaobsymbol}}
\newcommand\multinst{\vectorobject{\instancesymbol}}
\newcommand\multinstoo[1]{\mbox{$\multinst=(\inst{1},\ldots,\inst{#1})$}}

\newcommand\multiUni{\vectorobject{\universesymbol}}
\newcommand\multiRel{\vectorobject{\relschemaobsymbol}}
\newcommand\multiuni{\vectorobject{u}}
\newcommand\multirel{\vectorobject{r}}
\newcommand\multiu{\vectorobject{u}}
\newcommand\multir{\vectorobject{r}}
\newcommand\multiroo[1]{\mbox{$\multir=(r_1,\ldots,r_{#1})$}}


%== Operators
\newcommand\operator[1]{\mbox{\sf #1}}
\newcommand\operatorInIndex[1]{{\sf #1}}

\newcommand\heoperator[1]{\mbox{\sf\bfseries #1}}
\newcommand\match{\operator{match}}

\newcommand\indexedoperator[3]{\mbox{\operator{#1}$_{#2}^{#3}$}}
\newcommand\indexedoperatorInIndex[3]{\operatorInIndex{#1}_{#2}^{#3}}

\newcommand\der[2]{\indexedoperator{der}{#1}{#2}}
\newcommand\dero[1]{\indexedoperator{der}{}{#1}}
\newcommand\derInIndex[2]{\indexedoperatorInIndex{der}{#1}{#2}}

%\newcommand\proj[1]{\indexedoperator{p}{#1}{}}
%\newcommand\merge{\operator{merge}}
%\newcommand\modgen{\operator{modelGen}}
%\newcommand\datatrans{\operator{dataTransf}}
%\renewcommand\self{\operator{self}}


\newcommand\SFW[3]{\mbox{\operator{Select} #1
                         \operator{from} #2
                         \operator{where} #3}
                         }

%=====================
%\input{../../Tools/Macros/m20-newMacros}
%\renewcommand\em[1]{\emph{#1}}

%\newcommand\vect[1]{\textbf{#1}}
\newcommand\veg{\vect{G}}
\newcommand\vef{\vect{f}}
\newcommand\ver{\vect{R}}
\newcommand\ves{\vect{S}}
\newcommand\vehh{\vect{H}}
\newcommand\veho{\vect{\ovr{H}}}
\newcommand\veh{\vect{h}}

\newcommand\ovr[1]{\mbox{$\overline{\mathstrut#1}$}}
\newcommand\ovri[1]{\overline{#1}}
\newcommand\ovh[1]{\ovr{H}_{#1}}
%\newcommand\ovri[1]{\mb{\ovr{\iota'}_{#1}}}

\newcommand\edge[1]{\ittt{Edge}\mb{_{#1}}}
\newcommand\Edge[2]{\ittt{Edge}\mb{_{#1}^{#2}}}


\newcommand\univarr[1]{\mb{!_{#1}}}
\newcommand\doublearrow[5]{\mbox{$#1\stackrel{#4}{\rightarrow}
                                 #2\stackrel{#5}{\rightarrow}#3$
}}
\newcommand\arrdou[5]{\doublearrow{#1}{#2}{#3}{#4}{#5}}
\newcommand\arrarr{\arrdou{\gra{2}}{\gra{3}}{\gra{4}}{h_2}{h_3}}
\newcommand\scearr{\arrdou{\gra{2}}{\gra{1}}{\gra{0}}{\tau_1}{\tau_0}}
\newcommand\arrsce{\arrdou{\gra{2}}{\gra{1}}{\gra{0}}{\tau_1}{\tau_0}} % the same as above

\newcommand\arrspan[5]{\fbox{$#1\stackrel{#4}{\leftarrow}
                                 #2\stackrel{#5}{\rightarrow}#3$
}}
\newcommand\arrcospan[5]{\fbox{$#1\stackrel{#4}{\rightarrow}
                                 #2\stackrel{#5}{\leftarrow}#3$
}}

%\renewcommand\span[1]{\textbf{R}\mb{_{#1}}}
\newcommand\cospan[1]{\textbf{S}\mb{_{#1}}}
\newcommand\set[2]{\mb{#1=\{#2\}}}

\newcommand\integr[3]{\mb{#1\bigoplus_#3 #2}}

\newcommand\gran[1]{\mb{G_{{#1}N}}}
\newcommand\gred[1]{\mb{G_{{#1}E}}}
\newcommand\graman[1]{\mb{f_{{#1}N}}}
\newcommand\gramed[1]{\mb{f_{{#1}E}}}
\newcommand\grinman[1]{\mb{\iota'_{{#1}N}}}
\newcommand\grinmed[1]{\mb{\iota'_{{#1}E}}}

% changing from \mathsl to \mathit
\renewcommand\object[2]{\mbox{${\mathit{#1}}_{#2}$}}
\renewcommand\objectind[1]{\mathit{#1}}
\renewcommand\objectmath[1]{\mathit{#1}}

%\newcommand\DOM[1]{\Box #1}
%\newcommand\COD[1]{#1 \Box}


\newcommand\mb[1]{\mbox{$#1$}}
\newcommand\nin{\mb{\cal N}}
\newcommand\nix{\mb{\cal X}}
\newcommand\nil{\mb{\cal L}}
\newcommand\nik{\mb{\cal K}}
\newcommand\dvet{\mbox{:}}
\newcommand\ddvet{\dvet\dvet}
%\newcommand\n{\mb{n}}

\renewcommand\x{\mb{X}}

\newcommand\proxx[2]{\mb{\prod_{#1}{#2}}}
\newcommand\prox{\proxx{}{\vex}}
\newcommand\proy{\proxx{}{\vey}}
\newcommand\prodxn{\proxx{\cal L}{\vex}}
\newcommand\prodxm{\proxx{\cal K}{\vex}}

\newcommand\unixx[2]{\mb{\bigcup_{#1}{#2}}}
\newcommand\unix{\unixx{}{\vex}}

\newcommand\proj[1]{\mb{\ell_{#1}}}
\newcommand\proji{\proj{i}}






\renewcommand\ext{\mbox{\textsf{ext}}}








\newcommand\oclar{\mbox{\footnotesize $>$}}
\newcommand\myendset[1]{\mbox{$\{#1_1..#1_m\}$}}
\newcommand\fens{\myendset{f}}





\newcommand\fulla[1]{\mbox{${\mathbf F}_{#1}$}}
\newcommand\rmap[1]{\mbox{$#1^\rightarrow$}}
\newcommand\lmap[1]{\mbox{$^\leftarrow #1$}}
\newcommand\basemap[1]{\mbox{\textit{base}$_{#1}$}}


\newcommand\seq[1]{\textsf{seq}\mbox{$#1$}}
\newcommand\coll[2]{\textsf{coll}\mbox{$_{#1}(#2)$}}

\newcommand\tabschema{\mbox{$D=\{a_1:D_1,...,a_n:D_n\}$}}
\newcommand\tabschemamap{\mbox{\lar{D}{\attrset{}}{\setcat}}}



%=====================
%\input{../../Tools/Macros/m21--labelsnewMacros}
%(left) labels for formulas
\newcommand\equationNumber[1]{(\textsf{#1})}
\newcommand\eqnumber[1]{\equationNumber{#1}}
\newcommand\eqn[1]{\equationNumber{#1}}


%\newcommand\mafo[2]\mathform{#1}{#2}
\newcommand\mathfo[2]{$$#2\leqno{\mbox{(\textsf{#1})}} $$}
\newcommand\mafo[2]{$$#2 \leqno{\mbox{\eqn{#1}}} $$}


\newcommand\selflab{\eqn{self}}
\newcommand\looplab{\eqn{loop}}
\newcommand\idlelab{\eqn{idle}}
\newcommand\dolab{\eqn{do}}
\newcommand\triglab{\eqn{trigger}}

\newcommand\assonla{\eqn{fullAsson}}
\newcommand\tabla{\eqn{TAB}}
\newcommand\invla{\eqn{inverse}}
\newcommand\extla{\eqn{extension}}
\newcommand\tablatup{\eqn{TABrow}}
\newcommand\tablapro{\eqn{TABattr}}
\newcommand\sepla{\eqn{1-1}}
%=====================================
\newcommand\classn{\eqnumber{classn}}
\newcommand\indexn{\eqnumber{indexng}}

\newcommand\igralabel{\eqnumber{instGra}}
\newcommand\schemaGeneralLabel{\eqnumber{schemaGen}}
\newcommand\stlabel{\schemaGeneralLabel}
\newcommand\itablabel{\eqnumber{instTab}}
%\renewcommand\uniob[1]{\mbox{${\mathsf\universesymbol}_{#1}$}}
\newcommand\igratablabel{\eqnumber{instGraTab}}
\newcommand\igragralabel{\eqnumber{instGraGra}}
\newcommand\itabtablabel{\eqnumber{instTabTab}}

%=====================
%\input{../Tools/Macros/m21--abbrev4formulas}
%\input{../Tools/Macros/m22--abbrev4text}
%--------------------------------
%\renewcommand\zdmargin[1]{}
%\renewenvironment{razd}[2]{\subsubsection{#1}}{}
%\nocite{}
\renewenvironment{razD}[2]{\beginRazD{{%\itshape
                                      \bfseries #1}}}{\EndRazD}

%% sle
%%%%%%%%%% sle09 macros
%\newcommand\diagi[1]{#1\mbox{$'$}}
%\newcommand\diagii[1]{#1\mbox{$''$}}
%
%\newcommand\ari[1]{\mbox{\textsl{ar}$(#1)$}}
%\newcommand\mmname[1]{\textsf{#1}}
%\newcommand\mmcd{\mmname{CD}}
%\newcommand\mmsd{\mmname{SD}}
%\newcommand\mmsc{\mmname{SC}}
%\newcommand\mmca{\mmname{CA}}
%\newcommand\mmamt{\mmname{CAT}}
%\newcommand\mmcat{\mmname{CAT}}
%\newcommand\cd{\mmname{cd}}
%\renewcommand\sd{\mmname{sd}}
%\renewcommand\sc{\mmname{sc}}
%\newcommand\ca{\mmname{ca}}
%\newcommand\amt{\mmname{cat}}
%\renewcommand\cat{\mmname{cat}}
%\newcommand\cdi{\diagi{\cd}}
%\renewcommand\sdi{\diagi{\sd}}
%\newcommand\sci{\diagi{\sc}}
%\newcommand\cdii{\diagii{\cd}}
%\newcommand\sdii{\diagii{\sd}}
%\newcommand\scii{\diagii{\sc}}





\newcommand\base{\mbox{$\pmb{MM}$}}
\newcommand\p{\textbf{P}}
\newcommand\ps{\mbox{$P$}}
\newcommand\leqnoo[1]{\leqno{\mbox{#1}}}

\newcommand\keyword[1]{{\itshape\textsf{#1}}}
\newcommand\nam{\keyword{name}}
\renewcommand\owner{\keyword{owner}}
\newcommand\type{\keyword{type}}
\newcommand\val{\keyword{value}}
\newcommand\Class{\keyword{Class}}
\renewcommand\Attr{\keyword{Attr}}
\newcommand\Type{\keyword{Type}}
\newcommand\elm[1]{\mbox{$\mathit{El}(#1)$}}

\newcommand\ueq{\mbox{$\leftrightarrow$}}
\newcommand\uneq{\mbox{$\rightsquigarrow$}}

\newcommand\meq{\mbox{$=$}}
\newcommand\mneq{\mbox{$\neq$}}


\newcommand\shot{\textsl{shot}}
\newcommand\reltile{\textsl{relTile}}
%\newcommand\tauh{\mbox{$\tau_{\textsf{h}}$}}
%\newcommand\tauv{\mbox{$\tau_{\textsf{v}}$}}



\newcommand\vso{\textsf{v}\mbox{$\partial_0$}}
\newcommand\vta{\textsf{v}\mbox{$\partial_1$}}
\newcommand\hso{\textsf{h}\mbox{$\partial_0$}}
\newcommand\hta{\textsf{h}\mbox{$\partial_1$}}

\newcommand\mmod{\nicex{ M$}}
\newcommand\id{\textsl{id}}
\renewcommand\id{\mbox{$\iota$}}
\newcommand\recon[1]{\mbox{$#1$\textbf{!}}}

\newcommand\oidd[1]{\mbox{$\overline{#1}$}}
\newcommand\oiddi[1]{\mbox{$\overline{#1}'$}}

\renewcommand\oidd[1]{\mbox{${#1}$}}
\renewcommand\oiddi[1]{\mbox{${#1}'$}}

\newcommand\oa{\oidd{a}}
\newcommand\ob{\oidd{b}}
\newcommand\oP{\oidd{P}}
\newcommand\oQ{\oidd{Q}}

\newcommand\oai{\oiddi{a}}
\newcommand\obi{\oiddi{b}}
\newcommand\oPi{\oiddi{P}}
\newcommand\oQi{\oiddi{Q}}

% icmt

%%% icmt09 macros
% the % piece below  was moved to newMacros ---
\newcommand\mrkoprr[1]{\mrkopr{\mrkopr{#1}}}
%\der{}{Q}
%\newcommand\mmview[1]{\mbox{$\textsl{v}_{#1}$}}
%\newcommand\mmarr{v}
\newcommand\mmf{\mbox{$m$}} % to be used in the row
%\renewcommand\mmview[1]{\mbox{$\pmb{\mmarr}_{#1}$}}
%%\newcommand\mmv[1]{{\pmb{\mmarr}_{#1}}} %for subscripts
%\newcommand\mmmap[1]{\mbox{$\pmb{\mmarr}_{#1}$}}
%\renewcommand\mmm{m}  % to be used for sub-sup-indexes
%\newcommand\mmap[1]{\mbox{${\mmarr}_{#1}$}}

\newcommand\unde[1]{\underline{#1}}

\newcommand\oversi[1]{\overline{\sigma}^{#1}}

\newcommand\oversig[1]{\overline{\sigma}^{Q#1}}
\newcommand\overtau[1]{\overline{\tau}^{Q#1}}
\newcommand\overover{\overline{\oversig{1}}}
\newcommand\doublesig{{\overover^{Q2}}} %
\newcommand\votono{{\overline{\oversig{}}^{R}}}

\newcommand\derqq[2]{\mbox{$\dero{Q#1}#2$}}
\newcommand\dermms[1]{\derqq{#1}{\mms}}
\newcommand\derms[1]{\derqq{#1}{\ms{}}}
\newcommand\derqmms{\derqq{}{\mms}}
\newcommand\derqms{\derqq{}{\ms{}}}
\newcommand\derq[1]{\mbox{$\der{}{Q}#1$}}
\newcommand\doubleder[1]{\derqq{1;Q2}{#1}}

\newcommand\augtymaps{\flar%
{\overline{\sigma}^{Q}}%
{\dero{Q}\ms{}}%
{\dero{Q}\mms}%
}
%\newcommand\mmarr{\mbox{$m$}}

%
\newcommand\tracemap[1]{\mbox{$\stackrel{\rightsquigarrow}{#1}$}}
\renewcommand\tracemap[1]{\mbox{$\mathit{tr}_{#1}$}}
\renewcommand\tracemap[1]{\mbox{$#1^{*}$}}
\newcommand\tram{\tracemap{\mmmap}}
%
\newcommand\reversemap[1]{\mbox{\spf$_{#1}$}}
%\newcommand\revem{\reversemap{\mmview{}}}
\newcommand\revem[1]{\mbox{$\semm{\mmmap{#1}}$}}

\renewcommand\s[1]{\mbox{$S_{#1}$}}
\renewcommand\ms[1]{\mbox{$S_{#1}$}}
\newcommand\mos[1]{\mbox{$\overline{S}_{#1}$}}
\renewcommand\mt[1]{\mbox{$T_{#1}$}}
\newcommand\mot[1]{\mbox{$\overline{T}_{#1}$}}
\newcommand\mh[1]{\mbox{$H_{#1}$}}
\renewcommand\ml[1]{\mbox{$L_{#1}$}}

\newcommand\pbop{\operator{PB}}

\newcommand\msarr{\flar{\sigma}{S}{\mms}}
\newcommand\msarrq{\flar{\overline{\sigma}^{Q}}{\der{}{Q}S}{\der{}{Q}\mms}}
\newcommand\mssym{\mbox{$\overline{\sigma}$}}
\newcommand\mssymq{\mbox{$\overline{\sigma}^Q$}}

\newcommand\mtarr{\flar{\tau}{T}{\mmt}}
\newcommand\srelarr{\flar{\sigma}{S}{\mmrel}}
\newcommand\erdarr{\flar{\tau}{D}{\mmer}}
\newcommand\srelderarr[1]{\flar{\overline{\sigma}^{Q#1}}{\der{}{Q#1}S}{\der{}{Q#1}\mmrel}}



\newcommand\ertorel[1]{\flar{\textsf{er2rel}_{#1}}{\mmer}{\mmrel}}
\newcommand\ertorelder[1]{\flar{\textsf{er2rel}_{#1}}{\mmer}{\der{}{{Q#1}}\mmrel}}

% gttse

%\renewcommand\mmname[1]{\mbox{$\pmb{\cal #1}$}}
%\newcommand\mmmapname[1]{\mbox{$\pmb{#1}$}}
%\newcommand\mma{\mmname{M}}
%\newcommand\mmb{\mmname{N}}
%\newcommand\mmc{\mmname{O}}
%\newcommand\mmr[1]{\mbox{\mmname{R}$_{#1}$}}
%\renewcommand\mmr[1]{\mbox{$\pmb{r}_{#1}$}}
%\newcommand\mmab{\mmname{MN}}
%\newcommand\mmac{\mmname{MO}}
%\newcommand\mmv{\mmmapname{v}}
%\newcommand\mmw{\mmmapname{w}}
%\newcommand\mmp{\mmmapname{p}}
%\newcommand\mmq{\mmmapname{q}}

\renewcommand\dvet{\mbox{:\,}}

\newcommand\newrevem[1]{\mbox{$\semm{\mmmapname{#1}}$}}
\newcommand\rev{\newrevem{v}}
\newcommand\rew{\newrevem{w}}
\newcommand\rep{\newrevem{p}}
\newcommand\req{\newrevem{q}}


\newcommand\mmnamei[1]{\pmb{\cal #1}}
\newcommand\mmabi{\mmnamei{MN}}
\newcommand\mmaci{\mmnamei{MO}}
\newcommand\amn{\mbox{$A_{\mmabi}$}}
\newcommand\bmn{\mbox{$B_{\mmabi}$}}
\newcommand\amnprim{\mbox{$A'_{\mmabi}$}}
\newcommand\bmnprim{\mbox{$B'_{\mmabi}$}}
\newcommand\amo{\mbox{$A_{\mmaci}$}}
\newcommand\cmo{\mbox{$C_{\mmaci}$}}
\newcommand\umn{\mbox{$u_{\mmabi}$}}
\newcommand\vmn{\mbox{$v_{\mmabi}$}}

\newcommand\lmmes{\left] \respace\left] }
\newcommand\rmmes{\right[\respace\right[}
\newcommand\mmes[1]{\mbox{$\lmmes\, \mathit{#1} \, \rmmes$}}

% spans

\newcommand\spancat{\category{Span}}
\newcommand\spansa{\scat\spancat}
\newcommand\spanset{\setcat\spancat}
\newcommand\cospancat{\category{Cospan}}
\newcommand\cospansa{\scat\cospancat}
\newcommand\cospanset{\setcat\cospancat}


\newcommand\spanfull[4]{\mbox{${\cal #1}$=(\flar{#2_i}{#3}{#4 i},
$i=1,2)$}}

\newcommand\lKleisly{\Leftarrow}
\newcommand\rKleisly{\Rightarrow}
\newcommand\spandiag[5]  {\fbox{$#1\lTo^{#2} #3 \rTo^{#4} #5$}}
\newcommand\kleispandiag[5]{\fbox{$#1\lKleisly^{#2} #3 \rKleisly^{#4} #5$}}
\newcommand\kleislispandiag[5]{\fbox{$#1\lKleisly^{#2} #3 \rKleisly^{#4} #5$}}
\newcommand\cospandiag[5]{\fbox{$#1\rTo^{#2} #3 \lTo^{#4} #5$}}
\newcommand\kleicospandiag[5]{\fbox{$#1\rKleisly^{#2} #3 \lKleisly^{#4} #5$}}
\newcommand\kleislicospandiag[5]{\fbox{$#1\rKleisly^{#2} #3 \lKleisly^{#4} #5$}}


\newcommand\flarsemm[3]{\flar{#1}{\semm{#2}}{\semm{#3}}}
\newcommand\spandiagsemm[5]{\fbox{$\semm{#1}\lTo^{#2} \semm{#3} \rTo^{#4} \semm{#5}$}}
\newcommand\cospandiagsemm[5]{\fbox{$\semm{#1}\rTo^{#2} \semm{#3} \lTo^{#4} \semm{#5}$}}


%=== with brackets
\newcommand\spandiagbra[5]
{\mbox{$%\left %
(#1\stackrel{~#2}{\leftarrow} #3
                                           \stackrel{#4~}{\rightarrow} #5%\right
)$}}
\renewcommand\kleispandiag[5]{\mbox{$\left(#1\stackrel{~#2}{\lKleisly} #3
                                             \stackrel{#4~}{\rKleisly} #5
                                             \right)$}}
\renewcommand\kleislispandiag[5]{\mbox{$\left(#1\stackrel{#2}{\lKleisly} #3
                                             \stackrel{#4}{\rKleisly} #5
                                             \right)$}}
\renewcommand\kleicospandiag[5]{\mbox{$\left(#1\stackrel{#2}{\rKleisly} #3
                                             \stackrel{#4}{\lKleisly} #5
                                             \right)$}}
\renewcommand\kleislicospandiag[5]{\mbox{$\left(#1\stackrel{#2}{\rKleisly} #3
                                             \stackrel{#4}{\lKleisly} #5
                                             \right)$}}

\renewcommand\cospandiag[5]{\mbox{$\left(#1\rTo^{#2} #3 \lTo^{#4} #5\right)$}}
\renewcommand\cospandiag[5]  {\mbox{$\left(#1\stackrel{~#2}{\rightarrow} #3
                                           \stackrel{#4~}{\leftarrow} #5\right)$}}

% without brackets
\renewcommand\spandiag[5]  {\mbox{$#1\stackrel{~#2}{\leftarrow} #3
                                           \stackrel{#4~}{\rightarrow} #5$}}
\renewcommand\cospandiag[5]  {\mbox{$#1\stackrel{~#2}{\rightarrow} #3
                                           \stackrel{#4~}{\leftarrow} #5$}}


%\renewcommand\kleislycospandiag[5]{\mbox{$\left(#1\rKleisly^{#2} #3 \lKleisly^{#4} #5\right)$}}

\renewcommand\flarsemm[3]{\flar{#1}{\semm{#2}}{\semm{#3}}}
\renewcommand\spandiagsemm[5]{\mbox{$\left(\semm{#1}\lTo^{#2} \semm{#3}\rTo^{#4} \semm{#5}\right)$}}
\renewcommand\cospandiagsemm[5]{\mbox{$\left(\semm{#1}\rTo^{#2} \semm{#3}\lTo^{#4} \semm{#5}\right)$}}


%% end macros



%%==== end newMacros


==> macros/macros4thisPaper-0.tex <==
\newcommand\incal{incremental}
\newcommand\mbcon{\ensuremath{\sim}}
\newcommand\hgg[1]{}
\newcommand\info{\ensuremath{\mathrm{inf}}}



\newcommand\boldsubsubsection[1]{\subsubsection*{\textbf{#1}}}
\renewcommand\boldsubsubsection[1]{\subsubsection*{{#1}}}
\newcommand\goup{\vspace{-7.5pt}}
\newcommand\rich{\ensuremath{\mathrm{+}}}
\newcommand\poor{\ensuremath{\mathrm{-}}}
\newcommand\ohtri{\ensuremath{(\ohafra\ohafra\ohafra)}}



\newcommand\alens{\ensuremath{\lambda}}
\newcommand\dbox[1]{\fbox{$#1$}}
% sub and super scripts
\newcommand\indname[1]{\ensuremath\mathrm{#1}}
\newcommand\priv{{\indname{prv}}}
\newcommand\pub{{\indname{pub}}}

\endinput













==> sections/TR/anti-gsn-newTR.tex <==
\subsection{\wfp\ vs. GSN}\label{sec:anti-gsn}

==> sections/TR/aspectRTR.tex <==
\subsection{Reviewing as an aspect}
\label{sec:aspects}
\newcommand\figrR{\figref{fig:aspectR}}
\newcommand\citeR{\cite{?}\footnote{ref to paper[*]}}
\newcommand\citeRR{\cite{?}\footnote{ref to paper[**]}}

\input{figures/TR/aspectRTR}
\zd{Needs a discussion with Alan}


Reviewing is a fundamental aspect of assurance: each subprocess execution of SEP must be reviewed on quality of execution and the executors qualifications, and all critical elements produced must be checked for semantic validity. While syntactic conformance checks that an execution is well structured, these reviews complete the story of a SEP being acceptably well executed by checking that quality of execution, qualifications of executors and semantic validity of critical elements are all acceptable. 

Reviewing appears as a typical cross-curring concern of assurance, which is scattered and partially repeated in many different places of a typical SC, and thus should be appropriately managed along the lines developed by the aspect-oriented programming community (AOSD), \cite{AspOrProg}. In our context, we need a mechanism of enriching a core metamodel with an aspect metamodel ({\em advice}, in AOSD terms) developed separately and weaved into the core metamodel at specified points  ({\em pointcuts}). We are not aware of any AO-\fwk s for metamodeling presented in the literature, and leave development of such for future work. Below we will use the main idea of aspect weaving \cite{advWeav} for metamodel weaving in the following sense. 

A crosscutting concern is specified by an advice metamodel $M_\adv$, whose part $M_\entry\subset M_\adv$ specifies an entry, to which the advice is to be applied. Formally, we model this as an embedding mapping \incrar{e}{M_\entry}{M_\adv}. Now, having a main metamodel $M_\main$ with a set of entry points in it, for each such point we specify a mapping \flar{w}{M_\main}{M_\entry} and apply the pushout operation (PO) to the pair $(e,w)$, which will result in the merge $M_\main+_{(e,v)}M_\adv$ modulo the common (shared) part $M_\entry$. 

Figure~\ref{fig:aspectR} presents a simplified example of an advice metamodel. In it, we see that performance data of a process, including when and how it was executed and who the executor(s) were, are reviewed alongside the inputs and outputs of that process. The review process then outputs the semantic validity of the critical data produced by the process being reviewed, from which we can derive if the execution was acceptable. In \figref{fig:normative}, purple cirlces with horizontal bars labelled Review indicate entry points. 


==> sections/TR/conformToNormTR.tex <==
\subsection{Conformance to Normative doc}\label{sec:conformToNorm}


\input{figures/normative}
One difficult but essential question remains - how do we know the SEP is acceptably well defined (cf. \defref{main}a)? Current best-practice tackles this issue by drawing from expert knowledge and empirical  evidence of effectiveness of techniques \zdmodok{to make a genuine attempt to do everything possible to ensure safety.}{used in SEP }{} \zdmoddok{This does not guarantee safety, but rather gives confidence that a best effort was made given the limitations of current knowledge.}{}{see the main \defref{main}}{-3em} 

In \wfc, we need to encode expert knowledge as a (normative) workflow metamodel \wfnorm, and \figref{fig:normative} presents such,  
%We simulated a normative workflow 
based mainly on our understanding of the domain (and simplifications to make it brief) rather than data in the GSN Example: the appropriateness of the arguments made, techniques used, and other meta-meta issues are not addressed in the Example. Below we will refer to this particular workflow as to \wfnorm*. %\figref{fig:gsnEx-main}. 
This document \zdmodok{which would be produced by domain experts by drawing on research, expert knowledge and empirical evidence,}{}{} defines the way in which systems of a particular type in a particular application must be developed, and which properties it must possess. Manufacturers developing their SEPs by instantiating \wfnorm' %the normative workflow 
are free to make decisions allowed by \wfnorm* (\eg, FHA vs STPA), but must conform to all restrictions placed in \wfnorm* by regulators. \zdhll{Conformance in this sense has two components. a) Syntactic conformance is shown by demonstrating that the SEP metamodel is indeed a refinement of the normative metamodel. b) Semantic conformance is up to reviewers - they must use their knowledge to determine if a SEP satisfies the intent of the normative metamodel.}{important. to think about}{-7em} 

\wfnorm* serves as an example to illustrate its concept, and is far too simple to provide any meaningful guidance to manufacturers implementing it or reviewers checking an implementation. Enriching the model by adding more details and consequently encoding semantics syntactically will allow for more semantic conformance checking tasks to be done syntactically. 


==> sections/TR/gsn2wf-introTR.tex <==
Figure~\ref{fig:gsnEx-main} shows a GSN goal structure taken from the GSN Community Standard \cite{gsn11}; we will refer to it as to the (GSN) Example. In this section, we will interpret the Example as a sketch of a simple safety case, extract its semantic meaning and present it in \wfp\ terms, and then compare the two cases, as schematically shown in \figgsntowf. 

We first recover semantics (wavy mapping in \figrii) in (sub)\secref{recoverSem}. We then reformulate this semantics in \wfc-terms as two conformance checks between three workflows (note the curved block arrow) 
This is the content of five subsections \secref{GSNWF+}-\sectref{aspects}. \zdmoddok{Note that in \sectref{conformToNorm} we consider an important component of assurance which is mainly omitted in a majority of GSN cases we are aware of, namely, conformance of the SEP definition to some normative workflow.}{}{important remark but doesn't belong here}{-5em}   
Finally, in \sectref{anti-gsn} we will compare the two specifications focusing on how information is represented and arguments are formed.
%Throughout this section, elements of \figref{fig:gsnEx-main} will be referenced by their title in italicized text, for example \gone.


==> sections/TR/gsn2wf-newTR.tex <==
% to ease ref to figs
\newcommand\figgsn{\figref{fig:gsnEx-main}}
\newcommand\figrecsem{\figref{fig:gsn2wf}}
\newcommand\figgsntowf{\figref{fig:gsn2wf}}
\renewcommand\figrii{\figgsntowf}
\newcommand\figgsnann{\figref{fig:GSNannotated}}
\newcommand\figann{\figgsnann}
\newcommand\figgsnanni{\figref{fig:GSNAnnotated-1}}
\newcommand\figgsnannii{\figref{fig:GSNAnnotated-2}}
\newcommand\figsepdefi{\figref{fig:metamodel}}
\newcommand\figsepdefii{\figref{fig:inference}}
\newcommand\sectsepdef{\sectref{GSNWF+}}

\section{From GSN to Workflow+}\label{sec:wfba}
\input{figures/TR/gsnEx-mainTR}

\input{sections/TR/gsn2wf-introTR}
\input{sections/TR/recoverSemTR}
\input{sections/TR/metamodel-mainTR}
\input{sections/TR/inferenceTR}
\input{sections/TR/instConformTR}	
\input{sections/TR/conformToNormTR}
\input{sections/TR/aspectRTR}
\input{sections/TR/anti-gsn-newTR}


\endinput

%We agreed this is not needed.
%(A more complex version is on \figref{fig:gsn2wf2gsn} but I am not sure it's needed)

==> sections/TR/gsn2wfTR.tex <==
% note \endinout on l.152

% to ease ref to figs
\renewcommand\figri{\figref{fig:gsnEx-main}}
\renewcommand\figrii{\figref{fig:recoverSem}}
%\renewcommand\figriii{\figref{fig:wfMetamod-flow}}
%\renewcommand\figriv{\figref{fig:wfExample-dataFlow}}

\section{From GSN to Workflow+}\label{sec:wfba}
\input{figures/gsnEx-main}


Figure~\ref{fig:gsnEx-main} shows a GSN goal structure taken from the GSN Community Standard \cite{gsn11}. We interpret the diagram as a sketch of a safety case, and will extract its semantic meaning and rebuild it in WF+ terms as schematically shown in \figrii. 

We will first recover semantics (wavy mapping in \figrii) in \secref{recoverSem}. We then reformulate this semantics in terms of workflow+  as illustrated by the upward vertical arrow in \figrii (\sectref{GSNWF+}). The latter semantics can accurately be specified as a conformance of WFs as shown by the horizontal right arrows in the schema. This is the content of five subsections \secref{GSNWF+}-\sectref{aspects}. Note that in \sectref{conformToNorm} we consider an important component of assurance which is mainly omitted in a majority of GSN cases we are aware of, namely, conformance of the SEP definition to some normative workflow. %  \sectref{sec:GSNWF+}.  
Finally, in \sectref{anti-gsn} we will compare the two specifications focusing on how information is represented and arguments are formed.
Throughout this section, elements of \figref{fig:gsnEx-main} will be referenced by their title in italicized text, for example \gone.
\input{figures/recoverSem}

\shortlong
{%short
\subsection{Recover Semantics}
\label{sec:recoverSem}
\input{figures/GSNannotated}
Figure~\ref{fig:GSNAnnotated} presents an annotated version of \figref{fig:gsnEx-main}. In this diagram we show the implicit structure in \figref{fig:gsnEx-main}, namely process flow(green for generic processes, purple for reviews) and dataflow(orange). Constraints(red), inference(blue) and data from standards(grey) are explicitely stated in the safety case and are annotated to show their relationship with the case's implicit structure. 

 Beginning with process and data flow, we see that an instance of a control system's definition and its operating role and context are input to a hazard analyisis(FHA) to generate a list of hazards. These hazards are subjected to SIL assessment and grouped by SIL apportionment(SA). These hazard groups are then allocated to protection systems responsible for mitigating them, which will be developed to the SIL appropriate to the group covered(PSD). 
 
 Both Protection systems mitigate hazards, so they are assessed to determine the probability of their mitigated hazards occuring(FTA). Once these probabilities are determined, hazards are checked by a simple process to determine if they are is indeed mitigated given based on their SIL and tolerability targets, which outputs mit(H)=True. Note that mit(H2) and mit(H3) are not attached to \gfi\ or \gsi\ respectively as the notion that a probability being lower than some tolerance constitutes mitigation is not mentioned in \gfi\ or \gsi.  The primary protection system is subjected to formal verification(FV) to determine that H1 has indeed been eliminated, which outputs that the claim \gfo\ is true.
 
 For some claims, truth is determined by reviewing. \snth\ and \snfo\ produce evidence supporting \gse\ and \gei\ respectively by reviewing the execution of PSD(R'') in the context of its inputs and outputs(\sectref{aspects} discusses how reviews can be included). These reviews output the truth of their respective claims. \jone\ mentions the correctness of SA, which we interpret to mean that SA must be subjected to reviewing to determine its correctness(R'). Similarly, \aone\ requires that the process FHA must the correctness and completeness of its execution reviewed to provide confidence in the completeness of the hazard list produced(R). Note that in this example, \aone\ isn't required to support the claim \gtw; having all hazards identified does not contribute to showing that all identified hazards are mitigated. This logical discrepancy is likely due to the fact that \figref{fig:gsnEx-main} is just an example to illustrate GSN constructs, but it is bad practice to illustrate a concept with a flawed example, just as one should not illustrate the concept of addition with the example 1+1=3.
 
 Now considering blue inferences, the truth \gfo, \gfi, \gsi\ and \aone\ are used to infer the truth of \gtw. Similarly, the truth of \jone, \gse\ and \gei\ are used infer the truth of \gth. Finally, the truth of \gtw\ and \gth\ are used to infer that the control system is safe. 
 
\csi\ is ignored as the lack of information about its use would unnecessarily complicate the story and require far too much speculation to be beneficial. 
}
{%long
\subsection{Recover Semantics, 1
	%Our Interpretation of the GSN Standard Example
}\label{sec:recoverSem-1}
As with all GSN safety cases, the story begins at the top. \zdmoddok{\gone}{The top goal \gone}{}{-1em} is a claim that the control system of interest is safe, given with \zdmoddok{\cone\ and \ctw}{contexts \cone\ and \ctw,}{}{-1em} which explain its operating purpose/environment and its functional architecture respectively. To show that the control system is safe, it is required to show that all hazards are appropriately mitigated/eliminated (\gtw) and that the level of rigour in the development process is appropriate to the hazards involved (\gth). Context \cfo\ is given for both \gtw\ and \gth: the hazards of the control system are identified by some functional hazard analysis FHA.

Goal/claim \gth\ is also given SIL guidelines(\cfi) as its context, which presumably includes information on how to assess the \namodok{SIL of hazards from SIL 1 to SIL 4, with SIL 4 being the most severe}{safety integrity level (SIL) of hazards, which we assume to be from SIL 1 to SIL 4, with SIL 4 being the most severe,}{} and how to develop systems of different SILs. We interpret  justification \jone\ and strategy \stw\ to mean that hazards have their SIL assessed and are grouped together. Each of these groups are allocated to a protection system intended to mitigate all hazards in that group. Each of these protection systems will then be developed to the highest SIL of all hazards in the group allocated to it(\gse, \gei). Then, for each protection system, artifacts from the software development process, \snth\ and \snfo, are provided as evidence that protection systems were properly developed. \zdnewwok{GSN calls such artifacts {\em solutions} (hence the abbreviation {\em Sn})}{}{-2em}.  \csi\ is ignored as the lack of information about its use would unnecessarily complicate the story to little benefit. 

Strategy \stw\ tells us that to demonstrate \gtw, it is shown that for each hazard(\gone, \gtw, \gth), the probability of occurrence is less than the tolarability target (given by \cth) corresponding to its SIL. From the handling of H1, H2 and H3(see \gfo, \gfi\ and \gsi\ respectively), we assume that H1 is SIL 4 and is to be eliminated, H2 is SIL 3 and has a target probability of $10^{-6}$, and H3 is SIL 2 and has a target probability of $10^{-3}$. Although SIL 1 doesn't appear in the safety case, for the sake of completeness we assume SIL 1 has a target probability of $10^{-2}$. The assumption that all hazards have been identified does not contribute to showing that all identified hazards have been mitigated. The meaning of \aone\ will appear in the next section. 
%Could also say SIL 4 is 10^-9, but they chose to eliminate it instead. 

\subsection{Recover Semantics, 2} %: The Rest of the Iceberg}
\label{sec:recoverSem-2}
%\input{figures/GSNannotated}
 \figref{fig:GSNAnnotated} presents a version of the example from the GSN community standard annotated with a block diagram where blocks are overlapping with the element that gave rise to them. In this diagram, we graphically represent the multi-dimensional meaning of the safety case outlined in \sectref{sec:recoverSem-1}. Orange blocks represent data, where instance-level data is orange and meta-level data is grey. Green blocks represent processes, with directed arrows representing input/output data. Purple blocks represent review processes, see \sectref{sec:aspects} for more on how reviews are included. Red blocks represent constraints on processes and data, where the goal is to demonstrate that each claim is True(T). Blue blocks represents inferences used to form an argument, with input and output logical elements denoted by directed arrows. 

 Beginning with process and data flow, we see that instances of a control system definition and it's operating role and context are input to a hazard analyisis(FHA) to generate a list of hazards. These hazards are subjected to SIL assessment and grouped by SIL apportionment(SA). These hazard groups are then allocated to protection systems which will be developed to the SIL appropriate to the group covered(PSD). Both Protection systems mitigate hazards, so they are assessed to determine the probability of their mitigated hazards occuring(FTA). Once these probabilities are determined, they are checked by a simple process to determine if their hazard is indeed mitigated given its SIL and tolerability targets, which outputs mit(H)=True. Note that mit(H2) and mit(H3) are not attached to \gfi\ or \gsi\ respectively as the notion that a probability being lower than some tolerance constitutes mitigation is not mentioned in \gfi\ or \gsi.  The primary protection system is subjected to formal verification(FV) to determine that H1 has indeed been eliminated, which outputs that the claim \gfo\ is true.
 
For some claims, truth is determined by reviewing. \snth\ and \snfo\ produce evidence supporting \gse\ and \gei\ respectively by assessing the execution of PSD(R'') in the context of its inputs and outputs(\sectref{aspects} discusses how reviews can be included). These reviews output the truth of their respective claims. \jone\ mentions the correctness of SA, which we interpret to mean that SA must be subjected to reviewing to determine its correctness(R'). Similarly, \aone\ requires that the process FHA must the correctness and completeness of its execution reviewed to provide confidence in the completeness of the hazard list produced(R). Again, note that in this example, \aone\ isn't required to support the claim \gtw; having all hazards identified does not contribute to showing that all identified hazards are mitigated. This logical discrepancy is likely due to the fact that \figref{fig:gsnEx-main} is just an example to illustrate GSN constructs, but it is bad practice to illustrate a concept with a flawed example, just as one should not illustrate the concept of addition with the example 1+1=3.

Now considering blue inferences, the truth \gfo, \gfi, \gsi\ and \aone\ are used to infer the truth of \gtw. Similarly, the truth of \jone, \gse\ and \gei\ are used infer the truth of \gth. Finally, the truth of \gtw\ and \gth\ are used to infer that the control system is safe. 
}%endlong


\subsection{GSN Example Modeled as WF+}\label{sec:GSNWF+}
\input{figures/metamodel}
This section presents WF+ as an alternative way to represent the multi-dimensional information presented in \figref{fig:GSNAnnotated}. Our WF+ representation of the GSN example comes as a package of five diagrams - a WF+ metamodel(\figref{fig:metamodel}, referred to as SEP for processes and dataflow, a WF+ metamodel with data, inferences over constraints and reviews(\figref{fig:inference}), an instance of the WF+ metamodel(\figref{fig:instance}), a WF+ metamodel of a normative document(\figref{fig:normative}) and a model of reviewing(\figref{fig:aspectR} see \sectref{aspects}). Figure~\ref{fig:metamodel} and \figref{fig:inference} are two views of the same model, but are separated to ease reading. Black boxes with white text are used to indicate the correspondence with elements of \figref{fig:GSNAnnotated}.

\subsubsection{WF+ Syntax}
\shortlong{%SHORT
There are three main components to WF+ models presented: process classes, data classes, and constraints. Green processes are classes whose instances are executions of a process, which takes input data to produce output data, denoted by directed arrows to and from the process respectively. The order of execution of processes is denoted by numbering in their titles. WF+ allows processes to produce new data, associations between input data, associations between input and output data, new attributs for data, or any combination thereof. Green frames denote different stages of the SEP. As a whole, these processes form the SEP to be followed during the development of a safety-critical system. 
}
{%LONG
There are three main components to WF+ models presented: process classes, data classes, and constraints. Processes, stereotyped <<Process>>, are classes whose instances are executions of a process, which takes input data to produce output data, denoted by directed arrows to and from the process respectively. The order of execution of processes is denoted by numbering in their titles. WF+ allows processes to produce new data, associations between input data, associations between input and output data, new attributs for data, or any combination thereof. If associations are output by a process, they are refied as an association class and an output arrow is directed there. If an attribute of data is output, an arrow is directed to the new data created, which will be an attribute of input data.

Green frames denote that the process in its top left corner was decomposed into the processes contained by the frame. That is, the process in the top left corner of a frame is a black-box representation of a process, which can be implemented by the internal processes within the frame. As a whole, these processes form the SEP to be followed during the development of a safety-critical system. In their current simplified form, these processes would not be very instructive to an engineer attempting to execute the process. Through enrichment and decomposition of the model, these processes can become as well-defined(or undefined) as is desired. This flexibility can be useful to engineers designing these processes for several reasons: it allows safety-critcal components of processes to be as prescriptive as possible, it allows creative processes to be left as "free" as is acceptable, and enables a "graceful" transition for organizations adopting this technology who are unable to convert their entire practice to this style in one fell swoop. 
}%ENDLONG

\shortlong
{%SHORT
Data classes represent data produced and/or used by processes during the execution of a SEP. Orange data indicates that it is given as input to the SEP. Any associations between non-process classes are standard UML associations(directed arrows are reserved to annotate process flow). Boundary objects(circle with a vertical line attached) are used as aliases for data to reduce the number of crossing lines in the model. 
}
{%LONG
Data classes represent data produced and/or used by processes during the execution of a SEP. Orange data indicates that it is given as input, not produced by any modelled process, and yellow data indicates that it is produced by a modelled process. Any associations between non-process classes are standard UML associations(directed arrows are reserved to annotate process flow). Occasionally, boundary objects(circle with a vertical line attached) are used as aliases for classes with the same name to reduce the number of crossing lines in the model. 
}%ENDLONG

Constraints are used to restrict the structure of instantiations of the SEP. Multiplicities typical of UML are used to specify how many data classes are related to each other, and how many instances of data are input/output to/from processes. OCL-style constraints are used between classes and associations, which can be complex and will be explained on a case-by-case basis.

\subsubsection{WF+ 1 - Metamodel}

\figref{fig:metamodel} shows a WF+ representation of the green and orange elements from \figref{fig:GSNAnnotated}. Bold red lines are used as constraints, where black, grey and blue lines are used for dataflow and associations. Black and grey lines are used solely to ease reading of crossing lines.  
\shortlong{%SHORT
\paragraph{HARA}
The topmost green frame, HARA, contains three processes: \fha, \dersil and \silapp. Just as in the GSN example, \fha uses the control system of interest(more accurately its functional architecture) and operating role and context to identify hazards. We have introduced four attributes for \hazard\, including whether it should be mitigated or eliminated, that are common artifacts of hazard analyses.
Following this, each \hazard\ is assessed as per the \silguide\ by \dersil\ to identify its \sil. Notice that through multiplicity constraints, there will be one execution of \dersil\ for each hazard, and one \sil\ output. Then, every hazard(notice that \sil\ is included by virtue of being an attribute) is input to \silapp\ to produce \hazgr s and a \containment\ association to show which hazards belong to which group. \hazgr\ has a method $\backslash$\sil\ that calculates the \sil\ of the group, which is the highest \sil\ of all \hazard s in the group.
}
{%LONG
\paragraph{HARA}

The first step in the GSN example can be interpreted as performing a hazard analysis and risk assessment(HARA). The topmost green frame, HARA, contains three processes: \fha, \dersil and \silapp. Just as in the GSN example, \fha uses the control system of interest(more accurately its functional architecture) and operating role and context to identify hazards. We have introduced four attributes for \hazard\ that are common artifacts of hazard analyses and are helpful for assessing a \hazard s \sil. \hazdesc\ is a description of \hazard\ and its consequences, \severity\ is a description of how severe the consequences of \hazard\ are, \likelihood\ is how often the hazard would occur if \cs\ was left as is, and \mitorelim\ dictates whether \hazard\ should be mitigated or eliminated as determined by \fha. 
Following this, each \hazard\ is assessed as per the \silguide\ by \dersil\ to identify its \sil, which is output as an attribute of  \hazard. Notice that through multiplicity constraints, there will be exactly one execution of \dersil\ for each hazard, and exactly one \sil\ output. Then, every hazard(notice the multiplicity constraint \namefont{all} and that \sil\ is included by virtue of being an attribute) is input to \silapp\ to produce \hazgr s and a \containment\ association to show which hazards belong to which group. Notice that the multiplicities on \containment\ limit hazards to being part of exactly one \hazgr. \hazgr\ has a method $\backslash$\sil\ that calculates the \sil\ of the group, which is the highest \sil\ of all \hazard s in the group.
}%ENDLONG

\shortlong{%SHORT
\paragraph{Design}
Once \hazard s are grouped, the next step is to develop a \protsys\ for each \hazgr\ to mitigate or eliminate every \hazard\ in it. This is done through \devprotsys, which is executed once for each \hazgr\ while following \silproc\ to produce a \protsys\ for the \hazgr\ input and a traceability association \grprot\ to the group it is protecting. Through \grprot\ and \containment,  \elim\ and \mitig\ are derived, indicating which hazards are eliminated or mitigated by which systems. The multiplicity constraint $1$ between \elim\ and \mitig\ means that each hazard is either mitigated or eliminated by one \protsys.
}
{%LONG
\paragraph{Design}
Once \hazard s are grouped, the next step is to develop a \protsys\ for each \hazgr\ to mitigate or eliminate every \hazard\ in it. This is done through \devprotsys, which is executed once for each \hazgr\ while following \silproc\ to produce a \protsys\ for the \hazgr\ input and a traceability association \grprot\ to the group it is protecting. Now, through \grprot\ and \containment, associations \elim\ and \mitig\ can be automatically derived, indicating which hazards are eliminated or mitigated by which systems. The multiplicity constraint $1$ between \elim\ and \mitig\ means that each hazard is either mitigated or eliminated by one \protsys.
}%ENDLONG

\shortlong{%SHORT
\paragraph{Verification}
Finally, the SEP verifies that each \hazard\ is eliminated or sufficiently mitigated. The constraint \namefont{XOR} between inputs to \formverif\ and \fta\ means that each hazard is verified by exactly one method; \hazard s to be eliminated must undergo formal verification(\sse in the model) and those to be mitigated must be assessed using fault tree anaylsis. For each \hazard\, \namefont{self.\mitorelim} can be used to determine which verification process should be used, and the \protsys\ to be used can be found through \namefont{self.\mitig} or \namefont{self.\elim}(only one can exist in an instance).

If \sse\ deems that the hazard has indeed been eliminated, it outputs the attribute \valid\ of the \elim\ association with \Value =$True$. If the \hazard\ is not eliminated, the same attribute is crated but with \Value=$False$.
	
\fta\ outputs the actual probability, \realprob\, of the \hazard occuring with the \protsys\ in place. \vermit\ then compares \realprob\ to the target probability from \tolgui\ to check that for \hazard 's \sil, the probability of \hazard occuring is indeed low enough. If it is low enough, it outputs the attribute \valid\ of the \mitig\ association with \Value =$True$. If the \hazard\ is not mitigated, the same attribute is crated but with \Value=$False$.
}
{%LONG
\paragraph{Verification}
Finally, the SEP verifies that each \hazard\ is eliminated or adequately mitigated. The constraint \namefont{XOR} between inputs to \formverif\ and \fta\ means that each hazard is verified by exactly one method.

For each \hazard\ to be eliminated, that is, each \hazard\ with \namefont{self.\mitorelim=elim}, the \protsys\ covering that \hazard\ undergoes formal verification through an execution of \sse(The correct \protsys can be systematically found through the link \hazard.\elim). If \sse\ deems that the hazard has indeed been eliminated by the \protsys, it outputs the attribute \valid\ of the \elim\ association between the input \hazard\ and its \protsys\ with \Value =$True$. If the \hazard\ is not eliminated, the same attribute is crated but with \Value=$False$.

Similarly, for every \hazard\ with \namefont{self.\mitorelim=mit}, the corresponding \protsys\ is subjected to a fault tree analysis through execution of \fta. \fta\ outputs the actual probability, \realprob\, of the \hazard occuring with the \protsys\ in place. \vermit\ then compares \realprob\ to the target probability from \tolgui\ to check that for \hazard 's \sil, the probability of \hazard occuring is indeed low enough. If it is low enough, it outputs the attribute \valid\ of the \mitig\ association between the input \hazard\ and its \protsys\ with \Value =$True$. If the \hazard\ is not mitigated, the same attribute is crated but with \Value=$False$.
}%ENDLONG
\shortlong{%SHORT
\subsection{Inference Over Data}
\input{figures/inference}
WF+ allows for inferences to be made over constraints on meta-level data, illustrated in \figref{fig:inference}. Light pink constraints are "normal" constraints, dark pink constraints are constraints on values, and blue constraints are derived.

Something about completeness constraints being special

Inferences are made from the bottom up, where two or more constraints are used to infer a derived constraint. For example, consider the derived constraint that all hazards are grouped appropriately(C1). C1 depends on two conditions: each hazard must be contained by a group(apportionment complete) and that each containment is correct.  If these two constraints are satisfied, then we can infer that all hazards are indeed grouped appropriately. 
}
{%LONG
\subsection{Inference Over Data}
\input{figures/inference}
WF+ allows for inferences to be made over constraints on meta-level data, illustrated in \figref{fig:inference}. Light pink constraints are "normal" constraints, dark pink constraints are constraints on values, and blue constraints are derived from multiplicity and value constraints. Black rectangles with white text map elements of \figref{fig:instance} to \figref{fig:gsnEx-main}. For the time being, we will ignore the role played by reviews as they will be explained in \sect{?}.

Inferences are made from the bottom up, where two or more constraints are determined to imply a derive constraint. Consider the derived constraint that all hazards are grouped appropriately(C1). C1 depends on two conditions: each hazard must be contained by a group(apportionment complete) and that each containment is correct.  If these two constraints are satisfied, then we can conclude that all hazards are indeed grouped appropriately. Similarly, C2 depends on two conditions: Each hazard group must be protected by a system, and the system must be appropriate for protecting that group. If these two conditions are satisfied, we can infer that all hazard groups are assigned to the appropriate protection system. From both C1 and C2, we can infer that all hazards are assigned to the appropriate protection system(C5).

C3 depends on two conditions: that the mitigation(or elimination) of each hazard by the assigned protection system is verified. If these two conditions are satisfied, we can infer that all protection systems verifiably mitigate(or eliminate) all hazards they are intended to mitigate(or eliminate). 

C4 depends on two conditions: The SIL each protection system is developed to must be appropriate given the hazard group it protects, and the development of each must indeed follow the guidelines for its SIL. From this, we can infer that each protection system was developed to the appropriate SIL. 

Given C3, C4 ad C5, we can infer that all identified are effectively eliminated or mitigated(C6). Finally, if all hazards are effectively eliminated or mitigated(C6) and all hazards are identified, we infer the top constraint that the control system is indeed safe.

In this setting, arguments, their origin and their relationships are presented unambiguously with no flexibility in how they are structured. Making inferences about systems in this way is not an attempt to allow one to formally prove the safety of a system. It is certainly possible, if not probable, that an expert would disagree with the inferences made in \figref{fig:instance}. In fact, this is exactly the point; presenting inferences with access to all relevant data, associations, and processes used allows these inferences to be analyzed critically. 
}%ENDLONG

\shortlong{%SHORT
	
	\endinput
\subsection{ An instance and Conformance to MM}
\label{sec:instance}
\input{figures/instance}
The instance in \figref{fig:instance} is the result executing the process in \figref{fig:metamodel} . We ommit dataflow links from all processes but two to avoid clutter but still demonstrate dataflow in the instance. Here, we see product-level details appear. Detailed information ommitted in \figref{fig:gsnEx-main} was "made up" for the sake of the example(such as \textit{Prob1: \realprob)}. 

Once an instance is complete, or at any desired point along the way, tools can be used to automatically verifiy syntactic contraints. An example of this is shown by horizontal red lines attached to the associations being verified. 

If all syntactic contraints are satisfied, we can conclude that condition b in DEFENITION 1 REF is satisfied. It may seem strange to say that the satisfaction of syntactic constraints can be used to conclude that the SEP was well executed, but as the metamodel encodes all semantics syntactically(eg. the validity of data through reviewing), confidence in the instance is reduced to a simple conformance check. There is no magic; everything important to safe development must be done, but checking that it is done is reduced to the well-known concept of conformance.

\nanew{More on constraints, conformance from zinovy probably}{}
}
{%LONG
\subsection{ An instance and Conformance to MM}
\label{sec:instance}
\input{figures/instance}
The instance in \figref{fig:instance} is the result executing the process in \figref{fig:metamodel} . We ommit dataflow links from all processes but two to avoid clutter but still demonstrate dataflow in the instance. Here, we see product-level details appear. Detailed information hidden within solutions in \figref{fig:gsnEx-main} was "made up" for the sake of the example(such as \textit{Prob1: \realprob)}. 


In the instance, \hazard s \textit{H1} and \textit{H2} were grouped together. From \figref{fig:gsnEx-main}, \textit{H1} and \textit{H2} are assumed to be the most severe, because their probability of occurance is made the lowest. Then, because in \figref{fig:gsnEx-main} there are three hazards and only two protection systems, it makes the most sense to assume the most severe hazards are addressed by the primary protection system. \nahll{The remainder of the instance is self-explanatory as it follows the logic of its WF+ metamodel directly.}{maybe a bit bold}{-3em}

Figure~\ref{fig:instance} is a view of the completed instance. In reality, it would be completed incrementally as engineers work their way through the process. Tooling designed for WF+ would allow for automated in-process syntactic checks to be implemented with the purpose of informing engineers that something went wrong or was missed while they are working. Two examples of constraint satisfaction verification are shown by horizontal red lines attached to the associations being verified. The topmost verification checks that all \containment s are syntactically correct. That is, that each \hazard\ is in one \hazgr\ and no \hazgr s are empty. Similarly, the lower verification checks \elim\ and \mitig\ associations to ensure all hazards are either eliminated or mitigated, but not both. 

\nahl{Instance inheriting derived constraints on MM}{For zinovy.}
}%ENDLONG


%\subsection{ASpects}\label{sec:aspects}
\input{sections/conformToNorm}
\input{sections/aspectR}

%\input{sections/anti-gsn}


\endinput

%We agreed this is not needed.
%(A more complex version is on \figref{fig:gsn2wf2gsn} but I am not sure it's needed)

==> sections/TR/inferenceTR.tex <==
\subsection{Recover semantics 3: Inference Over Data}
\input{figures/TR/inferenceTR}
WF+ allows for inferences to be made over constraints on meta-level data, illustrated in \figref{fig:inference}. Light pink constraints are "normal" constraints, dark pink constraints are constraints on values, and blue constraints are derived.

Something about completeness constraints being special

Inferences are made from the bottom up, where two or more constraints are used to infer a derived constraint. For example, consider the derived constraint that all hazards are grouped appropriately(C1). C1 depends on two conditions: each hazard must be contained by a group(apportionment complete) and that each containment is correct.  If these two constraints are satisfied, then we can infer that all hazards are indeed grouped appropriately. 


==> sections/TR/instConformTR.tex <==
\subsection{ An instance and Conformance to MM}
\label{sec:instance}
\input{figures/TR/instanceTR}
The instance in \figref{fig:instance} is the result executing the process in \figref{fig:metamodel} . We omit dataflow links from all processes but two to avoid clutter but still demonstrate dataflow in the instance. Here, we see product-level details appear. Detailed information ommitted in \figref{fig:gsnEx-main} was "made up" for the sake of the example(such as \textit{Prob1: \realprob)}. 

Once an instance is complete, or at any desired point along the way, tools can be used to automatically verifiy syntactic contraints. An example of this is shown by horizontal red lines attached to the associations being verified. 

If all syntactic contraints are satisfied, we can conclude that condition b in DEFENITION 1 REF is satisfied. It may seem strange to say that the satisfaction of syntactic constraints can be used to conclude that the SEP was well executed, but as the metamodel encodes all semantics syntactically(eg. the validity of data through reviewing), confidence in the instance is reduced to a simple conformance check. There is no magic; everything important to safe development must be done, but checking that it is done is reduced to the well-known concept of conformance.

\nanew{More on constraints, conformance from zinovy probably}{}


==> sections/TR/metamodel-mainTR.tex <==
\subsection{Recover semantics 2: Process\& Dataflow from GSN to \wfp} 
\label{sec:GSNWF+}

This section presents \wfp\ as an alternative way to represent the multi-dimensional information presented in \figref{fig:GSNAnnotated}. Our WF+ representation of the GSN example comes as a package of five diagrams - a WF+ metamodel(\figref{fig:metamodel}, referred to as SEP for processes and dataflow, a WF+ metamodel with data, inferences over constraints and reviews(\figref{fig:inference}), an instance of the WF+ metamodel(\figref{fig:instance}), a WF+ metamodel of a normative document(\figref{fig:normative}) and a model of reviewing(\figref{fig:aspectR} see \sectref{aspects}). Figure~\ref{fig:metamodel} and \figref{fig:inference} are two views of the same model, but are separated to ease reading. Black boxes with white text are used to indicate the correspondence with elements of \figref{fig:GSNAnnotated}.


\input{figures/TR/metamodelTR}

\endinput

\subsubsection{WF+ Syntax}
There are three main components to WF+ models presented: process classes, data classes, and constraints. Green processes are classes whose instances are executions of a process, which takes input data to produce output data, denoted by directed arrows to and from the process respectively. The order of execution of processes is denoted by numbering in their titles. WF+ allows processes to produce new data, associations between input data, associations between input and output data, new attributs for data, or any combination thereof. Green frames denote different stages of the SEP. As a whole, these processes form the SEP to be followed during the development of a safety-critical system. 

Data classes represent data produced and/or used by processes during the execution of a SEP. Orange data indicates that it is given as input to the SEP. Any associations between non-process classes are standard UML associations(directed arrows are reserved to annotate process flow). Boundary objects(circle with a vertical line attached) are used as aliases for data to reduce the number of crossing lines in the model. 

Constraints are used to restrict the structure of instantiations of the SEP. Multiplicities typical of UML are used to specify how many data classes are related to each other, and how many instances of data are input/output to/from processes. OCL-style constraints are used between classes and associations, which can be complex and will be explained on a case-by-case basis.

\subsubsection{WF+ 1 - Metamodel}

\figref{fig:metamodel} shows a WF+ representation of the green and orange elements from \figref{fig:GSNAnnotated}. Bold red lines are used as constraints, where black, grey and blue lines are used for dataflow and associations. Black and grey lines are used solely to ease reading of crossing lines.  

\paragraph{HARA}
The topmost green frame, HARA, contains three processes: \fha, \dersil and \silapp. Just as in the GSN example, \fha uses the control system of interest(more accurately its functional architecture) and operating role and context to identify hazards. We have introduced four attributes for \hazard\, including whether it should be mitigated or eliminated, that are common artifacts of hazard analyses.
Following this, each \hazard\ is assessed as per the \silguide\ by \dersil\ to identify its \sil. Notice that through multiplicity constraints, there will be one execution of \dersil\ for each hazard, and one \sil\ output. Then, every hazard(notice that \sil\ is included by virtue of being an attribute) is input to \silapp\ to produce \hazgr s and a \containment\ association to show which hazards belong to which group. \hazgr\ has a method $\backslash$\sil\ that calculates the \sil\ of the group, which is the highest \sil\ of all \hazard s in the group.

\paragraph{Design}
Once \hazard s are grouped, the next step is to develop a \protsys\ for each \hazgr\ to mitigate or eliminate every \hazard\ in it. This is done through \devprotsys, which is executed once for each \hazgr\ while following \silproc\ to produce a \protsys\ for the \hazgr\ input and a traceability association \grprot\ to the group it is protecting. Through \grprot\ and \containment,  \elim\ and \mitig\ are derived, indicating which hazards are eliminated or mitigated by which systems. The multiplicity constraint $1$ between \elim\ and \mitig\ means that each hazard is either mitigated or eliminated by one \protsys.

\paragraph{Verification}
Finally, the SEP verifies that each \hazard\ is eliminated or sufficiently mitigated. The constraint \namefont{XOR} between inputs to \formverif\ and \fta\ means that each hazard is verified by exactly one method; \hazard s to be eliminated must undergo formal verification(\sse in the model) and those to be mitigated must be assessed using fault tree anaylsis. For each \hazard\, \namefont{self.\mitorelim} can be used to determine which verification process should be used, and the \protsys\ to be used can be found through \namefont{self.\mitig} or \namefont{self.\elim}(only one can exist in an instance).

If \sse\ deems that the hazard has indeed been eliminated, it outputs the attribute \valid\ of the \elim\ association with \Value =$True$. If the \hazard\ is not eliminated, the same attribute is crated but with \Value=$False$.
	
\fta\ outputs the actual probability, \realprob\, of the \hazard occuring with the \protsys\ in place. \vermit\ then compares \realprob\ to the target probability from \tolgui\ to check that for \hazard 's \sil, the probability of \hazard occuring is indeed low enough. If it is low enough, it outputs the attribute \valid\ of the \mitig\ association with \Value =$True$. If the \hazard\ is not mitigated, the same attribute is crated but with \Value=$False$.



==> sections/TR/recoverSemTR.tex <==
\subsection{Recover Semantics}
\label{sec:recoverSem}
\input{figures/TR/recoverSemTR}
\input{figures/TR/GSNannotatedTR}

Even a surfaced inspection of the Example's elements  shows that they (directly or indirectly) refer to entities of several basic types. There are processes, \eg, context node C4 mentions FHA (Functional Hazard Analysis), justification J1 mentions the process of SIL Apportionment (SA), solution node Sn2 mentions FTA (Fault Tree Analysis), and goals G7, G8 talk about Protection Systems Development (PSD). % realized by some process abbreviated below as PSD. 
There are also data, \eg, from context node C4, we conclude that FHA produces a set of hazards, and strategy S1 together with goals G4-6 say that this set consists of three hazards, H=\{H1, H2, H3\}, while goals G5-6 refer to probabilities of hazards H2-H3 occurrences.  
The results of this inspection are shown in \figann, where references to processes and data are labelled by green and orange block resp., and  special data residing in normative documents, Tolerability Targets in C3 and SIL Guidelines in C5, are shown in grey (ignore blocks of other colours for a while). In contrast to processes, data names are not specified to keep blocks compact.  

Note colon prefixes in block labels: they say that the Example talks about {\em instances} of processes and data, \ie, individual executions of processes and individual data objects consumed and produced by processes. For example, we have an execution of some formal verification procedure FV, which takes as its input data about the Primary protection system (note the data block on the left-down of G7 node) and produces a boolean value T; the latter resides within node G4 and denotes the statement Elim(H1)=T, where Elim refers to the proposition specified in G4. 

A more interesting dataflow is hidden behind goals G5-G6. Each of them assumes a separate FTA execution for the \corring\ hazard (note two green FTA blocks), which input  data about the \corring\ protection system (two orange arrows going left-down) and output the probability of the hazard occurrence (two green arrows resulting in p2:D and p3:D). These probabilities are compared with 
 the \corring\ normative values, $10^{-6}$ for hazards H2 having SIL=4 (see goal G7) and $10^{-3}$ for H3 with SIL=2 (see goal G8); these normative values are taken from the Tolerability document (note the grey arrows from the leftmost grey data block). If the comparison returns True, we conclude that the \corring\ hazard {\em has been sufficiently mitigated} (see goal G2 and strategy S1) and set Mit(Hi)=T for i=2,3, where Mit denotes the italicized  proposition above. We coloured the Mit-blocks differently from blocks T:B as the latter propositions are directly stated by the goal owning a red block
 % (\eg, red block in goal G4 abbreviates statement Elim(H1)=T) 
 while statements Mit(Hi)=T required, besides reading goals G5-6, also a) reading  elements G2, S1, C3, and b) having some domain knowledge merging all information involved into a reasonable workflow. Some domain knowledge is also needed to recover the dataflow between blocks FHA, SA, PSD and FV, FTA -- we will consider it in more detail later in \sectsepdef\ and \figref{fig:metamodel}. 
 
 An important type of processes assumed by the Example are {\em reviews} denoted in \figann\ by purple round blocks labelled :R. For example, to assure the statement required by justification J1, the process SA is to be reviewed, and similarly achieving goals G7 and G8 needs reviewing the \corring\ two executions of PSD. A review R of process P (we omit colons) takes P's execution data as its input%
 \footnote{To simplify notation, we omit the \corring\ data block and connect P and R immediately; an accurate worklfow model will be considered later in \sectref{aspectR}.}
   and outputs a Boolean value for the \corring\ proposition about P (typically, correctness and/or completeness phrased in context dependent terms, \eg, completeness of FHA is usually phrased as in assumption A1). Note a logical error in the Example: assumption A1 is not needed for strategy S1, but is necessary for deriving G1 from G2 and G3, \ie, it is a fundamental assumption of strategy S0 justifying this derivation (S0 is missing from the Example and was added by us). 
   
   The last entity important for the story is logical inference: note light-blue blocks I residing in strategy nodes and light-blue arrows connecting it to propositions. The inference in strategy S0 can be specified by logical formula $A1\Rightarrow(G2 \,\& \,G3 \Rightarrow G1)$,  and similarly for the two other strategy nodes (S1 is unconditional while S2 requires a side condition J1). Although inference goes bottom-up, we show it with top-bottom arrows following the GSN notation to reduce clutter. \zdhll{The logical content of inference nodes is rather trivial, the challenge is in establishing the truth of their operands. For sub-goals, this challenge is manageable by their decomposition toward simpler and simpler subgoals, while the truth of side conditions such as A1 and J1......}{to be completed or eliminated}{-10em} 
   
   Process-data annotation of even the simple example as above, reveals a major ``root-cause'' problem of GSN. Dataflow is a crucial component of SEP and its assurance, but it is ignored in GSN: indeed, a majority of data blocks in \figann\ refer to sufficiently complex data structures (encompassing multiple classes, attributes and associations--- we will see it below) but not anyhow specified in GSN diagrams. Moreover, even with a very abstract view of dataflow as shown in \figann\ (only data and process nodes), the resulting workflow does not fit in the hierarchical structure of the GSN diagram-- they significantly mismatch. \zd{to be completed}.
   %The latter specifies a logical flow in isolation of the underlying workflow ...
   
   In the next section, we will convert our process-data annotations into an accurate workflow model, and then in \sectref{?} will discuss the logical flow over the dataflow. 
      






\endinput


Figure~\ref{fig:GSNAnnotated} presents an annotated version of \figref{fig:gsnEx-main}. In this diagram we show the implicit structure in \figref{fig:gsnEx-main}, namely process flow(green for generic processes, purple for reviews) and dataflow(orange). Constraints(red), inference(blue) and data from standards(grey) are explicitely stated in the safety case and are annotated to show their relationship with the case's implicit structure. 

Beginning with process and data flow, we see that an instance of a control system's definition and its operating role and context are input to a hazard analyisis(FHA) to generate a list of hazards. These hazards are subjected to SIL assessment and grouped by SIL apportionment(SA). These hazard groups are then allocated to protection systems responsible for mitigating them, which will be developed to the SIL appropriate to the group covered(PSD). 

Both Protection systems mitigate hazards, so they are assessed to determine the probability of their mitigated hazards occuring(FTA). Once these probabilities are determined, hazards are checked by a simple process to determine if they are is indeed mitigated given based on their SIL and tolerability targets, which outputs mit(H)=True. Note that mit(H2) and mit(H3) are not attached to \gfi\ or \gsi\ respectively as the notion that a probability being lower than some tolerance constitutes mitigation is not mentioned in \gfi\ or \gsi.  The primary protection system is subjected to formal verification(FV) to determine that H1 has indeed been eliminated, which outputs that the claim \gfo\ is true.

For some claims, truth is determined by reviewing. \snth\ and \snfo\ produce evidence supporting \gse\ and \gei\ respectively by reviewing the execution of PSD(R'') in the context of its inputs and outputs(\sectref{aspects} discusses how reviews can be included). These reviews output the truth of their respective claims. \jone\ mentions the correctness of SA, which we interpret to mean that SA must be subjected to reviewing to determine its correctness(R'). Similarly, \aone\ requires that the process FHA must the correctness and completeness of its execution reviewed to provide confidence in the completeness of the hazard list produced(R). Note that in this example, \aone\ isn't required to support the claim \gtw; having all hazards identified does not contribute to showing that all identified hazards are mitigated. This logical discrepancy is likely due to the fact that \figref{fig:gsnEx-main} is just an example to illustrate GSN constructs, but it is bad practice to illustrate a concept with a flawed example, just as one should not illustrate the concept of addition with the example 1+1=3.

Now considering blue inferences, the truth \gfo, \gfi, \gsi\ and \aone\ are used to infer the truth of \gtw. Similarly, the truth of \jone, \gse\ and \gei\ are used infer the truth of \gth. Finally, the truth of \gtw\ and \gth\ are used to infer that the control system is safe. 

\csi\ is ignored as the lack of information about its use would unnecessarily complicate the story and require far too much speculation to be beneficial. 


==> sections/anti-gsn-new.tex <==
\subsection{\wfp\ vs. GSN}\label{sec:anti-gsn}

(o) \zdhll{The logical content of inference nodes is rather trivial, the challenge is in establishing the truth of their operands. For sub-goals, this challenge is manageable by their decomposition toward simpler and simpler subgoals, while the truth of side conditions such as A1 and J1......}{to be completed or eliminated}{-10em} 


  Process-data annotation of even the simple example as above reveals a major ``root-cause'' problem of GSN. Dataflow is a crucial component of SEP and its assurance, but it is ignored in GSN: indeed, a majority of data blocks in \figann\ refer to sufficiently complex data structures (encompassing multiple classes, attributes and associations--- we will see it below) but not anyhow specified in GSN diagrams. Moreover, even with a very abstract view of dataflow as shown in \figann\ (only data and process nodes), the resulting workflow does not fit in the hierarchical structure of the GSN diagram. For instance, the Example shows goal decomposition below G2 and below G3 as two separate branches while the dataflow shows that the left branch depends on the right one. % , -- they significantly mismatch. \zd{to be completed}.
%The latter specifies a logical flow in isolation of the underlying workflow ...

==> sections/anti-gsn.tex <==
\newcommand\wfbf{{\bf\em \wcfa}}
\newcommand\gsnbf{{\bf\em GSN}}

%\subsection{\wcfa\ vs. GSN}\label{sec:anti-gsn}
%We will begin with listing major GSN flaws

We will consecutively analyze seven major issues with safety cases identified in a survey on safety case use in practice [ref to survey] and being quite common  according to our own experience of doing safety assurance in the industrial setting and consultancy. We will provide an italicized summary of each issue identified in the survey, followed by the applicability of \wcfa\ in corroborating and/or addressing the issue followed by GSN's inapplicability to manage or, worse, abolity to create the issue.   

\subsubsection{\textbf{Scalability}}
{\em Navigation and comprehension of SC  is difficult. Current tools either fail to deliver features to handle scalability, or are domain-specific and not generalizable.} 

\wfbf: a) All traceability is explicit, thereby improving understandability, b) The \fwk\ is b) model-based, and moreover, c) allows for compositionality and hence decomposition and modularization %ing for the adoption of multi-view modelling to modularize, and hence improve, understandability of safety cases. 
%
\gsnbf: SCs are difficult to comprehend due to the amount of implicit information and its irregular representation  appearing even in simple SCs (see \figref{fig:GSNAnnotated}); for big industrial SCs, these deficiencies can accumulate enormously and really prevent understanding. %which may become . As GSN-style safety cases become large, they quickly become incomprehensible. The lack of primitives to represent basic concepts such as process flow and dataflow are major contributors to this issue with GSN. 


\subsubsection{\textbf{Managing Change}}
\textit{There are no effective mechanisms to manage changes in SCs. Lack of integration of processes and inadequate tool support are contributing factors.}

\wfbf: Complete traceability between model elements, explicit dataflow and explicit process flow, all of which are crucial for impact analysis and change management. \gsnbf: traceability is almost entirely omitted,
making change management a very difficult task. Moreover, the lack of well defined semantics of syntactic elements, %(again, see \figref{fig:GSNAnnotated}) - No GSN elements play well defined roles), 
makes the development of tools supporting automatic change management very difficult.  

\subsubsection{\textbf{Requiring special skills to create}}
\textit{Graphic notations of SCs are typically intuitive to understand, but creating a well-structured, convincing SC requires special skills and experience. The privacy of information in SCs prevents the sharing of knowledge on effective patterns and strategies.}

\wfbf: a) Workflows are a natural way for engineers to understand their work. As a result, \wcfa\ provides an intuitive and easily understandable framework for building SCs. b) A strict separation of instance and meta- (and metameta-) levels  of modelling allows experts to create templates and share effective patterns and strategies \zdmoddok{without fear of revealing sensitive information about products}{so that the fear of revealing sensitive information about products can be essentially mitigated.}{}{-3em}
\gsnbf: It is unnatural, and hence difficult, for engineers to convert their intuitive understanding of the story of a system's safety into the one-dimensional structure of GSN-style safety cases.

\subsubsection{\textbf{Complexity of the system}}
\textit{Identifying safety concerns is extremely difficult in complex systems due to the difficulty of managing and identifying interactions between different subsystems. Multidisciplinary collaboration is also challenging.}

On complexity. \wfbf: \zdmodd{WF+ remedies this issue by a) including the traceability required to manage complex interactions and b)supporting the modularity necessary for humans to be able to interpret complex structures.}
{a) Traceability does help to identify interactions b) Compositionality of WF+ allows for decomposition --- a classical engineering approach to manage complexity.}
{just to show how it works}{-5em}
\gsnbf:\zdmodd{
GSN-style SCs do not support the traceability necessary to effectively analyze interactions between different components unless the reader was deeply involved in the creation of this system. 
}{The actual absence of traceability links makes interaction analysis very difficult unless the SC assessor was deeply involved in the creation of this system. But then the assessment can suffer from confirmation bias. 
}{}{-5em}

On collaboration. \wfbf:An intuitive common language allows experts to share different perspectives and facilitate discussions
\gsnbf:Ad-hoc structure and implicit information leaves room for ambiguity, potentially impeding communication between teams

%old: WF+ provides the means for multidisciplinary collaboration by allowing experts to work with an intuitive common language to share different considerations and facilitate discussions.GSN offers an easily understandable graphical notation, but its ad-hoc strucutre and amount of implicit information leaves room for ambiguity, potentially impeding communication between teams. 

\subsubsection{\textbf{Uncertainty, trust, confidence}}
\textit{Issues of confidence and trust are seen as intangible. This leaves room for doubt about the efficacy of SCs and makes it difficult to establish trust}

Confidence and trust cannot be quantified in the context of assurance, and have long been a topic of debate(citation needed) 

\wfbf:  a) Manufacturers can be confident that their SEP is acceptably well defined, follows best practices and provides appropriate evidence by conforming to this normative document. b)\nahl{ For Zinovy: "we do real inference, not pseudo inference. Creating argument flow in wf+ is more difficult, but if you manage to do it you can trust it because it's logic"}{}

\gsnbf: The ability of manufacturers to generate trust in their safety cases is dependent upon their ability to express what has been done to reviewers. \nahll{GSN-style SCs are fundamentally unequipped to do this as they lack support for basic primitives such as processes, data and constraints(As demonstrated in \figref{fig:GSNAnnotated}, much of the information is left implicit). In the context of safety, leaving information crucial to assessment implicit unreasonably reduces the assessers ability to make conclusive verdicts.}{not too sure about this point}{-10em}

\subsubsection{\textbf{Too flexible}}
\textit{Flexebility can be dangerous because manufacturers can overlook aspects of safety. Conflicts of interest and confirmation bias contribute to this danger. This is closely related to establishing trust and confidence.}

Independent assessment has been shown to be effective in reducing confirmation bias(\cite{levesonSCinCertif}\nahl{The citation generated by the mcmaster library website is weird. Should i leave it as is, or find another link to it online?}{})
\wfbf: A well-defined structure for safety cases and the ability to offer templates to guide their development, allowing assessers to gain expertise in evaluating SCs. 

\gsnbf: The ad-hoc structure of GSN-style safety cases makes it very difficult to develop expertise in analyzing these safety cases, making it far too likely that holes in arguments will go unnoticed. 

\subsubsection{\textbf{Incomplete information}}
\textit{Survey: Limited integration of SC management into the software development process causes challenges in collecting sufficient and accurate information for safety arguments. Incomplete traceability, insufficiencies in testing and flawed safety requirements are all issues that arise as a result of this.} 

\wfbf: Processes and complete traceability between data are incorporated. This enables integration of the SEP and SC development, allowing for systematic change impact analysis and, with proper tooling, automated updating of SCs in response to changes in data and gathering of data, ensuring information is properly managed.

\gsnbf: a) GSN-style safety cases argue over instnace-level data. The notion of processes flow and dataflow are ommitted almost entirely. b) implicit traceability leaves room for data to be left behind or forgotten. \nahll{As all engineers know, design is an interative process - it is not hard to imagine that without traceability, data appearing a single time in the middle of a huge document could be forgotten, potentially leading to dire consequences.}{Would be nice to ref that boeing example, but the official investigation hasnt been released}{-18em} 


\subsubsection{Other Considerations not in survey}

\nahll{complexity is not accidental, its intentional. It definitely takes a lot of work to implement this, but the work is already being done during the creation of safety cases today - all that is missing is a proper way to document it}{Not sure what to say about these points}{-3em}


\endinput 

%NOTES WHILE READING SURVEY
\begin{itemize}
\item WF+ does not undermine the benefits!
\item CHALLENGES:

\item Scalability
\begin{itemize}
\item Survey: Navigation and comprehension are difficult. Current tools fail to deliver features for handling scalability, or are domain-specific and not generalizable. 
\item WF+:  Because it's UML-based, multiview modelling is easy to incorporate, which is helpful for understandability(ref?). This is generalizable to any domain, all that would be different are the views created, where good tooling could support the selection of different views.
\end{itemize}

\item Managing Change
\begin{itemize}
	\item Survey: No effective mechanisms to manage change. Due to lack of integration into software dev process? not quite sure how this would contribute. Lack of tool support also a contributing factor.
	\item WF+: We identified the same issue, but by a different approach. Ad-hoc structure prevents any systematic analysis of GSN safety cases. Implicit information prevents traceability. Together, these would make it next to impossible to automate any change management. 
\end{itemize}

\item Requireing special skills to create
\begin{itemize}
	\item Survey: Easy to understand SCs, but limited knowledge transfer and lack of access to real-world examples makes it difficult to learn how to make them. 
	\item From experience: This is closely related to the issue of templates. Lack of access to useful patterns (templates) often leaves practitioners on their own when creating these. Assuming not everyone has this expertise, it's inevitable that poorly structured safety cases will be created. Needs more thought
	\item WF+: Allowing structure, strategies, and patterns to be modelled at a meta-level, as opposed to the instance level, allows for knowledge sharing without the fear of releasing companies secrets. 
	
	The inherent expressiveness of UML allows domain experts participating in the creation of WF+ metamodels to encode semantics syntactically through constraints. These constraints, which can be checked automatically, allow developers and reviewers to gain confidence in the correctness of a system, i.e. an instantiation of the SEP, "for free" through conformance to its metamodel.
	
\end{itemize}
\item Complexity of the system
\begin{itemize}
	\item Survey: Capturing safety concerns is difficult in complex systems. Most likely referring to managing interactions between different subsystems. 
	\item WF+: We observed that GSN does not support the traceability to be able to effectively analyze interactions between different components, unless you were deeply involved in the creation of this system. Traceability and interaction is "easily" manageble when based on a solid model-based foundation. 
	
	multiview allows you to approach interactions in a managable way
\end{itemize}

\item Uncertainty, trust, confidence
\begin{itemize}
	\item Survey: Issues of confidence and trust are seen as intangible. This leaves room for doubt about the efficacy of SCs and makes it difficult to establish trust. 
	\item WF+: Also closely related to the issue of templates. Confidence and trust cannot be quantified, the best to be done is to follow best practices as determiend by regulators and experts. The inability to create templates prevents these best practices to be passed on to manufacturers. WF+ introduces the concept of a normative doc as a template for manufacturers. As far as a manufacturer is concerned, the issue of trust is reduced to conformance to the normative document. Trust in WF+-style normative documents is easier to show, as it allows for all considerations to be out in the open and to be critically analyzed. 
	
	we do real inference, not pseudo inference. Creating argument flow in wf+ is more difficult, but if you manage to do it you can trust it because it's logic
	
	These missing details are of great importance to those reviewing a safety case. Knowledge of how data was produced, the data it depends on and the order in which data was processed is essential when determining the suitability of data to support a claim. GSN-style safety cases are not equipped to express such information. In the context of safety, leaving information crucial to assessment implicit unreasonably reduces the assessers ability to make conclusive verdicts.
	
	In this setting, arguments, their origin and their relationships are presented unambiguously with no flexibility in how they are structured. Making inferences about systems in this way is not an attempt to allow one to formally prove the safety of a system. It is certainly possible, if not probable, that an expert would disagree with the inferences made in \figref{fig:instance}. In fact, this is exactly the point; presenting inferences with access to all relevant data, associations, and processes used allows these inferences to be analyzed critically.
	
\end{itemize}

\item Too flexible
\begin{itemize}
	\item Survey: Flexebility can be dangerous because manufacturers can overlook safety aspects. Conflicts of interest, confirmation bias contribute to this. This is closely related to establishing trust and confidence.
	\item WF+: Again, related to the issue of templates. Independent assessment is crucial for reducing confirmation bias(ref to nancy leveson's stuff?) As shown in GSN-Annotated, there are almost no restrictions on the role GSN elements can play. They can be processes, data, constraints, or any combination thereof. With ad-hoc structures, it's next to impossible to develop expertise in analyzing these safety cases, making it far too likely that holes in arguments will go unnoticed.
\end{itemize}

\item Incomplete information
\begin{itemize}
	\item Survey: Limited integration of SC management into the software dev process causes challenges in collecting sufficient and accurate information for safety arguments. Incomplete traceability, insufficiencies in testing and flawed safety requirements are all issues that arise as a result of this.
	\item WF+: As GSN-style safety cases argue over instnace-level data, the notion of processes flow and dataflow are ommitted almost entirely. In \figref{fig:GSNAnnotated} we have reconstructed both of these missing components. The true depth and complexity of the safety case becomes clear once this missing information is restored. WF+ allows for processes to be incorporated and complete traceability between data. This enables integration of the SEP and SC development, allowing for systematic change impact analysis and, with proper tooling, automated updating of SCs in response to changes in data. 
	
	On a similar note, all traceability between data is either left implicit or ommitted entirely, which can cause many negative outcomes. The lack of explicit traceability results in the assessment of a safety being dependent upon the assesser's ability to sift through massive quantities of data to find all information relevant to some particular claim, which is unreliable at best. Implicit traceability also leaves room for data in some documents to be forgotten. As all engineers know, design is an interative process - it is not hard to imagine that data appearing a single time in the middle of a huge document could be forgotten, potentially leading to dire consequences. in \sectref{??} we will discuss how the model-based nature of WF+ solves these problems.
	
\end{itemize}
	
\item Add something about recommendations for best practices?

\end{itemize}




%WORK IN PROGRESS, GENERAL THOUGHTS, IDEAS. NOT TO BE INCLUDED
We consecutively discuss major GSN flaws -- one subsubsection per a flaw. 
%\begin{itemize}
%	\item Ad hocness: the basic concepts such as Context, Assumption are too flexible and do not actually guide the SC writer
%	\item Deficiency: on the other hand, basic concepts of safety engineering in the modelling view (process, data, constraints) are not provided as promitives
%	\item no separation between meta
%\end{itemize}

\subsubsection{Ad hoc ness} The basic concepts such as Context, Assumption are too flexible and do not actually guide the SC writer

\subsubsection{Deficiency} On the other hand, basic concepts of safety engineering in the modelling view (process, data, constraints) are not provided as promitives

\subsubsection{No process flow nor dataflow}As GSN-style safety cases argue over instnace-level data, the notion of processes flow and dataflow are ommitted almost entirely. In \figref{fig:GSNAnnotated} we have reconstructed both of these missing components. The true depth and complexity of the safety case becomes clear once this missing information is restored.

\subsubsection{The iceberg metaphor}

=======

These missing details are of great importance to those reviewing a safety case. Knowledge of how data was produced, the data it depends on and the order in which data was processed is essential when determining the suitability of data to support a claim. GSN-style safety cases are not equipped to express such information. In the context of safety, leaving information crucial to assessment implicit unreasonably reduces the assessers ability to make conclusive verdicts.  For instance, consider \gfi. An assesser would first look at \gfi, search documents for H2's SIL, check that the target probability was right, search Sn2 for the applicable fault tree analysis, search documents to find which protection system covers H2 to make sure the fault tree analysis was done with the right system, check that the analysis was properly done, and finally make sure the probability is in fact low enough, all while hoping to not get lost or confused along the way.


On a similar note, all traceability between data is either left implicit or ommitted entirely, which can cause many negative outcomes. The lack of explicit traceability results in the assessment of a safety being dependent upon the assesser's ability to sift through massive quantities of data to find all information relevant to some particular claim, which is unreliable at best. Implicit traceability also leaves room for data in some documents to be forgotten. As all engineers know, design is an interative process - it is not hard to imagine that data appearing a single time in the middle of a huge document could be forgotten, potentially leading to dire consequences. in \sectref{??} we will discuss how the model-based nature of WF+ solves these problems.

Secondly, as a well-informed reader would have already noticed from our example, interpretation of these GSN-style safety cases is highly subjective. Without well-defined semantics for the syntax used, creators of safety cases are free to chose(or invent) the patterns/approaches used to support claims. As a result, GSN-style safety cases in practice containing thousands of elements, all potentially organized in a unique way, are extremely difficult to understand without assistance from their creator. Independent assessment of safety cases by regulators has been shown to be important{confirmation bias or something?}, but it is almost impossible to do so when assessing safety cases presented in this way. Moreover, the ability of assessers to gain expertise in identifying weak points in designs and holes in reasoning is dependent upon their ability to recognize patterns characteristic of poor design or reasoning. When every safety case is unique, it is very difficult to develop such expertise. As a result, it is inevitable that faults in safety cases will go unnoticed. 

\nanew{The inherent expressiveness of UML allows domain experts participating in the creation of WF+ metamodels to encode semantics syntactically through constraints. These constraints, which can be checked automatically, allow developers and reviewers to gain confidence in the correctness of a system, i.e. an instantiation of the SEP, "for free" through conformance to its metamodel. For example, consider the constraint that every \hazard\ with \sil =4 must undergo formal verification. Conformance of the instance to the metamodel implies that each \hazard\ with \sil =4 was properly verified without needing to manually check. This obviously will not aleviate the need for humans to check that the formal verificatin was done correctly, but the more detailed the syntactic constraints on formal verification, the more the assurance process can be automated. See future work? An easy-to-imagine hypothetical: In standards like ISO26262, different SILs require different architectures. It is easy to imagine that a detailed architectural MM would allow semantics to be syntactically checked, such as checking required properties such as redundancy, restricted size of interfaces, restricted coupling between components, etc. are satisfied by design.just a thought. 
}{WF+ benefit}

\nanew{Another issue is that GSN-style safety cases apply constraints to data.}{for zinovy}


%\input{figures/gsnEx-modified2}

%As demonstrated by \figref{fig:gsnEx-modified2}, 
GSN flattens the following structures:

--- instance vs. model 

--- dataflow vs. process flow vs. argument flow

\zd{this section is important but am not sure we need \figref{fig:gsnEx-modified2}. Perhaps, referring to the labelled GSN diagram would be enough. So, I removed \figref{fig:gsnEx-modified2} as it takes too much space and needs a lot of polishing -- no time }

\nahl{In their current simplified form, these processes would not be very instructive to an engineer attempting to execute the process. Through enrichment and decomposition of the model, these processes can become as well-defined(or undefined) as is desired. This flexibility can be useful to engineers designing these processes for several reasons: it allows safety-critcal components of processes to be as prescriptive as possible, it allows creative processes to be left as "free" as is acceptable, and enables a "graceful" transition for organizations adopting this technology who are unable to convert their entire practice to this style in one fell swoop. \\  \\ In this setting, arguments, their origin and their relationships are presented unambiguously with no flexibility in how they are structured. Making inferences about systems in this way is not an attempt to allow one to formally prove the safety of a system. It is certainly possible, if not probable, that an expert would disagree with the inferences made in \figref{fig:instance}. In fact, this is exactly the point; presenting inferences with access to all relevant data, associations, and processes used allows these inferences to be analyzed critically. }{Stuff from section 3 that was out of place}



==> sections/backgr-from-fase19.tex <==


\newcommand\citePPPF[1]{\cite[#1]{pppf-bloomf-scss10}}
\newcommand\citemleg{\cite{multileg-bloomf-dsn03}}
\newcommand\citevschema{\cite{?}\par\zd{DoT book https://ops.fhwa.dot.gov/publications/seitsguide/index.htm}}



%\renewcommand\topcla{``system $X$ is $S$}

\section{Introduction}
%\zd{It needs a rewrite to make it shorter}

The metaphor of the modern car as ``a computer on wheels'' is actually a precise description of the real situation..... mlns lines of codes, ... recalls due to software faults, ....,....  Hence, safety issues in software engineering...


The long history of safety assurance can roughly be divided in two periods. In the first one, the certifying authority regulated the design (D) and manufacturing process (M) so that the product had been considered safe if D and M satisfied the \req s. However, such prescriptive regulations turned out limiting technical innovations (including safety innovations if designed after the time of regulation is written; an in-depth discussion of  these and other deficiencies can be found in \cite{pppf-bloomf-10}). A better solution was found in the mid-nineties by requiring the (original equipment) manufacturer (OEM) to submit to the certifying authority a {\em safety case (SC)}: ``a documented body of evidence that provides a convincing and valid argument that a system is adequately safe for a given application in a given environment'' \zdhll{\cite{?}}{ref to ASCAD, 1998}{-3ex}. The approach turned out effective and currently dominates the assurance domain \zdhll{\cite{?,?}.}{1-2 refs are needed, Alan?}{0.5ex}

 Switching to SCs means switching the focus of regulation rather than its cancellation: to be properly built and assessed, an SC should follow the corresponding guidelines and norms, that is, should reveal (or instantiate) a predefined structure described in one or several normative documents that we will collectively refer to as a Standard. Importantly, the notion of an SC's conformance to a Standard should allow having both a formal prescriptive mechanism and a sufficient freedom of its implementation; a proper realization of this goal needs having SCs and Standards built on accurately specified similar structural foundations. The latter %Having proper structural foundations 
 would also be instrumental for managing yet another issue of safety assurance---an effective tool support  for the development and maintenance of SCs, whose cost can be enormous and, in some cases, be greater than those needed to build the system \cite{multileg-bloomf-dsn03}.
% For example, as pointed out in \cite{multileg-bloomf-dsn03}, the French RER railway in Paris contains a safety-critical system with about 20,000 lines of code with 100 person years spent on safety assurance, and NASA quoted several years ago a figure of more than \$1,000 per line for production and assurance of Space Shuttle code. %, and it is known that this contains many faults \cite{multileg-bloomf-14}.
Indeed, effective tools need well thought and well designed metamodels based on predefined mathematical rather than ad hoc patterns. %(underlying, \eg, the current OMG standard \zdhl{SACM \cite{?}}{ref to SACM}).  

In the paper, we aim at defining a mathematical model of assurance that would provide a basic  structure for both SCs and their normative documents so that conformance to a standard could be seen as a structure preserving (sp) mapping. It will allow us to model conformance as a well known formal construct of refinement. %--- a procedure $P$ implements (or refines) a specification $S$, more specifically, $P$ instantiates (the metamodel) $S$.  
Importantly, metamodels based on the structure we develop would capture much more of SC's semantic content %(more accurately, the flow of evidence underlying an SC) 
than their mainly syntactical arrangement in the Goal-Structured Notation (GSN) terms  as is done in the recent OMG standard SACM \cite{?}. % The latter specifies an SC as a GSN document, which---seen semantically---is like a UML model in which behaviour of the system is encoded in class names rather than being specified by state machines attached to classes. 
\zdhll{In our formal \fwk, the GSN-based syntax for SCs can accurately be located within a line of mathematical models for assurance as the most abstract model, in which allocation of requirements to (sub)systems, and the dynamic nature of the latter, are ignored (more accurately, are hidden in claim names but not captured anyhow formally and hence lost for tools based on metamodels).}{I guess this is what Mark always wanted to have :)}{-5em}
  
In the nutshell, the \fwk\ we propose is based on the observation that pieces of evidence can be seen as arrows between claims, which can be composed sequentially and in parallel thus endowing an SC with a structure of a (symmetric) monoidal category. Modelling the allocation of claims to (sub)systems that are, in their turn, are modelled as functional blocks (or processes in the technical sense of process algebra), 
converts the evidential structure into a monoidal double category. Then conformance to a standard amounts to having a monoidal double functor. Despite possibly frightening categorical sounding, these notions are based on simple metamodels and have a clear semantic meaning, thus opening the door for an algebraic theory of assurance and an effective tool support based on it.  

Our plan for the paper is as follows. The next section briefly overviews our \fwk: motivates and described its main ingredients. Specifically, it divides assurance ({\em A}) into {\em inferential, IA}, and {\em procedural, PA}. The former deals mainly with requirement decomposition (RD) and their subsequent verification, the latter deals with completeness of hazard analyses and their subsequent validation. Although the two assurance types are semantically very different, we consider both in the light of RD. \sectref{sec:escEx} presents our running example: a case of RD for embedded software. In \sectref{sec:prop}, we consider a propositional model of the example, and in \sectref{sec:proc},
 a much more accurate model based on the process refinement hierarchy. Related work is discussed in \sectref{sec:related} and \sectref{sec:concl} concludes. 

\endinput

\vspace{1cm}

*** From regulating Design to regulating Assurance cases cf. \citePPPF{p.51} 

-- Def of safety case \citePPPF{p.53}

*** Building AC is expensive  


%This led to the first software safety case publication and, in 1998, to ASCAD (Bloomfield et al. 1998, Bishop and Bloomfield 1998), a safety case development manual (still the only one). ASCAD provided the now customary definition of a case as ‘a documented body of evidence that provides a convincing and valid argument that a system is adequately safe for a given application in a given environment’. [Bloomfield RE, Bishop PG, Jones CCM, Froome PKD (1998) ASCAD – Adelard safety case development manual. Adelard]

From \cite{multileg-bloomf-dsn03}
-- P.1 In this paper we consider the use of diversity in arguments – so-called multi-legged arguments, specifically arguments that are used to make claims about the dependability (safety, reliability, etc) of a system. Our intention is to begin to formalise understanding of this use of diversity, so that greater confidence can be placed in the dependability claims that are made about systems.

P.3  Although we do not have answers to questions of this kind right now, their importance is without doubt. 

P.3 In critical systems, particularly, the costs of justifying safety claims can be enormous, and are likely to grow. In some cases, these costs can be greater than those needed to build the system. For example, the French RER railway in Paris contains a safety-critical system with about 20,000 lines of code [8]; 100 person years was spent on safety assurance. NASA quoted several years ago a figure of more than \$1,000 per line for production and assurance of Space Shuttle code, and it is known that this contains many faults. 

P.3 For some systems, the levels of confidence needed seem so high as to be beyond what can be claimed from the deployment of feasible amounts of evidence in conventional arguments. Can the use of argument diversity be shown to justify significantly stronger claims like these without requiring more evidence?

In the next section, we introduce the language we employ in the paper with a simple example, and then overview the technical content of the paper in Sect.3-6. In \sectref{sec:rel}, we discuss related work, and \sectref{sec:concl} concludes. 

\endinput

\zd{just a piece from Models paper, outdated}
... {\em X is S},..building  {\em assurance cases (ACs)} --- documents aimed at demonstrating \topcla\ which are written by the manufacturer of $S$  and assessed by certifying bodies% 
\footnote{The latter can be an independent agency or a group of experts at the manufacturer disjoint from the AC writers.}.
In a typical AC, the top claim \topcla\ is decomposed into subclaims involving either subsystems of $S$ or subproperties of $P$ or both, and so on, until we reach the level of ``atomic'' claims (about simple properties of simple subsystems), whose truth is ensured by immediate evidence. %This decomposition is usually framed in logical terms as the assurance argument flow so that an $i$th decomposition step is interpreted as a conjunctive implication: if a subsystem $S_i$ is composed from subsystems $S^{i1}...S_{ik_i}$, then satisfaction $S_i\models P_i$ is provided by the conjunction of satisfaction statements $S_{ij} \models P_{ij}$ ($j=1...k_i$) for appropriate subproperties $P_{ij}$  
%%$$
%%S_{i1} \models P_{11} \wedge  ...\wedge P^i_{1n_1},
%%S^i_{2} \models P^i_{21} \wedge  ...\wedge P^i_{2n_2},
%% ...,
%%S^i_{k} \models P^i_{k1} \wedge  ...\wedge P_{kn_k}
%%$$ 
%under the assumption that the metalogical information justifying this decomposition is true. 
If the correctness of every decomposition step, and the atomic claims, is validated, then the top claim is considered to be valid as well. This gives the writer and the reviewer of the AC a way to manage the sheer complexity of assurance. 
Building ACs based on decomposition is now supported by several notations and tools, 
% that allow the user to build and edit the hierarchical structures as above in a graphical way; 
\replaced{primarily}{specifically, the} Goal-Structuring Notation (GSN) and Claims-Arguments-Evidence notation \added{CAE}\added{. These methods}
and tools \cite{gsn11,cae15} 
are becoming a {\em de facto} standard in safety assurance.
  

 
The combination of two ideas --- delegating the assurance argument to the manufacturer and the decomposition approach outlined above --- gave rise to the growing popularity of ACs, which have lately emerged as a widely-used technique for assurance justification and assessment (see, \eg, surveys \cite{adelard-mss10,RushbySRI2015} on safety  cases. 




==> sections/backgr.tex <==
\section{Running Example} 

\input{figures/gsnEx-main}
%The long history of safety assurance can roughly be divided in two periods. In the first one, the certifying authority regulated the design (D) and manufacturing process (M) so that the product had been considered safe if D and M satisfied the prescribed \req s. However, such prescriptive regulations turned out limiting technical innovations (including safety innovations if designed after the time of regulation is written; an in-depth discussion of  these and other deficiencies can be found in \cite{pppf-bloomf-10}). Another approach had been getting popular since the mid-nineties by requiring the (original equipment) manufacturer (OEM) to submit to the certifying authority a {\em safety case (SC)}: ``a documented body of evidence that provides a convincing and valid argument that a system is adequately safe for a given application in a given environment'' \zdhll{\cite{?}}{ref to ASCAD, 1998}{-3ex}. The approach turned out effective and currently dominates the assurance domain \zdhll{\cite{?,?}.}{1-2 refs are needed}{0.5ex}

%Switching to SCs means switching the focus of regulation rather than its cancellation: to be properly built and assessed, an SC should follow the corresponding guidelines and norms, that is, should reveal (or instantiate) a predefined structure described in one or several normative documents that we will collectively refer to as a Standard. Importantly, the notion of an SC's conformance to a Standard should allow having both a formal prescriptive mechanism and a sufficient freedom of its implementation; a proper realization of this goal needs having SCs and Standards built on accurately specified similar structural foundations. The latter would also be instrumental for managing yet another issue of safety assurance---an effective tool support  for the development and maintenance of SCs, whose cost can be enormous and, in some cases, be greater than those needed to build the system \cite{multileg-bloomf-dsn03}.
% For example, as pointed out in \cite{multileg-bloomf-dsn03}, the French RER railway in Paris contains a safety-critical system with about 20,000 lines of code with 100 person years spent on safety assurance, and NASA quoted several years ago a figure of more than \$1,000 per line for production and assurance of Space Shuttle code. %, and it is known that this contains many faults \cite{multileg-bloomf-14}.
%Indeed, effective tools need well thought and well designed metamodels based on predefined mathematical rather than ad hoc patterns. %(underlying, \eg, the current OMG standard \zdhl{SACM \cite{?}}{ref to SACM}).  

%\input{figures/gsnEx-main}
Figure~\ref{fig:gsnEx-main} presents ...

\endinput


==> sections/comparative-survey.tex <==
%\renewcommand\wfbf{{\bf\em \wfp}}
\newcommand\gsnbf{{\bf\em GSN}}

%\subsection{\wcfa\ vs. GSN}\label{sec:anti-gsn}
%We will begin with listing major GSN flaws

We \awmodok{will consecutively analyze}{have analyzed}{} seven major issues with safety cases identified in a survey on safety case use in practice \cite{jcheng-corr18}. \namodok{These issues correspond well with our own experience of safety cases in industry.}{These issues correspond well with our own experience of safety cases in industry and overlap with our requirements described on p.1.}{} We \awmodok{will}{}{} provide an italicized summary of each issue identified in the survey \nanewok{with a reference to our requirements that are similar}{}, followed by the applicability of \wcfa\ in corroborating and/or addressing the issue, followed by GSN's \awmodok{inapplicability}{very limited (if at all) ability}{} to manage or, worse, \awmodok{}{its}{} ability to create the issue.  

\newcommand\citsur[1]{{\small\em #1}}
\subsubsection{\textbf{Scalability}}
\citsur{Navigation and comprehension of the SC is difficult. Current tools either fail to deliver features to handle scalability, or are domain-specific and not generalizable.}  

\nanew{\textbf{R4}. \textbf{R6}: Comprehensibility is essential for safety engineering.}{}

\nanew{\wfbf: a) All traceability is explicit and extends into the development process, the product artifacts and even the environment, thereby improving detailed understandability, b) The \fwk\ is model-based and  allows for compositionality and hence decomposition and modularization and so, in spite of the complexity of the system and its trace-links, there are built in constructs for managing this.}{}%ing for the adoption of multi-view modelling to modularize, and hence improve, understandability of safety cases. 
%

\gsnbf: SCs are difficult to comprehend due to the amount of implicit information and their ad hoc structure that is evident even in simple SCs (see \figref{fig:GSNannotated}); for large industrial SCs, these deficiencies can accumulate enormously and really prevent understanding. %which may become . As GSN-style safety cases become large, they quickly become incomprehensible. The lack of primitives to represent basic concepts such as process flow and dataflow are major contributors to this issue with GSN. 


\subsubsection{\textbf{Managing Change}}
\citsur{There are no effective mechanisms to manage changes in SCs. Lack of integration of processes and inadequate tool support are contributing factors.} 

\nanew{\textbf{R1}: Design iterations require reusability, and are a common trigger for changes in SCs. \textbf{R2}. \textbf{R5}: Managing change is a well-known challenge in systems engineering.}{}

\wfbf: Complete traceability between model elements, explicit dataflow and explicit process flow, all of which are crucial for impact analysis and change management.

\gsnbf: traceability is almost entirely omitted,
making change management a very difficult task. Moreover, the lack of well defined semantics of syntactic elements, %(again, see \figref{fig:GSNAnnotated}) - No GSN elements play well defined roles), 
makes the development of tools supporting automatic change management very difficult.  

\subsubsection{\textbf{Requiring special skills to create}}
\citsur{\small Graphic notations of SCs are typically intuitive to understand, but creating a well-structured, convincing SC requires special skills and experience. The privacy of information in SCs prevents the sharing of knowledge on effective patterns and strategies.} 

\nanew{\textbf{R3}: A unified approach reduces the need for special skills.}{}

\wfbf: a) Workflows are a natural way for engineers to understand their work. As a result, \wcfa\ provides an intuitive and easily understandable framework for building SCs. b) A strict separation of instance and meta- (and metameta-) levels  of modelling allows experts to create templates and share effective patterns and strategies \zdmoddok{without fear of revealing sensitive information about products}{so that the fear of revealing sensitive information about products can be essentially mitigated.}{}{-3em}

\gsnbf: It is unnatural, and hence difficult, for engineers to convert their intuitive understanding of the story of a system's safety into the one-dimensional structure of GSN-style safety cases.

\subsubsection{\textbf{Complexity of the system}}
\citsur{Identifying safety concerns is extremely difficult in complex systems due to the difficulty of managing and identifying interactions between different subsystems. Multidisciplinary collaboration is also challenging.} 

\nanew{\textbf{R2}. \textbf{R4}. \textbf{R5}.}{}

On complexity. \wfbf: \zdmoddok{WF+ remedies this issue by a) including the traceability required to manage complex interactions and b)supporting the modularity necessary for humans to be able to interpret complex structures.}
{a) Traceability does help to identify interactions b) Compositionality of WF+ allows for decomposition --- a classical engineering approach to manage complexity.}
{just to show how it works}{-5em}
\gsnbf:\zdmoddok{
GSN-style SCs do not support the traceability necessary to effectively analyze interactions between different components unless the reader was deeply involved in the creation of this system. 
}{The actual absence of traceability links makes interaction analysis very difficult unless the SC assessor was deeply involved in the creation of this system. But then the assessment can suffer from confirmation bias. 
}{}{-5em}

On collaboration. \wfbf:An intuitive common language allows experts to share different perspectives and facilitate discussions

\gsnbf:Ad-hoc structure and implicit information leaves room for ambiguity, potentially impeding communication between teams

%old: WF+ provides the means for multidisciplinary collaboration by allowing experts to work with an intuitive common language to share different considerations and facilitate discussions.GSN offers an easily understandable graphical notation, but its ad-hoc strucutre and amount of implicit information leaves room for ambiguity, potentially impeding communication between teams. 

\subsubsection{\textbf{Uncertainty, trust, confidence}}
\citsur{\small Issues of confidence and trust are seen as intangible. This leaves room for doubt about the efficacy of SCs and makes it difficult to establish trust} 

\nanew{\textbf{(R2, R3, R4, R6)}: These requirements must be addressed to allow understandable, accurate and convincing arguments to be made}{}

\nanew{Confidence and trust cannot be quantified in the context of assurance, and have long been a topic of debate(citation needed)}{}
%

\wfbf:  a) Conformance of the SEP-definition to normative documents makes a  ``half'' of the \fwk\ and thus directly addresses the issues above. %Manufacturers can be confident that their SEP is acceptably well defined, follows best practices and provides appropriate evidence by conforming to this normative document. 
b) Creating data-driven argument flow in \wfp\ is difficult (in an order of magnitude than in GSN), but if it is managed well, it provides a high level of confidence and trust because it is explicit and formalized.
%

\gsnbf: The ability of manufacturers to generate trust in their safety cases is dependent upon their ability to express what has been done to reviewers. GSN-style SCs provide little support for this as they leave massive arrays of data, process and dataflow details implicit. %they lack support for basic primitives such as processes, data and constraints(As demonstrated in \figref{fig:GSNAnnotated}, much of the information is left implicit). In the context of safety, leaving information crucial to assessment implicit unreasonably reduces the assessers ability to make conclusive verdicts.}{not too sure about this point}{-10em}

\subsubsection{\textbf{Too flexible}}
\citsur{\small Flexibility can be dangerous because manufacturers can overlook aspects of safety. Conflicts of interest and confirmation bias contribute to this danger. This is closely related to establishing trust and confidence.} 

\nanew{\textbf{R6}: Allowing too much flexibility is the opposite of observing reasonable conservatism}{}

Independent assessment has been shown to be effective in reducing confirmation bias(\cite{levesonSCinCertif}%
\wfbf: A well-defined structure for SCs and the ability to offer templates to guide their development, allowing assessors to gain expertise in evaluating SCs. 
%
\gsnbf: The ad-hoc structure of GSN-style safety cases makes it very difficult to develop expertise in analyzing these safety cases, making it far too likely that holes in arguments will go unnoticed. 

\subsubsection{\textbf{Incomplete information}}
\citsur{Survey: Limited integration of SC management into the software development process causes challenges in collecting sufficient and accurate information for safety arguments. Incomplete traceability, insufficiencies in testing and flawed safety requirements are all issues that arise as a result of this.} 

\nanew{\textbf{R2}}{}

\wfbf: Processes and complete traceability between data are incorporated. This enables integration of the SEP and SC development, allowing for systematic change impact analysis and, with proper tooling, automated updating of SCs in response to changes in data and gathering of data, ensuring information is properly managed.

\gsnbf: a) GSN-style safety cases argue over instnace-level data. The notion of processes flow and dataflow are ommitted almost entirely. b) implicit traceability leaves room for data to be left behind or forgotten. 


\subsubsection{Other Considerations not in survey}

\nahll{Complexity of \wfp\ is not accidental, it's intentional. It definitely takes a lot of work to implement this, but the work is already being done during the creation of safety cases today - all that is missing is a proper way to document it}{Not sure what to say about these points}{-3em}


\endinput 

%NOTES WHILE READING SURVEY
\begin{itemize}
\item WF+ does not undermine the benefits!
\item CHALLENGES:

\item Scalability
\begin{itemize}
\item Survey: Navigation and comprehension are difficult. Current tools fail to deliver features for handling scalability, or are domain-specific and not generalizable. 
\item WF+:  Because it's UML-based, multiview modelling is easy to incorporate, which is helpful for understandability(ref?). This is generalizable to any domain, all that would be different are the views created, where good tooling could support the selection of different views.
\end{itemize}

\item Managing Change
\begin{itemize}
	\item Survey: No effective mechanisms to manage change. Due to lack of integration into software dev process? not quite sure how this would contribute. Lack of tool support also a contributing factor.
	\item WF+: We identified the same issue, but by a different approach. Ad-hoc structure prevents any systematic analysis of GSN safety cases. Implicit information prevents traceability. Together, these would make it next to impossible to automate any change management. 
\end{itemize}

\item Requireing special skills to create
\begin{itemize}
	\item Survey: Easy to understand SCs, but limited knowledge transfer and lack of access to real-world examples makes it difficult to learn how to make them. 
	\item From experience: This is closely related to the issue of templates. Lack of access to useful patterns (templates) often leaves practitioners on their own when creating these. Assuming not everyone has this expertise, it's inevitable that poorly structured safety cases will be created. Needs more thought
	\item WF+: Allowing structure, strategies, and patterns to be modelled at a meta-level, as opposed to the instance level, allows for knowledge sharing without the fear of releasing companies secrets. 
	
	The inherent expressiveness of UML allows domain experts participating in the creation of WF+ metamodels to encode semantics syntactically through constraints. These constraints, which can be checked automatically, allow developers and reviewers to gain confidence in the correctness of a system, i.e. an instantiation of the SEP, "for free" through conformance to its metamodel.
	
\end{itemize}
\item Complexity of the system
\begin{itemize}
	\item Survey: Capturing safety concerns is difficult in complex systems. Most likely referring to managing interactions between different subsystems. 
	\item WF+: We observed that GSN does not support the traceability to be able to effectively analyze interactions between different components, unless you were deeply involved in the creation of this system. Traceability and interaction is "easily" manageble when based on a solid model-based foundation. 
	
	multiview allows you to approach interactions in a managable way
\end{itemize}

\item Uncertainty, trust, confidence
\begin{itemize}
	\item Survey: Issues of confidence and trust are seen as intangible. This leaves room for doubt about the efficacy of SCs and makes it difficult to establish trust. 
	\item WF+: Also closely related to the issue of templates. Confidence and trust cannot be quantified, the best to be done is to follow best practices as determiend by regulators and experts. The inability to create templates prevents these best practices to be passed on to manufacturers. WF+ introduces the concept of a normative doc as a template for manufacturers. As far as a manufacturer is concerned, the issue of trust is reduced to conformance to the normative document. Trust in WF+-style normative documents is easier to show, as it allows for all considerations to be out in the open and to be critically analyzed. 
	
	we do real inference, not pseudo inference. Creating argument flow in wf+ is more difficult, but if you manage to do it you can trust it because it's logic
	
	These missing details are of great importance to those reviewing a safety case. Knowledge of how data was produced, the data it depends on and the order in which data was processed is essential when determining the suitability of data to support a claim. GSN-style safety cases are not equipped to express such information. In the context of safety, leaving information crucial to assessment implicit unreasonably reduces the assessers ability to make conclusive verdicts.
	
	In this setting, arguments, their origin and their relationships are presented unambiguously with no flexibility in how they are structured. Making inferences about systems in this way is not an attempt to allow one to formally prove the safety of a system. It is certainly possible, if not probable, that an expert would disagree with the inferences made in \figref{fig:instance}. In fact, this is exactly the point; presenting inferences with access to all relevant data, associations, and processes used allows these inferences to be analyzed critically.
	
\end{itemize}

\item Too flexible
\begin{itemize}
	\item Survey: Flexebility can be dangerous because manufacturers can overlook safety aspects. Conflicts of interest, confirmation bias contribute to this. This is closely related to establishing trust and confidence.
	\item WF+: Again, related to the issue of templates. Independent assessment is crucial for reducing confirmation bias(ref to nancy leveson's stuff?) As shown in GSN-Annotated, there are almost no restrictions on the role GSN elements can play. They can be processes, data, constraints, or any combination thereof. With ad-hoc structures, it's next to impossible to develop expertise in analyzing these safety cases, making it far too likely that holes in arguments will go unnoticed.
\end{itemize}

\item Incomplete information
\begin{itemize}
	\item Survey: Limited integration of SC management into the software dev process causes challenges in collecting sufficient and accurate information for safety arguments. Incomplete traceability, insufficiencies in testing and flawed safety requirements are all issues that arise as a result of this.
	\item WF+: As GSN-style safety cases argue over instnace-level data, the notion of processes flow and dataflow are ommitted almost entirely. In \figref{fig:GSNAnnotated} we have reconstructed both of these missing components. The true depth and complexity of the safety case becomes clear once this missing information is restored. WF+ allows for processes to be incorporated and complete traceability between data. This enables integration of the SEP and SC development, allowing for systematic change impact analysis and, with proper tooling, automated updating of SCs in response to changes in data. 
	
	On a similar note, all traceability between data is either left implicit or ommitted entirely, which can cause many negative outcomes. The lack of explicit traceability results in the assessment of a safety being dependent upon the assesser's ability to sift through massive quantities of data to find all information relevant to some particular claim, which is unreliable at best. Implicit traceability also leaves room for data in some documents to be forgotten. As all engineers know, design is an interative process - it is not hard to imagine that data appearing a single time in the middle of a huge document could be forgotten, potentially leading to dire consequences. in \sectref{??} we will discuss how the model-based nature of WF+ solves these problems.
	
\end{itemize}
	
\item Add something about recommendations for best practices?

\end{itemize}




%WORK IN PROGRESS, GENERAL THOUGHTS, IDEAS. NOT TO BE INCLUDED
We consecutively discuss major GSN flaws -- one subsubsection per a flaw. 
%\begin{itemize}
%	\item Ad hocness: the basic concepts such as Context, Assumption are too flexible and do not actually guide the SC writer
%	\item Deficiency: on the other hand, basic concepts of safety engineering in the modelling view (process, data, constraints) are not provided as promitives
%	\item no separation between meta
%\end{itemize}

\subsubsection{Ad hoc ness} The basic concepts such as Context, Assumption are too flexible and do not actually guide the SC writer

\subsubsection{Deficiency} On the other hand, basic concepts of safety engineering in the modelling view (process, data, constraints) are not provided as promitives

\subsubsection{No process flow nor dataflow}As GSN-style safety cases argue over instnace-level data, the notion of processes flow and dataflow are ommitted almost entirely. In \figref{fig:GSNAnnotated} we have reconstructed both of these missing components. The true depth and complexity of the safety case becomes clear once this missing information is restored.

\subsubsection{The iceberg metaphor}

=======

These missing details are of great importance to those reviewing a safety case. Knowledge of how data was produced, the data it depends on and the order in which data was processed is essential when determining the suitability of data to support a claim. GSN-style safety cases are not equipped to express such information. In the context of safety, leaving information crucial to assessment implicit unreasonably reduces the assessers ability to make conclusive verdicts.  For instance, consider \gfi. An assesser would first look at \gfi, search documents for H2's SIL, check that the target probability was right, search Sn2 for the applicable fault tree analysis, search documents to find which protection system covers H2 to make sure the fault tree analysis was done with the right system, check that the analysis was properly done, and finally make sure the probability is in fact low enough, all while hoping to not get lost or confused along the way.


On a similar note, all traceability between data is either left implicit or ommitted entirely, which can cause many negative outcomes. The lack of explicit traceability results in the assessment of a safety being dependent upon the assesser's ability to sift through massive quantities of data to find all information relevant to some particular claim, which is unreliable at best. Implicit traceability also leaves room for data in some documents to be forgotten. As all engineers know, design is an interative process - it is not hard to imagine that data appearing a single time in the middle of a huge document could be forgotten, potentially leading to dire consequences. in \sectref{??} we will discuss how the model-based nature of WF+ solves these problems.

Secondly, as a well-informed reader would have already noticed from our example, interpretation of these GSN-style safety cases is highly subjective. Without well-defined semantics for the syntax used, creators of safety cases are free to chose(or invent) the patterns/approaches used to support claims. As a result, GSN-style safety cases in practice containing thousands of elements, all potentially organized in a unique way, are extremely difficult to understand without assistance from their creator. Independent assessment of safety cases by regulators has been shown to be important{confirmation bias or something?}, but it is almost impossible to do so when assessing safety cases presented in this way. Moreover, the ability of assessers to gain expertise in identifying weak points in designs and holes in reasoning is dependent upon their ability to recognize patterns characteristic of poor design or reasoning. When every safety case is unique, it is very difficult to develop such expertise. As a result, it is inevitable that faults in safety cases will go unnoticed. 

\nanew{The inherent expressiveness of UML allows domain experts participating in the creation of WF+ metamodels to encode semantics syntactically through constraints. These constraints, which can be checked automatically, allow developers and reviewers to gain confidence in the correctness of a system, i.e. an instantiation of the SEP, "for free" through conformance to its metamodel. For example, consider the constraint that every \hazard\ with \sil =4 must undergo formal verification. Conformance of the instance to the metamodel implies that each \hazard\ with \sil =4 was properly verified without needing to manually check. This obviously will not aleviate the need for humans to check that the formal verificatin was done correctly, but the more detailed the syntactic constraints on formal verification, the more the assurance process can be automated. See future work? An easy-to-imagine hypothetical: In standards like ISO26262, different SILs require different architectures. It is easy to imagine that a detailed architectural MM would allow semantics to be syntactically checked, such as checking required properties such as redundancy, restricted size of interfaces, restricted coupling between components, etc. are satisfied by design.just a thought. 
}{WF+ benefit}

\nanew{Another issue is that GSN-style safety cases apply constraints to data.}{for zinovy}


%\input{figures/gsnEx-modified2}

%As demonstrated by \figref{fig:gsnEx-modified2}, 
GSN flattens the following structures:

--- instance vs. model 

--- dataflow vs. process flow vs. argument flow

\zd{this section is important but am not sure we need \figref{fig:gsnEx-modified2}. Perhaps, referring to the labelled GSN diagram would be enough. So, I removed \figref{fig:gsnEx-modified2} as it takes too much space and needs a lot of polishing -- no time }

\nahl{In their current simplified form, these processes would not be very instructive to an engineer attempting to execute the process. Through enrichment and decomposition of the model, these processes can become as well-defined(or undefined) as is desired. This flexibility can be useful to engineers designing these processes for several reasons: it allows safety-critcal components of processes to be as prescriptive as possible, it allows creative processes to be left as "free" as is acceptable, and enables a "graceful" transition for organizations adopting this technology who are unable to convert their entire practice to this style in one fell swoop. \\  \\ In this setting, arguments, their origin and their relationships are presented unambiguously with no flexibility in how they are structured. Making inferences about systems in this way is not an attempt to allow one to formally prove the safety of a system. It is certainly possible, if not probable, that an expert would disagree with the inferences made in \figref{fig:instance}. In fact, this is exactly the point; presenting inferences with access to all relevant data, associations, and processes used allows these inferences to be analyzed critically. }{Stuff from section 3 that was out of place}



==> sections/conf1-syntax.tex <==
\subsection{Instance Conformance: Syntax
	%The metamodel of the Example's \wfsep%
	%Making Process \& Dataflow accurate 
} 
\label{sec:inst-conf-syn}

%This section presents \wfp\ as an alternative way to represent the multi-dimensional information presented in \figref{fig:GSNAnnotated}. Our WF+ representation of the GSN example comes as a package of five diagrams - a WF+ metamodel(\figref{fig:metamodel}, referred to as SEP for processes and dataflow, a WF+ metamodel with data, inferences over constraints and reviews(\figref{fig:inference}), an instance of the WF+ metamodel(\figref{fig:instance}), a WF+ metamodel of a normative document(\figref{fig:normative}) and a model of reviewing(\figref{fig:aspectR} see \sectref{aspects}). Figure~\ref{fig:metamodel} and \figref{fig:inference} are two views of the same model, but are separated to ease reading. Black boxes with white text are used to indicate the correspondence with elements of \figref{fig:GSNAnnotated}.

\input{figures/metamodel}
Process and data blocks in \figann\ sketch some workflow, which in this section we treat as an instance of some workflow definition/metamodel (\wfsep\ in term of \secref{ass-as-conf}). Making the latter syntactically accurate and semantically reasonable needs some domain knowledge beyond the workflow sketch in \figann, but we tried to keep the extension beyond the Example story as minimal as possible. 

We build the metamodel as a class diagram with a special type of classes stereotyped Process (green in \figsepi), whose instances are process executions. Dataflow to and from processes is shown with directed associations, while ordinary (static) \asson s between data classes (yellow and orange) are all undirected and oriented vertically. Orange data are input to the entire SEP process, consisting from three components, HARA, Design, Verification (note three green rectangles in \figsepi), which are further decomposed as shown. The order of processes is shown with numbers prefixing process names (and can be inferred from the dataflow)  
%The metamodel has the following special layout. Process are moved to the left and their order is shown by numbers prefixing their names. 
We use rectangle frames to show decomposition, \eg, process HARA consists of three subprocesses. %Data classes (yellow and orange) represent data produced and/or used by processes during their execution (orange data are input to the entire SEP) indicates that it is given as input to the SEP. Any associations between non-process classes are standard UML associations(directed arrows are reserved to annotate process flow). 
Boundary objects (circle with a vertical line attached) are used as aliases for data to reduce the number of crossing lines in the model. 

The diagram is mainly a self-explainable completion of the annotated Example (\figann); black-box labels show the backward mapping to the GSN diagram. We only mention several points. Note attribute mitORelim of class Hazard and its \multy\  [1], which says that each hazard is to be eliminated or mitigated but not both. If a hazard is to eliminated, then by composing \asson s \nmf{occursIn} and \nmf{protectedBy}, we obtain a derived \asson\ \nmf{Elimination} of \multy\ 0..1 as not each hazard is to be eliminated; similarly for hazards to be mitigated we obtain a derived \asson\ \nmf{Mitigation}.  Now \multy\ [1] implied \multy\ [1] spanning the two \asson\ ends (shown blue as it is derived)  says that each hazard is to eliminated or mitigated by exactly one PS. The inverse multiplicity 1..* is derived from \multi es of \nmf{protecs} and \nmf{consistsOf} and demands a protection system to protect against at least one hazard.
Also, process FV in \figann\ is specialized as a state space exploration, which assures hazard elimination iff the hazardous state is not reachable. The comparisons residing in goals G5, G6 are specified as executions of the query specified in box 3b.2, which is defined to assure hazard mitigation. 


Note a special feature of the workflow: data produced by a process are connected to its input data, \eg, processes 1.2 and 1.3 take Hazard at the input and produce, resp., their  SIL attributes and (for process 1.3) HazardGroup together with as \asson\ linking it to Hazard. Or, process 3a takes a pair (H,PS) consisting of a hazard H and a PS intended to eliminate H, using these data build a state machine, explores whether hazardous states leading to H are reachable, and outputs the \corring\ Boolean value into the attribute slot Verified?.      



%=== inst piece
\input{figures/instance}
The metamodel in \figmetamod\ defines a workflow, which can be executed for any data correctly instantiating the orange part of the diagram, and thus instantiate the yellow part of the class diagram (ISO 26262 refers to these as to WorkProducts). The GSN Example actually tells us a story about such an instance \exeinst\ and \zdmodd{, and \figinst\ presents its fragment: to save space, we cut off part of the data rekated to hazard H3} {and \figinst\ shows it}{}{-2em}(ignore round purple elements for a while) . It is easy o see that the instance workflow \exeinst\ satisfies all constraints declared in the metamodel workflow \wfsep.

\subsection{Instance conformance: Semantic validity}
In assurance, there are two main questions about instances. The first is its syntactic correctness: whether all constraints declared in the metamodel such as \wfsep\ in \figmetamod\ are satisfied. This task can be done automatically with modern MDE tools. The second question is more challenging: syntactically correct data can be semantically invalid \eg, for instance \wfexex, a hazard can be missing from set {\sf Hazard.allInstances}=\{H1, H2, H3\}, or the SIL of hazard H1 is to be 2 rather than 4 so that hazard grouping must be changed, or if even all SILs are valid, grouping was done incorrectly and hazard H2 is to be grouped with H3 rather than H1, etc. In fact, a majority of the instance elements are to be checked for semantic validity (we will say {\em validated}), including the results of verification. Validation of an element $x$ in instance \wfexex\ is done by reviewing the process that produced $x$, \eg, FHA for the hazard set completeness, SIL Determination for SILs validity \etc. Review processes (we say {\em reviews}) are denoted by purple circles in the metamodel \figmetamod\ (we only show three of the total six (not seven as Query is computed automatically and does not need reviewing) ). Review executions in \figinst\ are also purple.  
 To simplify notation, we show the dataflow from a process to its review by an arrow and omit the intermediate data block: this is just a syntactic sugar for a detailed specification considered in the next subsection. 


\endinput







The instance in \figref{fig:instance} is the result executing the process in \figref{fig:metamodel} . We omit dataflow links from all processes but two to avoid clutter but still demonstrate dataflow in the instance. Here, we see product-level details appear. Detailed information ommitted in \figref{fig:gsnEx-main} was "made up" for the sake of the example(such as \textit{Prob1: \realprob)}. 

Once an instance is complete, or at any desired point along the way, tools can be used to automatically verifiy syntactic contraints. An example of this is shown by horizontal red lines attached to the associations being verified. 

If all syntactic contraints are satisfied, we can conclude that condition a) \defref{main}  is satisfied. It may seem strange to say that the satisfaction of syntactic constraints can be used to conclude that the SEP was well executed, but as the metamodel encodes all semantics syntactically(eg. the validity of data through reviewing), confidence in the instance is reduced to a simple conformance check. There is no magic; everything important to safe development must be done, but checking that it is done is reduced to the well-known concept of conformance.

\nanew{More on constraints, conformance from zinovy probably}{}



\endinput

\subsubsection{WF+ Syntax}
There are three main components to WF+ models presented: process classes, data classes, and constraints. Green processes are classes whose instances are executions of a process, which takes input data to produce output data, denoted by directed arrows to and from the process respectively. The order of execution of processes is denoted by numbering in their titles. WF+ allows processes to produce new data, associations between input data, associations between input and output data, new attributs for data, or any combination thereof. Green frames denote different stages of the SEP. As a whole, these processes form the SEP to be followed during the development of a safety-critical system. 

Data classes represent data produced and/or used by processes during the execution of a SEP. Orange data indicates that it is given as input to the SEP. Any associations between non-process classes are standard UML associations(directed arrows are reserved to annotate process flow). Boundary objects(circle with a vertical line attached) are used as aliases for data to reduce the number of crossing lines in the model. 

Constraints are used to restrict the structure of instantiations of the SEP. Multiplicities typical of UML are used to specify how many data classes are related to each other, and how many instances of data are input/output to/from processes. OCL-style constraints are used between classes and associations, which can be complex and will be explained on a case-by-case basis.

\subsubsection{WF+ 1 - Metamodel}

\figref{fig:metamodel} shows a WF+ representation of the green and orange elements from \figref{fig:GSNAnnotated}. Bold red lines are used as constraints, where black, grey and blue lines are used for dataflow and associations. Black and grey lines are used solely to ease reading of crossing lines.  

\paragraph{HARA}
The topmost green frame, HARA, contains three processes: \fha, \dersil and \silapp. Just as in the GSN example, \fha uses the control system of interest(more accurately its functional architecture) and operating role and context to identify hazards. We have introduced four attributes for \hazard\, including whether it should be mitigated or eliminated, that are common artifacts of hazard analyses.
Following this, each \hazard\ is assessed as per the \silguide\ by \dersil\ to identify its \sil. Notice that through multiplicity constraints, there will be one execution of \dersil\ for each hazard, and one \sil\ output. Then, every hazard(notice that \sil\ is included by virtue of being an attribute) is input to \silapp\ to produce \hazgr s and a \containment\ association to show which hazards belong to which group. \hazgr\ has a method $\backslash$\sil\ that calculates the \sil\ of the group, which is the highest \sil\ of all \hazard s in the group.

\paragraph{Design}
Once \hazard s are grouped, the next step is to develop a \protsys\ for each \hazgr\ to mitigate or eliminate every \hazard\ in it. This is done through \devprotsys, which is executed once for each \hazgr\ while following \silproc\ to produce a \protsys\ for the \hazgr\ input and a traceability association \grprot\ to the group it is protecting. Through \grprot\ and \containment,  \elim\ and \mitig\ are derived, indicating which hazards are eliminated or mitigated by which systems. The multiplicity constraint $1$ between \elim\ and \mitig\ means that each hazard is either mitigated or eliminated by one \protsys.

\paragraph{Verification}
Finally, the SEP verifies that each \hazard\ is eliminated or sufficiently mitigated. The constraint \namefont{XOR} between inputs to \formverif\ and \fta\ means that each hazard is verified by exactly one method; \hazard s to be eliminated must undergo formal verification(\sse in the model) and those to be mitigated must be assessed using fault tree anaylsis. For each \hazard\, \namefont{self.\mitorelim} can be used to determine which verification process should be used, and the \protsys\ to be used can be found through \namefont{self.\mitig} or \namefont{self.\elim}(only one can exist in an instance).

If \sse\ deems that the hazard has indeed been eliminated, it outputs the attribute \valid\ of the \elim\ association with \Value =$True$. If the \hazard\ is not eliminated, the same attribute is crated but with \Value=$False$.
	
\fta\ outputs the actual probability, \realprob\, of the \hazard occuring with the \protsys\ in place. \vermit\ then compares \realprob\ to the target probability from \tolgui\ to check that for \hazard 's \sil, the probability of \hazard occuring is indeed low enough. If it is low enough, it outputs the attribute \valid\ of the \mitig\ association with \Value =$True$. If the \hazard\ is not mitigated, the same attribute is crated but with \Value=$False$.



==> sections/contentList.tex <==

\input{sections/introNew1-zd}
%\input{sections/intro-tr}
\renewcommand\figrii{\figref{fig:recoverSem}}
\input{sections/assr-as-conf}
%=== commands to ref to figs
\newcommand\figinfer{\figref{fig:inference}}
\newcommand\figinf{\figref{fig:inference}}
\newcommand\figann{\figref{fig:GSNannotated-full}}
\newcommand\figanni{\figref{fig:GSNannotated-PD}}
\newcommand\figannii{\figref{fig:GSNannotated-PDD}}
\newcommand\figanniii{\figref{fig:GSNannotated-PDDR}}
\newcommand\figannlast{\figref{fig:GSNannotated-full}}
\newcommand\figtwotriangles{\figref{fig:two-triangles}}
\newcommand\figannlastlast{\figtwotriangles}
\newcommand\figmm{\figmetamod}
\newcommand\figrec{\figref{fig:gsn2wf}}
\newcommand\figgw{\figrec}
\input{sections/gsn2wf-new}
%\input{sections/gsn2wf}
\input{sections/gsn2wf-logicflow-new}
\input{sections/summary-zd}
\input{sections/umlProfile}
{  % begin \renewcommand \subsubsection[1] 
\paperGM{
	\input{sections/applicability} %formerly discussion
}{}
} % end \renewcomm \subsubsection
%\paperGM{
%\input{sections/work-in-progress}
%}{}
%\newpage
%\input{sections/wfp-meta-new}
\paperGM{
\input{sections/relWork}
}{}
\input{sections/concl}


==> sections/discussion.tex <==
\section{Applicability and Possible Impact
%:\wcfa\ vs. GSN
}\label{sec:compara-survey} 

%\renewcommand\awmod[3]{#2}

\input{sections/comparative-survey}


\endinput

%%%%%\zd{Below is a rather unordered piece about how \wfp\ meets the \req s R1-6}
%Workflows are a classical engineering idea, and different workflow formalisms have an excellent record in various branches of  engineering (electrical, chemical, software,...) thus providing a common ground for different stakeholders from business analysts to electrical to system engineers. We thus satisfy requirements R3 (partially), and R4-6 (R5 is provided by the compositionality of workflows).    

%\zd{what is below is a repetition of sect 2}
%Process-based assurance has long traditions but was often criticized for indirectness and hence unreliability \citealan. We mitigate this problem by a detailed process modelling focused on data; our processes are more like (multiary) model \trafon s: they consume data conforming to input metamodels and produce data conforming to output metamodels. 
%Importantly, in general, the output data are related to input data% 
%\footnote{a typical example is when the input to a process is specified by a class or several classes, while the output provides new attributes for the input classes and/or new associations between them}. Because of this special feature of our workflow models, we refer to them as {\em workflow$^+$ (\wfp)}. 
%%%%%The argument flow (mandatory for SC) in \wfp\ is realized as derivation of OCL constraint over the \corring\ data, and is thus data-driven.  %(which moves the underlying logic beyond the boundaries of propositional logic customary for modern SCs). 
%
%%%%%A typical \wfp-model comprises three (interrelated) lanes: (i) process and control flow, (ii) dataflow (with input-output relationships), and (iii) argument flow or constraint derivation. It is the dataflow lane that bounds all ingredients into a single \WF-model and makes our assurance methodology essentially product-oriented. Thus, \wfp\ satisfies R3 (completed)
%%%%%and R7 (sect 2 discusses that process-orientation is reasonably conservative).

%%%%%As for the major requiremenst R1-2,...  ...\wfp\ being a truly UML/MOF-\fwk based on metamodeling, class diagram s,.... 
%%%%%\zd{====== the unordered piece ends here}
%\input{sections/anti-gsn}


==> sections/empirical.tex <==
\subsection{XXXX}
In Models18 paper, we used the result of some survey-- we can try something similar again.

==> sections/eval.tex <==
\section{Evaluation}\label{sec:eval}

Do an evaluation based on the shortfalls of safety cases similar to the evaluation done in the models 18 paper. 

==> sections/gsn2wf-logicflow.tex <==
\section{From GSN to Workflow+, 2: Argument Flow}\label{sec:gsn2wf2}


%%\endinput
%\newcommand\figinfer{\figref{fig:inference}}
%\newcommand\figinf{\figref{fig:inference}}
%\newcommand\given{\nmf{given}}
%\newcommand\der{\nmf{der}}
%\renewcommand\data{\nmf{data}}
%\newcommand\val{\nmf{val}}
%\newcommand\cset[1]{\ensuremath{{\mathbf{C}}_{#1}}}

\input{figures/inference}
In this section we reproduce the argument flow of the Example by treating it as a constraint derivation procedure $\cset{\given}\vdash\cset{\der}$, where  \cset{\given} is a set of constraints initially specified ({\em given}) in the metamodel \wfsep\ and \cset{\der} consists of those ({\em derived}) constraints that we need to infer logically in order to reconstruct the logical flow of the Example. As the logic we will use for inference is obviously sound
(in the sense of mathematical logic), if an instance \wfexex\ satisfies the given constraints, then it is automatically satisfies all derived constraints. \zdhl{A great advantage of this approach in comparison with GSN is its reusabilty:  ...}{should go to the end}



% (it is, in fact, the definition of soundness). 
We will show how the top claim of system's safety $C0$ % (goal G1 in the Example) 
can be inferred from given constraints and thus build a \wfp-based safety case.  

Set \cset{\given} consists of two group of constraints: %$\cset{\given}=\cset{\data}{\cup}\cset{\val}$, where 
constraints over data in \wfsep\ (in our case, multiplicities)
% plus implicit constraints embodied in black-white diamond symbols) 
are grouped into set \cset{\data}, and constraints stating validity of data as discussed in \sectref{sem-val} are grouped into set \cset{\val}. Thus, we need to show an inference tree for    
$(\cset{\data}\cup \cset{\val})\vdash C1$, which we do with \figinfer.

Figure~\ref{fig:inference} shows the metamodel \wfsep, in which green process blocks are omitted (and several blue-boxes with white font are added but ignore them for a while), and data constraints are supplied with {\em claims}---formulations of constraints' semantics in common assurance-motivated terms (note pink boxes with a black-font text). We have also added a composed (and hence derived) \asson\ 
\begin{equation}\label{eq:protect-def}
\Protn = \Contt \Join  \grPrtn
\end{equation}
 from Hazard to HazardGroup to ProtectionSystem with (derived) multiplicities [1] at the bottom and [1..*] at the top end, which we will need for inference.
%; we will refer to them as to {\em claims}.  
Note also six purle aliases of six review processes 1.1-3, 2.1, 3a and 3b (as the second step in 3b is a query, \ie, an automatic operation over data that does not need a semantic check), which provide six respective Boolean-valued validity attributes. A requirement for such an attribute to be true is a constraint written as a ``stamp'' \stamp\ (red if it is given and blue if it is derived), and the respective claims are written in deep-red notes with white font. % (the colour is bolder to distinguish validity claims from (pink) claims  \corring\ to data constraints, and to emphasize the challenge of getting them satisfied). 
Claim derivation as such is shown with bold blue arrows:  
%(of lighter colour when they originate from a data constraint claim):
the common target claim  of a set of co-targeted blue arrows \frar{a_i}{\mathrm{C_i}}{\mathrm{C}}, $i=1...n$, means that C is derived from conjunction of C$_i$ %1,..,C_n$ 
and we write C \implBy C1\&.. \& Cn. 

When we need to distinguish a constraint $C$ and its claim, we will write the latter in the roman font as C. 




Now we are ready to reconstruct the style of the argument flow in the Example (but, unfortunately, not literally due to some logical discrepancies we have found in the Example, and our formal derivation procedure does not allow us to reproduce them). The top inference step is well-known in the SC literature \cite{}[J.Rushby]: C0\implBy C1 \& C2. %
%\footnote{There is no}
 Claim C1 is given, it remains to derive C2. This latter claim can be represented as a conjunction
 $ \claf{C2}   = \cmul{C2}{\hPro} \wedge \cval{C2}{\hPro}$
whose first component is \multy\ constraint [1] on the lower end of \asson\ \hPrtn: this is the data constraint part of C2,  and \cval{C2}{\hPr} is semantic validity check of \hPrtn\ \asson: the semantic part of claim C2. Identifying the data component part of a claim is 
 a principle step: we leave the land of propositional logic of claims and enter the land of first-order logic (FOL) over data, in which data drive the logical inference. Indeed, \asson\ \hPr\ can be represented as the sequential composition of \asson\ \Contt\ and \grProtn\ (further abbreviated as \ctt\ and \gPr) from Hazard to HazardGroup to ProtectionSystem. Hence, mutiplicity [1] of \hPr\ is a direct consequence of \multi s [1] on the lower ends of component associations \ctt\ and \gPr, \ie, $\cmul{C2}{\hPr}\implBy \cmul{A}{\ctt}\wedge\cmul{P}{\gpr}$ (see \figinf\ for claims A and P) 
 %
  Similarly, for semantic checks 
 $\cval{C2}{\hPr}\implBy \cval{A}{\ctt}\wedge\cval{P}{\gpr}$. Thus, 
 deriving C2 splits into two branches: the upper one deals with apportionment (hazard grouping) and we will refer to its constraints and claims by A with indexes, and the lower one deals with hazard group protection and we will refer to its constraints/claims by P with indexes. 
 
 Now we have pratically formal inference procedure:   









%\input{sections/inference}
\input{sections/anti-gsn-new}

==> sections/gsn2wf.tex <==
% note \endinout on l.152

% to ease ref to figs
\renewcommand\figri{\figref{fig:gsnEx-main}}
\renewcommand\figrii{\figref{fig:recoverSem}}
%\renewcommand\figriii{\figref{fig:wfMetamod-flow}}
%\renewcommand\figriv{\figref{fig:wfExample-dataFlow}}

\section{From GSN to Workflow+}\label{sec:wfba}
\input{figures/gsnEx-main}


Figure~\ref{fig:gsnEx-main} shows a GSN goal structure taken from the GSN Community Standard \cite{gsn11}. We interpret the diagram as a sketch of a safety case, and will extract its semantic meaning and rebuild it in WF+ terms as schematically shown in \figrii. 

We will first recover semantics (wavy mapping in \figrii) in \secref{recoverSem}. We then reformulate this semantics in terms of workflow+  as illustrated by the upward vertical arrow in \figrii (\sectref{GSNWF+}). The latter semantics can accurately be specified as a conformance of WFs as shown by the horizontal right arrows in the schema. This is the content of five subsections \secref{GSNWF+}-\sectref{aspects}. Note that in \sectref{conformToNorm} we consider an important component of assurance which is mainly omitted in a majority of GSN cases we are aware of, namely, conformance of the SEP definition to some normative workflow. %  \sectref{sec:GSNWF+}.  
Finally, in \sectref{anti-gsn} we will compare the two specifications focusing on how information is represented and arguments are formed.
Throughout this section, elements of \figref{fig:gsnEx-main} will be referenced by their title in italicized text, for example \gone.
\input{figures/recoverSem}

\shortlong
{%short
\subsection{Recover Semantics}
\label{sec:recoverSem}
\input{figures/GSNannotated}
Figure~\ref{fig:GSNAnnotated} presents an annotated version of \figref{fig:gsnEx-main}. In this diagram we show the implicit structure in \figref{fig:gsnEx-main}, namely process flow(green for generic processes, purple for reviews) and dataflow(orange). Constraints(red), inference(blue) and data from standards(grey) are explicitely stated in the safety case and are annotated to show their relationship with the case's implicit structure. 

 Beginning with process and data flow, we see that an instance of a control system's definition and its operating role and context are input to a hazard analyisis(FHA) to generate a list of hazards. These hazards are subjected to SIL assessment and grouped by SIL apportionment(SA). These hazard groups are then allocated to protection systems responsible for mitigating them, which will be developed to the SIL appropriate to the group covered(PSD). 
 
 Both Protection systems mitigate hazards, so they are assessed to determine the probability of their mitigated hazards occuring(FTA). Once these probabilities are determined, hazards are checked by a simple process to determine if they are is indeed mitigated given based on their SIL and tolerability targets, which outputs mit(H)=True. Note that mit(H2) and mit(H3) are not attached to \gfi\ or \gsi\ respectively as the notion that a probability being lower than some tolerance constitutes mitigation is not mentioned in \gfi\ or \gsi.  The primary protection system is subjected to formal verification(FV) to determine that H1 has indeed been eliminated, which outputs that the claim \gfo\ is true.
 
 For some claims, truth is determined by reviewing. \snth\ and \snfo\ produce evidence supporting \gse\ and \gei\ respectively by reviewing the execution of PSD(R'') in the context of its inputs and outputs(\sectref{aspects} discusses how reviews can be included). These reviews output the truth of their respective claims. \jone\ mentions the correctness of SA, which we interpret to mean that SA must be subjected to reviewing to determine its correctness(R'). Similarly, \aone\ requires that the process FHA must the correctness and completeness of its execution reviewed to provide confidence in the completeness of the hazard list produced(R). Note that in this example, \aone\ isn't required to support the claim \gtw; having all hazards identified does not contribute to showing that all identified hazards are mitigated. This logical discrepancy is likely due to the fact that \figref{fig:gsnEx-main} is just an example to illustrate GSN constructs, but it is bad practice to illustrate a concept with a flawed example, just as one should not illustrate the concept of addition with the example 1+1=3.
 
 Now considering blue inferences, the truth \gfo, \gfi, \gsi\ and \aone\ are used to infer the truth of \gtw. Similarly, the truth of \jone, \gse\ and \gei\ are used infer the truth of \gth. Finally, the truth of \gtw\ and \gth\ are used to infer that the control system is safe. 
 
\csi\ is ignored as the lack of information about its use would unnecessarily complicate the story and require far too much speculation to be beneficial. 
}
{%long
\subsection{Recover Semantics, 1
	%Our Interpretation of the GSN Standard Example
}\label{sec:recoverSem-1}
As with all GSN safety cases, the story begins at the top. \zdmoddok{\gone}{The top goal \gone}{}{-1em} is a claim that the control system of interest is safe, given with \zdmoddok{\cone\ and \ctw}{contexts \cone\ and \ctw,}{}{-1em} which explain its operating purpose/environment and its functional architecture respectively. To show that the control system is safe, it is required to show that all hazards are appropriately mitigated/eliminated (\gtw) and that the level of rigour in the development process is appropriate to the hazards involved (\gth). Context \cfo\ is given for both \gtw\ and \gth: the hazards of the control system are identified by some functional hazard analysis FHA.

Goal/claim \gth\ is also given SIL guidelines(\cfi) as its context, which presumably includes information on how to assess the \namodok{SIL of hazards from SIL 1 to SIL 4, with SIL 4 being the most severe}{safety integrity level (SIL) of hazards, which we assume to be from SIL 1 to SIL 4, with SIL 4 being the most severe,}{} and how to develop systems of different SILs. We interpret  justification \jone\ and strategy \stw\ to mean that hazards have their SIL assessed and are grouped together. Each of these groups are allocated to a protection system intended to mitigate all hazards in that group. Each of these protection systems will then be developed to the highest SIL of all hazards in the group allocated to it(\gse, \gei). Then, for each protection system, artifacts from the software development process, \snth\ and \snfo, are provided as evidence that protection systems were properly developed. \zdnewwok{GSN calls such artifacts {\em solutions} (hence the abbreviation {\em Sn})}{}{-2em}.  \csi\ is ignored as the lack of information about its use would unnecessarily complicate the story to little benefit. 

Strategy \stw\ tells us that to demonstrate \gtw, it is shown that for each hazard(\gone, \gtw, \gth), the probability of occurrence is less than the tolarability target (given by \cth) corresponding to its SIL. From the handling of H1, H2 and H3(see \gfo, \gfi\ and \gsi\ respectively), we assume that H1 is SIL 4 and is to be eliminated, H2 is SIL 3 and has a target probability of $10^{-6}$, and H3 is SIL 2 and has a target probability of $10^{-3}$. Although SIL 1 doesn't appear in the safety case, for the sake of completeness we assume SIL 1 has a target probability of $10^{-2}$. The assumption that all hazards have been identified does not contribute to showing that all identified hazards have been mitigated. The meaning of \aone\ will appear in the next section. 
%Could also say SIL 4 is 10^-9, but they chose to eliminate it instead. 

\subsection{Recover Semantics, 2} %: The Rest of the Iceberg}
\label{sec:recoverSem-2}
%\input{figures/GSNannotated}
 \figref{fig:GSNAnnotated} presents a version of the example from the GSN community standard annotated with a block diagram where blocks are overlapping with the element that gave rise to them. In this diagram, we graphically represent the multi-dimensional meaning of the safety case outlined in \sectref{sec:recoverSem-1}. Orange blocks represent data, where instance-level data is orange and meta-level data is grey. Green blocks represent processes, with directed arrows representing input/output data. Purple blocks represent review processes, see \sectref{sec:aspects} for more on how reviews are included. Red blocks represent constraints on processes and data, where the goal is to demonstrate that each claim is True(T). Blue blocks represents inferences used to form an argument, with input and output logical elements denoted by directed arrows. 

 Beginning with process and data flow, we see that instances of a control system definition and it's operating role and context are input to a hazard analyisis(FHA) to generate a list of hazards. These hazards are subjected to SIL assessment and grouped by SIL apportionment(SA). These hazard groups are then allocated to protection systems which will be developed to the SIL appropriate to the group covered(PSD). Both Protection systems mitigate hazards, so they are assessed to determine the probability of their mitigated hazards occuring(FTA). Once these probabilities are determined, they are checked by a simple process to determine if their hazard is indeed mitigated given its SIL and tolerability targets, which outputs mit(H)=True. Note that mit(H2) and mit(H3) are not attached to \gfi\ or \gsi\ respectively as the notion that a probability being lower than some tolerance constitutes mitigation is not mentioned in \gfi\ or \gsi.  The primary protection system is subjected to formal verification(FV) to determine that H1 has indeed been eliminated, which outputs that the claim \gfo\ is true.
 
For some claims, truth is determined by reviewing. \snth\ and \snfo\ produce evidence supporting \gse\ and \gei\ respectively by assessing the execution of PSD(R'') in the context of its inputs and outputs(\sectref{aspects} discusses how reviews can be included). These reviews output the truth of their respective claims. \jone\ mentions the correctness of SA, which we interpret to mean that SA must be subjected to reviewing to determine its correctness(R'). Similarly, \aone\ requires that the process FHA must the correctness and completeness of its execution reviewed to provide confidence in the completeness of the hazard list produced(R). Again, note that in this example, \aone\ isn't required to support the claim \gtw; having all hazards identified does not contribute to showing that all identified hazards are mitigated. This logical discrepancy is likely due to the fact that \figref{fig:gsnEx-main} is just an example to illustrate GSN constructs, but it is bad practice to illustrate a concept with a flawed example, just as one should not illustrate the concept of addition with the example 1+1=3.

Now considering blue inferences, the truth \gfo, \gfi, \gsi\ and \aone\ are used to infer the truth of \gtw. Similarly, the truth of \jone, \gse\ and \gei\ are used infer the truth of \gth. Finally, the truth of \gtw\ and \gth\ are used to infer that the control system is safe. 
}%endlong


\subsection{GSN Example Modeled as WF+}\label{sec:GSNWF+}
\input{figures/metamodel}
This section presents WF+ as an alternative way to represent the multi-dimensional information presented in \figref{fig:GSNAnnotated}. Our WF+ representation of the GSN example comes as a package of five diagrams - a WF+ metamodel(\figref{fig:metamodel}, referred to as SEP for processes and dataflow, a WF+ metamodel with data, inferences over constraints and reviews(\figref{fig:inference}), an instance of the WF+ metamodel(\figref{fig:instance}), a WF+ metamodel of a normative document(\figref{fig:normative}) and a model of reviewing(\figref{fig:aspectR} see \sectref{aspects}). Figure~\ref{fig:metamodel} and \figref{fig:inference} are two views of the same model, but are separated to ease reading. Black boxes with white text are used to indicate the correspondence with elements of \figref{fig:GSNAnnotated}.

\subsubsection{WF+ Syntax}
\shortlong{%SHORT
There are three main components to WF+ models presented: process classes, data classes, and constraints. Green processes are classes whose instances are executions of a process, which takes input data to produce output data, denoted by directed arrows to and from the process respectively. The order of execution of processes is denoted by numbering in their titles. WF+ allows processes to produce new data, associations between input data, associations between input and output data, new attributs for data, or any combination thereof. Green frames denote different stages of the SEP. As a whole, these processes form the SEP to be followed during the development of a safety-critical system. 
}
{%LONG
There are three main components to WF+ models presented: process classes, data classes, and constraints. Processes, stereotyped <<Process>>, are classes whose instances are executions of a process, which takes input data to produce output data, denoted by directed arrows to and from the process respectively. The order of execution of processes is denoted by numbering in their titles. WF+ allows processes to produce new data, associations between input data, associations between input and output data, new attributs for data, or any combination thereof. If associations are output by a process, they are refied as an association class and an output arrow is directed there. If an attribute of data is output, an arrow is directed to the new data created, which will be an attribute of input data.

Green frames denote that the process in its top left corner was decomposed into the processes contained by the frame. That is, the process in the top left corner of a frame is a black-box representation of a process, which can be implemented by the internal processes within the frame. As a whole, these processes form the SEP to be followed during the development of a safety-critical system. In their current simplified form, these processes would not be very instructive to an engineer attempting to execute the process. Through enrichment and decomposition of the model, these processes can become as well-defined(or undefined) as is desired. This flexibility can be useful to engineers designing these processes for several reasons: it allows safety-critcal components of processes to be as prescriptive as possible, it allows creative processes to be left as "free" as is acceptable, and enables a "graceful" transition for organizations adopting this technology who are unable to convert their entire practice to this style in one fell swoop. 
}%ENDLONG

\shortlong
{%SHORT
Data classes represent data produced and/or used by processes during the execution of a SEP. Orange data indicates that it is given as input to the SEP. Any associations between non-process classes are standard UML associations(directed arrows are reserved to annotate process flow). Boundary objects(circle with a vertical line attached) are used as aliases for data to reduce the number of crossing lines in the model. 
}
{%LONG
Data classes represent data produced and/or used by processes during the execution of a SEP. Orange data indicates that it is given as input, not produced by any modelled process, and yellow data indicates that it is produced by a modelled process. Any associations between non-process classes are standard UML associations(directed arrows are reserved to annotate process flow). Occasionally, boundary objects(circle with a vertical line attached) are used as aliases for classes with the same name to reduce the number of crossing lines in the model. 
}%ENDLONG

Constraints are used to restrict the structure of instantiations of the SEP. Multiplicities typical of UML are used to specify how many data classes are related to each other, and how many instances of data are input/output to/from processes. OCL-style constraints are used between classes and associations, which can be complex and will be explained on a case-by-case basis.

\subsubsection{WF+ 1 - Metamodel}

\figref{fig:metamodel} shows a WF+ representation of the green and orange elements from \figref{fig:GSNAnnotated}. Bold red lines are used as constraints, where black, grey and blue lines are used for dataflow and associations. Black and grey lines are used solely to ease reading of crossing lines.  
\shortlong{%SHORT
\paragraph{HARA}
The topmost green frame, HARA, contains three processes: \fha, \dersil and \silapp. Just as in the GSN example, \fha uses the control system of interest(more accurately its functional architecture) and operating role and context to identify hazards. We have introduced four attributes for \hazard\, including whether it should be mitigated or eliminated, that are common artifacts of hazard analyses.
Following this, each \hazard\ is assessed as per the \silguide\ by \dersil\ to identify its \sil. Notice that through multiplicity constraints, there will be one execution of \dersil\ for each hazard, and one \sil\ output. Then, every hazard(notice that \sil\ is included by virtue of being an attribute) is input to \silapp\ to produce \hazgr s and a \containment\ association to show which hazards belong to which group. \hazgr\ has a method $\backslash$\sil\ that calculates the \sil\ of the group, which is the highest \sil\ of all \hazard s in the group.
}
{%LONG
\paragraph{HARA}

The first step in the GSN example can be interpreted as performing a hazard analysis and risk assessment(HARA). The topmost green frame, HARA, contains three processes: \fha, \dersil and \silapp. Just as in the GSN example, \fha uses the control system of interest(more accurately its functional architecture) and operating role and context to identify hazards. We have introduced four attributes for \hazard\ that are common artifacts of hazard analyses and are helpful for assessing a \hazard s \sil. \hazdesc\ is a description of \hazard\ and its consequences, \severity\ is a description of how severe the consequences of \hazard\ are, \likelihood\ is how often the hazard would occur if \cs\ was left as is, and \mitorelim\ dictates whether \hazard\ should be mitigated or eliminated as determined by \fha. 
Following this, each \hazard\ is assessed as per the \silguide\ by \dersil\ to identify its \sil, which is output as an attribute of  \hazard. Notice that through multiplicity constraints, there will be exactly one execution of \dersil\ for each hazard, and exactly one \sil\ output. Then, every hazard(notice the multiplicity constraint \namefont{all} and that \sil\ is included by virtue of being an attribute) is input to \silapp\ to produce \hazgr s and a \containment\ association to show which hazards belong to which group. Notice that the multiplicities on \containment\ limit hazards to being part of exactly one \hazgr. \hazgr\ has a method $\backslash$\sil\ that calculates the \sil\ of the group, which is the highest \sil\ of all \hazard s in the group.
}%ENDLONG

\shortlong{%SHORT
\paragraph{Design}
Once \hazard s are grouped, the next step is to develop a \protsys\ for each \hazgr\ to mitigate or eliminate every \hazard\ in it. This is done through \devprotsys, which is executed once for each \hazgr\ while following \silproc\ to produce a \protsys\ for the \hazgr\ input and a traceability association \grprot\ to the group it is protecting. Through \grprot\ and \containment,  \elim\ and \mitig\ are derived, indicating which hazards are eliminated or mitigated by which systems. The multiplicity constraint $1$ between \elim\ and \mitig\ means that each hazard is either mitigated or eliminated by one \protsys.
}
{%LONG
\paragraph{Design}
Once \hazard s are grouped, the next step is to develop a \protsys\ for each \hazgr\ to mitigate or eliminate every \hazard\ in it. This is done through \devprotsys, which is executed once for each \hazgr\ while following \silproc\ to produce a \protsys\ for the \hazgr\ input and a traceability association \grprot\ to the group it is protecting. Now, through \grprot\ and \containment, associations \elim\ and \mitig\ can be automatically derived, indicating which hazards are eliminated or mitigated by which systems. The multiplicity constraint $1$ between \elim\ and \mitig\ means that each hazard is either mitigated or eliminated by one \protsys.
}%ENDLONG

\shortlong{%SHORT
\paragraph{Verification}
Finally, the SEP verifies that each \hazard\ is eliminated or sufficiently mitigated. The constraint \namefont{XOR} between inputs to \formverif\ and \fta\ means that each hazard is verified by exactly one method; \hazard s to be eliminated must undergo formal verification(\sse in the model) and those to be mitigated must be assessed using fault tree anaylsis. For each \hazard\, \namefont{self.\mitorelim} can be used to determine which verification process should be used, and the \protsys\ to be used can be found through \namefont{self.\mitig} or \namefont{self.\elim}(only one can exist in an instance).

If \sse\ deems that the hazard has indeed been eliminated, it outputs the attribute \valid\ of the \elim\ association with \Value =$True$. If the \hazard\ is not eliminated, the same attribute is crated but with \Value=$False$.
	
\fta\ outputs the actual probability, \realprob\, of the \hazard occuring with the \protsys\ in place. \vermit\ then compares \realprob\ to the target probability from \tolgui\ to check that for \hazard 's \sil, the probability of \hazard occuring is indeed low enough. If it is low enough, it outputs the attribute \valid\ of the \mitig\ association with \Value =$True$. If the \hazard\ is not mitigated, the same attribute is crated but with \Value=$False$.
}
{%LONG
\paragraph{Verification}
Finally, the SEP verifies that each \hazard\ is eliminated or adequately mitigated. The constraint \namefont{XOR} between inputs to \formverif\ and \fta\ means that each hazard is verified by exactly one method.

For each \hazard\ to be eliminated, that is, each \hazard\ with \namefont{self.\mitorelim=elim}, the \protsys\ covering that \hazard\ undergoes formal verification through an execution of \sse(The correct \protsys can be systematically found through the link \hazard.\elim). If \sse\ deems that the hazard has indeed been eliminated by the \protsys, it outputs the attribute \valid\ of the \elim\ association between the input \hazard\ and its \protsys\ with \Value =$True$. If the \hazard\ is not eliminated, the same attribute is crated but with \Value=$False$.

Similarly, for every \hazard\ with \namefont{self.\mitorelim=mit}, the corresponding \protsys\ is subjected to a fault tree analysis through execution of \fta. \fta\ outputs the actual probability, \realprob\, of the \hazard occuring with the \protsys\ in place. \vermit\ then compares \realprob\ to the target probability from \tolgui\ to check that for \hazard 's \sil, the probability of \hazard occuring is indeed low enough. If it is low enough, it outputs the attribute \valid\ of the \mitig\ association between the input \hazard\ and its \protsys\ with \Value =$True$. If the \hazard\ is not mitigated, the same attribute is crated but with \Value=$False$.
}%ENDLONG
\shortlong{%SHORT
\subsection{Inference Over Data}
\input{figures/inference}
WF+ allows for inferences to be made over constraints on meta-level data, illustrated in \figref{fig:inference}. Light pink constraints are "normal" constraints, dark pink constraints are constraints on values, and blue constraints are derived.

Something about completeness constraints being special

Inferences are made from the bottom up, where two or more constraints are used to infer a derived constraint. For example, consider the derived constraint that all hazards are grouped appropriately(C1). C1 depends on two conditions: each hazard must be contained by a group(apportionment complete) and that each containment is correct.  If these two constraints are satisfied, then we can infer that all hazards are indeed grouped appropriately. 
}
{%LONG
\subsection{Inference Over Data}
\input{figures/inference}
WF+ allows for inferences to be made over constraints on meta-level data, illustrated in \figref{fig:inference}. Light pink constraints are "normal" constraints, dark pink constraints are constraints on values, and blue constraints are derived from multiplicity and value constraints. Black rectangles with white text map elements of \figref{fig:instance} to \figref{fig:gsnEx-main}. For the time being, we will ignore the role played by reviews as they will be explained in \sect{?}.

Inferences are made from the bottom up, where two or more constraints are determined to imply a derive constraint. Consider the derived constraint that all hazards are grouped appropriately(C1). C1 depends on two conditions: each hazard must be contained by a group(apportionment complete) and that each containment is correct.  If these two constraints are satisfied, then we can conclude that all hazards are indeed grouped appropriately. Similarly, C2 depends on two conditions: Each hazard group must be protected by a system, and the system must be appropriate for protecting that group. If these two conditions are satisfied, we can infer that all hazard groups are assigned to the appropriate protection system. From both C1 and C2, we can infer that all hazards are assigned to the appropriate protection system(C5).

C3 depends on two conditions: that the mitigation(or elimination) of each hazard by the assigned protection system is verified. If these two conditions are satisfied, we can infer that all protection systems verifiably mitigate(or eliminate) all hazards they are intended to mitigate(or eliminate). 

C4 depends on two conditions: The SIL each protection system is developed to must be appropriate given the hazard group it protects, and the development of each must indeed follow the guidelines for its SIL. From this, we can infer that each protection system was developed to the appropriate SIL. 

Given C3, C4 ad C5, we can infer that all identified are effectively eliminated or mitigated(C6). Finally, if all hazards are effectively eliminated or mitigated(C6) and all hazards are identified, we infer the top constraint that the control system is indeed safe.

In this setting, arguments, their origin and their relationships are presented unambiguously with no flexibility in how they are structured. Making inferences about systems in this way is not an attempt to allow one to formally prove the safety of a system. It is certainly possible, if not probable, that an expert would disagree with the inferences made in \figref{fig:instance}. In fact, this is exactly the point; presenting inferences with access to all relevant data, associations, and processes used allows these inferences to be analyzed critically. 
}%ENDLONG

\shortlong{%SHORT
	
	\endinput
\subsection{ An instance and Conformance to MM}
\label{sec:instance}
\input{figures/instance}
The instance in \figref{fig:instance} is the result executing the process in \figref{fig:metamodel} . We ommit dataflow links from all processes but two to avoid clutter but still demonstrate dataflow in the instance. Here, we see product-level details appear. Detailed information ommitted in \figref{fig:gsnEx-main} was "made up" for the sake of the example(such as \textit{Prob1: \realprob)}. 

Once an instance is complete, or at any desired point along the way, tools can be used to automatically verifiy syntactic contraints. An example of this is shown by horizontal red lines attached to the associations being verified. 

If all syntactic contraints are satisfied, we can conclude that condition b in DEFENITION 1 REF is satisfied. It may seem strange to say that the satisfaction of syntactic constraints can be used to conclude that the SEP was well executed, but as the metamodel encodes all semantics syntactically(eg. the validity of data through reviewing), confidence in the instance is reduced to a simple conformance check. There is no magic; everything important to safe development must be done, but checking that it is done is reduced to the well-known concept of conformance.

\nanew{More on constraints, conformance from zinovy probably}{}
}
{%LONG
\subsection{ An instance and Conformance to MM}
\label{sec:instance}
\input{figures/instance}
The instance in \figref{fig:instance} is the result executing the process in \figref{fig:metamodel} . We ommit dataflow links from all processes but two to avoid clutter but still demonstrate dataflow in the instance. Here, we see product-level details appear. Detailed information hidden within solutions in \figref{fig:gsnEx-main} was "made up" for the sake of the example(such as \textit{Prob1: \realprob)}. 


In the instance, \hazard s \textit{H1} and \textit{H2} were grouped together. From \figref{fig:gsnEx-main}, \textit{H1} and \textit{H2} are assumed to be the most severe, because their probability of occurance is made the lowest. Then, because in \figref{fig:gsnEx-main} there are three hazards and only two protection systems, it makes the most sense to assume the most severe hazards are addressed by the primary protection system. \nahll{The remainder of the instance is self-explanatory as it follows the logic of its WF+ metamodel directly.}{maybe a bit bold}{-3em}

Figure~\ref{fig:instance} is a view of the completed instance. In reality, it would be completed incrementally as engineers work their way through the process. Tooling designed for WF+ would allow for automated in-process syntactic checks to be implemented with the purpose of informing engineers that something went wrong or was missed while they are working. Two examples of constraint satisfaction verification are shown by horizontal red lines attached to the associations being verified. The topmost verification checks that all \containment s are syntactically correct. That is, that each \hazard\ is in one \hazgr\ and no \hazgr s are empty. Similarly, the lower verification checks \elim\ and \mitig\ associations to ensure all hazards are either eliminated or mitigated, but not both. 

\nahl{Instance inheriting derived constraints on MM}{For zinovy.}
}%ENDLONG


%\subsection{ASpects}\label{sec:aspects}
\input{sections/conformToNorm}
\input{sections/aspectR}

%\input{sections/anti-gsn}


\endinput

%We agreed this is not needed.
%(A more complex version is on \figref{fig:gsn2wf2gsn} but I am not sure it's needed)

==> sections/inference.tex <==
\subsection{From GSN to \wfc, 3: Inference Over Data}
\input{figures/inference}
WF+ allows for inferences to be made over constraints on meta-level data, illustrated in \figref{fig:inference}. Light pink constraints are "normal" constraints, dark pink constraints are constraints on values, and blue constraints are derived.

Something about completeness constraints being special

Inferences are made from the bottom up, where two or more constraints are used to infer a derived constraint. For example, consider the derived constraint that all hazards are grouped appropriately(C1). C1 depends on two conditions: each hazard must be contained by a group(apportionment complete) and that each containment is correct.  If these two constraints are satisfied, then we can infer that all hazards are indeed grouped appropriately. 


==> sections/info4relWork.tex <==
\section{Info for Related and future work}

\subsection{\href{https://www.researchgate.net/publication/284791681_Extracting_Models_from_ISO_26262_for_Reusable_Safety_Assurance}{Extracting Models from ISO 26262 for Reusable Safety Assurance}}
\begin{itemize}
	\item Says "Adherence to such standards is the basis for safety assurance and certification" with reference to 
	\item Discusses reuse of assurance artifacts, perhaps like the template idea?
	\item Interesting point: "In addition, the assurance artifacts themselves become more reliable with repeated reuse". 
	\item A conceptual model for the aeronautic standard DO 178B [2] is provided in \href{https://link.springer.com/article/10.1007/s10270-010-0164-x}{link} to improve communication and collaboration among safety engineers and software engineers.
	\item They also model the concept phase(HARA) - Might be useful to compare the methods and outcomes in my thesis
	\item Reference an Ontology-editor OWLGrEd - could be better than astah? worth looking into 
	\item They descibe a "snow ball approach", which seems to be about having refinements from general to more specific, growing like a snow ball. 
	\item In general their models are quite poor and do not reveal much of the underlying meaning of the standard or its datastructures/process flow. In a way their approach is naive in the sense that they assume away problems by considering certain concepts to be synonymous when they are clearly not.
\end{itemize}
\subsection{\href{http://www-users.cs.york.ac.uk/~ihabli/Papers/2012Sassur.pdf}{Towards a Case Based Reasoning approach for safety assurance  reuse}}
\begin{itemize}
	\item Proposes to identify patterns in cases(things whose safety needs to be argued) and to reuse the best practices accepted by experts in the past and then reuse the argument.
	\item uses GSN
\end{itemize}

\subsection{GSN}
\subsubsection{\href{http://www.goalstructuringnotation.info/wp-content/uploads/2013/02/YorkAssuranceCaseForum.pdf}{Tom's presentation}}

\subsubsection{\href{https://www.researchgate.net/publication/221541337_Software_Certification_Is_There_a_Case_against_Safety_Cases}{Case against safety cases}}

\subsubsection{\href{http://homepages.laas.fr/guiochet/telecharge/ERTS2012DOHOANG.pdf}{Human-robot interactions: model-based risk analysis and safety case construction}}
\begin{itemize}
	\item SUMMARY OF I (INTRO)
	\begin{itemize}
		\item Traditional methods of hazard analysis are difficult to apply to applications with constant human interaction, due to lack of data regarding frequency of failure of human interaction or certain types of system failures. They propose model-based analysis of interactions between humans and the system to properly identify hazards. Following this, they construct a GSN safety case providing a "structured and solid argument" arguing the mitigation of identified hazards. 
	\end{itemize}
	\item SUMMARY OF II(MODEL-BASED SAFETY ANALYSIS PROCESS)
	\begin{itemize}
		\item A combination of UML and HAZOP is used for model-based risk analysis. 
		\item with cutting-edge technology, information on failure rates is often missing. because of this they use argumentation supported by evidence(i.e. GSN) to justify that the risk is acceptable. 
	\end{itemize}
	\item SUMMARY OF III(RISK ANALYSIS WITH HAZOP-UML)
	\begin{itemize}
		\item  Systems are modelled with use case, sequence and statechart diagrams. In the authors experience these are most suitable for describing human-machine interaction(STPA??). It seems they use Use Case+Sequence to describe what happens between the user and system, then use a statechart to help identify the behaviour of the robot in the use cases which supposedly helps identify hazards from unwanted behaviour. 
		\item There are no system elements or parameters in the diagrams, they are purely functional. The guidewords are modified to fit behavioural UML diagrams. Then HAZOP proceeds as normal.
		\item 4670 deviations were found in their system, leading to 16 "main"(hazard grouping?) hazards and 57 safety recommendations. This large number of deviations was made possible through automation of their systematic approach. 
	\end{itemize}
	\item SUMMARY OF IV(Safety Case Construction)
	\begin{itemize}
		\item Says G2 is based on qualitative criteria because quantitative criteria is difficult to demonstrate. Looks quantitative to me?
		\item Their approach takes sw, hw, mechanical design and user into account. 
		\item The Goal is to show the system is safe by showing it is safer than it's socially-accepted alternative, a classical non-robotic walker. This is done by partitioning their identified risks(from earlier) as either new or also present in the classical design. It is not clear how this partitioning was done. 
		\item There is also mention of the standards met by the robot. These may be required by law or meant to improve confidence in safety.They do mention that compliance with standards is part of their safety case, implying that it does something to improve confidence in safety.
		\item The standard they reference puts forward requirements but no means to achieve them. This may always be the case for the standard or may be because they're dealing with a new type of system outside the standard's scope. Because of this they mapped severity levels to those of another standard, presumably to follow the guidance of the other standard but not sure.
		\item an excerpt of the safety case arguing the mitigation of a hazard  was provided. Acceptability criterion was obtained through discussion with medical experts. Markov models were used to show the acceptability criterion were met. They use P of hazard,  and compensation rate? to calculate acceptable failure rates and coverage of mitigation. They then argue there are no design faults by virtue of their rigorous development, the failure rate is low enough by evaluation(FTA,etc.), and the coverage of mitigation by testing. 
	\end{itemize}
	
	\item Fig 10 includes a snippit of the GSN case we used from the standard. It provides an instantiation of something similar.
\end{itemize}
\endinput


==> sections/instConform.tex <==
\subsection{ An instance and Conformance to MM}
\label{sec:instance}

\input{figures/instance}
The instance in \figref{fig:instance} is the result executing the process in \figref{fig:metamodel} . We omit dataflow links from all processes but two to avoid clutter but still demonstrate dataflow in the instance. Here, we see product-level details appear. Detailed information ommitted in \figref{fig:gsnEx-main} was "made up" for the sake of the example(such as \textit{Prob1: \realprob)}. 

Once an instance is complete, or at any desired point along the way, tools can be used to automatically verifiy syntactic contraints. An example of this is shown by horizontal red lines attached to the associations being verified. 

If all syntactic contraints are satisfied, we can conclude that condition b in DEFENITION 1 REF is satisfied. It may seem strange to say that the satisfaction of syntactic constraints can be used to conclude that the SEP was well executed, but as the metamodel encodes all semantics syntactically(eg. the validity of data through reviewing), confidence in the instance is reduced to a simple conformance check. There is no magic; everything important to safe development must be done, but checking that it is done is reduced to the well-known concept of conformance.

\nanew{More on constraints, conformance from zinovy probably}{}


==> sections/intro-tr-zd.tex <==
\section{Introduction: Consistency and traceability in safety assurance}

We will begin with a brief general overview of consistency management as a model management problem to set the stage (Section 1.1), and then consider its specific instantiation for safety cases (Sect. 1.2). 

\subsection{A primer on consistency management}
The presentation will be brief and thus rather formal, but many examples and details about consistency definition and checking can be found in \cite{me-staf16,me-staf16w,me-staf17,harald-progr18}, and about consistency restoration via change propagation in \cite{me-jot11,me-jss15,me-fase18,me-fase18tr}

Let $A_1,..., A_n$ be several interrelated artifacts (models, documents, datasets) to be kept in sync (we also say be {\em (mutually) consistent}) despite their independent changes. We assume that each of the artifacts $A_i$ is a valid instance of the \corring\ metamodel $M_i$, and we write $A_i\models M_i$. (In more detail, a metamodel $M_i$ consists of a graph $G_i$ of classes and associations, and a set of constraints $C_i$ over it so that $A_i\models M_i$ means that a) $A_i$ is properly typed over $G_i$ and b) all constraints $C_i$ are satisfied.) The challenge of consistency management is that although all artifacts $A_i$ can be perfectly valid locally, \ie, $A_i\models M_i$, taken together they may be inconsistent. A typical scenario begins with a consistent state $(A_1,..,A_n)$ of the artifacts involved (we will define this in a minute), then one of the artifacts changes to $A'_i$, which may violate consistency. The goal of consistency management is to change some or all other artifacts (including, perhaps, an amendment to $A'_i$) so that consistency between $A'_1,...,A'_n$ is restored. 

\newcommand\cmstage[1]{\par%\noindent 
	{\bf(#1)}~~~}
\newcommand\nig{\enma{\mathcal{G}}}
\newcommand\nigm{\enma{\nig_\nim}}
\renewcommand\nigm{\nim}

Consistency management consists of three major parts. 

The first is {\em consistency definition}. % (CDef)}. % which itself consists of two subparts.  

\cmstage{CDef}All traceability mappings/correspondences (or just {\em corrs}) $R_\nim$ between the metamodels are to be specified; we call the tuple $\nigm=(M_1,...,M_n, R_\nim)$  a {\em multi-metamodel} (or a {\em global} metamodel ), and sometime refer to {\em local} metamodels $M_i$ as to \nigm's {\em feet}.  Moreover, a %(CDef-2) 
set of {\em intermodel} constraints $C_\nim$ over $R_\nim$\ is to be defined so that their fulfillment by a multi-instance (see below) should ensure consistency. Thus, we redefine a {\em multi-metamodel} %({\em or a} global metamodel}) 
	to be a tuple $\nim=(M_1,...,M_n, R_\nim, C_\nim)$.

The second part of consistency management is {\em global instantiation}:

\cmstage{CInst} All traceability links/corrs $R_\nia$ between the artifacts are to be specified, and are assumed to be instantiating the metamodel corrs $R_\nim$. We call the tuple $\nia=(A_1,...,A_n, R_\nia)$ a {\em multi-artifact} or a {\em multi-instance}, and we say it is {\em consistent} if all intermodel constraints are satisfied, \ie, $\nia\models\nim$. 

Examples and details can be found in \cite{me-staf16,me-staf16w,me-staf17,harald-progr18} 

Finally, the third part of consistency management is {\em consistency restoration}, which is typically realized via {\em change propagation}.

\cmstage{CPpg} If an artifact $A_i$ changes to $A'_i$ and the global consistency is violated, \ie, $(A_1,..,A'_i, .., A_n, R_\nia)\nvDash \nim$, other artifacts are to be changed accordingly to restore consistency, \ie, $\nia'=(A'_1,...,A'_n, R'_\nia)\models \nim$ (note that the traceability links are also updated).  The case when the ``trouble-making'' artifact $A'_i$ is amended to $A''_i$ and thus $\nia'=(A'_1,..,A''_i,..,A'_n, R'_\nia)\models\nim$, is not excluded --- see \cite{me-fase18,me-fase18tr} for details.  

\subsection{Consistency management for safety cases}
\renewcommand\sc{\nmf{SC}}

\subsubsection{Safety case definition.}
<<<<<<< HEAD
The \fwk\ above shows that doing consistency management in a precise and automatable way needs precise definitions %/metamodels $M_i$ 
of all artifacts involved. The first of these artifacts is a metamodel $M_\sc$ for safety cases. In this regard, using a standard metamodel for GSN diagrams, \ie, %identifying safety cases with GSN diagram, would not work 
using GSN to describe a safety case, will not suffice since the GSN metamodel does not capture the semantics of its elements nor is it detailed enough to allow consistency management based on traceability and the consistency definition (indeed, traceability and constraints are missing from GSN). So, the first goal of deliverable D7 is to define a safety case metamodel. More accurately, we show how we can use a description of a safety engineering process (SEP) to define a safety case metamodel $M_\sc$, a safety case $A_\sc$ and check their consistency $A_\sc\models M_\sc$.  

As a SEP is a workflow, we prefer more suggestive names and notation for our (meta)artifacts: the SEP metamodel is called the SEP workflow definition and denoted by \wfsepdef, \corring ly, its instance is a SEP workflow execution and is denoted by \wfsepexex, where $X$ is the system for which SEP was executed. In this report we show how to build \wfsepdef\ and \wfsepexex\ with a simple example borrowed from the GSN community standard; in the deliverable D3b report %\cite{d3btr}, 
we showed how the same procedure can be applied for GM's SEP. 
=======
The \fwk\ above shows that doing consistency management in a precise and automatable way needs precise definitions/metamodels $M_i$ of all artifacts involved, first of all, a metamodel $M_\sc$ for safety cases. Clearly, using a standard metamodel for GSN diagrams, \ie, identifying safety cases with GSN diagram, would not work as the GSN metamodel does not capture the semantics of its elements nor is detailed enough to allow consistency management based on traceability and consistency definition (indeed, traceability and constraints are missing from GSN). So, the first goal of deliverable D7 is to define a safety case metamodel. More accurately, we will show how having a description of a safety engineering process (SEP), we can define a safety case metamodel $M_\sc$ and a safety case conforming to it, $A_\sc\models M_\sc$.  

As a SEP is a workflow, we prefer more suggestive names and notation for our (meta)artifacts: the SEP metamodel is called the SEP workflow definition and denoted by \wfsepdef, \corring ly, its instance is a SEP workflow execution and is denoted by \wfsepexex, where $X$ is the system for which SEP was executed. In the TR, we show how to build \wfsepdef\ and \wfsepexex\ with a simple example borrowed from the GSN community standard; in the deliverable D3b report \cite[Sect.4-5]{me-d3bTR}, we showed how the same procedure can be applied to GM's SEP. 
>>>>>>> fixed tites. Minor edits here and there.

The workflows used above are actually instances of a special workflow type called \wfp, in which data produced by a process are related to its input data. We need to bear in mind that that we have traceability within a model (intra-model traceability) and %To distinguish these (intra-model) traceability links from the 
traceability between models (inter-model traceability) $R_\nim$, $R_\nia$, as discussed in Sect. 1.1. %, we refer to the former as {\em vertical} and to the latter as {\em horizontal}.  
We will use the name \wfp\ to refer to the entire approach, in which a safety case is an instance \wfsepexex.  

Now several important remarks are in order.
\begin{remark}[On the notion of an instance] Our notion of a valid instance {\em includes} a verification that the instance satisfies the metamodel. For example, a safety case instance is a pair $(\wfsepexex, \pi)$ with $\pi$  a proof (verification procedure) showing that $\wfsepexex\models\wfsepdef$. To simplify notation, we will always assume the presence of such $\pi$ by default and refer to the pair by its first component. Thus, a safety case is an instance \wfsepexex\ of the SEP definition \wfsepdef. 
\end{remark}
\begin{remark}[On semantic validity of an instance]
	Semantic validity checks (fundamental for safey assurance) are included into the SEP definition (to wit: each SEP subprocess has a review process assigned to it) so that a valid instance of \wfsepdef\ includes reviewing and thus ensures both syntactic verification and semantic validation are done. 
\end{remark}
\begin{remark}[Consistency and traceability for safety cases]
  %\subsubsection{}
<<<<<<< HEAD
A special feature of the \wfp-approach is that in terms of Sect. 1.1, the SEP definition \wfsepdef\ is a multi-metamodel \nim\ rather than a local metamodel $M_i$ with all inter-model traceability mapping and constraints included through the SEP's intra-model traceability and constraints. In this report, we will see how the functional design data (dark-orange), the normative data (grey) and the safety engineering data (yellow), together with constraints defined over them, are seamlessly integrated into one artifact --- the SEP definition metamodel. Correspondingly, a safety case \wfsepexex\ is a multi-artifact \nia\ rather than a local artifact $A_i$, and checking its conformance $\wfsepexex\models\wfsepdef$ can be seen as consistency checking $\nia\models\nim$ considered in Sect. 1.1.  In this way, the \wfp-assurance reduces inter-model traceability and consistency management to a standard check of a (complex but still singular rather than  multi-) instanceOf-relationship.  Not much is gained technically w.r.t. tooling but a lot is gained conceptually.
\end{remark}
 
 Thus, the main goal of this report is to show how \wfsepdef\ and \wfsepexex\ can be defined given a (perhaps incomplete and scarce) SEP description, and thus produce a \wfp-based safety case for a toy example of a system $X$ and its SEP (the D3b report shows the path from this toy example to the GM SEP).
=======
A special feature of the \wfp-approach is that in terms of Sect. 1.1, the SEP definition \wfsepdef\ is a multi-metamodel \nim\ rather than a local metamodel $M_i$ with all inter-model traceability mapping and constraints included through the SEP's intra-model traceability and constraints. In the TR, we will see how the functional design data (dark-orange), the normative data (grey) and the safety engineering data (yellow), together with constraints defined over them, are seamlessly integrated into one artifact --- the SEP definition metamodel. Correspondingly, a safety case \wfsepexex\ is a multi-artifact \nia\ rather than a local artifact $A_i$, and checking its conformance $\wfsepexex\models\wfsepdef$ can be seen as consistency checking $\nia\models\nim$ considered in Sect. 1.1.  In this way, the \wfp-assurance reshapes inter-model traceability and consistency management to a standard check of a (complex but still singular rather than  multi-) instanceOf-relationship.  This allows us to use standard one-model EMF tools for consistency definition and checking. %Not much is gained technically w.r.t. tooling but a lot is gained conceptually.
\end{remark}
 
\subsection{The content of the TR}
 The main goal of the TR is to show how \wfsepdef\ and \wfsepexex\ can be defined given a (perhaps incomplete and scarce) SEP description, and thus produce a \wfp-based safety case. We will do it for a toy example of a system $X$ and its SEP, but the D3b TR \cite{me-d3bTR} shows the path from this toy example to the GM SEP).
>>>>>>> fixed tites. Minor edits here and there.
%The present TR has two goals. The first and the main one is to show how the {\em workflow plus} (\wfp) approach to assurance works with a simple ``toy'' example, and present a \wfp-based safety case assuring safety of a system $X$. 
%
We will render the safety case as a GSN diagram $\gsndiag$, 
%in a more or less typical GSN way, 
but as this GSN diagram is derived from SEP through the \wfp-glasses, we can denote it by %a safety engineering process (SEP) executed for $X$ and modelled as a \wfp%
%\footnote{so we use the acronym \wfp\ for both i) a type of workflow models and ii) an approach to assurance based on such models}.
%We can then write for the final GSN diagram something like 
a formula $\gsndiag_\wfp(X)$, and we will show the path from $X$ to $\wfp(X)$ to $\gsndiag_\wfp(X)$ including showing all dataflow (traceability) links and how they work for the safety case generation. 

Instead of designing an example of $X$ and its SEP ourselves, we employ the example used in the GSN community standard \citegsNp{p.14, Fig.7}, 
which can be encoded by a formula $\gsndiag_{\gsn}(X)$ 
similar to $\gsndiag_\wfp(X)$ above (where the subindex \gsn\ refers to the GSN approach to structuring safety cases). We thus have two safety cases based on basically the same SEP for the same system $X$%
\footnote{indeed, we will show how we extract $X$'s SEP from the GSN example without adding or deleting anything essential -- we just recover what is implicit in the example}.
%
 The only but crucial difference is that we model SEP as a \wfp\ with all traceability links and constraints explicit, while the GSN Standard keeps (as is typical for GSN safety cases) the SEP implicit and builds the safety case based on common GSN patterns. By comparing the two diagrams, $\gsndiag_\wfp(X)$ and $\gsndiag_\gsn(X)$, we can evaluate and compare the pros and cons of the two approaches to building and documenting safety cases ---this comparative analysis is the second goal of the paper.  
 
 The rest of this report is structured as follows. 
 %In the following, we describe the content of the paper and list its technical contributions. %The paper makes the following technical contributions.  
 In \sectref{assr-as-conf}, we give %define assurance as a workflow conformance enterprise, and give  
 a formalized definition of assurance based on the notions of \wfp-conformance and refinement. 
 %We are not aware of such model-based assurance definitions in the \awmodok{literature; perhaps, their absence had been a major obstacle in providing MDE foundations for assurance.}{literature.}{} 
 %
 In \sectref{gsn2wf1}-\ref{sec:gsn2wf2}, we show how the \wfp-method works with an \mlmodok{elaborated}{}{} example: we take a GSN diagram from the GSN Community 
 Standard~\citegsN{},  \awmodok{interpreted}{interpret it}{} as an SC, recover its semantics, rearrange it in \wfp-terms, and rebuild the case as \wfp-conformance. We show %(in \sectref{gsn2wf2}) 
 that the argument flow---a focal point of the GSN-based assurance---is a data-driven enterprise  (technically, the inference of derived OCL constraints over data they span from given OCL).
 %
 %\endinput
 This significantly differentiates \wfp\ from GSN, in which data and dataflow are mainly implicit. 
 %
 \sectref{anti-gsn} is a comparative analysis of \wfp\ vs. GSN: it can be seen as an evaluation of the new \fwk\ against an established one based on the standard example. We show that the argument flow in the example \awmodok{is significantly distorted and actually wrong}{is significantly distorted---a disappointing}{} observation for an example residing in a popular standard since 2011, Version 1  \citegsnp{p.5} until now in Version 2 \citegsNp{p.14}.  In Appendix, \sectref{compara-survey}, we comparatively analyse \wfp\ and GSN against the issues described in the empirical survey \cite{jcheng-corr18}.
 
 The report culminates in \sectref{assr-as-conf-rev}, where we explain how \wfp\ addresses the major question: Why a safety engineering process, if properly executed for a system $X$, results in a safe system $X$, and how this can be demonstrated with a safety case. Sect.7 concludes the report.
 
 % and satisfy our \req s above. Sections \ref{sec:WPF}-\ref{sec:relwork} \mlmodok{briefly observes}{are brief overviews of}{} our work in progress and future work, and related work resp. \sectref{concl} concludes. %and describes future work. 
 
% We extensively use colours in our diagrams as a visually convenient additional way to convey semantics of diagram elements, which is encoded by labels (specifically, UML's stereotypes) and shapes of elements. 
 \papertr{We extensively use colours in our diagrams as a visually convenient additional way to convey semantics of diagram elements, which is encoded by labels (specifically, UML's stereotypes) and shapes of elements. 
 	\wfp-diagrams contain large amounts of information and normally would span a full page but we made them smaller than  desired due to space limitations. The accompanying technical report  includes bigger versions of these diagrams, and two additional fragment of the material discussed in \sectref{compara-survey} but omitted due to space limits.
 }
 {}
 %\zdmarginn{they allow submitting accompanying material; we will use it}{-5em}
 
 \endinput
 

==> sections/intro-tr.tex <==
\section{Introduction: Consistency and traceability in safety assurance}

%\zd{the intro para below is taken from p.5 and edited as shown below.}

 Consistency issues arise during initial development of a system; as a result of changes for future systems; and during development of those future systems. Configuration management tools help us to keep physical control of various baselines---documents and related artifacts that together define a consistent system, but they do not help us in identifying whether or not \zdmoddok{the contents of a baseline really are mutually consistent.}{different versions of the artifacts involved are mutually consistent.}{}{-1em} This is the role of consistency management. This report shows \zdmoddok{the full context of a safety case approach in \wfp, and especially highlights the extensive traceability links generated in \wfp that enable us to implement effective consistency management throughout the stages discussed above.}{how the \wfp\ approach to assurance provides a solid foundation for consistency management by a) providing an extensive and accurate set of traceability links spanning the dataflow and the argument flow together with the process execution-definition conformance, and b) providing a set of constraints over those traceability links, which constitutes a semantically valid consistency definition.}{}{-1em} 

We will begin with a brief general overview of consistency management as a model management problem to set the stage (Section 1.1), and then consider its specific instantiation for safety cases (Sect. 1.2). 

\subsection{A primer on consistency management}
The presentation will be brief and thus rather formal, but many examples and details about consistency definition and checking can be found in \cite{me-staf16,me-staf16w,me-staf17,harald-progr18}, and about consistency restoration via change propagation in \cite{me-jot11,me-jss15,me-fase18,me-fase18tr}

Let $A_1,..., A_n$ be several interrelated artifacts (models, documents, datasets) to be kept in sync (we also say be {\em (mutually) consistent}) despite their independent changes. We assume that each of the artifacts $A_i$ is a valid instance of the \corring\ metamodel $M_i$, and we write $A_i\models M_i$. (In more detail, a metamodel $M_i$ consists of a graph $G_i$ of classes and associations, and a set of constraints $C_i$ over it so that $A_i\models M_i$ means that a) $A_i$ is properly typed over $G_i$ and b) all constraints $C_i$ are satisfied.) The challenge of consistency management is that although all artifacts $A_i$ can be perfectly valid locally, \ie, $A_i\models M_i$, taken together they may be inconsistent. A typical scenario begins with a consistent state $(A_1,..,A_n)$ of the artifacts involved (we will define this in a minute), then one of the artifacts changes to $A'_i$, which may violate consistency. The goal of consistency management is to change some or all other artifacts (including, perhaps, an amendment to $A'_i$) so that consistency between $A'_1,...,A'_n$ is restored. 

\newcommand\cmstage[1]{\par%\noindent 
	{\bf(#1)}~~~}
\newcommand\nig{\enma{\mathcal{G}}}
\newcommand\nigm{\enma{\nig_\nim}}
\renewcommand\nigm{\nim}

Consistency management consists of three major parts. 

The first is a {\em consistency definition}. % (CDef)}. % which itself consists of two subparts.  

\cmstage{CDef}All traceability mappings/correspondences (or just {\em corrs}) $R_\nim$ between the metamodels are to be specified; we call the tuple $\nigm=(M_1,...,M_n, R_\nim)$  a {\em multi-metamodel} (or a {\em global} metamodel ), and sometime refer to {\em local} metamodels $M_i$ as to \nigm's {\em feet}.  Moreover, a %(CDef-2) 
set of {\em intermodel} constraints $C_\nim$ over $R_\nim$\ is to be defined so that their fulfillment by a multi-instance (see below) should ensure consistency. Thus, we redefine a {\em multi-metamodel} to be a tuple $\nim=(M_1,...,M_n, R_\nim, C_\nim)$.

The second part of consistency management is {\em global instantiation}:

\cmstage{CInst} All traceability links/corrs $R_\nia$ between the artifacts are to be specified, and are assumed to be instantiating the metamodel corrs $R_\nim$. We call the tuple $\nia=(A_1,...,A_n, R_\nia)$ a {\em multi-artifact} or a {\em multi-instance}, and we say it is {\em consistent} if all intermodel constraints are satisfied, \ie, $\nia\models\nim$. 

Examples and details can be found in \cite{me-staf16,me-staf16w,me-staf17,harald-progr18} 

Finally, the third part of consistency management is {\em consistency restoration}, which is typically realized via {\em change propagation}.

\cmstage{CPpg} If an artifact $A_i$ changes to $A'_i$ and the global consistency is violated, \ie, $(A_1,..,A'_i, .., A_n, R_\nia)\nvDash \nim$, other artifacts are changed accordingly to restore consistency, \ie, $\nia'=(A'_1,...,A'_n, R'_\nia)\models \nim$ (note that the traceability links are also updated).  The case when the ``trouble-making'' artifact $A'_i$ is amended to $A''_i$ and thus $\nia'=(A'_1,..,A''_i,..,A'_n, R'_\nia)\models\nim$, is not excluded --- see \cite{me-fase18,me-fase18tr} for details.  

\subsection{Consistency management for safety cases}
\renewcommand\sc{\nmf{SC}}

\subsubsection{Safety case definition.}
The \fwk\ above shows that doing consistency management in a precise and automatable way needs precise definitions %/metamodels $M_i$ 
of all artifacts involved. The first of these artifacts is a metamodel $M_\sc$ for safety cases. In this regard, using a standard metamodel for GSN diagrams, \ie, %identifying safety cases with GSN diagram, would not work 
using GSN to describe a safety case, will not suffice since the GSN metamodel does not capture the semantics of its elements nor is it detailed enough to allow consistency management based on traceability and the consistency definition (indeed, traceability and constraints are missing from GSN). So, the first goal of deliverable D7 is to define a safety case metamodel. More accurately, we show how we can use a description of a safety engineering process (SEP) to define a safety case metamodel $M_\sc$, a safety case instance  $A_\sc$, and their consistency $A_\sc\models M_\sc$.  

As a SEP is a workflow, we prefer more suggestive names and notation for our (meta)artifacts: the SEP metamodel is called the SEP workflow definition and denoted by \wfsepdef. Correspondinglyly, its instance is a SEP workflow execution and is denoted by \wfsepexex, where $X$ is the system for which SEP was executed. In this report we show how to build \wfsepdef\ and \wfsepexex\ with a simple example borrowed from the GSN community standard; in Sect.4-5 of the deliverable D3b report, % \cite[Sect.4-5]{me-d3bTR}, 
we showed how the same procedure can be applied for GM's SEP. 

The workflows used above are actually instances of a special workflow type called \wfp, in which data produced by a process are related to its input data. We need to bear in mind that that we have traceability within a model (intra-model traceability) and %To distinguish these (intra-model) traceability links from the 
traceability between models (inter-model traceability) $R_\nim$, $R_\nia$, as discussed in Sect. 1.1. %, we refer to the former as {\em vertical} and to the latter as {\em horizontal}.  
We will use the name \wfp\ to refer to both a type of workflow and the entire approach, in which a safety case is an instance of \wfsepdef.  

%{
	Several important remarks are in order.
%\newenvironment[1]{remarks}{\subsubsection{#1}}{}
%\begin{remarks}{On the notion of an instance} 

\subsubsection{On the notion of an instance.} 
Our notion of a valid instance {\em includes} a verification that the instance satisfies the metamodel. For example, a safety case instance is a pair $(\wfsepexex, \pi)$ with $\pi$  a proof (verification procedure) showing that $\wfsepexex\models\wfsepdef$. To simplify notation, we will always assume the presence of such $\pi$ by default and refer to the pair by its first component. Thus, a safety case is an instance \wfsepexex\ of the SEP definition \wfsepdef. 
%\end{remarks}
%\begin{remarks}{}[On semantic validity of an instance]
\subsubsection{On semantic validity of an instance.}
	Semantic validity checks (fundamental for safety assurance) are included into the SEP definition (to wit: each SEP subprocess has a review process assigned to it) so that a valid instance of \wfsepdef\ includes reviewing and thus ensures both syntactic verification and semantic validation are done. 
%\end{remarks}
%\begin{remarks}[Consistency and traceability for safety cases]
  \subsubsection{Consistency and traceability for safety cases}
A special feature of the \wfp-approach is that in terms of Sect. 1.1, the SEP definition \wfsepdef\ is a multi-metamodel \nim\ rather than a local metamodel $M_i$ with all inter-model traceability mapping and constraints included through the SEP's intra-model traceability and constraints. In this report, we will see how the functional design data (dark-orange), the normative data (grey) and the safety engineering data (yellow), together with constraints defined over them, are integrated into one artifact --- the SEP definition metamodel. Correspondingly, a safety case \wfsepexex\ is a multi-artifact \nia\ rather than a local artifact $A_i$, and checking its conformance $\wfsepexex\models\wfsepdef$ can be seen as consistency checking $\nia\models\nim$ considered in Sect. 1.1.  In this way, the \wfp-assurance reshapes inter-model traceability and consistency management as a standard check of a (complex but still singular rather than  multi-) instanceOf-relationship.  This will later allow us to use standard one-model EMF tools for consistency definition and checking.
%\end{remarks}
%} % end group

To show why our approach to consistency management will be effective, this report demonstrates how a \wfp-based safety case is produced together with all the explicit traceability links required to support consistency management. We use an example safety case fragment in GSN to show how \wfsepdef\ and \wfsepexex\ can be defined given a (perhaps incomplete and scarce) SEP description, and we produce a \wfp-based safety case for that example system ($X$) and its SEP (while Sect.4-5 of the D3b report %\cite[Sect.4-5]{me-drbTR} 
shows the path from this toy example to the GM SEP).
%The present TR has two goals. The first and the main one is to show how the {\em workflow plus} (\wfp) approach to assurance works with a simple ``toy'' example, and present a \wfp-based safety case assuring safety of a system $X$. 
This safety case will be rendered as a GSN diagram $\gsndiag$, but as this GSN diagram is derived from SEP through the \wfp-glasses, we can denote it by %a safety engineering process (SEP) executed for $X$ and modelled as a \wfp%
%\footnote{so we use the acronym \wfp\ for both i) a type of workflow models and ii) an approach to assurance based on such models}.
%We can then write for the final GSN diagram something like 
a formula $\gsndiag_\wfp(X)$, and we will show the path from $X$ to $\wfp(X)$ to $\gsndiag_\wfp(X)$ including showing all dataflow (traceability) links and how they work for the safety case generation. 

Instead of designing an example of $X$ and its SEP ourselves, we employed the example used in the GSN community standard \citegsNp{p.14, Fig.7}, 
which can be encoded by a formula $\gsndiag_{\gsn}(X)$ 
similar to $\gsndiag_\wfp(X)$ above (where the subindex \gsn\ refers to the GSN approach to structuring safety cases). We thus have two safety cases based on basically the same SEP for the same system $X$%
\footnote{indeed, we will show how we extract $X$'s SEP from the GSN example without adding or deleting anything essential -- we just recover what is implicit in the example}.
%
 The only but crucial difference is that we model SEP as a \wfp\ with all traceability links and constraints explicit, while the GSN Standard keeps (as is typical for GSN safety cases) the SEP implicit and builds the safety case based on common GSN patterns. By comparing the two diagrams, $\gsndiag_\wfp(X)$ and $\gsndiag_\gsn(X)$, we can evaluate and compare the pros and cons of the two approaches to building and documenting safety cases, including the difference in their traceability mechanism crucial for consistency management. 
 
 The rest of this report is structured as follows. 
 %In the following, we describe the content of the paper and list its technical contributions. %The paper makes the following technical contributions.  
 In \sectref{assr-as-conf}, we give %define assurance as a workflow conformance enterprise, and give  
 a formal definition of assurance based on the notions of \wfp-conformance and refinement. 
 %We are not aware of such model-based assurance definitions in the \awmodok{literature; perhaps, their absence had been a major obstacle in providing MDE foundations for assurance.}{literature.}{} 
 %
 In \sectref{gsn2wf1}-\ref{sec:gsn2wf2}, we show how the \wfp-method works with an \mlmodok{elaborated}{}{} example: we take a GSN diagram from the GSN Community 
 Standard~\citegsN{},  \awmodok{interpreted}{interpret it}{} as a safety case, recover its semantics, rearrange it in \wfp-terms, and rebuild the case as \wfp-conformance. We show %(in \sectref{gsn2wf2}) 
 that the argument flow---a focal point of the GSN-based assurance---is a data-driven enterprise  (technically, the inference of derived OCL constraints over data they span from given OCL).
 %
 %\endinput
 This significantly differentiates \wfp\ from GSN, in which data and dataflow are mainly implicit. 
 %
 \sectref{anti-gsn} is a comparative analysis of \wfp\ vs. GSN: it can be seen as an evaluation of the new \fwk\ against an established one based on the standard example. This illustrates the built-in traceability of \wfp that generates links between processes, system data (can be thought of as parts of work products), reviewing (and hence people involved), and thus integrates all these constituents into a single consistent artifact---a safety case. In comparison, GSN-like safety cases build links between items in a safety case, but links between the safety case and processes, people or data (product) have to be constructed as separate tasks. We also show that the argument flow in the example \awmodok{is significantly distorted and actually wrong}{is significantly distorted---a disappointing}{} observation for an example residing in a popular standard since 2011, Version 1  \citegsnp{p.5} until now in Version 2 \citegsNp{p.14}.  
 
 In Appendix, \sectref{compara-survey}, we comparatively analyze \wfp\ and GSN against the issues described in the empirical survey \cite{jcheng-corr18}; several of them include traceability.
 
 \zdmoddok{
 Consistency issues arise during initial development of a system; as a result of changes for future systems; and during development of those future systems. Configuration management tools help us keep physical control of various baselines---documents and related artifacts that together define a consistent system, but they do not help in identifying whether or not the contents of a baseline really are mutually consistent. This is the role of consistency management. This report shows the full context of a safety case approach in \wfp, and especially highlights the extensive traceability links generated in \wfp that enable us to implement effective consistency management throughout the stages discussed above.
}{}{this piece doesn't belong here. I moved it to the very beginning, and amended accordingly}{-6em}
 
 The report culminates in \sectref{assr-as-conf-rev}, where we explain how \wfp\ addresses the major question: Why a safety engineering process, if properly executed for a system $X$, results in a safe system $X$, and how this can be demonstrated with a safety case. This enables us to show the role that effective consistency management plays in being able to produce a safe system. Sect.7 concludes the report.
 
 % and satisfy our \req s above. Sections \ref{sec:WPF}-\ref{sec:relwork} \mlmodok{briefly observes}{are brief overviews of}{} our work in progress and future work, and related work resp. \sectref{concl} concludes. %and describes future work. 
 
% We extensively use colours in our diagrams as a visually convenient additional way to convey semantics of diagram elements, which is encoded by labels (specifically, UML's stereotypes) and shapes of elements. 
 \papertr{We extensively use colours in our diagrams as a visually convenient additional way to convey semantics of diagram elements, which is encoded by labels (specifically, UML's stereotypes) and shapes of elements. 
 	\wfp-diagrams contain large amounts of information and normally would span a full page but we made them smaller than  desired due to space limitations. The accompanying technical report  includes bigger versions of these diagrams, and two additional fragment of the material discussed in \sectref{compara-survey} but omitted due to space limits.
 }
 {}
 %\zdmarginn{they allow submitting accompanying material; we will use it}{-5em}
 
 \endinput
 

==> sections/intro.tex <==
\section{Introduction}
\zd{this versuin of intro was written before the paper actually started. So, it should be revised, pergaps, essentially, when the paper is finished.}
%In the world of IoT, C2C, autonomous driving etc, assurance is getting more and more important. Nowadays, assurance is managed and regulated by assurance cases/safety cases (AC/SC) (see the next section)... But the cost of building an SC for a modern system can be enormous and, in some cases, be greater than those needed to build the system \cite{multileg-bloomf-dsn03}. Hence, to manage safety of embedded systems, we need an elaborated MBSE environment and an effective tool support. The work in this direction has began in \cite{??,??,??} and the present paper is within this line of work. 

Nowadays, safety cases (SC) are an established approach to certifying safety-critical systems in automotive, avionics, railway, and other domains where ... . However, the size and complexity, and hence the cost, of a typical SC for a modern system can be enormous and, in some cases, greater than the cost of building the system as such \cite{multileg-bloomf-dsn03}. This explains the long-standing demand for automation of SC building and maintenance, but the progress in this area is very slow and mainly focused on providing graphical editors (such as Astah GSN and Adelard ASCE) for presenting SCs as GSN/CAE diagrams, which became a de facto standard in structuring and specifying SCs. An OMG initiative in this direction, Structured Assurance Case Metamodel (SACM) \citesacm, can also be seen as an effort to standardize the GSN/CAE notation within the MOF \fwk.%
\footnote{There are some diiferences between GSN and CAE but their overall view of building SCs are similar; in the paper, we focus on GSN but the results of our analysis are applicable to CAE too.} \zdneww{However, we think that GSN foundations for assurance is a wrong way to go, and its automation would only speed up moving in the wrong direction. (Perhaps, it would also reveal some of inherited GSN problems, but it is cheaper to see the issues before the journey starts rather  than on the road.) The two general goals of the paper are a) to specify a proper specific place of the GSN in the overall assurance landscape and demonstrate its severe deficiencies when it's expanded and used as an integral approach to assurance as a whole, and b) describe an alternative approach, which is much more rigorous, detailed and, importantly for automation, based on MBE core ideas of metamodelling and model management.}{let's make it clear}{-12em}      

Several factors make automation of SC building inherently difficult  
 \citenasa: 
 \begin{enumerate}
 %a) the size of the case may grow super-linearly in the size of the underlying software, 
 \item the heterogeneity of the artifacts and tools to be integrated in the safety argument flow, including informal and domain-specific artifacts, 
 \item a multitude of implicit assumptions about functioning single subsystems and, especially, their interactions,  
 \item the necessity to coordinate the functional system development and its safety engineering side, and 
 \item the necessity to maintain a vast array of traceability links between all these artifacts and code. 
\end{enumerate}
 Managing the issues above needs  a solid MBSE \fwk\ based on truly MBE foundations (including accurately specified metamodels and models, their relationships and transformations). In contrast, GSN centered activities take into account mainly the purely logical part of the story and underestimate or neglect the intermodel relationships and dataflow parts%
 \footnote{In this sense, the GSN representation of an SC could be compared with a class diagram, whose semantics is hidden in the names of classes and associations rather than explicated in their attributes. A special section of the paper will be devoted to a technical analysis of GSN deficiencies.} 

A major obstacle in building the MBSE \fwk\ for assurance is the absence of a clear formalized definition of what assurance is, in other words, what an SC should demonstrate semantically, which would be a cornerstone for subsequent metamodeling and modelling activities. %
%\footnote{We again stress that the GSN representation of an SC leaves implicit an enormous amount of critical data and could be compared with a class diagram, whose semantics is hidden in the names of classes and associations rather than explicated in their attributes.} 
In the paper, we will give such a definition, and based on it, will develop foundation of an integral model management \fwk\ for assurance referred to as %We will refer to the \fwk\ we propose as to 
Workflow$^+$-Based Assurance, or \wfba\ in short. 

There are three important distinctive features of \wfba. {\bf First,} the assurance  philosophy underlying the approach can be seen as a trade-off between process-based and product-focused. Although we say that ``a system is safe if its safety-engineering process (SEP) is acceptably well done", our notion of SEP being {\em acceptably well done} is strongly product-oriented and  includes multiple and precisely specified pieces of evidence that the product possesses required measurable properties assuring its safety. {\bf Second,} our models of SEP and its subprocesses are workflows in the technical sense of the word and are specified as functional block diagrams with all dataflow accurately modelled. A special feature of a SEP dataflow is the presence of multiple relationships between the output data of a block/process and its input data; a typical example is when the input to a process is  specified by a class or several classes, while the output provides new attributes for the input classes and/or new associations between them. Because of this special feature of our workflow models, we refer to them as {\em workflow+ (WF+)}. {\bf Third,} the argument flow (mandatory for SC) in \wfba\ is heavily based on data, in fact, this is the flow of OCL constraint derivation (which moves the underlying logic beyond the boundaries of propositional logic customary for modern SCs). Thus, a typical WF+-model comprises three layers: (i) process and control flow, (ii) dataflow (with input-output relationships), and (iii) argument flow or constraint derivation. It is the dataflow layer that bounds all ingredients into a single WF+-model and makes our assurance methodology essentially product-oriented. Precise dataflow modelling signifies a crucial distinction of \wfba\ and GSN-based assurance, in which the data layer is mainly implicit so that a typical GSN-case appears as the tip of an iceberg. In our view, keeping the enormous dataflow layer of assuring complex systems implicit is as dangerous as neglecting the underwater part of an iceberg, and a strong anti-GSN stance can be seen as a  forth feature of \wfba. 

The paper makes the following technical contributions. In \sectref{sec:assr-as-conf}, we define assurance as a workflow conformance enterprise. In \sectref{sec:wfba}, we introduce \wfba\ and show how it works with a simple example: we take a sample safety case presented in the GSN Community Standard and rebuild it on \wfba-foundations. This will later allow us to make a comparative analysis of GSN and \wfba\ in \sectref{sec:anti-gsn}. In \sectref{sec:wfp-meta}, we formalize the notion of WF+ and build its metamodel. 

\zd{What is left behind is: 
	a) reviewing as an aspect and the aspect stuff as a contributuion; }
	%b) conformance as the cornerstone of assurance}
\endinput

==> sections/introNew-zd.tex <==
\section{Introduction-Previous}
%\zd{this version of intro was written before the paper actually started. So, it should be revised, perhaps essentially, when the paper is finished.}
%In the world of IoT, C2C, autonomous driving etc, assurance is getting more and more important. Nowadays, assurance is managed and regulated by assurance cases/safety cases (AC/SC) (see the next section)... But the cost of building an SC for a modern system can be enormous and, in some cases, be greater than those needed to build the system \cite{multileg-bloomf-dsn03}. Hence, to manage safety of embedded systems, we need an elaborated MBSE environment and an effective tool support. The work in this direction has began in \cite{??,??,??} and the present paper is within this line of work. 

Nowadays, safety cases (SC) are an established approach to certifying safety-critical systems in automotive, avionics, railway, nuclear and other domains\cite{adelard-mss10}. However, the size and complexity, and hence the cost, of a typical SC for a modern \nanewok{computer-controlled}{} system can be enormous and, in some cases, greater than the cost of building the system as such \cite{multileg-bloomf-dsn03}. This explains the long-standing demand for tooling to assist and automate the building and maintenance of SC \nahll{\cite{?,?}}{papers advocating tooling( AdvoCATE and other)}{-12em}. The activity in this domain is mainly based on GSN \citegsn\ or CAE \citecae\ diagrams (further collectively referred to as GSN-style diagrams), which became a de facto standard for structuring and specifying SCs.% 
\footnote{There are some differences between GSN and CAE but their overall view of building SCs are similar; in the paper, we focus on GSN but the results of our analysis are applicable to CAE too.} 
\zdmoddok{(such as Astah GSN, Adelard ASCE and advoCATE).}{}{}{-1cm}
An OMG initiative in this direction, Structured Assurance Case Metamodel (SACM)\cite{SACM2}, can also be seen as an effort to standardize the GSN notation within the MOF ecosystem.
 
%\zdneww{However, we think that GSN foundations for assurance is a wrong way to go, and its automation would only speed up moving in the wrong direction. (Perhaps, it would also reveal some of inherited GSN problems, but it is cheaper to see the issues before the journey starts rather  than on the road.) The two general goals of the paper are a) to specify a proper specific place of the GSN in the overall assurance landscape and demonstrate its severe deficiencies when it's expanded and used as an integral approach to assurance as a whole, and b) describe an alternative approach, which is much more rigorous, detailed and, importantly for automation, based on MBE core ideas of metamodelling and model management.}{let's make it clear}{-12em}      

\zdhll{
Several factors make automation of SC building inherently difficult  
 \citenasa:
 \numitem{a} the heterogeneity of the artifacts and tools to be integrated in the safety argument flow, including informal and domain-specific artifacts, 
 \numitem{b} a multitude of implicit assumptions about functioning single subsystems and, especially, their interactions,  
 \numitem{c} the necessity to coordinate the functional system development and its safety engineering side, and 
 \numitem{d} the necessity to maintain a vast array of traceability links between all these artifacts and code. 
}{to be shortened?}{-5em}
%\end{enumerate}
%
Managing the issues above needs  a solid MDE \fwk%
 	\footnote{we prefer to use a somewhat unpopular now acronym MDE rather than MBSE for model-based software engineering as the verb `based' will be often used in the context of XXX-based assurance} 
 	based on truly model-based foundations for system modelling, including accurately specified metamodels and models, their relationships and transformations, and extensive traceability management. We believe that the {\em Models} community has much to offer to assurance and can provide it with rigour, conceptual and technological clarity, and tool support. 
 	
 	The main goal of the paper is to lay theoretical foundations for this development by presenting a {\em Workflow$^+$ Conformance Framework for Assurance}, or {\em \wcfa}. %\ (Workflow conformance based assurance)}
% 	 in short. 
In \wca, assuring safety of a product $X$ consists of two parts. First, two workflows, which model how the safety engineering process (SEP) of $X$'s manufacturer is defined and executed for $X$, are to be specified and checked for  conformance: $\wfexe\Vdash^1\wfsep$. We specify \wfsep\ as a class diagram and \wfexe\ as an object diagram so that the conformance above is a usual model-metamodel conformance well known in MDE. Second, we need to build a third {\em normative} workflow \wfnorm\ that models how standards and other ``guiding documents'', including expert opinions, collectively prescribe SEP definition, and check conformance $\wfsep\Vdash^2\wfnorm$. We specify \wfnorm\ as a class diagram and conformance above appears as a refinement relation between two models. 
% ======    will be needed later
%To unify, we can consider an object model as a degenerated class diagram, whose all classed and associations are declared to be singletons (see \cite{me-sle13partial} for details) so that conformance $\models^1$ can also be seen as a refinement. 
%========
\zdmodd{Thus, we reduce assurance to the two well-known model management task of checking correctness of instantiation and refinement.}{only one is well-known}{}{-3em}
	
	 %$\Vdash^1$(meta)model refinement for correctness.   
%To make these general conditions technical and verifiable, we consider SEP definition as a huge model transformation definition, which is executed for a given system as a model instantiating the corresponding metamodel. Moreover, we model both artifacts as workflows so that checking condition b) amounts to a typical MOF/UML task: whether a (workflow) model conforms to a (workflow) metamodel.
%a) specifying three workflows modelling, resp., the Safety Engineering Process of the manufacturer (\wfsep),  its execution for particular product (\wfexe), and a set of standards and other normative documents collectively defining some {\em normative} workflow (\wfnorm), % normWfplaying the roles of an instance, metamodel, and meta-metamodel resp., 
% 	 and b) checking two conformance relationships between them
% 	\begin{equation}\label{eq:conf-conf}
% 	\mbox{$\wfexe\models^\VV\wfsep$ and  $\wfsep\models^\VV\wfnorm$},
%  	\end{equation}
% 	where the index \VV\ refers to the necessity to check both Validity of the instance data  and formal Verification of the instance to the (meta)model. %Workflows are modelled as class diagrams and thus, 
% 	Thus, at the centre of \wcfa\ is a well-known model management task of checking an instance-model conformance, enriched with a relatively unusual MDE task of checking data validity. % (we will motivate and detail this idea in \sectref{assr-as-conf}). 
 	
 	This goal is complemented in the paper with an analysis of the GSN-based assurance:  we show that GSN-style safety cases provide a dangerous false sense of confidence by presenting reasoning as if it is rigorous when it is in fact not. The investment of large quantities of time and money into the development of supporting tools and automation would further solidify GSN's position as the go-to for building assurance cases, resulting in the safety of more and more systems being subjected to its drawbacks. \wcba\ is an MDE-alternative to GSN, 
 	which we believe better achieves GSN's original goal of basing assurance on structured reasoning and %supporting it 
 	evidence.
 	
  %%%From a piece that got moved to antigsn. probably unneeded%%%
 %\footnote{In this sense, the GSN representation of an SC could be compared with a class diagram, whose semantics is hidden in the names of classes and associations rather than explicated in their attributes. A special section of the paper will be devoted to a technical analysis of GSN deficiencies.} 

\zdmoddok{A major obstacle in building the MBSE \fwk\ for assurance is the absence of a clear formalized definition of what assurance is, in other words, what an SC should demonstrate semantically, which would be a cornerstone for subsequent metamodeling and modelling activities. %
%\footnote{We again stress that the GSN representation of an SC leaves implicit an enormous amount of critical data and could be compared with a class diagram, whose semantics is hidden in the names of classes and associations rather than explicated in their attributes.} 
In the paper, we will give such a definition, and based on it, will develop foundation of an integral model management \fwk\ for assurance referred to as %We will refer to the \fwk\ we propose as to 
Workflow$^+$-Based Assurance, or \wfba\ in short.}{}{}{-2cm} 

We see four distinctive features of \wca. 
% needs package <<enumitem>>
\begin{enumerate}[label={\bf \alph*)}, %Step 
%\arabic{enumi}., ref=Step \arabic{enumi},% 
wide=0pt]
\item  It is based on a clear technical (even formal) definition (\ref{eq:conf-conf}) of what assurance is; %\ie, what an SC should demonstrate semantically,
we believe that the absence of such a definition was a major obstacle in providing MDE foundations for assurance.

\item The methodology underlying the approach can be seen as an integration of  the process-based and the product-focused approaches to assurance, which is a long-standing challenging issue in the domain (cf. \citealan). We will explain the challenge and our solution in \sectref{assr-as-conf}). % Although we say that ``a system is safe if its safety-engineering process (SEP) is acceptably well done", our notion of SEP being {\em acceptably well done} is strongly product-oriented and  includes multiple and precisely specified pieces of evidence that the product possesses required measurable properties assuring its safety. We are not aware of such an integrative view of assurance reported in the literature.

\item Our models of SEP and its subprocesses are workflows in the technical sense of the word and are specified as block diagrams with all dataflow accurately modelled. A special feature of a SEP dataflow is the presence of multiple relationships between the output data of a block/process and its input data%
\footnote{a typical example is when the input to a process is  specified by a class or several classes, while the output provides new attributes for the input classes and/or new associations between them}. Because of this special feature of our workflow models, we refer to them as {\em workflow+ (\WF)}. %
%and provide \WF with a formal semantics and an initial analysis of its foundations (we are not aware of an accurate analysis of \WF\ formalism reported in the literature). % (whereas we show in the paper that \WF essentially differs from ordinary workflows).

\item The argument flow (mandatory for SC) in \wca\ is heavily based on data, in fact, this is the flow of OCL constraint derivation over the \corring\ data (which moves the underlying logic beyond the boundaries of propositional logic customary for modern SCs). 
%
Thus, a typical \WF-model comprises three (interrelated) lanes: (i) process and control flow, (ii) dataflow (with input-output relationships), and (iii) argument flow or constraint derivation. It is the dataflow lane that bounds all ingredients into a single \WF-model and makes our assurance methodology essentially product-oriented. 
\item Precise dataflow modelling signifies a crucial distinction of \wca- and GSN-based assurance; in the latter, the dataflow part is mainly implicit so that a typical GSN-case appears as the tip of an iceberg. In our view, keeping the enormous dataflow part of assuring complex systems implicit is as dangerous as neglecting the underwater part of an iceberg, hence, a strong anti-GSN stance of this paper. %can be seen as a special forced feature of \wca. 
\end{enumerate}

The methodological novelties described above are supported with the following technical contributions reported in the paper. 
%
\numitem{a} We show how \WF\ modelling and conformance can effectively be done with class diagrams (which can further be developed into a specialized profile). 
%
\numitem{b} We show that \WF\ essentially differs from ordinary workflows, and provide \WF\ with precise metamodels, a formal semantics and an initial mathematical analysis of its foundations. Extending basic constructs well-known for functional block diagrams to make them applicable for \WF\ turns out mathematically challenging and requires sufficiently advanced category theory (CT) means discussed in \sectref{formal}.
%: categories with pullbacks (PB) and pushouts (PO) (and, more generally, limits and colimits), continuous functors compatible with them, and adhesive categories in which PBs and POs smoothly interact via Van Kampen squares. 
A notable result we obtained in this way is compositionality of \WF: a complex workflow can be encapsulated as a black-box process, which makes it possible to consider workflows of workflows (and so on) in the \WF\ setting as well as for classical workflows. 
%As we cannot assume an advanced knowledge of CT from a typical Models reader, we will describe the \WF\ mechanisms conceptually rather than formally, but accurate formal definitions and details can be found in a technical report (further, TR) \citetr\ accompanying the paper.  
%
\numitem{c} We manage the validation aspect of conformance checking by considering it as an aspect in the technical sense, \ie, as a cross-cutting concern spreading over the entire workflow. We present a simple metamodel weaving mechanism and show how it works with an example. 


The paper is structured as follows.
In \sectref{assr-as-conf}, we motivate and define assurance as a workflow conformance enterprise. In \sectref{wfba}, we introduce \wfba\ and show how it works with a simple example: we take a sample safety case presented in the GSN Community Standard and rebuild it on \wfba-foundations. This will later allow us to make a comparative analysis of GSN and \wfba\ in \sectref{anti-gsn}. In \sectref{wfFormalism}, we formalize the notion of \WF\ and build its metamodel. 

\zd{A remark about using colours in our diagrams}

\endinput

==> sections/metamodel-main.tex <==
\subsection{The metamodel of the Example's \wfsep%
	%Making Process \& Dataflow accurate 
} 
\label{sec:GSNWF+}

%This section presents \wfp\ as an alternative way to represent the multi-dimensional information presented in \figref{fig:GSNAnnotated}. Our WF+ representation of the GSN example comes as a package of five diagrams - a WF+ metamodel(\figref{fig:metamodel}, referred to as SEP for processes and dataflow, a WF+ metamodel with data, inferences over constraints and reviews(\figref{fig:inference}), an instance of the WF+ metamodel(\figref{fig:instance}), a WF+ metamodel of a normative document(\figref{fig:normative}) and a model of reviewing(\figref{fig:aspectR} see \sectref{aspects}). Figure~\ref{fig:metamodel} and \figref{fig:inference} are two views of the same model, but are separated to ease reading. Black boxes with white text are used to indicate the correspondence with elements of \figref{fig:GSNAnnotated}.

\input{figures/metamodel}
Process and data blocks in \figann\ sketch some workflow, which in this section we treat as an instance of some workflow definition/metamodel (\wfsep\ in term of \secref{ass-as-conf}). Making the latter syntactically accurate and semantically reasonable needs some domain knowledge beyond the workflow sketch in \figann, but we tried to keep the extension beyond the Example story as minimal as possible. 

We build the metamodel as a class diagram with a special type of classes stereotyped Process (green in \figsepi), whose instances are process executions. Dataflow to and from processes is shown with directed associations, while ordinary (static) \asson s between data classes (yellow and orange) are all undirected and oriented vertically. Orange data are input to the entire SEP process, consisting from three components, HARA, Design, Verification (note three green rectangles in \figsepi), which are further decomposed as shown. The order of processes is shown with numbers prefixing process names (and can be inferred from the dataflow)  
%The metamodel has the following special layout. Process are moved to the left and their order is shown by numbers prefixing their names. 
We use rectangle frames to show decomposition, \eg, process HARA consists of three subprocesses. %Data classes (yellow and orange) represent data produced and/or used by processes during their execution (orange data are input to the entire SEP) indicates that it is given as input to the SEP. Any associations between non-process classes are standard UML associations(directed arrows are reserved to annotate process flow). 
Boundary objects (circle with a vertical line attached) are used as aliases for data to reduce the number of crossing lines in the model. 

The diagram is hopefully a self-explainable completion of the annotated Example (\figann); black-box labels show the backward mapping to the GSN diagram. We just mention that we specialized process FV in \figann\ as a state space exploration process, which assures hazard elimination iff the hazardous state is not reachable. The comparisons residing in goals G5, G6 are specified as executions of the query specified in box 3b.2, which is defined to assure hazard mitigation. 
\zdhll{Note the lower multiplicity 1 spanning two \asson\ ends, which demands each hazard to be eliminated or mitigated. The inverse multiplicity demands a protection system to protect against at least one hazard.}{may be removed if fighting for space}{-5em}  

Note a special feature of the workflow: data produced by a process are connected to its input data, \eg, processes 1.2 and 1.3 take Hazard at the input and produce, resp., their  SIL attributes and (for process 1.3) HazardGroup together with as \asson\ linking it to Hazard. Or, process 3a takes information about hazards  and protection systems intended to eliminate them, and outputs an
\zd{to be completed .....}     



%=== inst piece
\input{figures/instance}
The metamodel above defines a workflow, which can be executed for any data correctly instantiating the orange part of the class diagram, and thus instantiate the yellow part of the class diagram (ISO 26262 refers to these as to WorkProducts). The GSN Example actually tells us a story about such an instance, say, $X$\zdmodd{, and \figinst\ presents its fragment: to save space, we only show the upper half of the instance for hazards H1, H2 while data about H3 are omitted.}{.}{}{-5em}

There are two main questions about $X$. The first is its syntactic correctness: whether all constraints declared in the metamodel \figsepi\ are satisfied. This task can be done automatically with modern MDE tools. Then second question is the semantic correctness of the instance data, for example, .... \zd{to be completed -- about reviewing-->goes to Nick} Or, how do we know that the set of Hazards objects appearing in the instance, \ie, \{H1, H2, H3\} , is complete enough, \ie, no bad hazards are missing. To answer such questions, we need a special procedure called reviewing \zd{to be completed-->Nick} 


\endinput
The instance in \figref{fig:instance} is the result executing the process in \figref{fig:metamodel} . We omit dataflow links from all processes but two to avoid clutter but still demonstrate dataflow in the instance. Here, we see product-level details appear. Detailed information ommitted in \figref{fig:gsnEx-main} was "made up" for the sake of the example(such as \textit{Prob1: \realprob)}. 

Once an instance is complete, or at any desired point along the way, tools can be used to automatically verifiy syntactic contraints. An example of this is shown by horizontal red lines attached to the associations being verified. 

If all syntactic contraints are satisfied, we can conclude that condition a) \defref{main}  is satisfied. It may seem strange to say that the satisfaction of syntactic constraints can be used to conclude that the SEP was well executed, but as the metamodel encodes all semantics syntactically(eg. the validity of data through reviewing), confidence in the instance is reduced to a simple conformance check. There is no magic; everything important to safe development must be done, but checking that it is done is reduced to the well-known concept of conformance.

\nanew{More on constraints, conformance from zinovy probably}{}


\endinput

\subsubsection{WF+ Syntax}
There are three main components to WF+ models presented: process classes, data classes, and constraints. Green processes are classes whose instances are executions of a process, which takes input data to produce output data, denoted by directed arrows to and from the process respectively. The order of execution of processes is denoted by numbering in their titles. WF+ allows processes to produce new data, associations between input data, associations between input and output data, new attributs for data, or any combination thereof. Green frames denote different stages of the SEP. As a whole, these processes form the SEP to be followed during the development of a safety-critical system. 

Data classes represent data produced and/or used by processes during the execution of a SEP. Orange data indicates that it is given as input to the SEP. Any associations between non-process classes are standard UML associations(directed arrows are reserved to annotate process flow). Boundary objects(circle with a vertical line attached) are used as aliases for data to reduce the number of crossing lines in the model. 

Constraints are used to restrict the structure of instantiations of the SEP. Multiplicities typical of UML are used to specify how many data classes are related to each other, and how many instances of data are input/output to/from processes. OCL-style constraints are used between classes and associations, which can be complex and will be explained on a case-by-case basis.

\subsubsection{WF+ 1 - Metamodel}

\figref{fig:metamodel} shows a WF+ representation of the green and orange elements from \figref{fig:GSNAnnotated}. Bold red lines are used as constraints, where black, grey and blue lines are used for dataflow and associations. Black and grey lines are used solely to ease reading of crossing lines.  

\paragraph{HARA}
The topmost green frame, HARA, contains three processes: \fha, \dersil and \silapp. Just as in the GSN example, \fha uses the control system of interest(more accurately its functional architecture) and operating role and context to identify hazards. We have introduced four attributes for \hazard\, including whether it should be mitigated or eliminated, that are common artifacts of hazard analyses.
Following this, each \hazard\ is assessed as per the \silguide\ by \dersil\ to identify its \sil. Notice that through multiplicity constraints, there will be one execution of \dersil\ for each hazard, and one \sil\ output. Then, every hazard(notice that \sil\ is included by virtue of being an attribute) is input to \silapp\ to produce \hazgr s and a \containment\ association to show which hazards belong to which group. \hazgr\ has a method $\backslash$\sil\ that calculates the \sil\ of the group, which is the highest \sil\ of all \hazard s in the group.

\paragraph{Design}
Once \hazard s are grouped, the next step is to develop a \protsys\ for each \hazgr\ to mitigate or eliminate every \hazard\ in it. This is done through \devprotsys, which is executed once for each \hazgr\ while following \silproc\ to produce a \protsys\ for the \hazgr\ input and a traceability association \grprot\ to the group it is protecting. Through \grprot\ and \containment,  \elim\ and \mitig\ are derived, indicating which hazards are eliminated or mitigated by which systems. The multiplicity constraint $1$ between \elim\ and \mitig\ means that each hazard is either mitigated or eliminated by one \protsys.

\paragraph{Verification}
Finally, the SEP verifies that each \hazard\ is eliminated or sufficiently mitigated. The constraint \namefont{XOR} between inputs to \formverif\ and \fta\ means that each hazard is verified by exactly one method; \hazard s to be eliminated must undergo formal verification(\sse in the model) and those to be mitigated must be assessed using fault tree anaylsis. For each \hazard\, \namefont{self.\mitorelim} can be used to determine which verification process should be used, and the \protsys\ to be used can be found through \namefont{self.\mitig} or \namefont{self.\elim}(only one can exist in an instance).

If \sse\ deems that the hazard has indeed been eliminated, it outputs the attribute \valid\ of the \elim\ association with \Value =$True$. If the \hazard\ is not eliminated, the same attribute is crated but with \Value=$False$.
	
\fta\ outputs the actual probability, \realprob\, of the \hazard occuring with the \protsys\ in place. \vermit\ then compares \realprob\ to the target probability from \tolgui\ to check that for \hazard 's \sil, the probability of \hazard occuring is indeed low enough. If it is low enough, it outputs the attribute \valid\ of the \mitig\ association with \Value =$True$. If the \hazard\ is not mitigated, the same attribute is crated but with \Value=$False$.



==> sections/old-unused.tex <==
\section{Old unused pieces}

 \subsection{Constraint derivation: From metamodels to instances}
 \label{sec:isnt-metamod}
 Constraints are elements of metamodels, and our derivation lives on the metamodel level while a typical GSN case builds an argument flow for a concrete system, \ie, an instance. The gap is easily bridged by the {\em soundness} of our derivation steps: we derive semantically rather than by syntactic rules.  %the logic used for inference: 
 %To explain  the notion, we will use simple mathematical models. 
 In more detail, suppose we have a metamodel $M=(\gbf^M,\csetx{M}{\given})$ with \gbf\ being its graph of types (classes and \asson s), and \csetx{M}{\given}  a set of constraints defined over \gbf. An inference tree can be schematically presented by a sequence of inference steps
 \begin{equation}\label{eq:inf-seq}
 \csetx{M}{\given}=\csetx{0}{\der}\models_1\csetx{1}{\der}\models_{2}\ldots\models_{n}\csetx{n}{\der}=\csetx{M}{\der}\ni C!
 \end{equation}
 %   $\cset{\given}\vdash^\nil\cset{\der}$, 
 where  $\models_i$ is an inference step extending a set of derived \namodok{constants}{constraints}{} \csetx{i}{\der} with a new constraint $C_i$ so that $\csetx{i+1}{\der}=\csetx{i}{\der}\cup \{C_i\}$; the initial set consists of all constraints initially given in the metamodel;  and \csetx{M}{\der} is the final set containing the top claim $C!$. Soundness of a step $i$ means that for any instance $I$ properly typed over $\gbf^M$,  if $I\models\csetx{i}{\der}$ then $I\models\csetx{i+1}{\der}$. By transitivity, if $I\models\csetx{M}{\given}$ and all steps are sound, then $I\models C!$. % 
%  \footnote{In a more accurate presentation of inference, an inference step $i$ consists of several steps $i_1,...,i_n$ performed in parallel, but the transitivity holds again -- it is a standard logical result.} 

Soundness of some of our derivation steps is based on simple logic, \eg, the inference 
CV\implBy EV \& MV is sound because of the data condition $\hPrtn=\nmf{Elimination}\cup\nmf{Mitigation}$, which is in turn implied by \multy\ 1 of Hazard's attribute elimORmit (see \figmetamod). Some inference steps can be seen as merely defintions, \eg, A1\implBy A11\&A12. And some derivations are semantically non-trivial, \eg, when we conclude that having a coverage link H-PS both verified and reviewed implies that PS really protects against H. A common approach to such derivations is to require strong validation criteria so that getting equality \valid?=T for an instance $I$ is not easy but being achieved would indeed mean that the semantic condition in question is satisfied. %, \eg, hazard H is indeed protected by PS (where H, PS are elements of instance $I$). 

Thus,  for a given system $X$, if $\wfexex\models\csetx{\wfsep}{\given}$, then $\wfexex\models C!$ so that the B) part of an \wfp-based safety case (see \defref{main}) consists of two major subparts: %

%\noindent 
\numitem{B1}  Constraint derivation over the SEP metamodel, $\csetx{\wfsep}{\given}\models C!$ % (in our case, derivation of blue constraints from the red/pink ones), 
  and 
  
  \numitem{B2} Checking instance conformance, $\wfexex\models \csetx{\wfsep}{\given}$, for a given system $X$, whose most challenging part is checking T for validity constraints (shown in red in \figinfer). % (which is fairly simple in our case, as all constraints are \multi es). 
 

  
\section{\wfp\ vs. GSN: A Comparative Discussion}\label{sec:anti-gsn}

\newcommand\exgsn{Ex.GSN}
\newcommand\exwfp{Ex.\wfp}
\newcommand\exg{\exgsn}
\newcommand\exw{\exwfp}
\newcommand\exgoal{\ensuremath{Z}}
\newcommand\exgaol{\exgoal} %l{\ensuremath{Z}}

We will begin with a brief survey of how we processed the material described in the Example (further \exgsn) and come to its \wfp-version (\exwfp) to set a stage for the discussion, then present the results of matching \exgsn\ and \exwfp, and conclude with some general observations about GSN. 

\renewcommand
\subsection{From \exgsn\ to \exwfp: defining the DCC}
We recognize that the main goal of the \exg\ diagram was to demonstrate the vocabulary of GSN elements and show how they can be put together to work for some purpose \exgoal\ rather than write an SC. However, for this \exgoal, they had chosen to specify in GSN terms an oversimplified SC, which a fully justifiable and reasonable choice: GSN is widely used for building and documenting SCs in many domains (including our partners in automotive industry). The \exg-authors did a good work for both facets: they describe the notation and they skilfully managed to present an interesting and seemingly well arranged SC with a small one-page diagram; the fact that the Example resides in the Standard without changes for nine years now is a good justification for this conclusion.  It also motivates and justify our idea to use \exg\ as a sample SC to show how \wfp\ works, and we processed it as schematically shown in \figref{fig:recoverSem}. For our comparative analysis, we need an accurate description of what our processing brought to  \exg. 


As \figann\ shows, \exg\ provides a listing of processes and data involved, and  \figmetamod\ shows that we did not intoduce in \exw\ new processes nor data classes (they all are labelled by the respective elements of \exg). However, classes (green and yellow) only give us a discrete view of the story without the dataflow between processes and data (green-yellow links), and \asson s  between classes (yellow-yellow); below we will refer to both types of links as dataflow and call its two specializations dp-dataflow and dd-dateflow.. We have restored the missing structural links based on our understanding of the domain knowledge (DK) and thus came to metamodel \wfsep\ in \figmm. As this DK is sufficiently common, it seems reasonable to assume that the authors of \exg\ based their SC on a very close dataflow picture but kept it implicit. In addition to this distinction, our \wfp-glasses revealed two more actors on the stage: a detailed specification of constraints for the \df, and splitting the argument flow into two parts: (data-driven) constraint derivation over the metamodel, and cheking the instance conformance $\wfexe(X)\confcheck{\inst}{}\,\wfsep$. (Recall that a typical GSN SC, including \exg, considers argument flow for a given system $X$ without any mentioning the two levels). We will briefly refer to the differences between the two \fwk s for SC buiding, GSN and \wfp, as DCC (Dataflow, Constraints, Conformance). Again, it seems reasonable to assume that all three actors are implicitly (and perhaps inaccurately) preset in the \exg\ so that the only real difference between the two \fwk s is that \wfp\ treats DCC as first-class citizens while GSN keeps them underground. We can schematically write something like \wfp=GSN + Explicit DCC.  Our next goal is to compare the two cases, \exg\ and \exw, to see whether DCC-explication is practically important or is mainly a theoretical bonus.  

\subsection{The Comparison}



 

\endinput


 
 
\subsection{Comparison of the two diagrams}
 It is worth reiterating that our criticisms of GSN-style SCs are entirely based on its structure - we are absolutely not attempting to criticize the content of \figref{fig:gsnEx-main} from a safety perspective, nor are we attempting to say that the \wfp\ representation would be a better SC than \figref{fig:gsnEx-main} if the Control System in the example were real; neither would be sufficient. Instead, we focus on analyzing the structures GSN uses to represent information and in this section will provide an objective, technical comparison of the structures of \wfp and GSN. 
 
 \begin{enumerate}[wide=0pt]
	 \item It can be seen in \figref{fig:GSNannotated} that GSN presents an after-the-fact, purely logical representation in which dataflow and traceability are left implicit, whereas in \wfp\ explicit traceability between all data and processes is central. For safety-critical systems it is essential to understand dataflow to be able to properly reason about safety. A concrete example of implicit dataflow can be seen in C3: it is provided as context for G2, but is ultimately used in G5 and G6. G5 and G6 do inherit the context from G2, allowing for the link to be reconstructed by the reader, but in large safety cases reconstructing these links becomes difficult and impractical. Another example is a cross-cutting reference where the SIL of hazards is implicitly used in the left branch by G5 and G6, who are never directed to any data about their Hazard's SIL. 
	 
	  \item  There is a lack of well defined semantics(\ie process, constraint or data) for syntactic elements of GSN, whereas \wfp\ provides prescise semantics for the syntactic elements(processes, data, constraints) necessary for safety-engineering. Loose semantics of syntax undermine the core purpose of SCs by introducing ambiguity into a model which is supposed to provide an understandable and compelling argument for safety. 
	  
	  \item The reasoning in the GSN example is distorted by the separation of interrelated components of the SC. For example, as shown in \figref{fig:inference}, it is clearly necessary to demonstrate that every hazard is covered by a protection system to show that all hazards are mitigated or eliminated. This type of distortion is typical of GSN SCs and is the result of an attempt to separate product-focused arguments(G2) from process-focused arguments(G3). On the surface this appears to be an effective way to strucutre safety cases, but, as we have shown, when the delicate relationships between processes and data(product) are considered, the logic of this separation is distorted.
	  
	  \item GSN reasoning is carried out in an ad-hoc manner, whereas \wfp\ reasons in a well-defined way over data. Data driven reasoning guides the development of arguments, and simultaneously allows the checking and discussion of arguments by presenting them in a discreet setting. We do not remove the difficulty inherint in reasoning, but rather provide a framework in which it can be managed effectively.
	  
  \end{enumerate}
  
  
  
  
  
 \endinput 
 
 
 
 
 \endinput 
 (and several blue-boxes with white font are added but ignore them for a while), and data constraints are supplied with {\em claims}---formulations of constraints' semantics in common assurance-motivated terms (note pink boxes with a black-font text). We have also added a composed (and hence derived) \asson\ 
 
 
%; we will refer to them as to {\em claims}.  
Note also six purle aliases of six review processes 1.1-3, 2.1, 3a and 3b (as the second step in 3b is a query, \ie, an automatic operation over data that does not need a semantic check), which provide six respective Boolean-valued validity attributes. A requirement for such an attribute to be true is a constraint written as a ``stamp'' \stamp\ (red if it is given and blue if it is derived), and the respective claims are written in deep-red notes with white font. % (the colour is bolder to distinguish validity claims from (pink) claims  \corring\ to data constraints, and to emphasize the challenge of getting them satisfied). 
Claim derivation as such is shown with bold blue arrows:  
%(of lighter colour when they originate from a data constraint claim):
the common target claim  of a set of co-targeted blue arrows \frar{a_i}{\mathrm{C_i}}{\mathrm{C}}, $i=1...n$, means that C is derived from conjunction of C$_i$ %1,..,C_n$ 
and we write C \implBy C1\&.. \& Cn. 

When we need to distinguish a constraint $C$ and its claim, we will write the latter in the roman font as C. 




Now we are ready to reconstruct the style of the argument flow in the Example (but, unfortunately, not literally due to some logical discrepancies we have found in the Example, and our formal derivation procedure does not allow us to reproduce them). The top inference step is well-known in the SC literature \cite{}[J.Rushby]: C0\implBy C1 \& C2. %
%\footnote{There is no}
 Claim C1 is given, it remains to derive C2. This latter claim can be represented as a conjunction
 $ \claf{C2}   = \cmul{C2}{\hPro} \wedge \cval{C2}{\hPro}$
whose first component is \multy\ constraint [1] on the lower end of \asson\ \hPrtn: this is the data constraint part of C2,  and \cval{C2}{\hPr} is semantic validity check of \hPrtn\ \asson: the semantic part of claim C2. Identifying the data component part of a claim is 
 a principle step: we leave the land of propositional logic of claims and enter the land of first-order logic (FOL) over data, in which data drive the logical inference. Indeed, \asson\ \hPr\ can be represented as the sequential composition of \asson\ \Contt\ and \grProtn\ (further abbreviated as \ctt\ and \gPr) from Hazard to HazardGroup to ProtectionSystem. Hence, mutiplicity [1] of \hPr\ is a direct consequence of \multi s [1] on the lower ends of component associations \ctt\ and \gPr, \ie, $\cmul{C2}{\hPr}\implBy \cmul{A}{\ctt}\wedge\cmul{P}{\gpr}$ (see \figinf\ for claims A and P) 
 %
  Similarly, for semantic checks 
 $\cval{C2}{\hPr}\implBy \cval{A}{\ctt}\wedge\cval{P}{\gpr}$. Thus, 
 deriving C2 splits into two branches: the upper one deals with apportionment (hazard grouping) and we will refer to its constraints and claims by A with indexes, and the lower one deals with hazard group protection and we will refer to its constraints/claims by P with indexes. 
 
 Now we have pratically formal inference procedure: 

==> sections/sect2.tex <==
\section{sect2}
something else
\endinput

==> sections/summary.tex <==
\section{Assurance as conformance, revisited: Parts and colours of safety assurance}
\label{sec:assr-as-conf-rev}

\subsection{The main question: conformance vs. logic}
GSN-inspired but \wfp-realized safety case would consist of three conceptually different parts. %assurance consists of three stages, which result in three main parts of a safety case.  

{\bf Part 1.} The SEP definition workflow \wfsepdef, is to be provided. It includes all process and dataflow (green and orange), including reviewing (violet), and, importantly, constraints (red) over data and dataflow. 

{\bf Part 1*.} From constraints given in Stage 1, new constraints/claims are derived (blue), and the corresponding inference tree eventually results in the top safety claim. 

{\bf Part 2.} The SEP execution workflow for system $X$ is to be provided, $\wfsepexe(X)$, and demonstrated that the execution conforms to the definition, $\wfsepexe(X)\confcheck{\instan}{}\wfsepdef$. Specifically, the execution instance has to satisfy all given (red) constraints (which GSN would call ``the body of evidence''). Then, by the transitive soundness of inference (see \secdercon), we conclude that the instance satisfies the top safety claim too. 

Importantly, the blue inference can be seen as a ``proof'' of the safety claim if only each inference step is sound (\secdercon)--- this fundamental aspect of the argument flow is often underestimated in the GSN literature and, we believe, in the practice of writing safety cases in the GSN notation. Indeed, assuring soundness requires a justified strategy assigned to each decomposition/inference step, \ie, a strategy and its justification at each decomposition step are to be mandatory elements of GSN-based safety cases. However, the GSN syntax does not make a justified strategy a mandatory element, and many safety cases appearing in practice do use this liberty, \eg, the GSN Community example we considered above. 

Moreover, a majority of GSN decomposition steps are not of logical nature and show a process decomposition rather than logical inference. For example, suppose we want to provide a more detailed evidence for the claim  {\em HI: All hazards have been identified} (see \figinf) rather than just FHA reviewing. Then we need to decompose FHA into smaller subprocesses, then decompose the latter into smaller subroutines and so on, and \corring ly, FHA reviewing will be composed from more elementary reviewing acts. The result will be a refined SEP definition, over which we can build a refined inference tree, but the latter is actually not needed: as we have seen in  \sectref{DDD}, inference is a straightforward (and practically trivial) consequence of the process and data decomposition. The essence of deriving claim HI is in the FHA decomposition, and each step of such a decomposition is to be justified and be assured to be semantically sound in the following sense: if all subprocesses P of a process P are well done, then the process P is well done. Hence, the real goal of Part 1* is to assure the validity of SEP definition rather than logical inference. 


Now the major question: {\bf\em Why \wfsepdef, if properly executed for a system $X$, results in a safe system $X$}, can be answered as follows. {\em A proper execution of $\wfsepexe(X)$ results in a safe system $X$ because: a) the SEP definition is based on successful previous experience in dealing with systems similar to $X$; b) all novelties brought by $X$ were analyzed by experts and addressed according to general patterns of addressing such novelties, and the SEP definition was appropriately amended; c) ... (place here anything you consider important)...}. 

In the \wfp\ approach to assurance, the requirements a), b), c) are subsumed by an appropriately defined notion of conformance of the SEP definition workflow \wfsepdef\ to some virtual workflow \wfnorm, which models and integrates the set of all relevant  normative and guiding (formal and informal) documents into a workflow \wfnorm\ (the next section provides some detail).  Thus, Parts 1 and  1* of a generic safety case can be combined into 

{\bf Part 1$^+$:} Assuring that the SEP is properly defined by showing its conformance (as a workflow \wfsepdef) to some normative workflow \wfnorm\ (both are actually \wfp-objects). 

In general, this conformance can be managed similarly to the instance conformance we considered in the TR (Sect. 3-4). The next section provides some details. 
\paperGM{}{
\input{sections/conformToNorm}
}


==> sections/wf-formalDefs.tex <==
\newpage
\subsection{Processes as multiary model \trafon s}\label{sec:wf-formalDefs}
Ordinary algebraic operations are specified by their {\em arity (schema)} and {\em semantic mapping}. For example, a binary operation $f$ may have a schema $(A_1,A_2;B)$ with $A_1,A_2$ being names of two input sets and $B$ the name of the output set; sometimes these names are called {\em sorts}. Semantics is a function \frar{\semm{f}}{\semm{A_1}\timm\semm{A_2}}{\semm{B}}, where \semm{X} denotes the set corresponding to a sort $X$. The above patterns is applicable to multiary model transformations (MTs) with sorts being metamodels, which can be see as ``names'' for the \corring\ sets of instances: if $X$ is a metamodel, then \semm{X} denotes its set of instances. An essential distinction from the ordinary algebra is that while set names are structureless tokens, metamodels are rich structures that can overlap and we need to take this into account. It is natural to assume that all input metamodels ($A,B$ for our case) are disjoint as otherwise it is reasonable to merge them into a single input metamodel. However, overlapping of $A{\cup}B$ and $C$ %or $B$ and $C$ or both 
is a typical case as we have seen above, but we cannot merge them as input and output metamodels play different roles. Thus, for MTs, we need a more intelligent notion of an arity schema. 

\zd{ref to background section on CT}
  We assume given some universe (a category) \mmodcat\ of metamodels and metamodel mappings.
  \begin{defin}%[Metamodelling \fwk]
  	A {\bf\em metamodelling \fwk} is given by the following two components. a) A category \mmodcat, whose objects are called {\em metamodels} and morphisms are {\em metamodel maps}. Moreover, \mmodcat\ has coproducts, \ie, any two metamodels $M$ and $N$ can be (disjointly) merged into $M+N$, and there is an empty metamodel 0 such that $M+0=M$ for any $M$. We will call monic maps {\em injections}  and say that metamodel $M$ is {\em embedded} into metamodel $N$ if there is an injection \frar{i}{M}{N}. 
  	
  	b) A coproduct compatible functor from category \mmodcat\ to category \setcat\ of sets and functions. In detail, the following two conditions hold. 
  	
  	\noindent b1) Every metamodel $M$ is assigned with a set of its {\em instances} \semm{M} so that $\semm{M+N}=\semm{M}\times\semm{N}$. As the empty metamodel can be seen as the merge of the empty set of metamodels, $0=\coprod^\mmodcat_\varnothing$, we have  $\semm{0}=\prod^\setcat_\varnothing=1$ where $1=\{*\}$ is a fixed singleton set. 
  	
  	\noindent b2) Every metamodel map \frar{f}{M}{N} is assigned with a mapping \flar{f^*}{\semm{M}}{\semm{N}} between instance sets (note the reversal of the arrow) which is functorial, \ie, given $X\rTo^f Y\rTo^g Z$, $(f.g)^*=g^*.f^*$ and if \frar{\id_M}{M}{M} is identity metamodel map, then \flar{\id_M^*}{\semm{M}}{\semm{M}} is identity mapping of set \semm{M}. 
  	
  	In addition, we assume that \mmodcat\ has all finite limits and colimits, which would allow us to talk about general forms of metamodel intersection (via limits) and union (via colimit).
  \end{defin}
\begin{remark}
	In all applications we are interested in, if map \frar{f}{M}{N} is injection, %, \ie, metamodel $M$ is embedded into $N$ and can be seen as $M$'s sub-metamodel, 
	and $I\in\semm{N}$ is an instance, then instance $f^*(I)\in\semm{M}$ can be seen as the part of instance $I$ typed over $M$ (we will say $I$ is {\em projected} onto $M$). If $f$ is not injection, and glues together some elements, \eg, for two classes $c, c' \inn M$, $f(c)=f(c')=d$ in $N$, then all instances of $d$ will be duplicated by $f^*$: if for $I\in\semm{N}$, $I(d)$ is the set of instances of class $d$, then $f^*(I)(c)=f^*(I)(c')=I(d)$. Details of how it works can be found in \cite[chapter xx]{ehrigbook06} 
\end{remark}
\begin{defin}[Process arity]\label{def:arity} A {\em process library} is a pair $\pslib=(|\pslib|, S)$ with |\pslib| a set whose elements are called {\em processes}, and $S$ a mapping that assigns to each process $P\in|\pslib|$ its {\bf\em arity schema}, \ie, a triple $S(P)=(N, \inx, \out)$ where $N$ is a metamodel called the {\em inner} metamodel of $P$, $\inx$ is a finite family of injective maps into $N$, \frar{\inx_i}{A_i}{N}, $i=1..n$, whose sources $A_i$ are disjoint and called $P$'s {\em input} metamodels, and \flar{\out}{N}{B} is metamodel map into $N$ whose source is called $P$'s {\em output} metamodel. Thus, arity schema is given by the following diagram:
	\begin{equation}\label{eq:arity}
	\begin{diagram}[small]
	A_i &\rTo^{\inx_i}_{i=1..n}&N&\lTo^\out&B
\end{diagram}
\end{equation}
and we require all images $\inx_i(A_i)$ to be disjoint in $N$. Categorically, it can be formally specified by requiring the pullback of any two maps $\inx_i$, $\inx_j$ %, $j\noteq i$ 
to be empty: 
\begin{equation}\label{eq:disj}
A_i\times^{\inx_i}_{\inx_j} A_j=0 \mbox{ for any $j\noteq i$}
\end{equation}
	Below we will write $P\in\pslib$ for $P\in|\pslib|$. If needed, elements of a schema $S(P)$ will be superscripted with $P$, \eg, $N^P$ etc.
\end{defin}	

\medskip	
	The intuition behind the definition above is that process $P$ takes a tuple of data instances over its input metamodels, computes from them an instance over the inner metamodel, and then projects it onto metamodel $B$. %returns a data instance over its output metamodel. 
	Formally,
	\begin{defin}\label{def:semMap}For any process $P$, we assume given some mapping \frar{\semm{P_\inx}}{\prod_{i\le n}\semm{A_i}}{\semm{N}} called $P$'s {\bf\em inner semantic mapping}. {\bf\em (Full) semantic mapping} of $P$ (denoted \semm{P}) is the composition 
\begin{equation}\label{eq:semmap}
% \frar{\semm{P}\eqdef\semm{P_\inx};\out^*}%
%{\prod_{i\le n}}{\semm{B}} 
\begin{diagram}[small]
\prod_{i\le n}\semm{A_i} &\rTo^{\semm{P_\inx}}&\semm{N}&\rTo^{\out^*}&\semm{B}
\end{diagram}
 \end{equation}
 whose second component is provided by the metamodelling \fwk\ (see condition (b2) in \defref{arity}. %We denote this composition by \semm{P}. 
 
 In addition, we need to require that input data are not changed, \ie, equality \eqref{nosideEff} below holds for any input tuple $X_i\in\semm{A_i}$, $i\le n$:
 \begin{equation}\label{eq:nosideEff}
 (X_1...X_n).\semm{P_\inx}.\inx_i^*= X_i \mbox{ for all $i$}
 \end{equation}
\end{defin}
\begin{remark}[Why the output metamodel is different from the inner one?] %If $B=N$ and map \out\ is identity, then $\out^*$ is also identity and $\semm{P}=\semm{P_\inx}$. 
	Distinguishing the inner and the output metamodels may seem artificial (why should we care about inner data, which are not visible at the process output?) but is well justified in the context of assurance. If even some inner data  are not needed for other processes, the assessor of a safety case must check their correctness and validity. Note that the standard case when $B=N$ is readily simulated by setting map \out\ to the identity of $N$. 
\end{remark}
\begin{defin}[Source and sink processes]\label{def:arity+}We modify \defref{arity} by allowing the number of input maps to be 0, $n=0$, and hence the family of inout maps is empty so that 
	$\prod_\varnothing\semm{A_i}=1={*}$. Then mapping \frar{\semm{P_\inx}}{1}{\semm{N}} just selects some specific instance over $N$, and then mapping $\out^*$ projects the required part of this instance. Hence, the case $n=0$ corresponds to having a fixed constant data instance, \eg, those data shown in grey in our metamodel \figref{fig:WF+-ADV}. We call such processes {\em sources}. Dually, we allow the output metamodel $B$ to be empty so that the process always produces the trivial predefined singleton instance 1 for any input data; such a process acts as a ``black hole'' or {\em sink}. 
\end{defin}

\medskip
For specifying networks of processes, it is convenient to introduce process' ports (input and output) coupled with the \corring\ (input and output) metamodels, \eg, process $P$ in \figrii\ has two input and one output port. All our processes will have just one output port as this settign simplifies technicalities without the loss of generality: a process with $n$ output ports can be decomposed into $n$ processes with one output port (it is a standard algebraic setting for modelling $n$-coary operations). A \corring\ reformulation of Def.~\ref{def:arity}, \ref{def:arity+}, \ref{def:semMap} is straightforward and we omit it, but introduce ports in the metamodel in \figri.  %(by a process library we mean set of processes each assigned with its arity schema and supplied with a semantic mapping). 
\begin{remark}%[On portfree processes]
A process may have neither input nor output ports and hence be  isolated, but it still has an arity schema $0\rightarrow N \leftarrow 0$. 
\end{remark}
\begin{remark}
There is an important difference between a constant process $P_c$ with no input ports, which denotes some constant instance $c=\semm{P}(*)$ over the output metamodel, and a process $P_c^0$ with one input port and hence one input metamodel equal to 0. Such a process will produce instance $c=\semm{P}(*)$ only if signal $*$ is received at the input port and stay idle otherwise. Similarly, a process without the output port, simply absrobs all received data without producing anything visible while a process with the empty output metamodel produces a signal * at the output port (which can be seen as notification that some input data instance is received and processed). 
\end{remark}
=========

\zd{there is some piece in the source below this line but it's commented}

\endinput

Next we consider how processes are composed into a workflow.  We will begin with a high-level view of process composition in \sectref{wfMetamod-depFlow} and then refine it in an accurate data modelling \fwk\ in \sectref{wfMetamod-dataFlow}.

%\subsection{Composing processes into workflow}

%\input{figures/wfMetamod-full}
%\input{figures/wfExample-depFlow}

\subsection{Composing processes into workflow, 1: Dependency flow}\label{sec:wfMetamod-depFlow}
The world of assurance consists of processes (Ps) and work products (WP) (cf. \citeiso): the former produce the latter, which are then used to feed the former. A generic example is shown in \figrii, which says that each of the products WP1, WP2 is jointly created by processes $P$ and $P'$, some part of WP1 is the input for $Q$ and another part is an input for $Q'$, but the latter also need the second input from WP2. Note that an arrow from a WP to a port means that some part of WP is fed to that port, and two arrows from WP0 to $P$ mean that the latter processes two parts of WP0 (in general, different, but it may happen that the same part is fed to different ports-- we will explain how it works later in \sectref{wfMetamod-dataFlow}). 


 Arrows specifying the flow will be referred to as {\em wires} and they are of two types: wires from ports to WP and from WP to ports. 
 \begin{defin}[Dependency flow] A {\em dependency flow} over a process library (\pslib, \iptset, \optset)  is given by a set of metamodels $\wpset\subset\xob{\mmodcat}$ called {\em work product metamodels} or just {\em WPs}, and two flow relations , $\wptopt\subset\wpset\times\iptset$ and $\pttowp\subset\optset\times\wpset$, whose elements are called wires. 
\end{defin}
 The left half of \figriii\ (shaded in grey) presents the \corring\ metamodel, in which wires are specified by (white) classes \wptopt\ and \pttowp\ supplied with \from\ and \too\ associations, % to WP and in/outPort classes, 
 and two [key] constraints say that a wire is fully determined by its ends, \ie,  sharing a source port or a target port is allowed, but sharing both ends is prohibited (hence, classes \wptopt\ and \pttowp\ are relations rather than multirelations). Associations $\from'$ and $\too'$ to class Process shown in blue are derived by composition: %(note also backslash prefixes in their names): 
these associations specify the dependency flow between WP and processes, and we will denote the \corring\ relations by \wptops\ and \pstowp\ (the former is actually a multirelation as miltiple wires from a WP to a Process are possible, \eg, from WP0 to P in \figrii.). Relational composition $\pstops\eqdef \pstowp\Join \wptops$ is a binary (multi)relation on processes, and we require it to be acyclic. This assumption greatly simplifies the mathematical model, and holds in all SEP instances we have been dealing with. 

We will also need the following dependability relation \wptowp\ between WPs. We first consider processes as relationships between input and outports (note dashed arrows between ports within process blocks in \figrii). Then we compose three relations: $\wptowp\eqdef\wptopt\Join\Process\Join\pttowp$. It can be shown that if \pstops\ si acyclic, then \wptowp\ is acyclic and conversely. 
\begin{defin} A dependency flow is {\em acyclic} if relations \pstops\ and \wptowp\ are acyclic.
\end{defin}

%\input{figures/wfMetamod-flow}
%\input{figures/wfMetamod-full}
%\input{figures/wfExample-dataFlow}

\subsection{Composing processes into workflow, 2: Data algebra underlying the dependency flow}\label{sec:wfMetamod-dataFlow}

\begin{defin}The {\em metamodeling carrier} of a dependency flow 
	
\end{defin}
%\zd{not finished yet} % ; i guess it'd take about yet another page}

==> sections/wfExample-comp.tex <==
\subsection{Compositionality of WF+}\label{sec:comp}

{\em Compositionality} of a workflow formalism refers to the possibility of considering a complex workflow as an elementary block so that we can consider a workflow of workflows, and reiterate this again. For example, we may need to consider the entire workflow \niw\ in \figri\ as a process, say, \wasp, with two input ports with metamodels $\In_1(\wasp)\eqdef\MM(W)$ and $\In_2(\wasp)\eqdef\MM(W')$, and the output port with $\Out(\wasp)=\MM(U)$. 
We need also to define metamodel $\Inner(P)$ and the semantic function, which is non-trivial. Compositionality is a fundamental requirement allowing us to manage complex behaviours by their hierarchical decomposition. Due to space limitations, we will juts present a rough sketch of how WF+ models can be encapsulated as process and refer to \citetr\ for details. %Below we describe a compositional mechanism for WF+ using our running example. %The construction is essentially categorical, and we will describe it semi-formally referring to \citetr\ for details.%

\zd{the peice below is too long, it should be just a brief para}

\zd{A few words why using CT is unavoidable}


 \zdhll{The inner metamodel is the colimit of the entire diagram of metamodels and maps in \figri(b): $\Inner(\wasp)\eqdef \colim\niw$ (= the disjoint union of all metamodels involved modulo factorization by all maps between the metamodels). As with any colimit, all metamodel in \figri(b), inclusing $\MM(W)$, $\MM(W')$ and $\MM(U)$, are mapped into it, which gives us the arity schema \eqref{arity} of process 
\wasp. %maps \frar{\inx_i}{\In_i(\wasp)}{\Inner(\wasp)}, $i=1,2$ and \flar{\out}{\Inner(\wasp)}{\Out(\wasp)}. 
\\
Now we need to define the semantic function of \wasp,
$$\frar{\semm{\wasp_\inx}}
{\semm{\MM(W)}\times\semm{\MM(W')}}
	{\semm{\colim\niw}}.$$ 
For this, let us consider how instances are processed step by step. Suppose we have instances $X\in\semm{\MMx{W}}$, $X'\in\semm{\MMx{W'}}$ (%we again write $\MMx(W)$ for $\MM(W)$).
By projecting them along maps $\mm1$, $\mm2$, etc., we obtain instances over metamodels $\In1(P)$, $\In2(P)$ etc. These instances are processed by $P, P', P''$, which gives us instances $Y, Y', Y''$ over $\Out(P)$, $\Out(P')$, $\Out(P'')$. To instantiate metamodels $V$ and $V'$ we need to merge $Y$ with $Y'$ and $Y'$ with $Y''$, but due to the vertical overlapping considered above, we need intelligent merges modulo suitable \corring\ spans between instances. Thus, before we approach merging, we need to instantiate all \corring\ spans involved. This is done by applying PB operations to data graphs (see \citetr\ for detail), after which merging modulo \corrce s (colimit) provides correct instances $Y+Y'\in\semm{V}$ and $Y'+Y''\in\semm{V'}$. Then we repeat the procedure for processes $Q, Q'$ and instantiate all relevant metamodels including $U$ (via merging modulo \corrce s). 
\\
The last problem we need to manage is to prove the initial data preservation condition \eqref{putget}. The most challenging issue here is the interaction between PB and colimit operations, \eg, we need to prove that pulling back instance $Y'+Y''$ along maps $\nn''$ and $\nn'''$ results in, resp., instances  $Y'$ and $Y''$. It is known that this nice property does not hold in an arbitrary category, but it does hold when instances are specifiable as attributed types graphs---see textbook \cite{ehrigbook06} for details. %
Now, as processes $P'$ and $P''$ satisfy condition \eqref{putget} and by standard categorical results about pullbacks, we can prove that condition \eqref{putget} holds for $Y+Y''$ and similarly for $Y+Y'$ and then for $Z+Z'$ too. This finally proves that we have condition \eqref{putget} for the entire process \wasp. 
	\\
We assume that assigning sets of instances to metamodels is a) functorial and b) continuous (see \cite{me-entcs08} and \cite{uwe-acs15} for motivating discussion), so that  $\semm{\colim\niw}=\lim(\niw^{\op};\semm{\_})$, where the latter set is a subset of all those tuples $$(X_1\in\semm{M_1},\ldots,X_i\in\semm{M_i},\ldots, X_n\in\semm{M_n})$$ with $i$ running over all nodes in \niw, which 
%\comprfam{X\in\semm{M}}{M \in Nodes(\niw)}, which 	respect the maps in \niw, \eg, for $i=\In(P')$, $j=\Out(P')$ and $k=\Out(P'')$ equalities  $X_i.\ii^*=X_j.\oo^*$ and  $X_j.r'^*=X_k.r''^*$ hold. Thus, for any two instances $X\in\semm{\MMx{W}}$ and $X'\in\semm{\MMx{W'}}$, we need to define instances $X_i\in\semm{M_i}$ for all other nodes $i$ and prove the \corrce\ equalities as above. We show this in \citetr. 
}{the peice is too long, it should be just a brief para}{-25em}


==> sections/wfExample-corrs.tex <==
\subsubsection{Dataflow correspondences}\label{sec:corrs}

A distinctive feature of WF+ is the overlap of the input and output data, or {\em horizontal} overlapping if the dataflow is oriented horizontally as in \figri. Somewhat unexpectedly, it implies {\em vertical} overlapping between metamodels. % To ease reading formulas below, we will merely write $W$ for the metamodel $\MM(W)$ of a work product $W$. 

\zd{The rest of the section is outdated and to be updated, and shortened as much as possible.}
Consider, \eg, metamodel $\MMx{V'}$ in \figri(b). It is produced by processes $P'$ and $P''$, which may use the same input data if (images of) maps $\mm'2$ and $\mm''$ overlap  in $\MMx{W'}$. 
%
This overlap causes overlap between $P'$'s and $P''$'s outputs due to the following. In each of the processes $P', P''$, we can specify the intersection of the input and output metamodels, $\Inout{}(P)$ and $\Inout{}(P'')$, resp. More accurately, an intersection is a span \eg, the upper one is the span $(\Inout{2}(P'), \ii'_2,\oo'_2)$ whose legs map the shared part into the resp. metamodels, and analogously for $\Inout{}(P'')$. The heads of the intersection spans are mapped to $W'$ by composed maps $\im'2=\ii'2.\mm'2$ and $\im''=\ii''.\mm''$.  If these two mappings have a non-empty overlap in $\MMx{W'}$, say, $O$, then when an instance $X'\in\semm{W'}$ is projected to $X'_2\in \semm{\In_2(P')}$ along $\mm'2$ and to $X''\in\semm{ \In(P'')}$ along $\mm''$, then elements of $X'$ typed over $O$ (which form a sub-instance $X'_O\subset X$) will be preserved in both outputs, %
$Y'= \semm{P'}(X, X')\in\semm{\Out(P')} $ (where $X$ is an arbitrary instance over \MMx{W}) and 
$Y''=\semm{P''}(X')    \in\semm{\Out(P'')}$. 
%
 Hence, to avoid their duplication when the two outputs are merged to form product $V'$, we need to specify the \corrce s between them explicitly by span $$\nicorrinst(V')=\left( (X'_O)^*,\ovr{r'},\ovr{r''}\right)$$ whose elements are derived by applying a series of pullbacks: $\Corr(V')=\pbop(\im'2,\im'')$, $(X'_O)^*=X'_O.(\im2,\im'')^*$ and $\ovr{r'}, \ovr{r''}$ are lifts of maps $r'', r''$ (cf. \figro) so that the  data span \nicorrinst\ is typed over metamodel span $$\nicorrmmod(V')=(\Corr(V'), r', r''),$$
 and, moreover, the head of the instance span is the common projection of the two instances at the targets of legs, \ie, $(X'_O)^*=Y'.\r'^*=Y''.r''^*$. Then we write $\nicorrinst\inn\semm{\nicorrmmod}$.
 In \citetr\ we show how all these instances and mappings are formally derived by applying categorical operations.
%
% $\Inout(P')$ and $\Inout(P'')$ have {\em semantically shared} elements collected in metamodel $\Corr(V')$ (recall that we begin our analysis from metamodel $\MMx{V'}$). 
%
%By composing maps from \Corr\ to \Inout s with maps from \Inout s to \Out s, we get maps $r', r''$ from $\Corr$ to \Out s so that the triple $(\Corr(V'), r', r'')$ specify a relationship between $\Out(P')$ and $\Out(P'')$; we will call such triples {\em correspondence spans} (with {\em head} $\Corr(V')$ and {\em legs} $r', r''$).  
%\endinput

%===
We emphasize that span $\nicorrinst\inn\semm{\nicorrmmod}$ is an important part of the dataflow as it essentially affects product $V'\in\semm{\MMx{V'}}$: the latter is obtained by merging instances $Y'\in\semm{\Out(P')}$ and $Y''\in\semm{\Out(P'')}$ modulo \nicorrinst\ data, \ie, we first merge $Y'$ and $Y''$ disjointly and then glue together elements that are images of the same element in $(X'_O)^*$. In CT, the operation of merging without duplication modulo a \corring\ span is called {\em colimit} (note the label in the diagram). 

%===
In the same way, we specify correspondences over horizontal overlap between metamodels $\MMx{V}$ and $\MMx{W}$, but as there are two paths from the latter to the former within process $P$, we have two \corrce\ spans $\Corr11(V)$ and $\Corr21(V)$ as shown  in \figri(b) (\Inout{}\ metamodels are omitted).  Then metamodel $\MMx{V}$ is formed by the colimit modulo two \corrce\ spans. 
%\endinput
Finally, note that the triple $(Out(P'), \nn', \nn'')$ is a span specifying \corrce s between metamodels $\MMx{V}$ and $\MMx{V'}$. 
%
Thus, if even two initial metamodels \MMx{W} and \MMx{W'} are disjoint, metamodels \MMx{V} and \MMx{V'} may overlap---this feature of WF+ essentially differs it from ordinary block diagrams. 

The constructs above are specified by the extension of the framed part in \figrii(a) to a full metamodel of WF+, which is the merge of parts (a) and (b). 


==> sections/wfExample-dataFlow.tex <==
%\subsection{WF+ via an example, 2}
\subsection{Semantics: Dataflow definition and execution in WF+}
\label{sec:dataflow}

The dataflow schema in \figri\ %(reproduced in \figriii(a))
is a very abstract view of workflow: it only shows directions of dataflow and hence dependencies between products and processes, but does not actually describe the content of dataflow. From the schema, we cannot infer what data constitute products, and how these data are fed to process ports, \eg, how product W's data fed to ports 1 and 2 overlap, and what part of V is provided by process P and what part by P'. To answer these questions, schema in \figri\  is to be supplied with a {\em dataflow definition} diagram shown in \figriii, whose nodes are metamodels and arrows are metamodel maps. %pings (we will say {\em maps}).

%\input{figures/wfExample-dataFlow}
\input{figures/wfExample-full} % #2
%All nodes in this diagram are metamodels: 
To visualize relationships between diagrams in \figri\ and \figriii,  metamodels \corring\ to products and ports are orange and yellow resp., black rectangles denote processes' {\em inner} metamodels, which together with \inx\ and \out\ mappings make process arity schemas. %, we will soon describe how they are related to input and output metamodels), and 
Blue rectangles denote metamodels specifying \corrce s between processes:  these metamodels are derived from other metamodels and maps in the diagram as we will describe below. %, but for a while, blue metamodels may be ignored). 

\endinput

All metamodels maps are assumed to be injective, \ie, arrows denote metamodel embeddings. Each such embedding, say, \flar{e}{M}{N} defines a simple data transformation %\flar{f^*}{\semm{M}}{\semm{N}} 
of the \corring\ instances: if $X$ is an instance of $N$, then by selecting its part typed over $M$, we get an instance $e^*(X)$ of $M$ (we will say $X$ is {\em projected to $M$ along} $e$). 
%
Formally, we specify an instance $X\in\semm{M}$ as a data graph $D_X$ with a typing mapping \frar{t_A}{D_X}{M}, and  the transformation is specified by applying the pullback operation (pb) to the pair of mappings $(t_A, e)$, which produces an instance $(D_Y, t_Y)$ over $N$ together with traceability map $\ovr{e}$ as shown in \figro, where nodes denoting derived data graphs are not framed and derived mappings are dashed. 
Hence, each metamodel map $e$ as above in assigned with a function \frar{e^*}{\semm{M}}{\semm{N}} where \semm{M}, \semm{N} denote sets of instances of the metamodels (note the reversal of direction of $e^*$). 
%\input{figures/sem-fwk}
Transformation via PB provides a compositional dataflow mechanism: having two consecutive maps $e, f$ as shown, the PB square (actually a rectangle) along composition $f.e$ is composed from two PB squares (it is a well-know fact, see, \eg, \cite{ehrigbook06}), \ie, for any instance $X\in\semm{M}$, we have $X.(f.e)^*= X.e^*.f^*$. 


Thus, according to \figri(b), a data instance $X$ over metamodel $\MM(W)$ will be transformed into instances $X1$ and $X2$ over ports 1 and 2 of process $P$  (\ie, over metamodels \corring\ to these ports) by projecting along maps $\mm1$ and $\mm2$. Data $X1$ and $X2$ may overlap or even coincide depending on how images of maps $\mm1$, $\mm2$ overlap in $\MM(W)$. But the internal data processing in process $P$ is defined irrespectively to whether data overlap or not, \ie, $P$ assumes the two data instances to be disjoint. Now we discuss how this internal procedure works. 

We suppose that all data produced by process $P$ are specified by a metamodel $\Inner(P)$ so that semantics of $P$ is given by a function \frar{\semm{P}}
    {\semm{\In_1(P)}\times\semm{\In_2(P)}}
	{\semm{\Inner(P)}}.
%
If the three metamodels above were discrete collections of classes, then we would require their disjointness to avoid side effects --- process $P$ should not  change the input data. However, typical data in our context are graphical, and a typical WF+ situation is when $P$ computes attributes of input data objects, or association links between them. As neither attributes nor associations can be declared without the \corring\ classes, the inner metamodel must include some or all of them. It may also happen that the inner metamodel must also include some input associations if, \eg, there is a constraint spanning an input association and a new computed association in $\Inner(P)$ (\eg, a joint multiplicity for two association ends). A general way to model such situations is to assume that each input metamodel is embeddable into the inner one by a map \frar{\inx_i}{\In_i(P)}{\Inner(P)}, $i=1..n$ where $n$ is  the number of input ports. 
But then we must require that input data are not changed by $P$, \ie, equality \eqref{putget} below holds for any tuple of input instances $X_i\in\semm{A_i}$, $i\le n$:
\begin{equation}\label{eq:putget}
(X_1...X_n).\semm{P_\inx}.\inx_i^*= X_i \mbox{ for all $i$}
\end{equation}
Finally, it may happen that not all of the inner data are actually needed at $P$'s output. The latter is specified by a metamodel $\Out(P)$ being a part of the inner metamodel given by a map \flar{\out}{\Inner(P)}{\Out(P)}. Then projection along \out\ would extract the part of the inner data to be visible at the output. 

In general, a process $P$ is given by its {\em arity schema} 
	\begin{equation}\label{eq:arity}
\begin{diagram}[small]
\In_i(P) &\rTo^{\inx_i}_{i=1..n}&\Inner(P)&\lTo^\out&\Out(P)
\end{diagram}
\end{equation}
and {\em semantic function} $\semm{P}=\semm{P_\inx}.\out^*$ as shown below
 \begin{equation}\label{eq:semmap}
 % \frar{\semm{P}\eqdef\semm{P_\inx};\out^*}%
 %{\prod_{i\le n}}{\semm{\Out(P)}} 
 \begin{diagram}[small]
 \prod_{i\le n}\semm{\In_i(P)} &\rTo^{\semm{P_\inx}}&\semm{N}&\rTo^{\out^*}&\semm{\Out(P)}
 \end{diagram}
 \end{equation}
(where symbol $\prod$ denotes the product operation on metamodels, see \citetr\ for details) such that condition \eqref{putget}  holds. 
\begin{remark}%[Why the output metamodel is different from the inner one?] %If $B=N$ and map \out\ is identity, then $\out^*$ is also identity and $\semm{P}=\semm{P_\inx}$. 
	Distinguishing the inner and the output metamodels may seem artificial (why should we care about inner data, which are not visible at the process output?) but is well justified in the context of assurance. If even some inner data  are not needed for other processes, the assessor of a safety case must check their correctness and validity. Note that the case when $\Out(P)=\Inner(P)$ is readily simulated by setting map \out\ to be the identity map. 
\end{remark}

\medskip
A metamodel specifying processes with their ports and metamodel assignment is shown in \figriv. Note that we admit processes without input or output ports, but they still have the input and the output metamodels considered to be empty. An accurate discussion of such processes can be found in \citetr. \zd{actually it's an important piece and it shoudl be in the paper if space allows. }




	  




 


%%\subsection{Composing processes into workflow, 2: Xata algebra underlying the dependency flow}\label{sec:wfMetamod-dataFlow}
%
%\begin{defin}The {\em metamodeling carrier} of a dependency flow 
%	\end{defin}

==> sections/wfExample-depFlow.tex <==
\subsection{Dataflow (dependency) schema}	\label{sec:depflow}

%Next we consider how processes are composed into a workflow.  We will begin with a high-level view of process composition in \sectref{wfMetamod-depFlow} and then refine it in an accurate data modelling \fwk\ in \sectref{wfMetamod-dataFlow}.

%\subsection{Composing processes into workflow}

\input{figures/wfExample-depFlow}
%\input{figures/wfExample-full} %#1
%\subsection{Composing processes into workflow, 1: Dependency flow}\label{sec:wfMetamod-depFlow}
The world of assurance consists of processes and work products  (cf. \citeiso): the former produce the latter, which are then used to feed the former. A generic example is shown in \figri(a) (ignore subfigure b) for a while), which shows five processes (green blocks) and five products (orange) interrelated by arrows or {\em wires} showing the dataflow. Process blocks actually refer to {\em occurrences} of processes $P, P'$ etc. (hence, colons) and the same process can occur in the same network multiple times; to simplify presentation,  we will assume that a process can occur in a network just once, and thus refer to blocks by their process names P, P' etc. %hence we can identify occurrences with process and refer to green blocks as to processes. 

Processes P, P' and Q' have two, and processes P'', Q one, {\em input} ports. All processes in \figri(a) have only one {\em output} port, which is our general assumption for any process---this setting simplifies technicalities without the actual loss of generality: a process with $n$ out-ports can be decomposed into $n$ processes with one out-port (it is a standard algebraic setting for modelling $n$-coary operations). Each of the wires WP1,WP2 and WP' says that some part of product W data goes to the \corring\ port (ports 1,2 in P and port 1 in P' resp.). The three parts  may coincide but, in general, are different and may overlap (or be disjoint) -- there are no general restrictions on this. Other wires from products to in-ports are treated similarly. Wires from out-ports to products show how products are built, \eg, wires PV and P'V  say that product V is composed from the output data of processes P and P' (and products V', U are produced by pairs (P',P'') and (Q,Q') resp.).  

Thus, a general schema of the data flow consists of a sequence of steps, each one consisting of three substeps: a) read data from w-products to in-ports, b) process data, c) write data from out-ports to w-products and merge them; \eg, in the example we have two steps 
$$(W,W')\rTo^{\mathrm{step 1}}_{\mathrm{a-b-c}}(V,V')
             \rTo^{\mathrm{step 2}}_{\mathrm{a-b-c}}U.
$$ We will discuss the underlying mechanisms in \secref{??}, but before that, some important technical details are in order. 

%\input{figures/wfMetamod-full-vert}
%\input{figures/wfMetamod-full-horiz}
An accurate metamodel specifying diagrams like in \figri(a) is shown in the framed fragment of \figrii(a).  Wires are specified by (dark grey) classes \wptopt\ and \pttowp\ supplied with \from\ and \too\ associations. Following CT, we call a triple like $(\wptopt,\from,\too)$ a {\em span}, node \wptopt\ is its {\em head}, arrows \from, \too\ are {\em legs} and legs' target nodes are {\em feet}. We will often refer to a span by its head if the legs are clear from the context. % to WP and in/outPort classes, 
 Thus, wires are specified by spans \wptopt\ and \pttowp. Two [key] constraints declared for these spans demand a wire to be fully determined by its ends, \ie,  two different wires can share the source or the  target, but sharing both ends is prohibited (\ie, classes \wptopt\ and \pttowp\ are relations rather than multirelations). Note associations $\from'$ and $\too'$ to class Process shown in blue, whcih are derived by composition: 
 %for a wire $w:\wptopt$, 
 $\too'=\too.\owner$ and $\from'=\from.\owner$ (where \owner\ is the black-diamond end name).%
 \footnote {We follow UML and prefix the names of derived elements by backslah, and colour them in blue to suggest ``mechanical/algebraic derivation''.}
  Then span $\wptopt'=(\wptopt,\from,\too')$ 
  %(we call such triples {\bf \em spans} with node \wptopt\ being its {\bf\em head} and arrows \from\ and $\too'$ its {\bf\em legs}) 
  gives us a (mutli)relation from WorkProduct to Process (note two wires between product W and process P in \figri(b) which show that the span is a multirelation). Similarly, span $\pttowp'=(\pttowp,\from',\too)$ is a relation from Process to WorkProduct (not a multi-relation as each process has only one out-port).   %these associations specify the dependency flow between products and processes, and we will denote the \corring\ relations by \wptops\ and \pstowp\ (the former is actually a multirelation as miltiple wires from a product to a process are possible, \eg, from W to P in \figri.). 
 Relational composition $\pstops\eqdef \pstowp'\Join \wptops'$ is a binary (multi)relation on processes, and we require it to be acyclic. This assumption greatly simplifies the mathematical model, and holds in all SEP instances we have been dealing with. 

%\zdmodd{We will also need the following relation \wptowp\ between WPs. We first consider processes as relationships between input and outports (note dashed white arrows between ports within process blocks in \figri). Then we compose three relations: $\wptowp\eqdef\wptopt\Join\Process\Join\pttowp$. It can be shown that if \pstops\ is acyclic, then \wptowp\ is acyclic and conversely, and we include this constraint in the metamodel. }{}{Maybe this piece is not needed}{-8em}
%\begin{defin} A dependency flow is {\em acyclic} if relations \pstops'\ and \wptowp\ are acyclic.
%\end{defin}
\begin{remark}
Note two encircled multiplicities in \figrii(a). The left one says that only one wire can come to an in-port, and hence an in-port reads one and only one piece of data; thus, there is no data merge at ports. The right one says that any out-port has at least one wire that takes its data and hence any out-port writes to at least one product.
\end{remark} 
\begin{remark}We admit processes without in-ports, which provide predefined information like in standards (such processes were coloured grey in \figref{?}). We also admit processes without out-ports, which can be seen as garbage collectors. 
\end{remark}




==> sections/wfExample-mech.tex <==
\subsection{Dataflow mechanisms, 1: Reading and Writing}
\label{sec:dataflow}

Let \flar{e}{M}{N} be an injective mapping from metamodel $N$ to metamodel $M$ (we will say $e$ is a map from $N$ to $M$). 
%Reading or translating a data instance $X$ over $M$ to $N$
%All metamodels maps are assumed to be injective, \ie, arrows denote metamodel embeddings. Each such embedding, say, \flar{e}{M}{N} defines a simple data transformation %\flar{f^*}{\semm{M}}{\semm{N}} 
%of the \corring\ instances: if 
If $X$ is an instance of $M$, then by selecting its part typed over $N$, we get an instance $e^*(X)$ of $N$: we will say $X$ is {\em projected} to $M$ (or {\em read} into $M$) along $e$. 
%
Formally, we specify an instance $X\in\semm{M}$ as a data graph $D_X$ with a typing mapping \frar{t_A}{D_X}{M} (see \figro(a)), and  the transformation is specified by applying the pullback operation (pb) to the pair of mappings $(t_A, e)$: this operations produces an instance $(D_Y, t_Y)$ over $N$ together with traceability map $\ovr{e}$ as shown in \figro(a). %, where nodes denoting derived data graphs are not framed and derived mappings are dashed. 
Hence, each metamodel map $e$ as above in assigned with a function \frar{e^*}{\semm{M}}{\semm{N}} where \semm{M}, \semm{N} denote sets of instances of metamodels (note that the arrow direction is reversed). %e reversal of direction of $e^*$). 
%%%%%%%%
\input{figures/sem-fwk}
%%%%%%%%
Transformation via PB provides a compositional dataflow mechanism: having two consecutive maps $e, f$ as shown, the PB square (actually a rectangle) along composition $f.e$ is composed from two PB squares (it is a well-know fact, see, \eg, \cite{ehrigbook06}), \ie, for any instance $X\in\semm{M}$, we have $X.(f.e)^*= X.e^*.f^*$. 

\papertr{}{% TR}
Writing is explained by diagram (b). In simple cases, writing is merely composition of mappings: if $Y=e_*(X)$ then $D_Y=D_X$ and $t_Y=t_x.e$. However, so obtained instance $Y$ can violate constraints in $N$ and hence should be amended. Thus, in general, writing is implemented by an operation \gen\ more intelligent than mapping composition. It is required to be compositional: $X.(e.f)_*=X.e_*.f_*$. Moreover, ... \Write\Read-law  ....  
}
Now we consider writing with merging specified in \figro(b).
\zd{To be written. It would need 0.5 column approx}

\zdmod{Thus, according to \figri(b), a data instance $X$ over metamodel $\MM(W)$ will be transformed into instances $X1$ and $X2$ over ports 1 and 2 of process $P$  (\ie, over metamodels \corring\ to these ports) by projecting along maps $\mm1$ and $\mm2$. Data $X1$ and $X2$ may overlap or even coincide depending on how images of maps $\mm1$, $\mm2$ overlap in $\MM(W)$. But the internal data processing in process $P$ is defined irrespectively to whether data overlap or not, \ie, $P$ assumes the two data instances to be disjoint. Now we discuss how this internal procedure works.}{to go below} {}

\subsection{Dataflow mechanisms 2: Inside of (custom) processes}
Let $P$ be a general process with two in-ports as in \figri. %We suppose that all data produced by $P$ are specified by a metamodel $\Inner(P)$ so that 
To specify semantics of $P$, we assume that each of the ports is assigned with a \corring\ metamodel, and then semantics is given by a function 
%Semantics of $P$ is given by a function 
\frar{\semm{P}}
    {\semm{\In_1(P)}\times\semm{\In_2(P)}}
	{\semm{\Out(P)}}.
%
If the three metamodels above were discrete collections of classes, then we would require their disjointness to avoid side effects --- process $P$ should not  change the input data. However, typical data in our context are graph-based, and a typical WF+ situation is when $P$ computes attributes of input data objects, or association links between them. As neither attributes nor associations can be declared without the \corring\ classes, the output metamodel must include some or all input classes. It may also happen that the output metamodel must also include some input associations if, \eg, there is a constraint spanning an input association and a newly computed association in $\Out(P)$ (\eg, a joint multiplicity for two association ends). Thus, metamodels $\In_i(P)$ and $\Out(P)$ may overlap, and a general way to model such situations is to assume that all three metamodels are embeddable into some all-embracing inner metamodel $\Inner(P)$; in the general case, we have the following diagram of metamodel maps
\begin{equation}\label{eq:arity}
\begin{diagram}[small]
\In_i(P) &\rTo^{\inx_i}_{i=1..n}&\Inner(P)&\lTo^\out&\Out(P)
\end{diagram}
\end{equation}
(where $n$ is the number of in-ports), which we call the {\em arity schema} of process $P$. 
%
Then semantic function of $P$ consists of two components: the first generates inner data from the input data and the second reads from the inner data to the output: %writes input data into the inner metamodel 
 \begin{equation}\label{eq:semmap}
\begin{diagram}[small]
\prod_{i\le n}\semm{\In_i(P)} &\rTo^{\semm{P_\inx}}&\semm{N}&\rTo^{\out^*}&\semm{\Out(P)}
\end{diagram}
\end{equation}
(where symbol $\prod$ denotes the product operation on metamodels, see \citetr\ for details) so that $\semm{P}=\semm{P_\inx}.\out^*$.

An important condition to impose on any semantic function is to require that input data are not changed by $P$, \ie, equality \eqref{putget} holds for any tuple of input instances $X_i\in\semm{A_i}$, $i\le n$:
\begin{equation}\label{eq:putget}
(X_1...X_n).\semm{P_\inx}.\inx_i^*= X_i \mbox{ for all $i$}
\end{equation}
%Finally, it may happen that not all of the inner data are actually needed at $P$'s output. The latter is specified by a metamodel $\Out(P)$ being a part of the inner metamodel given by a map \flar{\out}{\Inner(P)}{\Out(P)}. Then projection along \out\ would extract the part of the inner data to be visible at the output. 

\begin{remark}%[Why the output metamodel is different from the inner one?] %If $B=N$ and map \out\ is identity, then $\out^*$ is also identity and $\semm{P}=\semm{P_\inx}$. 
	We do  not require that output metamodel be isomorphic to the inner one, it can be smaller which means that only part of the inner data are sent to the out-port. This difference  may seem artificial (why should we care about inner data, which are not visible at the process output?) 
	but is well justified in the context of assurance. If even some inner data  are not needed for other processes, the assessor of a safety case must check their correctness and validity. Note also that the case when $\Out(P)=\Inner(P)$ is readily simulated by setting map \out\ to be the identity map. 
\end{remark}

\medskip
A metamodel specifying processes with their ports and metamodel assignment is shown in \figriv. Note that we admit processes without input or output ports, but they still have the input and the output metamodels considered to be empty. An accurate discussion of such processes can be found in \citetr. \zd{actually it's an important piece and it shoudl be in the paper if space allows. }


==> sections/wfExample-mechanisms.tex <==
%\subsection{WF+ via an example, 2}
\subsection{Dataflow mechanisms, 1: Reading and (joint) writing
	Semantics: Dataflow definition and execution}
\label{sec:dataflow}

The dataflow schema in \figri(a) is a very abstract view of workflow: it only shows directions of dataflow and hence dependencies between products and processes, but does not actually describe the content of dataflow. From the schema we cannot infer what data constitute products, and how these data are fed to process ports, \eg, how product W's data fed to ports 1 and 2 overlap, and what part of V is provided by process P and what part by P'. To answer these questions, schema (a)  is to be supplied with a {\em dataflow definition} diagram shown in \figri(b), whose nodes are metamodels and arrows are metamodel mappings (we will say {\em maps}).

%\input{figures/wfExample-dataFlow}
%\input{figures/wfExample-full} % #2
%All nodes in this diagram are metamodels: 
To visualize relationships between diagrams (a) and (b),  metamodels \corring\ to products and ports are orange and yellow resp., white rectangles denote processes' {\em inner} metamodels (roughly \corring\ to internal process arrows in \figri(a), we will soon describe how they are related to input and output metamodels), and blue rectangles denote metamodels specifying \corrce s between processes (these metamodels are derived from other metamodels and maps in the diagram as we will describe below, but for a while, blue metamodels may be ignored). 

All metamodels maps are assumed to be injective, \ie, arrows denote metamodel embeddings. Each such embedding, say, \flar{e}{M}{N} defines a simple data transformation %\flar{f^*}{\semm{M}}{\semm{N}} 
of the \corring\ instances: if $X$ is an instance of $N$, then by selecting its part typed over $M$, we get an instance $e^*(X)$ of $M$ (we will say $X$ is {\em projected to $M$ along} $e$). 
%
Formally, we specify an instance $X\in\semm{M}$ as a data graph $D_X$ with a typing mapping \frar{t_A}{D_X}{M}, and  the transformation is specified by applying the pullback operation (pb) to the pair of mappings $(t_A, e)$, which produces an instance $(D_Y, t_Y)$ over $N$ together with traceability map $\ovr{e}$ as shown in \figro, where nodes denoting derived data graphs are not framed and derived mappings are dashed. 
Hence, each metamodel map $e$ as above in assigned with a function \frar{e^*}{\semm{M}}{\semm{N}} where \semm{M}, \semm{N} denote sets of instances of the metamodels (note the reversal of direction of $e^*$). 
\input{figures/sem-fwk}
Transformation via PB provides a compositional dataflow mechanism: having two consecutive maps $e, f$ as shown, the PB square (actually a rectangle) along composition $f.e$ is composed from two PB squares (it is a well-know fact, see, \eg, \cite{ehrigbook06}), \ie, for any instance $X\in\semm{M}$, we have $X.(f.e)^*= X.e^*.f^*$. 


Thus, according to \figri(b), a data instance $X$ over metamodel $\MM(W)$ will be transformed into instances $X1$ and $X2$ over ports 1 and 2 of process $P$  (\ie, over metamodels \corring\ to these ports) by projecting along maps $\mm1$ and $\mm2$. Data $X1$ and $X2$ may overlap or even coincide depending on how images of maps $\mm1$, $\mm2$ overlap in $\MM(W)$. But the internal data processing in process $P$ is defined irrespectively to whether data overlap or not, \ie, $P$ assumes the two data instances to be disjoint. Now we discuss how this internal procedure works. 

We suppose that all data produced by process $P$ are specified by a metamodel $\Inner(P)$ so that semantics of $P$ is given by a function \frar{\semm{P}}
    {\semm{\In_1(P)}\times\semm{\In_2(P)}}
	{\semm{\Inner(P)}}.
%
If the three metamodels above were discrete collections of classes, then we would require their disjointness to avoid side effects --- process $P$ should not  change the input data. However, typical data in our context are graphical, and a typical WF+ situation is when $P$ computes attributes of input data objects, or association links between them. As neither attributes nor associations can be declared without the \corring\ classes, the inner metamodel must include some or all of them. It may also happen that the inner metamodel must also include some input associations if, \eg, there is a constraint spanning an input association and a new computed association in $\Inner(P)$ (\eg, a joint multiplicity for two association ends). A general way to model such situations is to assume that each input metamodel is embeddable into the inner one by a map \frar{\inx_i}{\In_i(P)}{\Inner(P)}, $i=1..n$ where $n$ is  the number of input ports. 
But then we must require that input data are not changed by $P$, \ie, equality \eqref{putget} below holds for any tuple of input instances $X_i\in\semm{A_i}$, $i\le n$:
\begin{equation}\label{eq:putget}
(X_1...X_n).\semm{P_\inx}.\inx_i^*= X_i \mbox{ for all $i$}
\end{equation}
Finally, it may happen that not all of the inner data are actually needed at $P$'s output. The latter is specified by a metamodel $\Out(P)$ being a part of the inner metamodel given by a map \flar{\out}{\Inner(P)}{\Out(P)}. Then projection along \out\ would extract the part of the inner data to be visible at the output. 

In general, a process $P$ is given by its {\em arity schema} 
	\begin{equation}\label{eq:arity}
\begin{diagram}[small]
\In_i(P) &\rTo^{\inx_i}_{i=1..n}&\Inner(P)&\lTo^\out&\Out(P)
\end{diagram}
\end{equation}
and {\em semantic function} $\semm{P}=\semm{P_\inx}.\out^*$ as shown below
 \begin{equation}\label{eq:semmap}
 % \frar{\semm{P}\eqdef\semm{P_\inx};\out^*}%
 %{\prod_{i\le n}}{\semm{\Out(P)}} 
 \begin{diagram}[small]
 \prod_{i\le n}\semm{\In_i(P)} &\rTo^{\semm{P_\inx}}&\semm{N}&\rTo^{\out^*}&\semm{\Out(P)}
 \end{diagram}
 \end{equation}
(where symbol $\prod$ denotes the product operation on metamodels, see \citetr\ for details) such that condition \eqref{putget}  holds. 
\begin{remark}%[Why the output metamodel is different from the inner one?] %If $B=N$ and map \out\ is identity, then $\out^*$ is also identity and $\semm{P}=\semm{P_\inx}$. 
	Distinguishing the inner and the output metamodels may seem artificial (why should we care about inner data, which are not visible at the process output?) but is well justified in the context of assurance. If even some inner data  are not needed for other processes, the assessor of a safety case must check their correctness and validity. Note that the case when $\Out(P)=\Inner(P)$ is readily simulated by setting map \out\ to be the identity map. 
\end{remark}

\medskip
A metamodel specifying processes with their ports and metamodel assignment is shown in \figriv. Note that we admit processes without input or output ports, but they still have the input and the output metamodels considered to be empty. An accurate discussion of such processes can be found in \citetr. \zd{actually it's an important piece and it shoudl be in the paper if space allows. }




	  




 


%%\subsection{Composing processes into workflow, 2: Xata algebra underlying the dependency flow}\label{sec:wfMetamod-dataFlow}
%
%\begin{defin}The {\em metamodeling carrier} of a dependency flow 
%	\end{defin}

==> sections/wfExample-schema.tex <==
\subsection{Dataflow (dependency) schema}	\label{sec:depflow}

%Next we consider how processes are composed into a workflow.  We will begin with a high-level view of process composition in \sectref{wfMetamod-depFlow} and then refine it in an accurate data modelling \fwk\ in \sectref{wfMetamod-dataFlow}.

%\subsection{Composing processes into workflow}

\input{figures/wfExample-schema}
%\input{figures/wfExample-full} %#1
%\subsection{Composing processes into workflow, 1: Dependency flow}\label{sec:wfMetamod-depFlow}
The world of assurance consists of processes and work products  (cf. \citeiso): the former produce the latter, which are then used to feed the former. A generic example is shown in \figri, %(ignore subfigure b) for a while), 
which shows five user-defined processes (green blocks), one predefined standard process Id (idle or identity), which outputs input data without any change,  and five products (orange) interrelated by arrows or {\em wires} showing the dataflow. Process blocks actually refer to {\em occurrences} of processes $P, P'$ etc. (hence, colons) and the same process can occur in the same network multiple times; to simplify presentation,  we will assume that a process can occur in a network just once, and thus refer to blocks by their process names P, P' etc. %hence we can identify occurrences with process and refer to green blocks as to processes. 

Processes P, P' and Q' have two, and processes P'', Q one, {\em input} ports. All processes in \figri\ have only one {\em output} port, which is our general assumption for any process---this setting simplifies technicalities without the actual loss of generality: a process with $n$ out-ports can be decomposed into $n$ processes with one out-port (it is a standard algebraic setting for modelling $n$-coary operations). Each of the wires WP1,WP2 and WP' says that some part of product W data goes to the \corring\ port (ports 1,2 in P and port 1 in P' resp.). The three parts  may coincide but, in general, are different and may overlap (or be disjoint) -- there are no general restrictions on this. Other wires from products to in-ports are treated similarly. Wires from out-ports to products show how products are built, \eg, wires PV and P'V  say that product V is composed from the output data of processes P and P' (and products V', U are produced by pairs (P',P'') and (Q,Q') resp.).  

Thus, a general schema of the data flow consists of a sequence of steps, each one consisting of three substeps: a) read data from products to in-ports, b) process data, c) write data from out-ports to products and merge them; \eg, in the example we have two steps 

\smallskip
$\qquad\qquad(W,W')\rTo^{\mathrm{step 1}}_{\mathrm{a-b-c}}(V,V')
             \rTo^{\mathrm{step 2}}_{\mathrm{a-b-c}}U,
$

\smallskip
\noindent  
each one consisting of several processes working in parallel but interacting due to data sharing (to wit: (P, P', P'') for step 1 and (Q,Q', Id) for step 2) and with several reading and writing subprocesses. In general, it is quite possible that data produced at step N will then be used at step N+K rather than N+1, but to unify the formalities, we introduce a chain of one or more idle processes (like, \eg, in \figri, a part of V'-data is not actually used at Step 2, but the idle process Id moves it further) so that we can assume that all data produced at Step N are consumed at Step N+1 (with Id processes added as needed). This assumption makes data provenance complete and thus has a direct assurance relevance. 
We will discuss the underlying mechanisms in \secref{??}, but before that, some important technical details are in order. 

%\input{figures/wfMetamod-full-vert}
%\input{figures/wfMetamod-full-horiz}
\zdhll{An accurate metamodel specifying diagrams like in \figri\ is shown in the framed fragment of \figrii(a).  Wires are specified by (dark grey) classes \wptopt\ and \pttowp\ supplied with \from\ and \too\ associations. Following CT, we call a triple like $(\wptopt,\from,\too)$ a {\em span}, node \wptopt\ is its {\em head}, arrows \from, \too\ are {\em legs} and legs' target nodes are {\em feet}. We will often refer to a span by its head if the legs are clear from the context. % to WP and in/outPort classes, 
 Thus, wires are specified by spans \wptopt\ and \pttowp. Two [key] constraints declared for these spans demand a wire to be fully determined by its ends, \ie,  two different wires can share the source or the  target, but sharing both ends is prohibited (\ie, classes \wptopt\ and \pttowp\ are relations rather than multirelations). Note associations $\from'$ and $\too'$ to class Process shown in blue, whcih are derived by composition: 
 %for a wire $w:\wptopt$, 
 $\too'=\too.\owner$ and $\from'=\from.\owner$ (where \owner\ is the black-diamond end name).%
 \footnote {We follow UML and prefix the names of derived elements by backslah, and colour them in blue to suggest ``mechanical/algebraic derivation''.}
  Then span $\wptopt'=(\wptopt,\from,\too')$ 
  %(we call such triples {\bf \em spans} with node \wptopt\ being its {\bf\em head} and arrows \from\ and $\too'$ its {\bf\em legs}) 
  gives us a (mutli)relation from WorkProduct to Process (note two wires between product W and process P in \figri(b) which show that the span is a multirelation). Similarly, span $\pttowp'=(\pttowp,\from',\too)$ is a relation from Process to WorkProduct (not a multi-relation as each process has only one out-port).   %these associations specify the dependency flow between products and processes, and we will denote the \corring\ relations by \wptops\ and \pstowp\ (the former is actually a multirelation as miltiple wires from a product to a process are possible, \eg, from W to P in \figri.). 
 Relational composition $\pstops\eqdef \pstowp'\Join \wptops'$ is a binary (multi)relation on processes, and we require it to be acyclic. This assumption greatly simplifies the mathematical model, and holds in all SEP instances we have been dealing with.}{probably this piece may be written shorter based on  self-explainability of the metamodel. But spans are to be explained}{-25em} 

%\zdmodd{We will also need the following relation \wptowp\ between WPs. We first consider processes as relationships between input and outports (note dashed white arrows between ports within process blocks in \figri). Then we compose three relations: $\wptowp\eqdef\wptopt\Join\Process\Join\pttowp$. It can be shown that if \pstops\ is acyclic, then \wptowp\ is acyclic and conversely, and we include this constraint in the metamodel. }{}{Maybe this piece is not needed}{-8em}
%\begin{defin} A dependency flow is {\em acyclic} if relations \pstops'\ and \wptowp\ are acyclic.
%\end{defin}
\begin{remark}
Note two encircled multiplicities in \figrii(a). The left one says that only one wire can come to an in-port, and hence an in-port reads one and only one piece of data; thus, there is no data merge at ports. The right one says that any out-port has at least one wire that takes its data and hence any out-port writes to at least one product.
\end{remark} 
\begin{remark}We admit processes without in-ports, which provide predefined information like in standards (such processes were coloured grey in \figref{?}). We also admit processes without out-ports, which can be seen as garbage collectors. 
\end{remark}




==> sections/wfFormalism.tex <==
%\renewcommand\figri{\figref{fig:wfMetamod-full}(a)}
%\renewcommand\figrii{\figref{fig:wfExample-depFlow}}
%\renewcommand\figriii{\figref{fig:wfMetamod-full}(b)}
%\renewcommand\figriv{\figref{fig:wfExample-dataFlow}}

%\subsection{Workflow$^+$ formalization and metamodel}


\subsection{Processes as multiary model \trafon s}\label{sec:wf-formalDefs}
Ordinary algebraic operations are specified by their {\em arity (schema)} and {\em semantic mapping}. For example, a binary operation $f$ may have a schema $(A_1,A_2;B)$ with $A_1,A_2$ being names of two input sets and $B$ the name of the output set; sometimes these names are called {\em sorts}. Semantics is a function \frar{\semm{f}}{\semm{A_1}\timm\semm{A_2}}{\semm{B}}, where \semm{X} denotes the set corresponding to a sort $X$. The above patterns is applicable to multiary model transformations (MTs) with sorts being metamodels, which can be see as ``names'' for the \corring\ sets of instances: if $X$ is a metamodel, then \semm{X} denotes its set of instances. An essential distinction from the ordinary algebra is that while set names are structureless tokens, metamodels are rich structures that can overlap and we need to take this into account. It is natural to assume that all input metamodels ($A,B$ for our case) are disjoint as otherwise it is reasonable to merge them into a single input metamodel. However, overlapping of $A{\cup}B$ and $C$ %or $B$ and $C$ or both 
is a typical case as we have seen above, but we cannot merge them as input and output metamodels play different roles. Thus, for MTs, we need a more intelligent notion of an arity schema. 

\zd{ref to background section on CT}
  We assume given some universe (a category) \mmodcat\ of metamodels and metamodel mappings.
  \begin{defin}%[Metamodelling \fwk]
  	A {\bf\em metamodelling \fwk} is given by the following two components. a) A category \mmodcat, whose objects are called {\em metamodels} and morphisms are {\em metamodel maps}. Moreover, \mmodcat\ has coproducts, \ie, any two metamodels $M$ and $N$ can be (disjointly) merged into $M+N$, and there is an empty metamodel 0 such that $M+0=M$ for any $M$. We will call monic maps {\em injections}  and say that metamodel $M$ is {\em embedded} into metamodel $N$ if there is an injection \frar{i}{M}{N}. 
  	
  	b) A coproduct compatible functor from category \mmodcat\ to category \setcat\ of sets and functions. In detail, the following two conditions hold. 
  	
  	\noindent b1) Every metamodel $M$ is assigned with a set of its {\em instances} \semm{M} so that $\semm{M+N}=\semm{M}\times\semm{N}$. As the empty metamodel can be seen as the merge of the empty set of metamodels, $0=\coprod^\mmodcat_\varnothing$, we have  $\semm{0}=\prod^\setcat_\varnothing=1$ where $1=\{*\}$ is a fixed singleton set. 
  	
  	\noindent b2) Every metamodel map \frar{f}{M}{N} is assigned with a mapping \flar{f^*}{\semm{M}}{\semm{N}} between instance sets (note the reversal of the arrow) which is functorial, \ie, given $X\rTo^f Y\rTo^g Z$, $(f.g)^*=g^*.f^*$ and if \frar{\id_M}{M}{M} is identity metamodel map, then \flar{\id_M^*}{\semm{M}}{\semm{M}} is identity mapping of set \semm{M}. 
  	
  	In addition, we assume that \mmodcat\ has all finite limits and colimits, which would allow us to talk about general forms of metamodel intersection (via limits) and union (via colimit).
  \end{defin}
\begin{remark}
	In all applications we are interested in, if map \frar{f}{M}{N} is injection, %, \ie, metamodel $M$ is embedded into $N$ and can be seen as $M$'s sub-metamodel, 
	and $I\in\semm{N}$ is an instance, then instance $f^*(I)\in\semm{M}$ can be seen as the part of instance $I$ typed over $M$ (we will say $I$ is {\em projected} onto $M$). If $f$ is not injection, and glues together some elements, \eg, for two classes $c, c' \inn M$, $f(c)=f(c')=d$ in $N$, then all instances of $d$ will be duplicated by $f^*$: if for $I\in\semm{N}$, $I(d)$ is the set of instances of class $d$, then $f^*(I)(c)=f^*(I)(c')=I(d)$. Details of how it works can be found in \cite[chapter xx]{ehrigbook06} 
\end{remark}
\begin{defin}[Process arity]\label{def:arity} A {\em process library} is a pair $\pslib=(|\pslib|, S)$ with |\pslib| a set whose elements are called {\em processes}, and $S$ a mapping that assigns to each process $P\in|\pslib|$ its {\bf\em arity schema}, \ie, a triple $S(P)=(N, \inx, \out)$ where $N$ is a metamodel called the {\em inner} metamodel of $P$, $\inx$ is a finite family of injective maps into $N$, \frar{\inx_i}{A_i}{N}, $i=1..n$, whose sources $A_i$ are disjoint and called $P$'s {\em input} metamodels, and \flar{\out}{N}{B} is metamodel map into $N$ whose source is called $P$'s {\em output} metamodel. Thus, arity schema is given by the following diagram:
	\begin{equation}\label{eq:arity}
	\begin{diagram}[small]
	A_i &\rTo^{\inx_i}_{i=1..n}&N&\lTo^\out&B
\end{diagram}
\end{equation}
and we require all images $\inx_i(A_i)$ to be disjoint in $N$. Categorically, it can be formally specified by requiring the pullback of any two maps $\inx_i$, $\inx_j$ %, $j\noteq i$ 
to be empty: 
\begin{equation}\label{eq:disj}
A_i\times^{\inx_i}_{\inx_j} A_j=0 \mbox{ for any $j\noteq i$}
\end{equation}
	Below we will write $P\in\pslib$ for $P\in|\pslib|$. If needed, elements of a schema $S(P)$ will be superscripted with $P$, \eg, $N^P$ etc.
\end{defin}	

\medskip	
	The intuition behind the definition above is that process $P$ takes a tuple of data instances over its input metamodels, computes from them an instance over the inner metamodel, and then projects it onto metamodel $B$. %returns a data instance over its output metamodel. 
	Formally,
	\begin{defin}\label{def:semMap}For any process $P$, we assume given some mapping \frar{\semm{P_\inx}}{\prod_{i\le n}\semm{A_i}}{\semm{N}} called $P$'s {\bf\em inner semantic mapping}. {\bf\em (Full) semantic mapping} of $P$ (denoted \semm{P}) is the composition 
\begin{equation}\label{eq:semmap}
% \frar{\semm{P}\eqdef\semm{P_\inx};\out^*}%
%{\prod_{i\le n}}{\semm{B}} 
\begin{diagram}[small]
\prod_{i\le n}\semm{A_i} &\rTo^{\semm{P_\inx}}&\semm{N}&\rTo^{\out^*}&\semm{B}
\end{diagram}
 \end{equation}
 whose second component is provided by the metamodelling \fwk\ (see condition (b2) in \defref{arity}. %We denote this composition by \semm{P}. 
 
 In addition, we need to require that input data are not changed, \ie, equality \eqref{nosideEff} below holds for any input tuple $X_i\in\semm{A_i}$, $i\le n$:
 \begin{equation}\label{eq:nosideEff}
 (X_1...X_n).\semm{P_\inx}.\inx_i^*= X_i \mbox{ for all $i$}
 \end{equation}
\end{defin}
\begin{remark}[Why the output metamodel is different from the inner one?] %If $B=N$ and map \out\ is identity, then $\out^*$ is also identity and $\semm{P}=\semm{P_\inx}$. 
	Distinguishing the inner and the output metamodels may seem artificial (why should we care about inner data, which are not visible at the process output?) but is well justified in the context of assurance. If even some inner data  are not needed for other processes, the assessor of a safety case must check their correctness and validity. Note that the standard case when $B=N$ is readily simulated by setting map \out\ to the identity of $N$. 
\end{remark}
\begin{defin}[Source and sink processes]\label{def:arity+}We modify \defref{arity} by allowing the number of input maps to be 0, $n=0$, and hence the family of inout maps is empty so that 
	$\prod_\varnothing\semm{A_i}=1={*}$. Then mapping \frar{\semm{P_\inx}}{1}{\semm{N}} just selects some specific instance over $N$, and then mapping $\out^*$ projects the required part of this instance. Hence, the case $n=0$ corresponds to having a fixed constant data instance, \eg, those data shown in grey in our metamodel \figref{fig:WF+-ADV}. We call such processes {\em sources}. Dually, we allow the output metamodel $B$ to be empty so that the process always produces the trivial predefined singleton instance 1 for any input data; such a process acts as a ``black hole'' or {\em sink}. 
\end{defin}

\medskip
For specifying networks of processes, it is convenient to introduce process' ports (input and output) coupled with the \corring\ (input and output) metamodels, \eg, process $P$ in \figrii\ has two input and one output port. All our processes will have just one output port as this settign simplifies technicalities without the loss of generality: a process with $n$ output ports can be decomposed into $n$ processes with one output port (it is a standard algebraic setting for modelling $n$-coary operations). A \corring\ reformulation of Def.~\ref{def:arity}, \ref{def:arity+}, \ref{def:semMap} is straightforward and we omit it, but introduce ports in the metamodel in \figri.  %(by a process library we mean set of processes each assigned with its arity schema and supplied with a semantic mapping). 
\begin{remark}%[On portfree processes]
A process may have neither input nor output ports and hence be  isolated, but it still has an arity schema $0\rightarrow N \leftarrow 0$. 
\end{remark}
\begin{remark}
There is an important difference between a constant process $P_c$ with no input ports, which denotes some constant instance $c=\semm{P}(*)$ over the output metamodel, and a process $P_c^0$ with one input port and hence one input metamodel equal to 0. Such a process will produce instance $c=\semm{P}(*)$ only if signal $*$ is received at the input port and stay idle otherwise. Similarly, a process without the output port, simply absrobs all received data without producing anything visible while a process with the empty output metamodel produces a signal * at the output port (which can be seen as notification that some input data instance is received and processed). 
\end{remark}
=========

\zd{there is some piece in the source below this line but it's commented}

\endinput

Next we consider how processes are composed into a workflow.  We will begin with a high-level view of process composition in \sectref{wfMetamod-depFlow} and then refine it in an accurate data modelling \fwk\ in \sectref{wfMetamod-dataFlow}.

%\subsection{Composing processes into workflow}

%\input{figures/wfMetamod-full}
%\input{figures/wfExample-depFlow}

\subsection{Composing processes into workflow, 1: Dependency flow}\label{sec:wfMetamod-depFlow}
The world of assurance consists of processes (Ps) and work products (WP) (cf. \citeiso): the former produce the latter, which are then used to feed the former. A generic example is shown in \figrii, which says that each of the products WP1, WP2 is jointly created by processes $P$ and $P'$, some part of WP1 is the input for $Q$ and another part is an input for $Q'$, but the latter also need the second input from WP2. Note that an arrow from a WP to a port means that some part of WP is fed to that port, and two arrows from WP0 to $P$ mean that the latter processes two parts of WP0 (in general, different, but it may happen that the same part is fed to different ports-- we will explain how it works later in \sectref{wfMetamod-dataFlow}). 


 Arrows specifying the flow will be referred to as {\em wires} and they are of two types: wires from ports to WP and from WP to ports. 
 \begin{defin}[Dependency flow] A {\em dependency flow} over a process library (\pslib, \iptset, \optset)  is given by a set of metamodels $\wpset\subset\xob{\mmodcat}$ called {\em work product metamodels} or just {\em WPs}, and two flow relations , $\wptopt\subset\wpset\times\iptset$ and $\pttowp\subset\optset\times\wpset$, whose elements are called wires. 
\end{defin}
 The left half of \figriii\ (shaded in grey) presents the \corring\ metamodel, in which wires are specified by (white) classes \wptopt\ and \pttowp\ supplied with \from\ and \too\ associations, % to WP and in/outPort classes, 
 and two [key] constraints say that a wire is fully determined by its ends, \ie,  sharing a source port or a target port is allowed, but sharing both ends is prohibited (hence, classes \wptopt\ and \pttowp\ are relations rather than multirelations). Associations $\from'$ and $\too'$ to class Process shown in blue are derived by composition: %(note also backslash prefixes in their names): 
these associations specify the dependency flow between WP and processes, and we will denote the \corring\ relations by \wptops\ and \pstowp\ (the former is actually a multirelation as miltiple wires from a WP to a Process are possible, \eg, from WP0 to P in \figrii.). Relational composition $\pstops\eqdef \pstowp\Join \wptops$ is a binary (multi)relation on processes, and we require it to be acyclic. This assumption greatly simplifies the mathematical model, and holds in all SEP instances we have been dealing with. 

We will also need the following dependability relation \wptowp\ between WPs. We first consider processes as relationships between input and outports (note dashed arrows between ports within process blocks in \figrii). Then we compose three relations: $\wptowp\eqdef\wptopt\Join\Process\Join\pttowp$. It can be shown that if \pstops\ si acyclic, then \wptowp\ is acyclic and conversely. 
\begin{defin} A dependency flow is {\em acyclic} if relations \pstops\ and \wptowp\ are acyclic.
\end{defin}

%\input{figures/wfMetamod-flow}
%\input{figures/wfMetamod-full}
%\input{figures/wfExample-dataFlow}

\subsection{Composing processes into workflow, 2: Data algebra underlying the dependency flow}\label{sec:wfMetamod-dataFlow}

\begin{defin}The {\em metamodeling carrier} of a dependency flow 
	
\end{defin}
%\zd{not finished yet} % ; i guess it'd take about yet another page}

==> sections/wfp-meta-new.tex <==
\renewcommand\figri{\figref{fig:wfExample-depFlow}}
\renewcommand\figrii{\figref{fig:wfMetamod-full}}
\renewcommand\figriii{\figref{fig:wfExample-dataFlow}}
\renewcommand\figriv{\figref{fig:wfMetamod-full}(b)}

\renewcommand\figro{\figref{fig:sem-fwk}}
\renewcommand\figri{\figref{fig:wfExample-schema}}
\renewcommand\figrii{\figref{fig:wfMetamod-full}}
\renewcommand\figriii{\figref{fig:wfExample-full}}


\section{Workflow$^+$ metamodel and formalization}
\label{sec:wfFormalism}

%\input{figures/wfPlane}
Even the simple example considered above shows two basic features of a typical SEP. First, the component (sub)processes operate complex data specifiable by metamodels employing full power of class diagrams; moreover, output data of a process can be essentially connected to the input data. Second, these processes are inter-connected into sufficiently complex networks. Thus, we deal with  high complexity in both intra- and inter-process dimensions of the entire workflow --- this is what we refer to as WF+ in this paper.  Somewhat surprisingly, mathematical and specificational foundations of WF+ are not presented in the literature and probably are not well understood. Indeed, processes with complex intra dataflow are sufficiently well studied by the MBD community as model \trafon s (MTs), but the semantic side is mainly operational rather than denotational. In the operational setting, understanding MT's composition to form complex MTs is especially challenging so that even sequential composition (MT chaining) is still being actively researched \cite{?} while studying general MT networking (both theoretical and practical) is in its  infancy  \cite{?}. 

\input{figures/wfPlane}
On the other hand, complex networks are well-studied in the domain of block diagrams with enormous literature (see, \eg, \cite{?,?,?}), but a typical functional block operates very simple data given by a set of input variables and a disjoint set of output variables%
\footnote{The two set can intersect if we have a feedback loop, but overlapping in WF+ is of different nature---it is static and has nothing to do with feedback.} 
%
%\input{figures/wfPlane}
The situation is schematically presented in the inset figure above, which shows that the case of WF+ is not covered by either of the \fwk s. 

In this section, we outline a formal \fwk\ in which WF+ can be precisely specified. The presentation will be based on a running example being sufficiently generic to show how all necessary mechanisms work, but metamodels we will present are general. In \sectref{depflow}, we present an abstract view of WF+ called schema, and how dataflow data are defined over a schema is shown in \sectref{dataflow}. Section~\ref{sec:corrs} is focused on what makes WF+ so special --- interactions between parallel processes. Finally, in \sectref{comp} we explain compositionality of WF+: a complex workflow can be encapsulated as a black-box process, which makes possible to consider workflows of workflows. Metamodels defining the syntax of WF+ models are specified, but an accurate formal presentation of semantics needs a relatively advanced category theory (CT) apparatus: limits and colimits (and specifically pullbacks and pushouts), continuous functors compatible with them, and adhesive categories in which PBs and POs smoothly interact (via Van Kampen squares). As we cannot assume knowledge of this material from a typical Models reader, we will describe the WF+ mechanisms conceptually rather than formally, but accurate formal definitions and details can be found in \citetr. 



%We will begin with an informal discussion of WF+ and its special features by considering a simple but generic enough example in \sectref{wfExample}. Then we will formalize the syntax by presenting its metamodel, and define the intended semantics formally in \sectref{wfMetamod}. 
%an accurate definition of the intra-structure of processes (considered as multiary MTs), and then proceed with the connectivity mechanism composing the processes into a workflow. 

\input{sections/wfExample-schema}%
\input{sections/wfExample-mech}
\input{sections/wfExample-dataFlow}
\input{figures/wfMetamod-full-vert}
\input{sections/wfExample-corrs}
\input{sections/wfExample-comp}
%\input{sections/wf-formalDefs}



==> sections/wfp-meta.tex <==
\renewcommand\figri{\figref{fig:wfMetamod-full}(a)}
\renewcommand\figrii{\figref{fig:wfExample-depFlow}}
\renewcommand\figriii{\figref{fig:wfMetamod-full}(b)}
\renewcommand\figriv{\figref{fig:wfExample-dataFlow}}

\section{Workflow$^+$ formalization and metamodel}
\label{sec:wfp-meta}

%Even the simple example considered above shows two basic features of a typical SEP. First, the component (sub)processes operate complex data specifiable by metamodels employing full power of class diagrams; moreover, output data of a process can be essentially connected to the input data. Second, these processes are connected into sufficiently complex networks. Thus, we deal with  high complexity in both intra- and inter-process dimensions of the entire workflow --- this is what we refer to as WF+ in this paper.  Somewhat surprisingly, mathematical and specificational foundations of WF+ are not presented in the literature and probably are not well understood. Indeed, processes with complex intra dataflow are sufficiently well studied by the MBD community as model \trafon s (MTs). However, composition of MTs to form complex MTs is in its infancy so that even sequential composition (MT chaining) is still being actively researched \cite{?}.  
%
%\input{figures/wfPlane}
%On the other hand, complex networks are well-studied in the domain of block diagrams with enormous literature (see, \eg, \cite{?,?,?}), but a typical functional block operates very simple data given by a set of input variables and a disjoint set of output variables%
%\footnote{The two set can intersect if we have a feedback loop, but overlapping in WF+ is of different nature---it is static and has nothing to do with feedback.} The situation is schematically presented in the inset figure above, which shows that the case of WF+ is not covered by either of the formalisms. 
%
%In this section, we outline a formal \fwk\ in which WF+ can be precisely specified. We will begin with an accurate definition of the intra-structure of processes (considered as multiary MTs), and then proceed with the connectivity mechanism composing the processes into a workflow. 

\subsection{Processes as multiary model \trafon s}
Ordinary algebraic operations are specified by their {\em arity (schema)} and {\em semantic mapping}. For example, a binary operation $f$ may have a schema $(A_1,A_2;B)$ with $A_1,A_2$ being names of two input sets and $B$ the name of the output set; sometimes these names are called {\em sorts}. Semantics is a function \frar{\semm{f}}{\semm{A_1}\timm\semm{A_2}}{\semm{B}}, where \semm{X} denotes the set corresponding to a sort $X$. The above patterns is applicable to multiary model transformations (MTs) with sorts being metamodels, which can be see as ``names'' for the \corring\ sets of instances: if $X$ is a metamodel, then \semm{X} denotes its set of instances. An essential distinction from the ordinary algebra is that while set names are structureless tokens, metamodels are rich structures that can overlap and we need to take this into account. It is natural to assume that all input metamodels ($A,B$ for our case) are disjoint as otherwise it is reasonable to merge them into a single input metamodel. However, overlapping of $A{\cup}B$ and $C$ %or $B$ and $C$ or both 
is a typical case as we have seen above, but we cannot merge them as input and output metamodels play different roles. Thus, for MTs, we need a more intelligent notion of an arity schema. 

\zd{ref to background section on CT}
  We assume given some universe (a category) \mmodcat\ of metamodels and metamodel mappings.
  \begin{defin}%[Metamodelling \fwk]
  	A {\bf\em metamodelling \fwk} is given by the following two components. a) A category \mmodcat, whose objects are called {\em metamodels} and morphisms are {\em metamodel maps}. Moreover, \mmodcat\ has coproducts, \ie, any two metamodels $M$ and $N$ can be (disjointly) merged into $M+N$, and there is an empty metamodel 0 such that $M+0=M$ for any $M$. We will call monic maps {\em injections}  and say that metamodel $M$ is {\em embedded} into metamodel $N$ if there is an injection \frar{i}{M}{N}. 
  	
  	b) A coproduct compatible functor from category \mmodcat\ to category \setcat\ of sets and functions. In detail, the following two conditions hold. 
  	
  	\noindent b1) Every metamodel $M$ is assigned with a set of its {\em instances} \semm{M} so that $\semm{M+N}=\semm{M}\times\semm{N}$. As the empty metamodel can be seen as the merge of the empty set of metamodels, $0=\coprod^\mmodcat_\varnothing$, we have  $\semm{0}=\prod^\setcat_\varnothing=1$ where $1=\{*\}$ is a fixed singleton set. 
  	
  	\noindent b2) Every metamodel map \frar{f}{M}{N} is assigned with a mapping \flar{f^*}{\semm{M}}{\semm{N}} between instance sets (note the reversal of the arrow) which is functorial, \ie, given $X\rTo^f Y\rTo^g Z$, $(f.g)^*=g^*.f^*$ and if \frar{\id_M}{M}{M} is identity metamodel map, then \flar{\id_M^*}{\semm{M}}{\semm{M}} is identity mapping of set \semm{M}. 
  	
  	In addition, we assume that \mmodcat\ has all finite limits and colimits, which would allow us to talk about general forms of metamodel intersection (via limits) and union (via colimit).
  \end{defin}
\begin{remark}
	In all applications we are interested in, if map \frar{f}{M}{N} is injection, %, \ie, metamodel $M$ is embedded into $N$ and can be seen as $M$'s sub-metamodel, 
	and $I\in\semm{N}$ is an instance, then instance $f^*(I)\in\semm{M}$ can be seen as the part of instance $I$ typed over $M$ (we will say $I$ is {\em projected} onto $M$). If $f$ is not injection, and glues together some elements, \eg, for two classes $c, c' \inn M$, $f(c)=f(c')=d$ in $N$, then all instances of $d$ will be duplicated by $f^*$: if for $I\in\semm{N}$, $I(d)$ is the set of instances of class $d$, then $f^*(I)(c)=f^*(I)(c')=I(d)$. Details of how it works can be found in \cite[chapter xx]{ehrigbook06} 
\end{remark}
\begin{defin}[Process arity]\label{def:arity} A {\em process library} is a pair $\pslib=(|\pslib|, S)$ with |\pslib| a set whose elements are called {\em processes}, and $S$ a mapping that assigns to each process $P\in|\pslib|$ its {\bf\em arity schema}, \ie, a triple $S(P)=(N, \inx, \out)$ where $N$ is a metamodel called the {\em inner} metamodel of $P$, $\inx$ is a finite family of injective maps into $N$, \frar{\inx_i}{A_i}{N}, $i=1..n$, whose sources $A_i$ are disjoint and called $P$'s {\em input} metamodels, and \flar{\out}{N}{B} is metamodel map into $N$ whose source is called $P$'s {\em output} metamodel. Thus, arity schema is given by the following diagram:
	\begin{equation}\label{eq:arity}
	\begin{diagram}[small]
	A_i &\rTo^{\inx_i}_{i=1..n}&N&\lTo^\out&B
\end{diagram}
\end{equation}
and we require all images $\inx_i(A_i)$ to be disjoint in $N$. Categorically, it can be formally specified by requiring the pullback of any two maps $\inx_i$, $\inx_j$ %, $j\noteq i$ 
to be empty: 
\begin{equation}\label{eq:disj}
A_i\times^{\inx_i}_{\inx_j} A_j=0 \mbox{ for any $j\noteq i$}
\end{equation}
	Below we will write $P\in\pslib$ for $P\in|\pslib|$. If needed, elements of a schema $S(P)$ will be superscripted with $P$, \eg, $N^P$ etc.
\end{defin}	

\medskip	
	The intuition behind the definition above is that process $P$ takes a tuple of data instances over its input metamodels, computes from them an instance over the inner metamodel, and then projects it onto metamodel $B$. %returns a data instance over its output metamodel. 
	Formally,
	\begin{defin}\label{def:semMap}For any process $P$, we assume given some mapping \frar{\semm{P_\inx}}{\prod_{i\le n}\semm{A_i}}{\semm{N}} called $P$'s {\bf\em inner semantic mapping}. {\bf\em (Full) semantic mapping} of $P$ (denoted \semm{P}) is the composition 
\begin{equation}\label{eq:semmap}
% \frar{\semm{P}\eqdef\semm{P_\inx};\out^*}%
%{\prod_{i\le n}}{\semm{B}} 
\begin{diagram}[small]
\prod_{i\le n}\semm{A_i} &\rTo^{\semm{P_\inx}}&\semm{N}&\rTo^{\out^*}&\semm{B}
\end{diagram}
 \end{equation}
 whose second component is provided by the metamodelling \fwk\ (see condition (b2) in \defref{arity}. %We denote this composition by \semm{P}. 
 
 In addition, we need to require that input data are not changed, \ie, equality \eqref{nosideEff} below holds for any input tuple $X_i\in\semm{A_i}$, $i\le n$:
 \begin{equation}\label{eq:nosideEff}
 (X_1...X_n).\semm{P_\inx}.\inx_i^*= X_i \mbox{ for all $i$}
 \end{equation}
\end{defin}
\begin{remark}[Why the output metamodel is different from the inner one?] %If $B=N$ and map \out\ is identity, then $\out^*$ is also identity and $\semm{P}=\semm{P_\inx}$. 
	Distinguishing the inner and the output metamodels may seem artificial (why should we care about inner data, which are not visible at the process output?) but is well justified in the context of assurance. If even some inner data  are not needed for other processes, the assessor of a safety case must check their correctness and validity. Note that the standard case when $B=N$ is readily simulated by setting map \out\ to the identity of $N$. 
\end{remark}
\begin{defin}[Source and sink processes]\label{def:arity+}We modify \defref{arity} by allowing the number of input maps to be 0, $n=0$, and hence the family of inout maps is empty so that 
	$\prod_\varnothing\semm{A_i}=1={*}$. Then mapping \frar{\semm{P_\inx}}{1}{\semm{N}} just selects some specific instance over $N$, and then mapping $\out^*$ projects the required part of this instance. Hence, the case $n=0$ corresponds to having a fixed constant data instance, \eg, those data shown in grey in our metamodel \figref{fig:WF+-ADV}. We call such processes {\em sources}. Dually, we allow the output metamodel $B$ to be empty so that the process always produces the trivial predefined singleton instance 1 for any input data; such a process acts as a ``black hole'' or {\em sink}. 
\end{defin}

\medskip
For specifying networks of processes, it is convenient to introduce process' ports (input and output) coupled with the \corring\ (input and output) metamodels, \eg, process $P$ in \figrii\ has two input and one output port. All our processes will have just one output port as this settign simplifies technicalities without the loss of generality: a process with $n$ output ports can be decomposed into $n$ processes with one output port (it is a standard algebraic setting for modelling $n$-coary operations). A \corring\ reformulation of Def.~\ref{def:arity}, \ref{def:arity+}, \ref{def:semMap} is straightforward and we omit it, but introduce ports in the metamodel in \figri.  %(by a process library we mean set of processes each assigned with its arity schema and supplied with a semantic mapping). 
\begin{remark}%[On portfree processes]
A process may have neither input nor output ports and hence be  isolated, but it still has an arity schema $0\rightarrow N \leftarrow 0$. 
\end{remark}
\begin{remark}
There is an important difference between a constant process $P_c$ with no input ports, which denotes some constant instance $c=\semm{P}(*)$ over the output metamodel, and a process $P_c^0$ with one input port and hence one input metamodel equal to 0. Such a process will produce instance $c=\semm{P}(*)$ only if signal $*$ is received at the input port and stay idle otherwise. Similarly, a process without the output port, simply absrobs all received data without producing anything visible while a process with the empty output metamodel produces a signal * at the output port (which can be seen as notification that some input data instance is received and processed). 
\end{remark}

%\input{figures/wfMetamod-lib}

Next we consider how processes are composed into a workflow.  We will begin with a high-level view of process composition in \sectref{wfMetamod-depFlow} and then refine it in an accurate data modelling \fwk\ in \sectref{wfMetamod-dataFlow}.

%\subsection{Composing processes into workflow}

%\input{figures/wfMetamod-full}
%\input{figures/wfExample-depFlow}

\subsection{Composing processes into workflow, 1: Dependency flow}\label{sec:wfMetamod-depFlow}
The world of assurance consists of processes (Ps) and work products (WP) (cf. \citeiso): the former produce the latter, which are then used to feed the former. A generic example is shown in \figrii, which says that each of the products WP1, WP2 is jointly created by processes $P$ and $P'$, some part of WP1 is the input for $Q$ and another part is an input for $Q'$, but the latter also need the second input from WP2. Note that an arrow from a WP to a port means that some part of WP is fed to that port, and two arrows from WP0 to $P$ mean that the latter processes two parts of WP0 (in general, different, but it may happen that the same part is fed to different ports-- we will explain how it works later in \sectref{wfMetamod-dataFlow}). 


 Arrows specifying the flow will be referred to as {\em wires} and they are of two types: wires from ports to WP and from WP to ports. 
 \begin{defin}[Dependency flow] A {\em dependency flow} over a process library (\pslib, \iptset, \optset)  is given by a set of metamodels $\wpset\subset\xob{\mmodcat}$ called {\em work product metamodels} or just {\em WPs}, and two flow relations , $\wptopt\subset\wpset\times\iptset$ and $\pttowp\subset\optset\times\wpset$, whose elements are called wires. 
\end{defin}
 The left half of \figriii\ (shaded in grey) presents the \corring\ metamodel, in which wires are specified by (white) classes \wptopt\ and \pttowp\ supplied with \from\ and \too\ associations, % to WP and in/outPort classes, 
 and two [key] constraints say that a wire is fully determined by its ends, \ie,  sharing a source port or a target port is allowed, but sharing both ends is prohibited (hence, classes \wptopt\ and \pttowp\ are relations rather than multirelations). Associations $\from'$ and $\too'$ to class Process shown in blue are derived by composition: %(note also backslash prefixes in their names): 
these associations specify the dependency flow between WP and processes, and we will denote the \corring\ relations by \wptops\ and \pstowp\ (the former is actually a multirelation as miltiple wires from a WP to a Process are possible, \eg, from WP0 to P in \figrii.). Relational composition $\pstops\eqdef \pstowp\Join \wptops$ is a binary (multi)relation on processes, and we require it to be acyclic. This assumption greatly simplifies the mathematical model, and holds in all SEP instances we have been dealing with. 

We will also need the following dependability relation \wptowp\ between WPs. We first consider processes as relationships between input and outports (note dashed arrows between ports within process blocks in \figrii). Then we compose three relations: $\wptowp\eqdef\wptopt\Join\Process\Join\pttowp$. It can be shown that if \pstops\ si acyclic, then \wptowp\ is acyclic and conversely. 
\begin{defin} A dependency flow is {\em acyclic} if relations \pstops\ and \wptowp\ are acyclic.
\end{defin}

%\input{figures/wfMetamod-flow}
%\input{figures/wfMetamod-full}
%\input{figures/wfExample-dataFlow}

\subsection{Composing processes into workflow, 2: Data algebra underlying the dependency flow}\label{sec:wfMetamod-dataFlow}

\begin{defin}The {\em metamodeling carrier} of a dependency flow 
	
\end{defin}
%\zd{not finished yet} % ; i guess it'd take about yet another page}

==> sections/work-in-progress.tex <==
\section{Work in Progress and future work}\label{sec:WPF}

%We present two important parts the \wfp\ landscape, which are in active development but not finished yet (\sectref{work-in}.A and B), and then briefly discuss future work (C).

\input{sections/conformToNorm}



%\subsection{Future work}
%\zd{A list of future work items with their brief descr. }
%\subsubsection{\wfp-Metamodel and formal semantics}

\subsection{Formal semantics for \wfp}

\wfp\ is a well-defined formalism; we did not include its metamodel into the paper due to space limits. It also has an intuitive semantics: a \wfp-process $P$ can be seen as a model transformation with $n$ ports, each with a metamodel assigned. Given$n$ instances  over those metamodels, $P$ transforms them into an instance over some output port metamodel.  Importantly, input and output metamodel may overlap (actually this is a typical case for SEPs we are dealing with), which adds $+$ to the name \wfp. An accurate, and manageable,  formalization of \wfp-semantics %needs category theory and 
is a work in progress. 

%. The 'plus' in \wfp-name is because 
%We believe it should also be provided with a clearly specified formal semantics
